The ACPATH Metric: Precise Estimation of the Number of Acyclic Paths in C-like Languages

NPATH is a metric introduced by Brian A. Nejmeh in [13] that is aimed at overcoming some important limitations of McCabe's cyclomatic complexity. Despite the fact that the declared NPATH objective is to count the number of acyclic execution paths through a function, the definition given for the C language in [13] fails to do so even for very simple programs. We show that counting the number of acyclic paths in CFG is unfeasible in general. Then we define a new metric for C-like languages, called ACPATH, that allows to quickly compute a very good estimation of the number of acyclic execution paths through the given function. We show that, if the function body does not contain backward gotos and does not contain jumps into a loop from outside the loop, then such estimation is actually exact.

==> pgf.revision.tex <==
\begingroup
\catcode`\-=12
\catcode`\/=12
\catcode`\.=12
\catcode`\:=12
\catcode`\+=12
\catcode`\-=12
\gdef\pgfrevision{3.1.9a}
\gdef\pgfversion{3.1.9a}
\gdef\pgfversiondatetime{2021-05-15 12:06:55 +0200}
\gdef\pgfrevisiondatetime{2021-05-15 12:06:55 +0200}
\gdef\pgf@glob@TMPa#1-#2-#3 #4\relax{#1/#2/#3}
\xdef\pgfversiondate{\expandafter\pgf@glob@TMPa\pgfversiondatetime\relax}
\xdef\pgfrevisiondate{\expandafter\pgf@glob@TMPa\pgfrevisiondatetime\relax}
\endgroup


==> pgfcore.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgfcore.code.tex}

\newif\ifpgf@draftmode
\def\pgf@typeout{\immediate\write0}

\input pgfmath.code.tex
\input pgfint.code.tex

\input pgfcorepoints.code.tex
\input pgfcorepathconstruct.code.tex
\input pgfcorepathusage.code.tex
\input pgfcorescopes.code.tex
\input pgfcoregraphicstate.code.tex
\input pgfcoretransformations.code.tex
\input pgfcorequick.code.tex
\input pgfcoreobjects.code.tex
\input pgfcorepathprocessing.code.tex
\input pgfcorearrows.code.tex
\input pgfcoreshade.code.tex
\input pgfcoreimage.code.tex
\input pgfcorelayers.code.tex
\input pgfcoretransparency.code.tex
\input pgfcorepatterns.code.tex
\input pgfcorerdf.code.tex

\pgfutil@ifundefined{pgf@texdist@protect}{%
    \def\pgf@texdist@protect{}%
}{}
\endinput


==> pgfcoreimage.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreimage.code.tex}



% Declare an image
%
% #1 = optional argument: width, height, page specification
% #2 = name of the image for later use
% #4 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF and .ps, .eps, .epsi for postscript.
%
% Description:
%
% This command declares an image file for later use. Even if the image
% is used several times in the document, in PDF it will only be stored
% once.
%
% Example:
%
% \pgfdeclareimage[width=2cm,page=2]{myimage}{imagefilename}

\def\pgfdeclareimage{\pgfutil@ifnextchar[{\pgf@declareimage}{\pgf@declareimage[]}}
\def\pgf@declareimage[#1]#2#3{%
  \pgfqkeys{/pgf/images}{height=,width=,page=,interpolate=false,mask=,#1}%
  % Try to find the file
  \gdef\pgf@filename{}%
  % If page= parameter is not empty, try that file first:
  \ifx\pgf@imagepage\pgfutil@empty%
  \else%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3.page\pgf@imagepage}%
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \else%
    \pgfkeys{/pgf/images/page=}% make page empty
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \pgfwarning%
    {File "#3" not found when defining image "#2".
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
    \pgf@declaredraftimage{#2}{#3}%
  \else%
    \ifpgf@draftmode%
      \pgf@declaredraftimage{#2}{#3}%
    \else%
      \pgfsys@defineimage%
    \fi%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@image@#2!\endcsname=\pgf@image%
}


\pgfkeys{
    /pgf/images/draft/.is if=pgf@draftmode,
    /pgf/images/draft/.default=true}
\pgfkeys{/pgf/images/width/.estore in=\pgf@imagewidth}
\pgfkeys{/pgf/images/height/.estore in=\pgf@imageheight}
\pgfkeys{/pgf/images/page/.estore in=\pgf@imagepage}
\pgfkeys{/pgf/images/interpolate/.cd,.code=\edef\pgf@imageinterpolate{#1},.default=true}
\let\pgf@imageinterpolate\pgfutil@empty
\pgfkeys{/pgf/images/mask/.code=%
  {%
    \edef\pgf@imagemask{#1}%
    \ifx\pgf@imagemask\pgfutil@empty%
    \else%
      \pgfutil@ifundefined{pgf@mask@#1}%
      {\pgferror{Undefined mask "#1".}%
        \edef\pgf@imagemask{}}%
      {\edef\pgf@imagemask{\csname pgf@mask@#1\endcsname}%
      }%
    \fi%
  }}


\def\pgf@findfile#1:#2+#3{%
  \pgfutil@IfFileExists{#3#1}%
  {\xdef\pgf@filename{#3#1}}%
  {\def\pgf@mightbeempty{#2}%
    \ifx\pgf@mightbeempty\pgfutil@empty\else%
    \pgf@findfile#2+{#3}%
    \fi}}

% #1: image name
% #2: file name
\def\pgf@declaredraftimage#1#2{%
  \ifx\pgf@imagewidth\pgfutil@empty%
    \pgfwarning{Missing width for image "#1" ("#2") in draft mode. Using 1cm instead}%
    \edef\pgf@imagewidth{1cm}%
  \fi%
  \ifx\pgf@imageheight\pgfutil@empty%
    \pgfwarning{Missing height for image "#1" ("#2") in draft mode. Using 1cm instead}%
    \edef\pgf@imageheight{1cm}%
  \fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepagetext{ page \pgf@imagepage}\fi%
  \edef\pgf@image{%
    \hbox to \pgf@imagewidth{%
      \vrule\kern-0.4pt%
      \vbox to \pgf@imageheight{%
        \hrule\vfil%
        \hbox to \pgf@imagewidth{\hskip-10cm\hfil\noexpand\pgfutil@font@tiny#2\pgf@imagepage\hfil\hskip-10cm}%
        \vfil\hrule}%
      \kern-0.4pt\vrule}%
  }%
}



% Declare a soft mask
%
% #1 = optional argument: matte specification. default matte is
%      white.
% #2 = name of the mask for later use
% #3 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF. Postscript is not supported.
%
% Description:
%
% This command declares a soft mask for later masking an image. The
% declared mask should be used together with an image of exactly the
% same height/width if matte is defined. Matte should be the
% preblended background color (see pdf spec for details).
%
% Example:
%
% \pgfdeclaremask[matte=white]{maskname}{maskfilename}
% \pgfdeclareimage[mask=maskname]{image}{imagefilename}

\def\pgfdeclaremask{\pgfutil@ifnextchar[\pgf@declaremask{\pgf@declaremask[]}}
\def\pgf@declaremask[#1]#2#3{%
  \pgfqkeys{/pgf/images/mask}{matte={1 1 1},#1}% defaults
  \def\pgf@mask{}%
  % Try to find the file
  \gdef\pgf@filename{}%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \ifx\pgf@filename\pgfutil@empty%
    \pgfwarning%
    {File "#3" not found when defining mask "#2".
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
  \else%
    \pgfsys@definemask%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@mask@#2\endcsname=\pgf@mask%
}

\pgfkeys{/pgf/images/mask/matte/.cd,.estore in=\pgf@maskmatte,.value required}



% Create an alias name for an image
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfdeclareimage{image}{1cm}{1cm}{filename
% \pgfaliasimage{alias}{image}
% \pgfuseimage{alias}

\def\pgfaliasimage#1#2{%
  \expandafter\global\expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@image@#2!\endcsname%
  \expandafter\global\expandafter\let\csname pgf@image@#1!\endcsname=\pgf@temp%
  }


% Use an image
%
% #1 = name of a previously declared image
%
% Example:
%
% \pgfputat{\pgforigin}{\pgfbox[left,base]{\pgfuseimage{myimage}}}

\def\pgfuseimage#1{%
  \def\pgf@imagename{pgf@image@#1}%
  \pgf@tryextensions{\pgf@imagename}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@imagename}%
  {\pgferror{Undefined image "#1"}}%
  {{\leavevmode\csname\pgf@imagename\endcsname}}}

\def\pgf@tryextensions#1#2{%
  \edef\pgf@args{[#2!]}\expandafter\pgf@@tryextensions\pgf@args{#1}}
\def\pgf@@tryextensions[#1!#2]#3{%
  \expandafter\pgfutil@ifundefined\expandafter{#3#1!#2}%
  {\def\pgf@temp{#2}%
    \ifx\pgf@temp\pgfutil@empty%
    \edef#3{#3!}%
    \else%
    \pgf@@tryextensions[#2]{#3}%
    \fi}%
  {\edef#3{#3#1!#2}}}


% Alternate image
%
% Description:
%
% When an image is used, pgf first attempts to use the image with the
% alternate extension added. If this fails, the original image is
% used. If the alternate extension contains ``!'', then the text up to
% the ! is successively removed and the remainder is tried as an
% alternate extension.
%
% Example:
%
% \def\pgfalternateextension{20!white}

\def\pgfalternateextension{}



% Directly insert an image
%
% #1 = optional argument: width, height, page specification
% #2 = file name
%
% Description:
%
% Directly inserts an image without declaration. You can, however,
% still access this image using the name pgflastimage. By using
% pgfaliasimage, you can also save this image for later.
%
% Example:
%
% \pgfimage[height=2cm]{filename}

\def\pgfimage{\pgfutil@ifnextchar[\pgf@imagecom{\pgf@imagecom[]}}
\def\pgf@imagecom[#1]#2{%
  \pgfdeclareimage[#1]{pgflastimage}{#2}%
  \pgfuseimage{pgflastimage}}


\input pgfcoreexternal.code.tex

\endinput


==> pgfcorequick.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorequick.code.tex}

% Quick version of basic drawing commands. Most high-level commands
% are not available if these commands are used.

% Move current point to (#1,#2).
%
% #1 = x dimension of new current point
% #2 = y dimension of new current point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqmoveto#1#2{\pgfsyssoftpath@moveto{#1}{#2}}


% Append a line to (#1,#2) to the current path.
%
% #1 = x dimension of target
% #2 = y dimension of target
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqlineto#1#2{\pgfsyssoftpath@lineto{#1}{#2}}


% Append a bezier spline to the current path.
%
% #1 = x dimension of first support point
% #2 = y dimension of first support point
% #3 = x dimension of second support point
% #4 = y dimension of second support point
% #5 = x dimension of target point
% #6 = y dimension of target point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqcurveto#1#2#3#4#5#6{\pgfsyssoftpath@curveto{#1}{#2}{#3}{#4}{#5}{#6}}




% Append a circle of the given radius around the origin.
%
% #1 = radius
% 
% Example:
%
% \pgfpathqcircle{10pt}
% is quicker than
% \pgfpathcircle{\pgforigin}{10pt}

\def\pgfpathqcircle#1{%
  {%
    \pgf@x=#1%
    \pgf@y=0.5522847\pgf@x%
    \pgfsyssoftpath@moveto{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@y}{\the\pgf@x}{0pt}{\the\pgf@x}%
    \pgfsyssoftpath@curveto{-\the\pgf@y}{\the\pgf@x}{-\the\pgf@x}{\the\pgf@y}{-\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{-\the\pgf@x}{-\the\pgf@y}{-\the\pgf@y}{-\the\pgf@x}{0pt}{-\the\pgf@x}%
    \pgfsyssoftpath@curveto{\the\pgf@y}{-\the\pgf@x}{\the\pgf@x}{-\the\pgf@y}{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@closepath%
  }%
}



% Stroke current path. No hooks called.
% 
% Example:
%
% \pgfpathqmoveto{0cm}{0cm}
% \pgfpathqlineto{1cm}{1cm}
% \pgfpathqcurveto{2cm}{1cm}{2cm}{2cm}{3cm}{2cm}
% \pgfqstroke

\def\pgfusepathqstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@stroke%
  \pgf@resetpathsizes%
}


% Quickly fill current path.

\def\pgfusepathqfill{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fill%
  \pgf@resetpathsizes%
}


% Quickly fill and stroke current path.

\def\pgfusepathqfillstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fillstroke%
  \pgf@resetpathsizes%
}

% Quickly clip current path.

\def\pgfusepathqclip{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@clipnext%
  \pgfsys@discardpath%
  \pgf@resetpathsizes%
}


\endinput


==> pgfcorerdf.code.tex <==
% Copyright 2018 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcorerdf.code.tex}



% 
%
% The Resource Description Framework (RDF) is a method of enriching
% output files with semantic information. In PGF, you can use the
% following commands to create RDF information that will be inserted
% into the output, provided the output format allows this (SVG
% does). You call any of these commands before an ID-scope and it will
% attach the attribute(s) to this id scope.
%
%
% Example:
%
% ...
% \pgfrdftypeof{http://purl.org/dc/dcmitype/Image}
% \pgfrdfresource{/paper/figures/1}
% \pgfidscope
%   % This ID scope will be flagged as the resource "/paper/figures/1"
%   % and typeof "Image" from the Dublin Core.
%   ...
% \endidscope





% Adds the rdf attribute "about" with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a SafeCURIEorCURIEorIRI, used for stating what
% the data is about (a 'subject' in RDF terminology);" 

\def\pgfrdfabout#1{\pgfsys@rdf@about{#1}}



% Adds the rdf attribute content with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a CDATA string, for supplying machine-readable
% content for a literal (a 'literal object', in RDF terminology);"  

\def\pgfrdfcontent#1{\pgfsys@rdf@content{#1}}



% Adds the rdf attribute datatype with value #1 to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a TERMorCURIEorAbsIRI representing a datatype,
% to express the datatype of a literal;" 

\def\pgfrdfdatatype#1{\pgfsys@rdf@datatype{#1}}



% Adds the rdf attribute href with value #1 to the next idscope
% The RDF-spec says: "a traditionally navigable IRI for
% expressing the partner resource of a relationship (a 'resource object', in RDF terminology);" 

\def\pgfrdfhref#1{\pgfsys@rdf@href{#1}}



% Adds the rdf attribute inlist to the next idscope.
%
% Description:
%
% The RDF-spec says: "An attribute used to indicate that the object
% associated with a rel or property attribute on the same element is
% to be added to the list for that predicate. Presence of this
% attribute causes a list to be created if it does not already exist."   

\def\pgfrdfinlist{\pgfsys@rdf@inlist}




% Adds #1 to the list of the rdf prefix attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called several times, in which case all values of #1 are
% concatenated with whitespaces. The RDF-spec says: "a white space
% separated list of prefix-name IRI pairs of the form NCName ':' ' '+
% xsd:anyURI"  

\def\pgfrdfprefix#1{\pgfsys@rdf@prefix{#1}}




% Adds #1 to the list of the rdf property attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between a subject and either a resource object if
% given or some literal text (also a 'predicate');"  

\def\pgfrdfproperty#1{\pgfsys@rdf@property{#1}}



% Adds #1 to the list of the rdf rel attribute to the next
% next idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between two resources ('predicates' in RDF
% terminology);" 

\def\pgfrdfrel#1{\pgfsys@rdf@rel{#1}}


% Adds the rdf attribute resource with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "a SafeCURIEorCURIEorIRI for expressing the
% partner resource of a relationship that is not intended to be
% navigable (e.g., a 'clickable' link) (also an 'object');"  

\def\pgfrdfresource#1{\pgfsys@rdf@resource{#1}}




% Adds #1 to the list of the rdf rev attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing reverse
% relationships between two resources (also 'predicates');

\def\pgfrdfrev#1{\pgfsys@rdf@rev{#1}}




% Adds an rdf attribute src with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "an IRI for expressing the partner resource of a
% relationship when the resource is embedded (also a 'resource object');" 

\def\pgfrdfsrc#1{\pgfsys@rdf@src{#1}}




% Adds #1 to the list of the rdf typeof attribute to the next
% idscope.
%
% #1 = A URL
%
% Description:
%
% Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs that indicate the RDF type(s)
% to associate with a subject;" 

\def\pgfrdftypeof#1{\pgfsys@rdf@typeof{#1}}




% Adds an rdf attribute vocab with value #1 to the next idscope.
%
% #1 = A URL
%
% Description:
%
% The RDF-spec says: "an IRI that defines the mapping to use when a
% TERM is referenced in an attribute value. See General Use of Terms
% in Attributes and the section on Vocabulary Expansion."  

\def\pgfrdfvocab#1{\pgfsys@rdf@vocab{#1}}





\endinput


==> pgfcoreshade.code.tex <==
% Copyright 2019 by Till Tantau
% CMYK and grayscale shadings adaptation copyright 2019 by David Purton
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfcoreshade.code.tex}

%
% Parsing functions
%
\newdimen\pgf@max
\newcount\pgf@sys@shading@range@num
\def\pgf@parsefunc#1{%
  \edef\temp{{#1}}%
  \expandafter\pgf@convertstring\temp%
  \edef\temp{{\pgf@conv}}%
  \expandafter\pgf@@parsefunc\temp}
\def\pgf@@parsefunc#1{%
  \let\pgf@bounds=\pgfutil@empty%
  \let\pgf@funcs=\pgfutil@empty%
  \let\pgf@psfuncs=\pgfutil@empty%
  \let\pgf@encode=\pgfutil@empty%
  \let\pgf@sys@shading@ranges=\pgfutil@empty%
  \pgf@sys@shading@range@num=0\relax%
  \csname pgf@parsefirst\pgf@shading@model\endcsname[#1; ]%
  \csname pgf@parselastdom\pgf@shading@model\endcsname[#1; ]%
  \csname pgf@parsemid\pgf@shading@model\endcsname[#1; ]%
  \ifx\pgf@bounds\pgfutil@empty%
    \edef\pgf@pdfparseddomain{0 1}%
    \edef\pgf@pdfparsedfunction{\pgf@singlefunc\space}%
  \else%
    \edef\pgf@pdfparseddomain{\pgf@doma\space\pgf@domb}%
    \edef\pgf@pdfparsedfunction{%
      << /FunctionType 3 /Domain [\pgf@doma\space\pgf@domb] /Functions
      [\pgf@funcs\space] /Bounds [\pgf@bounds] /Encode [0 1 \pgf@encode]
      >> }% <<
  \fi%
  \xdef\pgf@psfuncs{\pgf@psfuncs}%
  }
\def\pgf@parsefirstrgb[rgb(#1)=(#2,#3,#4)#5]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
  \edef\pgf@sys@shading@start@rgb{\pgf@sys@rgb}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@rgb%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@rgb}%
  \edef\pgf@firstcolor{\pgf@rgb}}
\def\pgf@parselastdomrgb[rgb(#1)=(#2,#3,#4); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@end@rgb{\pgf@sys@rgb}%
    \pgfutil@gobble}{\pgf@parselastdomrgb[}}
\def\pgf@parsemidrgb[rgb(#1)=(#2,#3,#4); {\pgf@parserestrgb[}
\def\pgf@parserestrgb[rgb(#1)=(#2,#3,#4); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@rgb}%
    \pgf@parserestrgb[}}

\def\pgf@getrgbtuplewithmixin#1#2#3{%
  \pgfutil@definecolor{pgfshadetemp}{rgb}{#1,#2,#3}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@getrgb@@\pgf@rgbcolor!}
\def\pgf@getrgb@@#1,#2,#3!{%
  \def\pgf@rgb{#1 #2 #3}%
  \def\pgf@sys@rgb{{#1}{#2}{#3}}%
}

\def\pgf@parsefirstcmyk[cmyk(#1)=(#2,#3,#4,#5)#6]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
  \edef\pgf@sys@shading@start@cmyk{\pgf@sys@cmyk}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@cmyk%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@cmyk}%
  \edef\pgf@firstcolor{\pgf@cmyk}}
\def\pgf@parselastdomcmyk[cmyk(#1)=(#2,#3,#4,#5); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@sys@shading@end@cmyk{\pgf@sys@cmyk}%
    \pgfutil@gobble}{\pgf@parselastdomcmyk[}}
\def\pgf@parsemidcmyk[cmyk(#1)=(#2,#3,#4,#5); {\pgf@parserestcmyk[}
\def\pgf@parserestcmyk[cmyk(#1)=(#2,#3,#4,#5); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space
      \pgf@cmyk\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@cmyk}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@cmyk%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getcmyktuplewithmixin{#2}{#3}{#4}{#5}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@cmyk}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@cmyk%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@cmyk\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@cmyk] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@cmyk}%
    \pgf@parserestcmyk[}}

\def\pgf@getcmyktuplewithmixin#1#2#3#4{%
  \pgfutil@definecolor{pgfshadetemp}{cmyk}{#1,#2,#3,#4}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{cmyk}{\pgf@cmykcolor}%
  \expandafter\pgf@getcmyk@@\pgf@cmykcolor!}
\def\pgf@getcmyk@@#1,#2,#3,#4!{%
  \def\pgf@cmyk{#1 #2 #3 #4}%
  \def\pgf@sys@cmyk{{#1}{#2}{#3}{#4}}%
}

\def\pgf@parsefirstgray[gray(#1)=(#2)#3]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getgraytuplewithmixin{#2}%
  \edef\pgf@sys@shading@start@gray{\pgf@sys@gray}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@gray%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@gray}%
  \edef\pgf@firstcolor{\pgf@gray}}
\def\pgf@parselastdomgray[gray(#1)=(#2); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@sys@shading@end@gray{\pgf@sys@gray}%
    \pgfutil@gobble}{\pgf@parselastdomgray[}}
\def\pgf@parsemidgray[gray(#1)=(#2); {\pgf@parserestgray[}
\def\pgf@parserestgray[gray(#1)=(#2); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@gray\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@gray}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@gray%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getgraytuplewithmixin{#2}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{%
      {\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@gray}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@gray%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@gray\space
      \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@gray] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@gray}%
    \pgf@parserestgray[}}

\def\pgf@getgraytuplewithmixin#1{%
  \pgfutil@definecolor{pgfshadetemp}{gray}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{gray}{\pgf@graycolor}%
  \expandafter\pgf@getgray@@\pgf@graycolor!}
\def\pgf@getgray@@#1!{%
  \def\pgf@gray{#1}%
  \def\pgf@sys@gray{{#1}}%
}

% Normalized a <color specification> argument for shadings into a
% series of color specifications in the current xcolor color model and write
% the result into \pgf@conv.
%
% Example:
% \pgf@convertstring{rgb(0cm)=(1,0,0); rgb(2cm)=(0,1,0); cmyk(4cm)=(1,0,0,0); gray(1cm)=(3);  color(2cm)=(green); }
% ->
% \pgf@conv = macro:->'rgb(0cm)=(1,0,0); rgb(2cm)=(0,1,0); rgb(4cm)=(0,1,1); rgb(1cm)=(3,3,3); rgb(2cm)=(0,1,0); '
\def\pgf@convertstring#1{%
  \def\pgf@conv{}%
  \pgf@convert#1]%
  }
\def\pgf@convert{%
  \pgfutil@ifnextchar]{\pgfutil@gobble}%done!
  {%
    \pgfutil@ifnextchar;{\pgf@grabsemicolor}%
    {%
      \pgfutil@ifnextchar c{\pgf@gobblec}%
      {%
        \pgfutil@ifnextchar g{\pgf@grabgray}%
        {%
          \pgfutil@ifnextchar o{\pgf@grabcolor}%
          {%
            \pgfutil@ifnextchar m{\pgf@grabcmyk}%
            {%
              \pgfutil@ifnextchar r{\pgf@grabrgb}%
                {\pgferror{Illformed shading
                 specification}\pgf@convert}%
            }%
          }%
        }%
      }%
    }%
  }%
}
\def\pgf@savecolor#1{%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor
    {\pgf@shading@model}{\pgf@color}%
  \expandafter\pgf@convget@\expandafter{\pgf@color}{#1}%
}
\def\pgf@grabsemicolor;{%
  \edef\pgf@conv{\pgf@conv; }\pgf@convert}
\def\pgf@gobblec c{\pgf@convert}
\def\pgf@grabrgb rgb(#1)=(#2,#3,#4){%
  \pgfutil@definecolor{pgf@tempcol}{rgb}{#2,#3,#4}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabcmyk myk(#1)=(#2,#3,#4,#5){%
  \pgfutil@definecolor{pgf@tempcol}{cmyk}{#2,#3,#4,#5}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabgray gray(#1)=(#2){%
  \pgfutil@definecolor{pgf@tempcol}{gray}{#2}%
  \pgf@savecolor{#1}%
}
\def\pgf@grabcolor olor(#1)=(#2){%
  \pgfutil@colorlet{pgf@tempcol}{#2}%
  \pgf@savecolor{#1}%
}
\def\pgf@convget@#1#2{%
  \edef\pgf@conv{\pgf@conv \pgf@shading@model(#2)=(#1)}\pgf@convert}


\newcount\pgf@shadingcount
\pgf@shadingcount=0
{
  \catcode`\/=0
  \catcode`\\=12
  /gdef/pgf@shadingnum{\/the/pgf@shadingcount\}
}

% Set up shading properties based on the current xcolor color model. This is
% called when shadings are declared and used. \ifpgfshadingmodelrgb,
% \ifpgfshadingmodelcmyk, and \ifpgfshadingmodelgray are set so that the type
% 4 function in functional shadings can be converted to the current color
% model. See \pgffuncshading*to* macros.

\newif\ifpgfshadingmodelrgb
\newif\ifpgfshadingmodelcmyk
\newif\ifpgfshadingmodelgray
\def\pgf@setup@shading@model{%
  \pgfshadingmodelrgbtrue
  \pgfshadingmodelcmykfalse
  \pgfshadingmodelgrayfalse
  \XC@sdef\pgf@mod@test{\XC@tgt@mod{natural}}%
  \def\pgf@shading@device{/DeviceRGB}%
  \def\pgf@shading@ps@device{setrgbcolor}%
  \def\pgf@shading@functional@range{0 1 0 1 0 1}%
  \def\pgf@shading@model{rgb}%
  \ifx\pgf@mod@test\XC@mod@cmyk
    \def\pgf@shading@device{/DeviceCMYK}%
    \def\pgf@shading@ps@device{setcmykcolor}%
    \def\pgf@shading@functional@range{0 1 0 1 0 1 0 1}%
    \def\pgf@shading@model{cmyk}%
    \pgfshadingmodelrgbfalse
    \pgfshadingmodelcmyktrue
  \fi
  \ifx\pgf@mod@test\XC@mod@gray
    \def\pgf@shading@device{/DeviceGray}%
    \def\pgf@shading@ps@device{setgray}%
    \def\pgf@shading@functional@range{0 1}%
    \def\pgf@shading@model{gray}%
    \pgfshadingmodelrgbfalse
    \pgfshadingmodelgraytrue
  \fi
  \edef\pgf@sys@driver@dvisvgm{pgfsys-dvisvgm.def}%
  \ifx\pgfsysdriver\pgf@sys@driver@dvisvgm
    \def\pgf@shading@model{rgb}%
  \fi
  \edef\pgf@sys@driver@texforht{pgfsys-tex4ht.def}%
  \ifx\pgfsysdriver\pgf@sys@driver@texforht
    \def\pgf@shading@model{rgb}%
  \fi
}


% Declares a horizontal shading for later use. The shading is a
% horizontal bar that changes its color.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification in the following format: A list of colors
%      that the bar should have at certain points. If the bar should
%      be red at 1cm, this is specified as
%      "rgb(1cm)=(1,0,0)". Multiple specifications are separated by a
%      semicolon and a space. At least two specifications must be
%      given. The specified positions must be given in increasing
%      order.
%
% Description:
%
% The optional dependencies have the following effect: If present, it
% should consist of a list of colors, separated by commas. Each time
% the shading is used, these colors will be reevaluated. It will be
% checked whether the colors still have their "original meaning". If
% the colors have changed, a new shading will be created internally to
% reflect the changed color's values.
%
% Example:
%
% \pgfdeclarehorizontalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm long: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclarehorizontalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declarehorizontalshading{\pgf@declarehorizontalshading[]}}
\def\pgf@declarehorizontalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname\pgfutil@empty
    \pgfsys@horishading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@horishading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a vertical shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification
%
% Example:
%
% \pgfdeclareverticalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm high: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareverticalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declareverticalshading{\pgf@declareverticalshading[]}}
\def\pgf@declareverticalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfsys@vertshading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@vertshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a radial shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = center of inner circle
% #4 = color specification
%
% Description:
%
% A radial shading creates a smooth color transition between two
% circles. The center of the inner circle is at the give position. Its
% radius is the start of the color specification. The
% center of the outer circle is at the center of the whole shading,
% whose radius is the end of the color specification. For example,
% suppose the color specification is "rgb(1cm)=(1,1,1); rgb(2cm)=(0,0,0)".
% Then the shading would be 4cm times 4cm large. The inner circle would
% have diameter 1cm and the outer circle would have diameter 2cm. The
% outer circle would be centered in the middle of the shading, whereas
% the outer circle would be centered at the given position.
%
% Example:
%
% \pgfdeclareradialshading{redtogreentoblue}{\pgfpoint{2cm}{2cm}}{%
%   rgb(10pt)=(1,0,0); % red
%   rgb(2cm)=(0,1,0); % green
%   rgb(3cm)=(0,0,1)}
%
% \begin{document}
%   The following ball has diameter 3cm: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareradialshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declareradialshading{\pgf@declareradialshading[]}}
\def\pgf@declareradialshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfsys@radialshading{#2}{#3}{#4}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@radialshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}




% Declares a functional shading for later use.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = lower left corner of the shading as a pgfpoint.
% #4 = upper right corner of the shading as a pgfpoint.
% #5 = Preparation code
% #6 = a PDF type 4 function (restricted Postscript function), see the
%      PDF-specification 1.7, section 3.9.4
%
% Description:
%
% This command creates a so-called functional shading. For such a
% shading the color of each point is calculated by calling a function
% for each point that gets the coordinates as input and yields the
% color as an output. Note that the function is evaluated by the
% *renderer*, not by PGF or TeX or someone else at compile-time. This
% means that the evaluation of this function has to be done *extremely
% quickly* and the function should be *very simple*. For this reason,
% only a very restricted set of operations are possible in the
% function (see 3.9.4 of the PDF-spec 1.7). Also functions should be
% kept small. Any errors in the function will only be noticed by the
% renderer.
%
% The function gets the coordinates of a point as input (as bp). This
% input consists of the top two elements of an otherwise empty
% (virtual, PostScript) stack. The function should then replace these
% two values by one value representing the gray color of the point for a
% grayscale shading, three values, representing the red, green, and blue color
% of the point for an RGB shading, or four values, representing the cyan,
% magenta, yellow, and black color of the point for a CMYK shading. The
% numbers should be real values, not integers since Apple's PDF renderer is
% broken in this regard (use cvr at the end if necessary).
%
% Conceptually, the function will be evaluated once for each point of
% the rectangle (#3) to (#4). A renderer may choose to evaluate the
% function at less points, but, in principle, the function will be
% evaluated for each pixel independently.
%
% Because of the rather difficult PostScript syntax, use this macro
% only *if you know what you are doing* (or if you are adventurous, of
% course).
%
% As for other shadings, the optional dependencies argument is used to
% determine whether a shading needs to be recalculated when a color
% has changed.
%
% The code #5 is executed each time a shading is
% (re)calculated. Typically, it will contain code to extract
% coordinates from colors (see below).
%
% Inside the PostScript function #6 you cannot use colors
% directly. Rather, you must push the color components on the
% stack. For this, it is useful to call \pgfshadecolortorgb,
% \pgfshadecolortocmyk, or \pgfshadecolortogray in the startup
% code #4. The macro takes a color name as input and stores the color's
% component real numbers between 0.0 and 1.0 separated
% by spaces (which is exactly what you need if you want to push it on
% a stack) in a macro.
%
% Example:
%
%\pgfdeclarefunctionalshading{twospots}{\pgfpointorigin}{\pgfpoint{200bp}{200bp}}{}{
%  2 copy
%  90 sub dup mul exch
%  80 sub dup mul add sqrt
%  dup mul neg 1.0005 exch exp 1.0 exch sub
%  3 1 roll
%  120 sub dup mul exch
%  100 sub dup mul add sqrt
%  dup mul neg 1.002 exch exp 1.0 exch sub
%  1.0
%}
%
% \pgfdeclarefunctionalshading[mycol]{sweep}{\pgfpointorigin}{\pgfpoint{100bp}{100bp}}
% {\pgfshadecolortorgb{mycol}{\myrgb}}{
%   add 150 div   % not very useful...
%   dup
%   \myrgb        % push mycol
%   5 4 roll      % multiply all components by calculated value
%   mul
%   3 1 roll
%   3 index
%   mul
%   3 1 roll
%   4 3 roll
%   mul
%   3 1 roll
% }
%
% \begin{document}
%   Have a look at this: \pgfuseshading{twospots}.
%   Here is \colorlet{mycol}{green!50}\pgfuseshading{sweep} in green
%   and in \colorlet{mycol}{red!50!blue}\pgfuseshading{sweep} in red/blue.
% \end{document}

\def\pgfdeclarefunctionalshading{%
  \pgf@setup@shading@model
  \pgfutil@ifnextchar[%
    \pgf@declarefunctionalshading{\pgf@declarefunctionalshading[]}}
\def\pgf@declarefunctionalshading[#1]#2#3#4#5#6{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \global\expandafter\let\csname pgf@num@pgfshading#2!\endcsname=\pgfutil@empty
    \pgfshade@functionaldo{#2}{#3}{#4}{#5}{#6}%
  \else%
    \global\advance\pgf@shadingcount 1\relax
    \global\expandafter\edef\csname pgf@num@pgfshading#2!\endcsname{\pgf@shadingnum}%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfshade@functionaldo}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}{#5}{#6}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}
\def\pgfshade@functionaldo#1#2#3#4#5{%
  \begingroup
    #4%
    \pgfsys@functionalshading{#1}{#2}{#3}{#5}%
    \expandafter\pgfmath@smuggleone\csname @pgfshading#1!\endcsname
  \endgroup
}

\def\pgfshadecolortorgb#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgfshading@rgb\pgf@rgbcolor\relax%
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space\pgf@sys@tonumber{\pgf@xb}\space\pgf@sys@tonumber{\pgf@xc}\space}%
  \c@pgf@counta\escapechar%
  \escapechar-1\relax%
  \expandafter\edef\csname\string#2red\endcsname{\pgf@sys@tonumber{\pgf@xa}\space}%
  \expandafter\edef\csname\string#2green\endcsname{\pgf@sys@tonumber{\pgf@xb}\space}%
  \expandafter\edef\csname\string#2blue\endcsname{\pgf@sys@tonumber{\pgf@xc}\space}%
  \escapechar\c@pgf@counta%
}
\def\pgfshading@rgb#1,#2,#3\relax{%
  \pgf@xa=#1pt%
  \pgf@xb=#2pt%
  \pgf@xc=#3pt%
}

\def\pgfshadecolortocmyk#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{cmyk}{\pgf@cmykcolor}%
  \expandafter\pgfshading@cmyk\pgf@cmykcolor\relax%
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space\pgf@sys@tonumber{\pgf@xb}\space
    \pgf@sys@tonumber{\pgf@xc}\space\pgf@sys@tonumber{\pgf@xd}\space}%
  \c@pgf@counta\escapechar%
  \escapechar-1\relax%
  \expandafter\edef\csname\string#2cyan\endcsname{%
    \pgf@sys@tonumber{\pgf@xa}\space}%
  \expandafter\edef\csname\string#2magenta\endcsname{%
    \pgf@sys@tonumber{\pgf@xb}\space}%
  \expandafter\edef\csname\string#2yellow\endcsname{%
    \pgf@sys@tonumber{\pgf@xc}\space}%
  \expandafter\edef\csname\string#2black\endcsname{%
    \pgf@sys@tonumber{\pgf@xd}\space}%
  \escapechar\c@pgf@counta
}
\def\pgfshading@cmyk#1,#2,#3,#4\relax{%
  \pgf@xa=#1pt%
  \pgf@xb=#2pt%
  \pgf@xc=#3pt%
  \pgf@xd=#4pt%
}

\def\pgfshadecolortogray#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{gray}{\pgf@graycolor}%
  \expandafter\pgfshading@gray\pgf@graycolor\relax
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space}%
  \c@pgf@counta\escapechar
  \escapechar-1\relax
  \expandafter\edef\csname\string#2gray\endcsname{%
    \pgf@sys@tonumber{\pgf@xa}\space}%
  \escapechar\c@pgf@counta
}
\def\pgfshading@gray#1\relax{%
  \pgf@xa=#1pt%
}

% Functions to convert between color models in the type 4 PostScript data of
% functional shadings.

\def\pgffuncshadingrgbtocmyk{%
  1.0 exch sub 3 1 roll
  1.0 exch sub 3 1 roll
  1.0 exch sub 3 1 roll
  3 copy
  2 copy gt { exch } if pop
  2 copy gt { exch } if pop
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll sub
  0.0 2 copy lt { exch } if pop
  1.0 2 copy gt { exch } if pop
  4 1 roll
}

\def\pgffuncshadingrgbtogray{%
  0.11 mul exch 0.59 mul add exch 0.3 mul add
}

\def\pgffuncshadingcmyktorgb{%
  % covert to CMY
  dup 3 1 roll add
  1.0 2 copy gt { exch } if pop
  4 1 roll
  dup 3 1 roll add
  1.0 2 copy gt { exch } if pop
  4 1 roll
  add
  1.0 2 copy gt { exch } if pop
  3 1 roll
  % covert to RGB
  1.0 exch sub
  3 1 roll
  1.0 exch sub
  3 1 roll
  1.0 exch sub
  3 1 roll
}

\def\pgffuncshadingcmyktogray{%
  exch 0.11 mul add exch 0.59 mul add exch 0.3 mul add
  1.0 2 copy gt { exch } if pop
  1.0 exch sub
}

\def\pgffuncshadinggraytorgb{%
  dup dup
}

\def\pgffuncshadinggraytocmyk{%
  0.0 0.0 0.0
  4 3 roll
}

% Inserts a box into the text that contains a previously defined
% shading.
%
% #1 = Name of a shading
%
% Example:
%
% \pgfuseshading{redtogreentoblue}

\def\pgfuseshading#1{%
  \edef\pgf@shadingname{@pgfshading#1}%
  \pgf@tryextensions{\pgf@shadingname}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@shadingname}%
  {\pgferror{Undefined shading "#1"}}%
  {%
    \edef\pgf@shade@adds{\csname pgf@num\pgf@shadingname\endcsname}%
    \pgfutil@ifundefined{pgf@deps\pgf@shadingname}%
    {}%
    {%
      \pgf@setup@shading@model
      \begingroup
        \pgfutil@globalcolorsfalse
        \edef\@list{\csname pgf@deps\pgf@shadingname\endcsname}%
        \pgfutil@for\@temp:=\@list\do{%
          \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{\@temp}}%
          \pgfutil@extractcolorspec{\@temp}{\pgf@tempcolor}%
          \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{\pgf@shading@model}{\pgf@color}%
          \edef\pgf@shade@adds{\pgf@shade@adds,\pgf@color}%
        }%
        \pgfmath@smuggleone\pgf@shade@adds
      \endgroup
    }%
    \expandafter\pgf@strip@shadename\pgf@shadingname!!%
    \edef\pgf@shadingxname{@pgfshading\pgf@basename\pgf@shade@adds!}%
    \pgfutil@ifundefined{\pgf@shadingxname}%
    {%
      \begingroup
        \edef\@temp{\expandafter\noexpand\csname pgf@func\pgf@shadingname\endcsname}%
        \edef\@args{{\pgf@basename\pgf@shade@adds}}%
        \expandafter\expandafter\expandafter\def
        \expandafter\expandafter\expandafter\@@args
        \expandafter\expandafter\expandafter{\csname pgf@args\pgf@shadingname\endcsname}%
        \expandafter\expandafter\expandafter\@temp\expandafter\@args\@@args
        \expandafter\pgfmath@smuggleone\csname\pgf@shadingxname\endcsname
      \endgroup
    }%
    {}%
    \pgf@invokeshading{\csname\pgf@shadingxname\endcsname}%
  }%
}

\def\pgf@strip@shadename @pgfshading#1!!!{\def\pgf@basename{#1}}

\def\pgf@invokeshading#1{%
  \ifpgfpicture%
    \pgfsys@shadinginsidepgfpicture{#1}%
  \else%
    \pgfsys@shadingoutsidepgfpicture{#1}%
  \fi%
}


% Create an alias name for a shading
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfaliasshading{shading!25}{shadingshaded}

\def\pgfaliasshading#1#2{%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname @pgfshading#2!\endcsname%
  \expandafter\let\csname @pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@num@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@num@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@deps@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@deps@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@func@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@func@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@args@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@args@pgfshading#1!\endcsname=\pgf@temp%
}




% Shades the current path, but does not discard it.
%
% #1 - a shading (see below)
% #2 - an angle
%
% Description:
%
% \pgfshadepath  ``tries'' to fill the
% current path with a shading. The shading's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% shading will be rotated by #2 and then rescaled so that it
% completely covers the path. Then the path will be used (locally) for
% clipping and the shading is drawn.
%
% In addition to the rotation, any transformation set by the
%\pgfsetadditionalshadetransform will also be applied.
%
% After all this, the path can still be used for the normal
% stroking/clipping operations.
%
% The shading is rotated around its middle. If no rotation occurs, the
% lower left corner of the path will lie on (25bp, 25bp), the upper
% right corner on (75bp, 75bp).
%
% Example:
%
% \pgfdeclareverticalshading{myshading}{100bp}{color(0pt)=(red); color(100bp)=(green)}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfshadepath{myshading}{0}
% \pgfusepath{stroke}

\def\pgfshadepath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    \pgfwarning{No path specified that can be filled}%
  \else%
    \begingroup%
      % Calculate center:
      \pgf@xb=.5\pgf@pathmaxx%
      \advance\pgf@xb by.5\pgf@pathminx%
      \pgf@yb=.5\pgf@pathmaxy%
      \advance\pgf@yb by.5\pgf@pathminy%
      % Calculate rotation:
      \pgfmathparse{#2}%
      \let\pgfshade@angle=\pgfmathresult
      \pgfmathsin@\pgfshade@angle
      \let\pgfshade@sin=\pgfmathresult
      \pgfmathcos@\pgfshade@angle
      \let\pgfshade@cos=\pgfmathresult
      % width and height of the bounding box
      \pgf@xa=\pgf@pathmaxx
      \advance\pgf@xa by-\pgf@pathminx
      \pgf@ya=\pgf@pathmaxy
      \advance\pgf@ya by-\pgf@pathminy
      % Calculate scaling:
      % xscale = 1pt/50bp * (w*|cos(a)|+h*|sin(a)|)/(|cos(a)|+|sin(a)|)
      % yscale = 1pt/50bp * (w*|sin(a)|+h*|cos(a)|)/(|cos(a)|+|sin(a)|)
      % 1pt/50bp = .01992528
      \pgfmathabs@\pgfshade@sin
      \let\pgfshade@abssin=\pgfmathresult
      \pgfmathabs@\pgfshade@cos
      \let\pgfshade@abscos=\pgfmathresult
      \pgf@xc=\pgfshade@abscos\pgf@xa
      \advance\pgf@xc by\pgfshade@abssin\pgf@ya
      \pgf@yc=\pgfshade@abssin\pgf@xa
      \advance\pgf@yc by\pgfshade@abscos\pgf@ya
      \pgfmathadd@\pgfshade@abscos\pgfshade@abssin
      \pgfmathdivide@{.01992528}{\pgfmathresult}%
      \pgf@xc=\pgfmathresult\pgf@xc
      \pgf@yc=\pgfmathresult\pgf@yc
      \ifdim\pgf@xc<0.0001pt
        \ifdim\pgf@xc>-0.0001pt
          \pgf@no@shadetrue
        \fi
      \fi
      \ifdim\pgf@yc<0.0001pt
        \ifdim\pgf@yc>-0.0001pt
          \pgf@no@shadetrue
        \fi
      \fi
      \ifpgf@no@shade\else
        \pgfsys@beginscope
          \pgfsyssoftpath@invokecurrentpath
          \pgfsys@clipnext
          \pgfsys@discardpath
          % Compute new transformation matrix:
          % shift
          \pgfsys@transformcm{1}{0}{0}{1}{\the\pgf@xb}{\the\pgf@yb}%
          % rotation
          \pgf@x=\pgfshade@sin pt%
          \pgf@xa=-\pgf@x%
          \pgfsys@transformcm{\pgfshade@cos}{\pgfshade@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgfshade@cos}{0pt}{0pt}%
          % scaling
          \pgfsys@transformcm{\pgf@sys@tonumber{\pgf@xc}}{0}{0}{\pgf@sys@tonumber{\pgf@yc}}{0pt}{0pt}%
          % This will actually be the first transformation of the shading.
          % Should it be applied first so that it becomes the last one?
          \ifx\pgf@shade@extra@transform\pgfutil@empty%
          \else%
            \pgflowlevel{\pgf@shade@extra@transform}%
          \fi%
          \pgfuseshading{#1}%
        \pgfsys@endscope%
      \fi%
    \endgroup%
  \fi%
}

\newif\ifpgf@no@shade

% Additionally transform shade paths
%
% #1 = Transformation code that is used in addition to the normal
%      shading transformation.
%
% Example:
%
% \pgfsetadditionalshadetransform{\pgftransformrotate{30}}

\def\pgfsetadditionalshadetransform#1{\def\pgf@shade@extra@transform{#1}}
\let\pgf@shade@extra@transform=\pgfutil@empty





\endinput


==> pgffor.code.tex <==
% Copyright 2019 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgffor.code.tex}

% pgfmath is needed
\input pgfmath.code.tex

\newdimen\pgffor@iter
\newdimen\pgffor@skip
\newif\ifpgffor@continue


\def\pgffor@reset@hooks{%
  \let\pgffor@beginhook=\relax%
  \let\pgffor@endhook=\relax%
  \let\pgffor@afterhook=\relax%
}
\pgffor@reset@hooks


% Stack emulation
%
\newtoks\pgffor@stack
\pgffor@stack={{}{}{}}

\def\pgffor@stackpush#1{%
    \def\pgffor@stacktemp{#1}%
    \expandafter\expandafter\expandafter\pgffor@stack\expandafter\expandafter\expandafter=%
    \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
        {\expandafter\pgffor@stacktemp\expandafter}\the\pgffor@stack}%
}

\def\pgffor@stackpop{\expandafter\pgffor@@stackpop\the\pgffor@stack\pgffor@stackstop}
\def\pgffor@@stackpop#1#2\pgffor@stackstop{\pgffor@stack{#2}#1}

\def\pgffor@emptyvalues{, \pgffor@stop,}%

\def\pgffor@foreach{%
    \pgffor@atbeginforeach%
    \let\pgffor@assign@before@code=\pgfutil@empty%
    \let\pgffor@assign@after@code=\pgfutil@empty%
    \let\pgffor@assign@once@code=\pgfutil@empty%
    \let\pgffor@remember@code=\pgfutil@empty%
    \let\pgffor@remember@once@code=\pgfutil@empty%
    \pgffor@alphabeticsequencefalse%
    \pgffor@contextfalse%
    %
    \let\pgffor@var=\pgfutil@empty
    %
    \pgffor@vars%
}

\let\foreach=\pgffor@foreach

\def\pgffor@vars{%
    \pgfutil@ifnextchar i{\pgffor@@vars@end}{%
        \pgfutil@ifnextchar[{\pgffor@@vars@opt}{%]
            \pgfutil@ifnextchar/{\pgffor@@vars@slash@gobble}{%
                \pgffor@@vars}}}}%

\def\pgffor@@vars@end in{\pgfutil@ifnextchar\bgroup{\pgffor@normal@list}{\pgffor@macro@list}}
\def\pgffor@@vars@opt[#1]{\pgfkeys{/pgf/foreach/.cd,#1}\pgffor@vars}
\def\pgffor@@vars#1{\pgffor@var@add#1\pgffor@stop\pgffor@vars}
\def\pgffor@@vars@slash@gobble/{\pgffor@@vars}

\def\pgffor@var@add#1#2\pgffor@stop{%
    \ifx\pgffor@var\pgfutil@empty%
        \def\pgffor@var{#1}%
        \def\pgffor@mainvar{#1}%
    \else%
        \expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@var/#1}%
    \fi%
}

\def\pgffor@expand@list@true{\let\pgffor@expand@list\edef}
\def\pgffor@expand@list@false{\let\pgffor@expand@list\def}
\def\pgffor@macro@list#1{%
  \expandafter\pgffor@normal@list\expandafter{#1}}
\def\pgffor@normal@list#1{%
  \pgffor@expand@list\pgffor@values{#1}%
  \expandafter\def\expandafter\pgffor@values\expandafter{\pgffor@values, \pgffor@stop,}%
  \ifx\pgffor@values\pgffor@emptyvalues
    \def\pgffor@values{\pgffor@stop,}%
  \fi%
  \let\pgffor@body=\pgfutil@empty%
  \global\pgffor@continuetrue%
  \pgffor@collectbody}
\def\pgffor@collectbody{%
  \pgfutil@ifnextchar\foreach{\pgffor@collectforeach}{%
    \pgfutil@ifnextchar\bgroup{\pgffor@collectargument}{\pgffor@collectsemicolon}}%
}

\def\pgffor@collectforeach\foreach#1in{%
  \pgfutil@ifnextchar\bgroup{\pgffor@collectforeach@normal{#1}}{\pgffor@collectforeach@macro{#1}}}
\def\pgffor@collectforeach@macro#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in#2}%
  \pgffor@collectbody%
}
\def\pgffor@collectforeach@normal#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in{#2}}%
  \pgffor@collectbody%
}
\long\def\pgffor@collectargument#1{%
    \expandafter\pgfutil@in@\expandafter\foreach\expandafter{\pgffor@body}%
    \ifpgfutil@in@%
        \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter%
    {\pgffor@body{#1}}%
    \else%
        \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter%
    {\pgffor@body#1}%
    \fi%
  \pgffor@iterate%
}

\def\pgffor@collectsemicolon{%
  \let\pgffor@next=\pgffor@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\pgffor@next=\pgffor@collectactivesemicolon%
  \fi%
  \pgffor@next%
}

\def\pgffor@collectnormalsemicolon#1;{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
  \pgffor@iterate%
}

{
  \catcode`\;=\active

  \gdef\pgffor@collectactivesemicolon#1;{%
    \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
    \pgffor@iterate%
  }
}

\def\pgffor@iterate{%
  % Must do all of these in case the internal stack is used.
  \let\pgffor@last=\pgfutil@empty%
  \let\pgffor@prevlast=\pgfutil@empty%
  \let\pgffor@dotsend=\pgfutil@empty%
  \let\pgffor@dots@pre=\pgfutil@empty%
  \let\pgffor@dots@post=\pgfutil@empty%
  %
  \expandafter\pgffor@scan\pgffor@values}

\def\pgffor@stop{\pgffor@stop}%
\def\pgffor@dots{...}%

\def\pgffor@scan{\pgfutil@ifnextchar({\pgffor@scanround}{\pgffor@scanone}}
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)#2}\pgffor@scanned}
\def\pgffor@scanone#1,{\def\pgffor@value{#1}\pgffor@scanned}


% Check for dots.
\newif\ifpgffor@dots@in@
\def\pgffor@dots@in@#1...#2#3\pgffor@stop{%
    \ifx\pgffor@dots@@#2%
        \pgffor@dots@in@false%
    \else%
        \pgffor@dots@in@true%
    \fi%
}

\def\pgffor@dots@@{\pgffor@dots@@}

\def\pgffor@scanned{%
  \ifx\pgffor@value\pgffor@stop%
    \let\pgffor@next=\pgffor@after% Done!
  \else%
    % Check for dots. Quicker than \pgfutil@in@ and not suceptable
        % to false-positives when a token sequence ends in a single full-stop.
    \expandafter\pgffor@dots@in@\pgffor@value\pgffor@dots@...\pgffor@dots@@\pgffor@stop%
    \ifpgffor@dots@in@%
      \let\pgffor@next=\pgffor@handledots%
    \else%
      \let\pgffor@next=\pgffor@handlevalue%
    \fi%
    \ifpgffor@continue%
    \else%
      \let\pgffor@next=\pgffor@scan% Done!
    \fi%
  \fi%
  \pgffor@next}


\def\pgffor@after{%
  \global\pgffor@continuetrue%
  \pgffor@atendforeach%
  \pgffor@afterhook}

\def\pgffor@handlevalue{%
    \let\pgffor@prevlast=\pgffor@last%
  \let\pgffor@last=\pgffor@value%
  \pgffor@invokebody%
  \pgffor@scan%
}


\def\pgffor@invokebody{%
  \pgffor@begingroup%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@value//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@value}%
    \fi%
    % Execute assign once code.
    \ifx\pgffor@assign@once@code\pgfutil@empty%
    \else%
        \pgffor@assign@once@code%
    \fi%
    % Execute assign before code.
    \ifx\pgffor@assign@before@code\pgfutil@empty%
    \else%
        \pgffor@assign@before@code%
    \fi%
    %
    \expandafter\expandafter\expandafter\pgffor@reset@hooks\expandafter\pgffor@beginhook\expandafter\pgffor@body\pgffor@endhook%
    % Execute assign after code.
    \ifx\pgffor@assign@after@code\pgfutil@empty%
    \else%
        \pgffor@assign@after@code%
    \fi%
    %
  \pgffor@endgroup%
}


\def\pgffor@multiassign#1/#2/\relax{%
  \def\pgffor@currentvar{#1}%
  \def\pgffor@rest{#2}%
  \ifx\pgffor@currentvar\pgffor@stop%
    \let\pgffor@next=\relax%
  \else%
    \let\pgffor@next=\pgffor@multiassignrest%
  \fi%
  \pgffor@next%
}

\def\pgffor@multiassignrest{\expandafter\pgffor@multiassignfinal\pgffor@valuerest}
\def\pgffor@multiassignfinal#1/#2/\relax{%
    \def\pgffor@temp{#1}%
    \ifx\pgffor@currentvar\pgffor@mainvar%
        \ifpgffor@alphabeticsequence%
        \pgffor@makealphabetic\pgffor@temp%
    \fi%
  \fi%
  \def\pgffor@test{#2}%
  \ifx\pgffor@test\pgfutil@empty%
    \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}% repeat
  \else%
    \def\pgffor@valuerest{#2/\relax}%
  \fi%
  \expandafter\expandafter\expandafter\def\expandafter\pgffor@currentvar\expandafter{\pgffor@temp}%
    %
  \expandafter\pgffor@multiassign\pgffor@rest/\relax%
}

\def\pgffor@gobblespaces#1{\pgfutil@ifnextchar x{#1}{#1}}

\def\pgffor@handledots{%
    \pgffor@gobblespaces{\expandafter\pgffor@@handledots\pgffor@value\pgffor@@stop}%
}

\newif\ifpgffor@context

\def\pgffor@@handledots#1...#2\pgffor@@stop{%
    % Define the context if any.
    \def\pgffor@dots@pre{#1}%
    \def\pgffor@dots@post{#2}%
    \def\pgffor@dots@stripcontext#1##1#2\pgffor@@stop{\def\pgffor@dotsvalue{##1}}%
    \pgffor@contexttrue%
    \ifx\pgffor@dots@pre\pgfutil@empty%
        \ifx\pgffor@dots@post\pgfutil@empty%
            \pgffor@contextfalse%
            \def\pgffor@dots@stripcontext##1\pgffor@@stop{\def\pgffor@dotsvalue{##1}}%
        \fi%
    \fi%
    \pgffor@gobblespaces{\pgffor@dotsscanend}%
}

\def\pgffor@dots@value@process#1{%
    \expandafter\pgffor@dots@stripcontext#1\pgffor@@stop%
    \expandafter\pgffor@dots@charcheck\pgffor@dotsvalue\pgffor@@stop%
  \ifpgffor@alphabeticsequence
  \else
    \ifpgffor@assign@parse
      \begingroup
      \pgfkeys{/pgf/fpu/false/.try}%
      \pgfmathparse{\pgffor@dotsvalue}%
      \pgfmath@smuggleone\pgfmathresult
      \endgroup
      \let\pgffor@dotsvalue=\pgfmathresult
    \fi
  \fi
  \let#1=\pgffor@dotsvalue%
}

\def\pgffor@dotsscanend#1,{%
    \pgffor@alphabeticsequencefalse%
    % Strip context and check for a character sequence.
    \def\pgffor@dotsend{#1}%
    \pgffor@dots@value@process{\pgffor@dotsend}%
  %
  \pgffor@dots@value@process{\pgffor@last}%
  %
  % calculate skip%
  \ifx\pgffor@prevlast\pgfutil@empty%
    \ifdim\pgffor@dotsend pt>\pgffor@last pt%
      \pgffor@skip=1pt%
    \else%
      \pgffor@skip=-1pt%
    \fi%
  \else%
    \pgffor@dots@value@process{\pgffor@prevlast}%
    \pgffor@skip=\pgffor@last pt%
    \pgffor@iter=\pgffor@prevlast pt%
    \advance\pgffor@skip by-\pgffor@iter%
  \fi%
  \pgffor@iter=\pgffor@last pt%
  % do loop
  \pgffor@loop%
}

\def\pgffor@loop{%
  \advance\pgffor@iter by\pgffor@skip%
  \let\pgffor@next=\pgffor@doloop%
  \ifdim\pgffor@skip<0pt%
    \ifdim\pgffor@iter<\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \else%
    \ifdim\pgffor@iter>\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \fi%
  \ifpgffor@continue%
  \else%
    \let\pgffor@next=\pgffor@endloop% Done!
  \fi%
  \pgffor@next%
}

\def\pgffor@endloop{%
    \pgffor@alphabeticsequencefalse%
    \pgffor@scan%
}

{\catcode`\p=12\catcode`\t=12\gdef\Pgffor@geT#1pt{#1}}

\def\pgffor@doloop{%
  \pgffor@begingroup
    \edef\pgffor@temp{\expandafter\Pgffor@geT\the\pgffor@iter}%
    \edef\pgffor@incheck{{.0/}{\pgffor@temp/}}%
    \expandafter\pgfutil@in@\pgffor@incheck%
    \ifpgfutil@in@%
      \expandafter\pgffor@strip\pgffor@temp%
    \fi%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
        % Convert to alphabetic sequence, if necessary.
        \ifpgffor@alphabeticsequence%
            \pgffor@makealphabetic\pgffor@temp%
            \expandafter\let\pgffor@var=\pgffor@temp%
        \else%
            \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@temp}%
      \fi%
    \fi%
    % Insert any context, if any.
    \ifpgffor@context%
      \let\pgffor@temp=\pgffor@dots@pre%
        \expandafter\pgfutil@append@macrotomacro\expandafter%
            {\expandafter\pgffor@temp\expandafter}\expandafter{\pgffor@var}%
        \expandafter\pgfutil@append@macrotomacro\expandafter%
            {\expandafter\pgffor@temp\expandafter}\expandafter{\pgffor@dots@post}%
        \expandafter\let\pgffor@var=\pgffor@temp%
      \fi%
      % Perform assignments before loop body.
      \ifx\pgffor@assign@before@code\pgfutil@empty%
    \else%
        \pgffor@assign@before@code%
    \fi%
    %
    \expandafter\expandafter\expandafter\pgffor@reset@hooks\expandafter\pgffor@beginhook\expandafter\pgffor@body\pgffor@endhook%
    %
    % Perform assignments after loop body.
      \ifx\pgffor@assign@after@code\pgfutil@empty%
    \else%
        \pgffor@assign@after@code%
    \fi%
  \pgffor@endgroup%
  \pgffor@loop%
}

\def\pgffor@strip#1.0{\def\pgffor@temp{#1}}

\def\breakforeach{\global\pgffor@continuefalse}

\def\pgffor@gobbletil@pgffor@@stop#1\pgffor@@stop{}


\newif\ifpgffor@registeriscount

\def\pgffor@ifcsregister#1{%
    \expandafter\pgffor@@ifcsregister\meaning#1\pgffor@stop}

\def\pgffor@@ifcsregister#1#2#3#4#5\pgffor@stop{%
    \if#1m% It is an ordinary (m)acro.
        \pgffor@registeriscountfalse%
        \let\pgffor@csnext=\pgfutil@secondoftwo%
    \else%
        \if#1u% It is (u)ndefined.
            \let\pgffor@csnext=\pgfutil@secondoftwo%
            \pgffor@registeriscountfalse%
        \else%
            \let\pgffor@csnext=\pgfutil@firstoftwo%
            \if#4u% It is a co(u)nt
                \pgffor@registeriscounttrue%
            \else% Assume it is a dimen or skip (bad assumption in the general case).
                \pgffor@registeriscountfalse%
                \let\pgffor@csnext=\pgfutil@firstoftwo%
            \fi%
        \fi%
    \fi%
    \pgffor@csnext}

\newif\ifpgffor@alphabeticsequence

%
\def\pgffor@dots@charcheck#1\pgffor@@stop{%
  \edef\pgffor@dots@charcheck@temp{#1}%
  \expandafter\expandafter\expandafter\pgffor@@dotscharcheck\expandafter\meaning\pgffor@dots@charcheck@temp\pgffor@@stop%
}
\def\pgffor@@dotscharcheck#1#2\pgffor@@stop{%
    \if#1t%
    \afterassignment\pgffor@gobbletil@pgffor@@stop%
      \expandafter\chardef\expandafter\pgffor@char\expandafter=\expandafter`\pgffor@dots@charcheck@temp\relax\pgffor@@stop%
      \edef\pgffor@char{\the\pgffor@char}%
      \ifnum\pgffor@char>64\relax% From A-Z?
        \ifnum\pgffor@char<91\relax%
          \let\pgffor@dotsvalue=\pgffor@char%
          \pgffor@alphabeticsequencetrue%
        \else%
          \ifnum\pgffor@char>96\relax% From a-z?
            \ifnum\pgffor@char<123\relax%
              \let\pgffor@dotsvalue=\pgffor@char%
              \pgffor@alphabeticsequencetrue%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
}

\def\pgffor@makealphabetic#1{%
    % Convert the number in the macro passed as #1 to a-z or A-Z.
    \pgfutil@tempcnta=#1\relax%
    \ifnum\pgfutil@tempcnta>95\relax%
        \advance\pgfutil@tempcnta by-96\relax%
        \edef#1{\pgffor@alpha\pgfutil@tempcnta}%
    \else%
        \advance\pgfutil@tempcnta by-64 %
        \edef#1{\pgffor@Alpha\pgfutil@tempcnta}%
    \fi%
}

\def\pgffor@Alpha#1{%
    \ifcase#1\relax\or A\or B\or C\or D\or E\or F\or G\or H\or I\or J\or K\or L\or M%
    \or N\or O\or P\or Q\or R\or S\or T\or U\or V\or W\or X\or Y\or Z\else?\fi%
}

\def\pgffor@alpha#1{%
    \ifcase#1\relax\or a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or l\or m%
    \or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or y\or z\else?\fi%
}

\newtoks\pgffor@toks

\def\pgffor@addcstotoks#1{%
    \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\expandafter\def\expandafter#1\expandafter{#1}}%
    \pgffor@@addcstotoks}

\def\pgffor@addregtotoks#1{%
    \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\expandafter#1\expandafter=\the#1}%
    \pgffor@@addcstotoks}

\def\pgffor@addiftotoks#1{%
    \begingroup%
        \escapechar=-1\relax%
            \expandafter\pgffor@@addiftotoks\string#1\pgffor@stop}
\def\pgffor@@addiftotoks#1#2#3#4\pgffor@stop{%
    \endgroup
    \csname if#3#4\endcsname%
        \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\csname#3#4true\endcsname}%
    \else%
        \expandafter\def\expandafter\pgffor@tokstemp\expandafter{\csname#3#4false\endcsname}%
    \fi%
    \pgffor@@addcstotoks%
}

\def\pgffor@@addcstotoks{%
    \expandafter\expandafter\expandafter\pgffor@toks\expandafter\expandafter\expandafter=%
    \expandafter\expandafter\expandafter{\expandafter\pgffor@tokstemp\the\pgffor@toks}%
}

% Set up the pgffor scopes.

\def\pgffor@atbeginforeach{%
    \begingroup%
}

\def\pgffor@atendforeach{%
        \global\edef\pgffor@remember@expanded{\pgffor@remember@code}%
        \ifx\pgffor@remember@expanded\pgfutil@empty%
        \else%
          \pgffor@remember@expanded%
          \global\let\pgffor@remember@expanded=\pgfutil@empty%
        \fi%
    \endgroup%
}
\def\pgffor@default@begingroup{%
    \begingroup%
}

\let\pgffor@remember@once@expanded=\pgfutil@empty
\let\pgffor@remember@expanded=\pgfutil@empty

\def\pgffor@default@endgroup{%
   \ifx\pgffor@remember@once@code\pgfutil@empty
   \else
     \xdef\pgffor@remember@once@expanded{\pgffor@remember@once@code}%
   \fi
   \ifx\pgffor@remember@code\pgfutil@empty
   \else
     \xdef\pgffor@remember@expanded{\pgffor@remember@code}%
   \fi
 \endgroup
 %
 \ifx\pgffor@remember@once@expanded\pgfutil@empty
 \else
   \pgffor@remember@once@expanded%
   % \let\pgffor@assign@once@code=\pgfutil@empty % Not needed anymore? (CJ)
   \global\let\pgffor@remember@once@expanded=\pgfutil@empty
 \fi
 \ifx\pgffor@assign@once@code\pgfutil@empty
 \else
   \global\let\pgffor@assign@once@code=\pgfutil@empty
 \fi
 %
 \ifx\pgffor@remember@expanded\pgfutil@empty
 \else
   \pgffor@remember@expanded%
   \global\let\pgffor@remember@expanded=\pgfutil@empty
 \fi
}

\let\pgffor@begingroup=\pgffor@default@begingroup
\let\pgffor@endgroup=\pgffor@default@endgroup


\def\pgffor@stack@begingroup{%
    \pgffor@toks={}%
    \pgffor@addcstotoks{\pgffor@mainvar}%
    \pgffor@addcstotoks{\pgffor@var}%
    \pgffor@addcstotoks{\pgffor@body}%
    %
    \pgffor@addcstotoks{\pgffor@last}%
    \pgffor@addcstotoks{\pgffor@prevlast}%
    \pgffor@addcstotoks{\pgffor@dotsend}%
    %
    \pgffor@addcstotoks{\pgffor@assign@before@code}%
    \pgffor@addcstotoks{\pgffor@assign@after@code}%
    \pgffor@addcstotoks{\pgffor@remember@code}%
    \pgffor@addcstotoks{\pgffor@remember@once@code}%
    \pgffor@addcstotoks{\pgffor@dots@pre}%
    \pgffor@addcstotoks{\pgffor@dots@post}%
    %
    \pgffor@addregtotoks{\pgffor@iter}%
    \pgffor@addregtotoks{\pgffor@skip}%
    %
    \pgffor@addiftotoks{\ifpgffor@alphabeticsequence}%
    \pgffor@addiftotoks{\ifpgffor@context}%
    \expandafter\pgffor@stackpush\expandafter{\the\pgffor@toks}%
}

\def\pgffor@stack@endgroup{\pgffor@stackpop}

% Keys stuff.

\newif\ifpgffor@assign@evaluate
\newif\ifpgffor@assign@once
\newif\ifpgffor@assign@parse

\pgfkeys{/pgf/foreach/.cd,
    var/.code=\pgffor@var@add#1\pgffor@stop,
    scope iterations/.code={
        \csname if#1\endcsname%
            \let\pgffor@begingroup=\pgffor@default@begingroup%
            \let\pgffor@endgroup=\pgffor@default@endgroup%
        \else%
            \let\pgffor@begingroup=\pgffor@stack@begingroup%
            \let\pgffor@endgroup=\pgffor@stack@endgroup%
        \fi%
    },
    evaluate/.code=\pgffor@assign@evaluatetrue\pgffor@assign@oncefalse\pgffor@assign@parse{#1},%
    assign/.code=\pgffor@assign@evaluatefalse\pgffor@assign@oncefalse\pgffor@assign@parse{#1},%
    evaluate once/.code=\pgffor@assign@evaluatetrue\pgffor@assign@oncetrue\pgffor@assign@parse{#1},%
    assign once/.code=\pgffor@assign@evaluatefalse\pgffor@assign@oncetrue\pgffor@assign@parse{#1},%
    remember/.code=\pgffor@remember@parse{#1},%
    count/.code=\pgffor@count@parse#1\pgffor@stop,
    parse/.is if=pgffor@assign@parse,
    parse/.default=false,
    expand list/.is if=pgffor@expand@list@,
    expand list/.default=true,
    expand list=false,
}

\def\pgffor@assign@parse#1{%
    \pgfutil@in@;{#1}%
    \ifpgfutil@in@%
    \else%
        \pgfutil@in@={#1}%
    \fi%
    \ifpgfutil@in@%
        \pgffor@assign@@parse#1;\pgffor@stop;%
    \else%
        \pgffor@assign@parse@old#1\pgffor@stop%%
    \fi%
}

\def\pgffor@stop{\pgffor@stop}
\def\pgffor@assign@@parse#1;{%
    \def\pgffor@test{#1}%
    \ifx\pgffor@test\pgffor@stop%
        \let\pgffor@next=\relax%
    \else%
        \let\pgffor@next=\pgffor@assign@@parse%
        \ifx\pgffor@test\pgfutil@empty%
        \else%
            \pgfutil@in@={#1}%
            \ifpgfutil@in@%
                \pgffor@assign@@@parse#1\pgffor@stop%
            \else%
                \pgffor@assign@@@parse#1=#1\pgffor@stop%
            \fi%
        \fi%
    \fi%
    \pgffor@next}

\def\pgffor@assign@@@parse#1=#2\pgffor@stop{%
    \ifpgffor@assign@evaluate%
        \ifpgffor@assign@once%
            \pgfutil@append@tomacro{\pgffor@assign@once@code}{\pgfmathparse{#2}\let#1=\pgfmathresult}%
            \pgfutil@append@tomacro{\pgffor@remember@once@code}{\noexpand\def\noexpand#1{#2}}%
        \else
            \pgfutil@append@tomacro{\pgffor@assign@before@code}{\pgfmathparse{#2}\let#1=\pgfmathresult}%
        \fi%
    \else%
        \ifpgffor@assign@once%
            \pgfutil@append@tomacro{\pgffor@assign@once@code}{\def#1{#2}}%
            \pgfutil@append@tomacro{\pgffor@remember@once@code}{\noexpand\def\noexpand#1{#2}}%
        \else
            \pgfutil@append@tomacro{\pgffor@assign@before@code}{\def#1{#2}}%
        \fi%
    \fi%
}

\def\pgffor@assign@parse@old#1#2\pgffor@stop{%
    \pgffor@assign@@parse@old#2\pgffor@stop as#1using #1\pgffor@@stop}

\def\pgffor@assign@@parse@old#1as#2#3\pgffor@@stop{%
    \pgffor@assign@@@parse@old{#2}#1#3\pgffor@stop\pgffor@@stop}

\def\pgffor@assign@@@parse@old#1#2using #3\pgffor@stop#4\pgffor@@stop{%
    \pgffor@assign@@@parse#1=#3\pgffor@stop}



\def\pgffor@remember@parse#1{%
    \pgfutil@in@ a{#1}% This matches the 'a' in 'as' or 'initially'.
    \ifpgfutil@in@%
        \pgffor@remember@parse@old#1\pgffor@stop%
    \else%
        \pgffor@remember@@parse#1;\pgffor@stop;%
    \fi%
}

\def\pgffor@remember@@parse#1;{%
    \def\pgffor@test{#1}%
    \ifx\pgffor@test\pgffor@stop%
        \let\pgffor@next=\relax%
    \else%
        \let\pgffor@next=\pgffor@remember@@parse%
        \ifx\pgffor@test\pgfutil@empty%
        \else%
            \pgfutil@in@={#1}%
            \ifpgfutil@in@%
                \pgffor@remember@@@parse#1\pgffor@stop%
            \else%
                \pgffor@ifcsregister{#1}{%
                    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand#1=\the#1\noexpand\relax}%
                }%
                {%
                    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
                }%
            \fi%
        \fi%
    \fi%
    \pgffor@next%
}

\def\pgffor@remember@@@parse#1=#2\pgffor@stop{%
    \pgffor@ifcsregister{#2}{%
        \pgfutil@append@tomacro{\pgffor@assign@after@code}{\expandafter\def\expandafter#1\expandafter{\the#2}}%
        \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
    }%
    {%
        \pgfutil@append@tomacro{\pgffor@assign@after@code}{\expandafter\def\expandafter#1\expandafter{#2}}%
        \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#1{#1}}%
    }%
}

\def\pgffor@remember@parse@old#1#2\pgffor@stop{%
    \pgffor@remember@@parse@old#1#2\pgffor@stop as#1(initially 0)\pgffor@@stop}

\def\pgffor@remember@@parse@old#1#2as#3#4\pgffor@@stop{%
    \pgffor@remember@@@parse@old{#1}{#3}#2#4\pgffor@stop\pgffor@@stop}

\def\pgffor@remember@@@parse@old#1#2#3(initially #4)#5\pgffor@stop#6\pgffor@@stop{%
    \pgfutil@append@tomacro{\pgffor@assign@after@code}{\edef#2{#1}}%
    \pgfutil@append@tomacro{\pgffor@remember@code}{\noexpand\def\noexpand#2{#2}}%
    \pgfutil@append@tomacro{\pgffor@assign@once@code}{\def#2{#4}}%
}

\def\pgffor@count@parse#1#2\pgffor@stop{%
    \pgffor@count@@parse#1#2\pgffor@stop from 1\pgffor@stop\pgffor@@stop}

\def\pgffor@count@@parse#1#2from#3\pgffor@stop#4\pgffor@@stop{%
    \pgfutil@append@tomacro\pgffor@remember@code{\noexpand\def\noexpand#1{#1}}%
    \pgfutil@append@tomacro\pgffor@assign@before@code{\pgfmathparse{int(#1+1)}\let#1=\pgfmathresult}%
    \pgfmathparse{int(#3-1)}\let#1=\pgfmathresult%
}


\def\pgfutil@append@macrotomacro#1#2{%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
        #1\expandafter\expandafter\expandafter{\expandafter#1#2}}

\def\pgfutil@append@tomacro#1#2{%
    \expandafter\def\expandafter#1\expandafter{#1#2}}


\endinput


==> pgfint.code.tex <==
% Copyright 2019 by Henri Menke
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% Guard against reading twice
\ifx\pgfintloaded\pgfutil@undefined
  \let\pgfintloaded=\relax
\else
  \expandafter\endinput
\fi

% This module is pretty much a rip-off of the LaTeX3 l3int module for integer
% calculations.  Since PGF supports e-TeX now, we can make use of those
% extended facilities.

% In contrast to l3int we will just admit that integers are regular TeX \count
% register and will not implement an extra "integer datatype".

% Evaluate an integer expression using \numexpr
\def\pgfinteval#1{\number\numexpr#1\relax}

% Get the absolute value of an integer by stripping off a leading minus sign
\def\pgfintabs#1{\number\expandafter\pgfint@abs\number\numexpr#1\relax}
\def\pgfint@abs#1{\ifx-#1\else\expandafter#1\fi}

% Minimum and maximum
\def\pgfintmax#1#2{%
  \number\expandafter\pgfint@minmax
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  >
}
\def\pgfintmin#1#2{%
  \number\expandafter\pgfint@minmax
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  <
}
\def\pgfint@minmax#1;#2;#3{%
  \ifnum#1#3#2
    #1%
  \else
    #2%
  \fi
}

% \numexpr has the annoying property to round divisions rather than truncating
% (as you would expect for integer arithmetic).  Therefore we need a truncating
% division function.
\def\pgfintdivtruncate#1#2{%
  \number\numexpr\expandafter\pgfint@divtruncate
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@divtruncate#1#2;#3#4;{%
  \ifx0#1
    0%
  \else
    (#1#2%
      \ifx-#1 +\else-\fi
      (\ifx-#3 -\fi#3#4-1)/2%
    )%
  \fi
  /#3#4%
}

% \pgfintdivtruncate always truncates the result which leads to a rounding
% towards zero.  Donald Knuth defines in TAoCP, Vol 1, 3rd Ed, Section 1.2.4
% that the modulo operation is
%
%    x mod y = x - y * floor(x/y)
%
% In contrast to truncated division, floored division always rounds towards
% -inf, i.e. floor(1/2) = 0 and floor(-1/2) = -1.  This is also how integer
% division is done in Lua.
\def\pgfintdivfloor#1#2{%
  \number\numexpr\expandafter\pgfint@divfloor
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@divfloor#1#2;#3#4;{%
  \ifx0#1
    0%
  \else
    \ifnum
      0\ifx-#1\ifx#3-\else1\fi\fi
      0\ifx-#3\ifx#1-\else1\fi\fi
      >0
      \pgfint@@divfloor#1#2;#3#4;-+%
    \else
      \pgfint@@divfloor#1#2;#3#4;+-%
    \fi
  \fi
  /#3#4%
}
\def\pgfint@@divfloor#1#2;#3#4;#5#6{%
  (#1#2%
  \ifx-#1 #5\else#6\fi
    (\ifx-#3 -\fi#3#4#61)/2%
  )%
}

% Round
\def\pgfintdivround#1#2{\number\numexpr(#1)/(#2)\relax}

% Modulo
\def\pgfintmod#1#2{%
  \number\numexpr\expandafter\pgfint@mod%
  \number\numexpr#1\expandafter;%
  \number\numexpr#2;%
  \relax
}
\def\pgfint@mod#1;#2;{#1-(\pgfint@divfloor#1;#2;)*#2}

% Setter function so we don't always have to write \pgfinteval
\def\pgfintset#1#2{#1 \numexpr#2\relax}

\endinput


==> pgfkeys.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% The files pgfkeys.code.tex and pgfkeysfiltered.code.tex are
% perfectly self-contained, except that the catcode of @
% should be made a letter.


% Guard against reading twice
\ifx\pgfkeysloaded\undefined
  \let\pgfkeysloaded=\relax
\else
  \expandafter\endinput
\fi

% The purpose of this file is to provide a general settings engine that
% works with all TeX formats and has no save-stack impact

\def\pgfkeys@empty{}
\long\def\pgfkeys@firstoftwo#1#2{#1}
\long\def\pgfkeys@secondoftwo#1#2{#2}

% This is useful:

\ifx\PackageError\undefined
  \def\pgfkeys@error#1{\errmessage{Package pgfkeys Error: #1}}%
\else
  \def\pgfkeys@error#1{\PackageError{pgfkeys}{#1}{}}%
\fi

\ifx\eTeXrevision\undefined%
  \pgfkeys@error{PGF requires etex in extended mode}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

\ifnum\eTeXversion<2
  \pgfkeys@error{PGF requires etex version 2}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

% e-TeX primitives and beyond

\ifx\contextversion\undefined
  \let\pgfkeys@expanded   \expanded
  \let\pgfkeys@unexpanded \unexpanded
\else
  \let\pgfkeys@expanded   \normalexpanded
  \let\pgfkeys@unexpanded \normalunexpanded
\fi


% Set a key to a value
%
% #1 = key
% #2 = tokens
%
% Description:
%
% This command sets the key to the given tokens. The tokens are stored as
% is and can even contain things like #9.
%
% Keys are organized hierarchically using something similar to Unix
% paths. Thus, a typically key might be called "/tikz/length" or
% "/tikz/length dimension/.@cmd". Some keys starting with a dot are
% special, so they should not be used as normal key names (they are
% similar to Unix files starting with a dot -- you can use them, but
% be careful).
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyssetvalue{/tikz/length}{2cm-3cm}
% \pgfkeyssetvalue{/algo/swap}{{#2}{#1}}

\long\def\pgfkeyssetvalue#1#2{%
  \pgfkeys@temptoks{#2}\expandafter\edef\csname pgfk@#1\endcsname{\the\pgfkeys@temptoks}%
}

\long\def\pgfkeyssetevalue#1#2{%
  \expandafter\edef\csname pgfk@#1\endcsname
  {\pgfkeys@unexpanded\expandafter{\pgfkeys@expanded{#2}}}%
}

% Add text to a key at the end
%
% #1 = key
% #2 = a value to be added at the beginning
% #3 = a value to be added at the end
%
% Description:
%
% This command adds #2 to the definition of the key. The key should
% have been set previously using \pgfkeyssetvalue.
%
% Example:
%
% \pgfkeysaddvalue{/tikz/length}{}{-3cm}

\long\def\pgfkeysaddvalue#1#2#3{%
  {%
    \toks0{#2}%
    \pgfkeysifdefined{#1}
    {\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@#1\endcsname}}%
    {\pgfkeys@temptoks{}}%
    \toks1{#3}%
    \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1}% believe or don't: the spaces are important
  }%
  \pgfkeyslet{#1}\pgfkeys@global@temp%
}



% Makes a key equal a given code
%
% #1 = key
% #2 = a code name
%
% Description:
%
% This command executes a \let command so that a key gets the same
% value as the parameter #2.
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyslet{/algo/swap}{\myswap}

\def\pgfkeyslet#1#2{%
  \expandafter\let\csname pgfk@#1\endcsname#2%
}


% Retrieve the code stored in a key into a code
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will set #2 to "point" to the value stored in the key.
%
% Example:
%
% \pgfkeysgetvalue{/tikz/swap}{\myswap}

\def\pgfkeysgetvalue#1#2{\expandafter\let\expandafter#2\csname pgfk@#1\endcsname}



% Retrieve the value stored in a key
%
% #1 = key
%
% Description:
%
% This command will expand to the value stored in the key. The key
% should previously have been set using \pgfkeyasetkey or \pgfkeyslet.
%
% Example:
%
% The length is \pgfkeysvalue{/tikz/length}.

\def\pgfkeysvalueof#1{\csname pgfk@#1\endcsname}



% If for testing whether a key exists
%
% #1 = key
% #2 = if-case
% #3 = else-case
%
% Description:
%
% This if will be executed if the key exists. In eTeX mode this works
% like a normal if, in normal TeX mode you need to provide an \else.
%
% Example:
%
% \pgfkeysifdefined{/tikz/length}{key exists}{does not exist}

\long\def\pgfkeysifdefined#1{%
  \ifcsname pgfk@#1\endcsname
    \expandafter\pgfkeys@firstoftwo
  \else
    \expandafter\pgfkeys@secondoftwo
  \fi
}

% Tests whether a key is assignable. For standard keys which just
% store their value, this is identical to \pgfkeysifdefined.
%
% But \pgfkeysifassignable is true for command keys as well (but not
% for handled keys).
\long\def\pgfkeysifassignable#1#2#3{%
  \pgfkeysifdefined{#1}%
    {#2}
  {\pgfkeysifdefined{#1/.@cmd}%
    {#2}%
    {#3}}%
}%



% Execute settings
%
% #1 = list of settings
%
% Description:
%
% The list of settings should contain comma-separated settings. Each
% setting has the following form:
%
% /path/key=value
%
% The parts "/path/" and "=value" are optional. When the path is not
% specified, the value of the token register "\pgfkeypath" is used. If
% "=value" is missing, the value of the setting "/path/key/.@def" is used
% instead. If this key is set to "\pgfvaluerequired", the key
% "/errors/value required/.@cmd" is executed. This error handler,
% like all other error handlers, will get the current key as its first
% parameter (unexpanded) and the current value as its second value
% (also unexpanded).
%
% Any spaces at the beginning and at the end and around the
% equals-sign are removed. The key with the complete path is set to
% the code \pgfcurrentkey.
%
% The setting is then processed according to the following rules:
%
% 1) If the key /path/key/.@cmd" is present, its code is executed
%    with the value computed above, followed by \pgfeov (end of
%    value). So, to handle
%
%    "/stuff/height=  1.5 ,"
%
%    /stuff/height/.@cmd should be set to some code, that can
%    handle the parameter
%
%    "1.5\pgfeov"
%
%    For instance, saying
%
%    \pgfkeys{/stuff/height/.@cmd}{#1\pgfeov}{\def\myheight{#1}}
%
%    will do nicely.
%
% 2) Otherwise, if the key /path/key is present, this key is
%    set to the value computed above.
%
% 3) Otherwise, if the key /handlers/key/.@cmd is present, it is executed
%    with the same parameters as in 1). Additionally, the
%    token register \pgfcurrentkeypath will be set to "/path/" and the
%    macro \pgfcurrentkeywithoutpath to "key". So, in the above
%    example if neither "/stuff/height/.@cmd" nor
%    "/stuff/height" is present, but "/handlers/height" is,
%    then "/handlers/height" is executed with the parameters:
%
%    "1.5\pgfeov"
%
%    and \pgfcurrentkey is set to "/stuff/height" and \pgfcurrentkeypath
%    is set to "/stuff/" and \pgfcurrentkeywithoutpath to "height".
%
% 4) Otherwise, if the key "/path/.unknown/.@cmd" is present, its code is
%    executed with the same parameters as in 3).
%
% 5) Otherwise, the key "/handlers/.unknown/.@cmd" is executed with the same
%    parameters as in 1).
%
% After all settings have been processed, the value of the token
% register \pgfdefaultkeypath is set to its original value. Thus, any local
% change of this token register has no effect outside the call.
%
% Example:
%
% \pgfkeys{/tikz/.is family}
% \pgfkeys{/tikz/line width/.cd,
%         .def=\pgfsetlinewidth{##1},
%         .set default=.4pt}
% \pgfkeys{tikz,line width=1pt}

\newtoks\pgfkeys@pathtoks
\def\pgfkeyscurrentpath{\the\pgfkeys@pathtoks}
\newtoks\pgfkeys@temptoks

\def\pgfkeys@root{/}
\let\pgfkeysdefaultpath\pgfkeys@root

\def\pgfkeys{\expandafter\pgfkeys@@set\expandafter{\pgfkeysdefaultpath}}%
\long\def\pgfkeys@@set#1#2{%
  \let\pgfkeysdefaultpath\pgfkeys@root%
  \pgfkeys@parse#2,\pgfkeys@mainstop%
  \def\pgfkeysdefaultpath{#1}}

\def\pgfkeys@parse{\futurelet\pgfkeys@possiblerelax\pgfkeys@parse@main}
\def\pgfkeys@parse@main{%
  \ifx\pgfkeys@possiblerelax\pgfkeys@mainstop%
    \expandafter\pgfkeys@cleanup%
  \else%
    \expandafter\pgfkeys@normal%
  \fi%
}
\newif\ifpgfkeys@syntax@handlers
\def\pgfkeys@normal{%
  \ifpgfkeys@syntax@handlers%
    \expandafter\pgfkeys@syntax@handlers%
  \else%
    \expandafter\pgfkeys@@normal%
  \fi%
}
\def\pgfkeys@syntax@handlers{\pgf@keys@utilifnextchar\relax\pgfkeys@syntax@@handlers\pgfkeys@syntax@@handlers}%get rid of spaces
\def\pgfkeys@syntax@@handlers{\futurelet\pgfkeys@first@char\pgfkeys@syntax@handlers@test}
\def\pgfkeys@syntax@handlers@test{%
  \pgfkeysgetvalue{/handlers/first char syntax/\meaning\pgfkeys@first@char}\pgfkeys@the@handler%
  \ifx\pgfkeys@the@handler\relax%
    \expandafter\pgfkeys@@normal%
  \else%
    \expandafter\pgfkeys@use@handler%
  \fi%
}
\long\def\pgfkeys@use@handler#1,{%
  \pgfkeys@the@handler{#1}%
  \pgfkeys@parse%
}

\long\def\pgfkeys@@normal#1,{%
  \pgfkeys@unpack#1=\pgfkeysnovalue=\pgfkeys@stop%
  \pgfkeys@parse%
}
\def\pgfkeys@cleanup\pgfkeys@mainstop{}

\def\pgfkeys@mainstop{\pgfkeys@mainstop} % equals only itself
\def\pgfkeys@novalue{}
\def\pgfkeysnovalue{\pgfkeys@novalue} % equals only itself
\def\pgfkeysnovalue@text{\pgfkeysnovalue}
\def\pgfkeysvaluerequired{\pgfkeysvaluerequired} % equals only itself

\long\def\pgfkeys@unpack#1=#2=#3\pgfkeys@stop{%
  \pgfkeys@spdef\pgfkeyscurrentkey{#1}%
  \edef\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
  \ifx\pgfkeyscurrentkey\pgfkeys@empty%
    % Skip
  \else%
    \pgfkeys@add@path@as@needed%
    \pgfkeys@spdef\pgfkeyscurrentvalue{#2}%
    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
      \pgfkeysifdefined{\pgfkeyscurrentkey/.@def}%
      {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@def}{\pgfkeyscurrentvalue}}
      {}% no default, so leave it
    \fi%
    \ifx\pgfkeyscurrentvalue\pgfkeysvaluerequired%
      \def\pgf@marshal{\pgfkeysvalueof{/errors/value required/.@cmd}}%
      \expandafter\pgf@marshal\expandafter{\pgfkeyscurrentkey}{}\pgfeov%
    \else%
      \pgfkeys@case@one%
    \fi%
  \fi}

\def\pgfkeys@case@one{%
  \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}%
  {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
   \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@case@two}%
}

\def\pgfkeys@case@two{%
  \pgfkeysifdefined{\pgfkeyscurrentkey}%
  {\pgfkeys@case@two@extern}%
  {\pgfkeys@case@three}%
}

\def\pgfkeys@case@two@extern{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
    \pgfkeysvalueof{\pgfkeyscurrentkey}%
  \else%
    \pgfkeyslet{\pgfkeyscurrentkey}\pgfkeyscurrentvalue%
  \fi%
}


% either handled key or unknown.
%
% This macro will be replaced by the /handler config/handle only existing
% configuration, see below.
\def\pgfkeys@case@three{%
  \pgfkeys@split@path%
  \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}%
  {\pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@unknown}%
}
\let\pgfkeys@case@three@handleall=\pgfkeys@case@three
\def\pgfkeys@case@three@handle@restricted{%
  \pgfkeys@split@path%
  \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
    \pgfkeys@ifexecutehandler{%
    \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
      \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
  }{%
      % this here is necessary:  /my search path/key/.code
      % won't be called, so \pgfkeyscurrentpath == '/my search path/key'
      % -> it should be one directory higher! We want to invoke the
    %  .unknown handler in
    % '/my search path'
    %
    % Idea:
    % set
    % - path := '/my search path'
    % - name := 'key/.code'
    % - key = '/my search path/key/.code'
    \let\pgfkeys@tempa=\pgfkeyscurrentkey
    \let\pgfkeys@tempb=\pgfkeyscurrentname
      \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}%
      \pgfkeys@split@path%
    \let\pgfkeyscurrentkey=\pgfkeys@tempa
    \edef\pgfkeyscurrentname{\pgfkeyscurrentname/\pgfkeys@tempb}%
      \pgfkeys@unknown
  }%
  }{%
    \pgfkeys@unknown
  }%
}

% this macro is to implement the |handle only existing| key in key filtering:
% #1: the code to invoke IF the key handler shall be executed
% #2: the code to invoke if it shall not run.
\def\pgfkeys@ifexecutehandler#1#2{#1}%
\let\pgfkeys@ifexecutehandler@handleall=\pgfkeys@ifexecutehandler
\def\pgfkeys@ifexecutehandler@handleonlyexisting#1#2{%
  \ifcsname pgfk@excpt@\pgfkeyscurrentname\endcsname%
     #1% ok, this particular key handler is known and should be processed in any case (for example .try)
  \else
     % implement the 'only existing' feature here:
     \pgfkeysifdefined{\pgfkeyscurrentpath}{#1}{%
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}{#1}{#2}%
     }{}%
  \fi%
}%
\def\pgfkeys@ifexecutehandler@handlefullorexisting#1#2{%
  \ifpgfkeysaddeddefaultpath
    \ifcsname pgfk@excpt@\pgfkeyscurrentname\endcsname%
       #1% ok, this particular key handler is known and be processed in any case (for example .try)
    \else
       % implement the 'only existing' feature here:
       \pgfkeysifdefined{\pgfkeyscurrentpath}{%
         #1%
       }{%
         \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}{%
           #1%
         }{%
           #2%
         }%
       }%
    \fi%
  \else
    #1% ok, always true if the USER explicitly provided the full key path.
  \fi
}%
\def\pgfkeysaddhandleonlyexistingexception#1{\expandafter\def\csname pgfk@excpt@#1\endcsname{1}}%

\def\pgfkeys@unknown{%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.unknown/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {%
    \pgfkeysgetvalue{/handlers/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
  }%
}


\long\def\pgfkey@argumentisspace#1{%
  \long\def\pgfkeys@spdef##1##2{%
    \futurelet\pgfkeys@possiblespace\pgfkeys@sp@a##2\pgfkeys@stop\pgfkeys@stop#1\pgfkeys@stop\relax##1}%
  \def\pgfkeys@sp@a{%
    \ifx\pgfkeys@possiblespace\pgfkeys@sptoken%
      \expandafter\pgfkeys@sp@b%
    \else%
      \expandafter\pgfkeys@sp@b\expandafter#1%
    \fi}%
  \long\def\pgfkeys@sp@b#1##1 \pgfkeys@stop{\pgfkeys@sp@c##1}%
}
\pgfkey@argumentisspace{ }
\long\def\pgfkeys@sp@c#1\pgfkeys@stop#2\relax#3{\pgfkeys@temptoks{#1}\edef#3{\the\pgfkeys@temptoks}}
{\def\:{\global\let\pgfkeys@sptoken= } \: }



\def\pgfkeys@add@path@as@needed{% Should add the path if the
  % \pgfkeyscurrentkey does not start with /
  \expandafter\futurelet\expandafter\pgfkeys@possibleslash\expandafter\pgfkeys@check@slash\pgfkeyscurrentkey\relax%
}
\newif\ifpgfkeysaddeddefaultpath
\def\pgfkeys@check@slash{%
  \ifx\pgfkeys@possibleslash/%
    \expandafter\pgfkeys@nevermind%
  \else%
    \expandafter\pgfkeys@addpath%
  \fi%
}

\def\pgfkeys@nevermind#1\relax{%
  \pgfkeysaddeddefaultpathfalse
  \let\pgfkeyscurrentkeyRAW\pgfkeyscurrentkey
}
\def\pgfkeys@addpath#1\relax{%
  \pgfkeysaddeddefaultpathtrue
  \def\pgfkeyscurrentkeyRAW{#1}%
  \edef\pgfkeyscurrentkey{\pgfkeysdefaultpath#1}%
}


\def\pgfkeys@split@path{% Should assign the two codes
                       % \pgfkeyscurrentname and \pgfcurrentlkeypath
  \pgfkeys@pathtoks{}%
  \expandafter\pgfkeys@splitter\pgfkeyscurrentkey//%
}
\def\pgfkeys@splitter#1/#2/{%
  \def\pgfkeys@temp{#2}%
  \ifx\pgfkeys@temp\pgfkeys@empty%
    % Ah. done
    \def\pgfkeyscurrentname{#1}%
    \expandafter\pgfkeys@gobbletoslash%
  \else%
    \expandafter\pgfkeys@pathtoks\expandafter{\the\pgfkeys@pathtoks#1/}%
  \fi%
  \pgfkeys@splitter#2/%
}
\def\pgfkeys@gobbletoslash\pgfkeys@splitter/{%
  \if\relax\detokenize\expandafter{\the\pgfkeys@pathtoks}\relax\else
    \expandafter\pgfkeys@remove@slash\the\pgfkeys@pathtoks\relax
  \fi
}%
\def\pgfkeys@remove@slash#1/\relax{\pgfkeys@pathtoks{#1}}



% Quickly set keys
%
% #1 = default path
% #2 = key-value pairs
%
% Description:
%
% This command starts the execution with the default path set to
% #1. This command should only be used when speed is important (like
% in a heavily used macro like \tikzset). Normally, keys should be
% used to set the path. Note that if #1 equals /, then \pgfkeys will
% actually be quicker!
%
% Example:
%
% \pgfqkeys{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\def\pgfqkeys{\expandafter\pgfkeys@@qset\expandafter{\pgfkeysdefaultpath}}%
\long\def\pgfkeys@@qset#1#2#3{\def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}}


% Sets keys while setting keys
%
% #1 = key-value pairs
%
% Description:
%
% This code may only be called inside the code that is executed for a
% key. The #1 should be a list of settings pairs. They will be executed
% as if they had been given as the argument to the \pgfkeys command.
%
% Example:
%
% \pgfkeys{tikz,myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\long\def\pgfkeysalso#1{\pgfkeys@parse#1,\pgfkeys@mainstop}



% Quickly sets keys while setting keys
%
% #1 = default path
% #2 = key-value pairs
%
% Description:
%
% This command executes #2 with the default path set to #1. This
% command will cause chaos if used incorrectly. The only safe
% place to use it instead of \pgfkeys is at the beginning of a TeX group.
%
% Example:
%
% \begingroup
%   \pgfqkeysalso{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\long\def\pgfqkeysalso#1#2{\def\pgfkeysdefaultpath{#1/}\pgfkeys@parse#2,\pgfkeys@mainstop}




% Now setup the default handlers and keys:

% Define a key macro with one argument (\def or \edef)
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes one parameter and has #2 as its code.
%
% Example:
%
% \pgfkeysdef{/my key}{\show#1}

\long\def\pgfkeysdef#1#2{%
  \long\def\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@body}{#2}%
}
\long\def\pgfkeysedef#1#2{%
  \long\edef\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetevalue{#1/.@body}{#2}%
}


% Define a key macro with multiple arguments (\def or \edef)
%
% #1 = key
% #2 = argument pattern
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes #2 as its parameter pattern and has #3 as its code.
%
% Example:
%
% \pgfkeysdefargs{/swap}{#1#2}{#2#1}

\long\def\pgfkeysdefargs#1#2#3{%
  \long\def\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetvalue{#1/.@body}{#3}%
}

\long\def\pgfkeysedefargs#1#2#3{%
  \long\edef\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetevalue{#1/.@body}{#3}%
}

% Like \pgfkeysdefargs, but `#2' is an integer denoting the expected
% *number* of arguments.
%
% There is a subtle difference between the 'args' command, when it
% comes to spaces:
%  a key defined with defargs{#1#2} must not have spaces between the
%  arguments when it is used.
%
% See this:
%
%--------------------------------------------------
% % defnargs:
% \pgfkeysdefnargs{/a}{2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /a=
%     {1}
%     {2}
% }
% ->defnargs: 1=`1', 2=`2'
%
% defargs:
% \pgfkeysdefargs{/b}{#1#2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /b=
%     {1}
%     {2}
% }
% ->defargs: 1=`1', 2=` 2'  (note the space!)
%
% defargs:
% \pgfkeysdefargs{/b}{#1#2}{1=`#1', 2=`#2'}
% \pgfkeys{
%   /b=
%     {1}%
%     {2}
% }
% ->defargs: 1=`1', 2=`2'
% --------------------------------------------------
\long\def\pgfkeysdefnargs#1#2#3{\pgfkeysdefnargs@{#1}{#2}{#3}{\def}{\pgfkeyssetvalue}}%
\long\def\pgfkeysedefnargs#1#2#3{\pgfkeysdefnargs@{#1}{#2}{#3}{\edef}{\pgfkeyssetevalue}}%
\long\def\pgfkeysdefnargs@#1#2#3#4#5{%
  \ifcase#2\relax
    \pgfkeyssetvalue{#1/.@args}{}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7##8}%
  \or
    \pgfkeyssetvalue{#1/.@args}{##1##2##3##4##5##6##7##8##9}%
  \else
    \pgfkeys@error{\string\pgfkeysdefnargs: expected  <= 9 arguments, got #2}%
  \fi
  \pgfkeysgetvalue{#1/.@args}\pgfkeys@tempargs
  \def\pgfkeys@temp{\expandafter\long\expandafter#4\csname pgfk@#1/.@@body\endcsname}%
  \expandafter\pgfkeys@temp\pgfkeys@tempargs{#3}%
  % eliminate the \pgfeov at the end such that TeX gobbles spaces
  % by using
  % \pgfkeysdef{#1}{\pgfkeysvalueof{#1/.@@body}##1}
  % (with expansion of '#1'):
  \edef\pgfkeys@tempargs{\noexpand\pgfkeysvalueof{#1/.@@body}}%
  \def\pgfkeys@temp{\pgfkeysdef{#1}}%
  \ifnum#2=1\relax
    \expandafter\pgfkeys@temp\expandafter{\pgfkeys@tempargs{##1}}%
  \else
    \expandafter\pgfkeys@temp\expandafter{\pgfkeys@tempargs##1}%
  \fi
  #5{#1/.@body}{#3}%
}

% Defining a key command

\pgfkeysdef{/handlers/.code}{\pgfkeysdef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.code 2 args}{\pgfkeysdefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdef{/handlers/.ecode}{\pgfkeysedef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.ecode 2 args}{\pgfkeysedefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdefnargs{/handlers/.code args}{2}{\pgfkeysdefargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.ecode args}{2}{\pgfkeysedefargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.code n args}{2}{\pgfkeysdefnargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefnargs{/handlers/.ecode n args}{2}{\pgfkeysedefnargs{\pgfkeyscurrentpath}{#1}{#2}}

% Adding to a key command

\pgfkeys{/handlers/.add code/.code 2 args=%
  % Find out, whether with args or not.
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@args}%
  {% Yes, so add to body and reuse args
  \pgfkeysaddvalue{\pgfkeyscurrentpath/.@body}{#1}{#2}%
  % Redefine code
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@args}{\pgfkeys@tempargs}%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@body}{\pgfkeys@tempbody}%
    \def\pgfkeys@marshal{\expandafter\long\expandafter\gdef\expandafter\pgfkeys@global@temp\pgfkeys@tempargs}%
    \expandafter\pgfkeys@marshal\expandafter{\pgfkeys@tempbody}%
  }%
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@@body}{%
    % support for \pgfkeysndefargs:
    \pgfkeyslet{\pgfkeyscurrentpath/.@@body}{\pgfkeys@global@temp}%
  }{%
    % support for \pgfkeysdefargs:
      \pgfkeyslet{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@global@temp}%
  }%
  }%
  {%
    % No, so single argument (simple \pgfkeysdef). Redefine accordingly.
    \edef\pgf@expanded@path{\pgfkeyscurrentpath}%
    {%
      \toks0{#1}%
      \pgfkeysifdefined{\pgf@expanded@path/.@cmd}%
      {\expandafter\expandafter\expandafter\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@\pgf@expanded@path/.@body\endcsname}}%
      {\expandafter\pgfkeys@temptoks\expandafter{\expandafter\pgfkeyssetvalue\expandafter{\pgf@expanded@path}{##1}}}%
      \toks1{#2}%
      \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1 }%
    }%
    \def\pgf@temp{\pgfkeyssetvalue{\pgf@expanded@path/.@body}}%
    \expandafter\pgf@temp\expandafter{\pgfkeys@global@temp}%
    \expandafter\long\expandafter\def\expandafter\pgfkeys@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
    \pgfkeyslet{\pgf@expanded@path/.@cmd}\pgfkeys@temp%
  }%
}
\pgfkeys{/handlers/.prefix code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={#1}{}}}%
\pgfkeys{/handlers/.append code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{#1}}}%


% Defining a style

\pgfkeys{/handlers/.style/.code=\pgfkeys{\pgfkeyscurrentpath/.code=\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.estyle/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\noexpand\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.style args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.code args={#1}{\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.estyle args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.ecode args={#1}{\noexpand\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.style 2 args/.code=\pgfkeys{\pgfkeyscurrentpath/.code 2 args=\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.style n args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.code n args={#1}{\pgfkeysalso{#2}}}}

% Adding to a style

\pgfkeys{/handlers/.add style/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{\pgfkeysalso{#2}}}}%
\pgfkeys{/handlers/.prefix style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{}}}%
\pgfkeys{/handlers/.append style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{\pgfkeysalso{#1}}}}%


% Defining a value

\pgfkeys{/handlers/.initial/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/handlers/.add/.code 2 args=\pgfkeysaddvalue{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeys{/handlers/.prefix/.code=\pgfkeysaddvalue{\pgfkeyscurrentpath}{#1}{}}
\pgfkeys{/handlers/.append/.code=\pgfkeysaddvalue{\pgfkeyscurrentpath}{}{#1}}
\pgfkeys{/handlers/.get/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/handlers/.link/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath}{\pgfkeysvalueof{#1}}}


% Defining a default

\pgfkeys{/handlers/.default/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{#1}}
\pgfkeys{/handlers/.value required/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeysvaluerequired}}
\pgfkeys{/handlers/.value forbidden/.code=\pgfkeys{\pgfkeyscurrentpath/.add code=%
{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
  \else%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/value forbidden/.@cmd}}%
    \expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkey\expandafter}\expandafter{\pgfkeyscurrentvalue}\pgfeov%
  \fi%
}{}}}


% High-level cmds

\pgfkeys{/handlers/.store in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\def#1{##1}}}
\pgfkeys{/handlers/.estore in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\edef#1{##1}}}

\pgfkeys{/handlers/.is if/.code=\pgfkeysalso{%
    \pgfkeyscurrentpath/.code=\pgfkeys@handle@boolean{#1}{##1},
    \pgfkeyscurrentpath/.default=true%
  }%
}
\def\pgfkeys@handle@boolean#1#2{%
  \ifcsname#1#2\endcsname%
    \csname#1#2\endcsname%
  \else%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/boolean expected/.@cmd}}%
    \expandafter\pgf@marshal\expandafter{\pgfkeyscurrentkey}{#2}\pgfeov%
  \fi
}

\pgfkeys{/handlers/.is choice/.code=%
  \pgfkeys{%
    \pgfkeyscurrentpath/.cd,%
    .code=\def\pgfkeys@was@choice{##1}\expandafter\pgfkeysalso\expandafter{\pgfkeyscurrentkey/##1},
    .unknown/.code={%
      \def\pgf@marshal{\pgfkeysvalueof{/errors/unknown choice value/.@cmd}}%
      {\expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@pathtoks\expandafter}\expandafter{\pgfkeys@was@choice}\pgfeov}%
    }%
  }%
}


% Repeatedly setting a key

\pgfkeys{/handlers/.list/.code=%
  {%
    \ifx\foreach\@undefined%
      \pgfkeys@error{You need to load the pgffor package to use the .list key syntax.}%
    \fi%
    % Use foreach to unfold the list
    \def\pgf@keys@temp{}%
    \foreach \pgf@keys@key in{#1}%
    {\expandafter\expandafter\expandafter\gdef%
      \expandafter\expandafter\expandafter\pgf@keys@temp%
      \expandafter\expandafter\expandafter{\expandafter\pgf@keys@temp\expandafter{\pgf@keys@key}}}%
    \edef\pgf@keys@list@path{\pgfkeyscurrentpath}%
    \expandafter\expandafter\expandafter\pgf@keys@do@list%
    \expandafter\expandafter\expandafter{\expandafter\pgf@keys@list@path\expandafter}\pgf@keys@temp\pgf@stop%
  }%
}
\def\pgf@keys@do@list#1{\pgf@keys@utilifnextchar\bgroup{\pgf@keys@do@list@item{#1}}\pgf@keys@gobble}
\def\pgf@keys@do@list@item#1#2{\pgfkeysalso{#1={#2}}\pgf@keys@do@list{#1}}


% Forwarding

\pgfkeys{/handlers/.forward to/.code=%
  \pgfkeys{\pgfkeyscurrentpath/.add code={}{\pgfkeys{#1={##1}}}}
}


% Inspection handlers

\pgfkeys{/handlers/.show value/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{\pgfkeysshower}\show\pgfkeysshower} % inspect the value
\pgfkeys{/handlers/.show code/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeysshower}\show\pgfkeysshower} % inspect the body of the command


% First char syntax handlers
\pgfkeys{/handlers/first char syntax/.is if=pgfkeys@syntax@handlers}

% Path handling

% Prepares the .unknown handler used by '.search also'.
% It will be stored into \pgfkeys@global@temp.
\def\pgfkeys@searchalso@prepare@unknown@handler#1{%
  \global\def\pgfkeys@global@temp##1\pgfeov{}%
  \pgfkeys@searchalso@parse#1,\pgfkeys@mainstop
  {%
    \toks0=\expandafter{\pgfkeys@global@temp##1\pgfeov}%
  \toks1={%
    \pgfkeysgetvalue{/handlers/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeys@searchalso@temp@value\pgfeov
  }%
  \xdef\pgfkeys@global@temp{%
    \noexpand\def\noexpand\pgfkeys@searchalso@temp@value{####1}%
    \noexpand\ifpgfkeysaddeddefaultpath
      \noexpand\expandafter\noexpand\pgfkeys@firstoftwo
    \noexpand\else
      \noexpand\expandafter\noexpand\pgfkeys@secondoftwo
    \noexpand\fi{%
      \noexpand\pgfkeyssuccessfalse
      \noexpand\let\noexpand\pgfkeys@searchalso@name=\noexpand\pgfkeyscurrentkeyRAW
      \the\toks0 % one or more /.try things; one for each path. The last element won't have a /.try
      %\noexpand\ifpgfkeyssuccess
      %\noexpand\else
      %  \the\toks1 % invoke /handlers/.unknown handler
      %\noexpand\fi
    }{%
      \the\toks1 % invoke /handlers/.unknown handler
    }%
  }%
  \expandafter\gdef\expandafter\pgfkeys@global@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
  }%
}%

\def\pgfkeys@searchalso@parse{\futurelet\pgfkeys@possiblerelax\pgfkeys@searchalso@parse@main}
\def\pgfkeys@searchalso@parse@main{%
  \ifx\pgfkeys@possiblerelax\pgfkeys@mainstop%
    \expandafter\pgfkeys@cleanup%
  \else%
    \expandafter\pgfkeys@searchalso@appendentry%
  \fi%
}
\def\pgfkeys@searchalso@appendentry#1,#2{%
  \def\pgfkeys@searchalso@nexttok{#2}%
  \pgfkeys@spdef\pgfkeys@temp{#1}%
  {%
    \toks0=\expandafter{\pgfkeys@global@temp##1\pgfeov}%
  \toks1=\expandafter{\pgfkeys@temp}%
  \xdef\pgfkeys@global@temp{%
    \the\toks0 % the space is important!
    \noexpand\ifpgfkeyssuccess\noexpand\else
      \noexpand\pgfqkeys{\the\toks1 }{\noexpand\pgfkeys@searchalso@name
               \ifx\pgfkeys@searchalso@nexttok\pgfkeys@mainstop\else/.try\fi /.expand once=\noexpand\pgfkeys@searchalso@temp@value}%
    \noexpand\fi}%
  \expandafter\gdef\expandafter\pgfkeys@global@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
  }%
  \pgfkeys@searchalso@parse#2%
}
\pgfkeys{%
  /handlers/.is family/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\edef\noexpand\pgfkeysdefaultpath{\pgfkeyscurrentpath/}},%
  /handlers/.cd/.code=\edef\pgfkeysdefaultpath{\pgfkeyscurrentpath/},%
  /handlers/.search also/.code={%
    \pgfkeys@searchalso@prepare@unknown@handler{#1}%
%\message{I prepared the '\pgfkeyscurrentpath/.unknown' handler \meaning\pgfkeys@global@temp\space for '#1'.}%
    \pgfkeyslet{\pgfkeyscurrentpath/.unknown/.@cmd}{\pgfkeys@global@temp}%
  }
}%


% Value expansion

\pgfkeys{/handlers/.expand once/.code=\expandafter\pgfkeys@exp@call\expandafter{#1}}
\pgfkeys{/handlers/.expand twice/.code=\expandafter\expandafter\expandafter\pgfkeys@exp@call\expandafter\expandafter\expandafter{#1}}
\pgfkeys{/handlers/.expanded/.code=\edef\pgfkeys@temp{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfkeys@temp}}

\long\def\pgfkeys@exp@call#1{\pgfkeysalso{\pgfkeyscurrentpath={#1}}}

\def\pgfkeys@mathparse{%
  \ifcsname pgfmathparse\endcsname
    \expandafter\pgfmathparse
  \else
    \pgfkeys@error{You have to load `pgfmath' to use \string\pgfmathparse}%
    \expandafter\def\expandafter\pgfmathresult
  \fi
}
\pgfkeys{/handlers/.evaluated/.code=\pgfkeys@mathparse{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfmathresult}}

% Try to set a key and do nothing if not define

\newif\ifpgfkeyssuccess
\pgfkeys{/handlers/.try/.code=\pgfkeys@try}
\pgfkeys{/handlers/.retry/.code=\ifpgfkeyssuccess\else\pgfkeys@try\fi}
\def\pgfkeys@try{%
  \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}% make sure that \pgfkeys@code doesn't know about 'try'. Important for .is choice
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
    \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
    {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
    {}% no default, so leave it
  \fi%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
    \pgfkeyssuccesstrue%
  }%
  {%
    \pgfkeysifdefined{\pgfkeyscurrentpath}%
    {%
      \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
        \pgfkeysvalueof{\pgfkeyscurrentpath}%
      \else%
        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
      \fi%
      \pgfkeyssuccesstrue%
    }%
    {%
      \pgfkeys@split@path%
      \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
      % in the standard configuration, this check here is redundant
      % because pgfkeys@ifexecutehandler === true.
    % It is only interesting for 'handle only existing'.
        \pgfkeys@ifexecutehandler{%
        \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
          \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
          \pgfkeyssuccesstrue%
      }{%
        \pgfkeyssuccessfalse
      }%
      }{%
      \pgfkeyssuccessfalse
      }%
  }%
  }%
}

% Utilities

\pgfkeys{/utils/exec/.code=#1} % simply execute the given code directly.


% Errors

\pgfkeys{
  /errors/boolean expected/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      Boolean parameter of key '\the\toks1' must be 'true' or 'false', not
      '\the\toks2'. I am going to ignore it%
    }%
  },
  /errors/value required/.code 2 args=%
  {%
    \toks1={#1}%
    \pgfkeys@error{%
      The key '\the\toks1' requires a value. I am going to ignore this
      key%
    }%
  },
  /errors/value forbidden/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      You may not specify a value for the key '\the\toks1'. I am going to ignore
      the value '\the\toks2' that you provided%
    }%
  },
  /errors/unknown choice value/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \pgfkeys@error{%
      Choice '\the\toks2' unknown in choice key '\the\toks1'. I am
      going to ignore this key%
    }%
  },
  /errors/unknown key/.code 2 args=%
  {%
    \toks1={#1}%
    \toks2={#2}%
    \def\pgf@temp{#2}%
    \pgfkeys@error{%
      I do not know the key '\the\toks1'\ifx\pgf@temp\pgfkeysnovalue@text\space\else, to which you passed
      '\the\toks2', \fi and I am going to ignore it. Perhaps you
      misspelled it%
    }%
  }
}

\pgfkeys{/handlers/.unknown/.code=%
  {%
    \def\pgf@marshal{\pgfkeysvalueof{/errors/unknown key/.@cmd}}%
    {\expandafter\expandafter\expandafter\pgf@marshal\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkey\expandafter}\expandafter{\pgfkeyscurrentvalue}\pgfeov}%
  }%
}

\pgfkeys{
  /handler config/.is choice,
  /handler config/all/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handleall
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handleall
  },
  /handler config/only existing/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handle@restricted
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handleonlyexisting
  },
  /handler config/full or existing/.code={%
    \let\pgfkeys@case@three=\pgfkeys@case@three@handle@restricted
    \let\pgfkeys@ifexecutehandler=\pgfkeys@ifexecutehandler@handlefullorexisting
  },
  /handler config/only existing/add exception/.code={\pgfkeysaddhandleonlyexistingexception{#1}},
}%
\pgfkeysaddhandleonlyexistingexception{.cd}%
\pgfkeysaddhandleonlyexistingexception{.try}%
\pgfkeysaddhandleonlyexistingexception{.retry}%
\pgfkeysaddhandleonlyexistingexception{.lastretry}%
\pgfkeysaddhandleonlyexistingexception{.unknown}%
\pgfkeysaddhandleonlyexistingexception{.expand once}%
\pgfkeysaddhandleonlyexistingexception{.expand twice}%
\pgfkeysaddhandleonlyexistingexception{.expanded}%


% Utilities for self-containment
\def\pgf@keys@gobble#1{}
\long\def\pgf@keys@utilifnextchar#1#2#3{%
  \let\pgf@keys@utilreserved@d=#1%
  \def\pgf@keys@utilreserved@a{#2}%
  \def\pgf@keys@utilreserved@b{#3}%
  \futurelet\pgf@keys@utillet@token\pgf@keys@utilifnch}
\def\pgf@keys@utilifnch{%
  \ifx\pgf@keys@utillet@token\pgf@keys@utilsptoken
    \let\pgf@keys@utilreserved@c\pgf@keys@utilxifnch
  \else
    \ifx\pgf@keys@utillet@token\pgf@keys@utilreserved@d
      \let\pgf@keys@utilreserved@c\pgf@keys@utilreserved@a
    \else
      \let\pgf@keys@utilreserved@c\pgf@keys@utilreserved@b
    \fi
  \fi
  \pgf@keys@utilreserved@c}
{%
  \def\:{\global\let\pgf@keys@utilsptoken= } \:
  \def\:{\pgf@keys@utilxifnch} \expandafter\gdef\: {\futurelet\pgf@keys@utillet@token\pgf@keys@utilifnch}
}


\input pgfkeysfiltered.code.tex

\endinput


==> pgfkeysfiltered.code.tex <==
% Copyright 2019 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file contains additions to pgfkeys.code.tex (loaded
% automatically at the end of pgfkeys.code.tex)
%
% Improvements:
%
% - option filtering
%   you provide
%     - a boolean predicate
%     - a "filter handler" which will be invoked for non-matching options,
%     - a key=value list as usual.
%   The filter sets only matching options and invokes the handler for
%   unmatching ones.
%
% - Fast family support as in xkeyval.
%   - A key like /my tree/my option  can be associated with /my family
%   - You can efficiently set keys which belong to a set of "active"
%     families.
%  Remaining options can be collected into a macro.

% WARNING:
% this file overwrites
% \pgfkeys@addpath
% \pgfkeys@nevermind
%
% all other features are 'additive'


% these implementations will be switched dynamically with their
% filtered versions (in \pgfkeys@install@filter@and@invoke)
\let\pgfkeys@orig@case@one=\pgfkeys@case@one
\let\pgfkeys@orig@@set=\pgfkeys@@set
\let\pgfkeys@orig@@qset=\pgfkeys@@qset
\let\pgfkeys@orig@try=\pgfkeys@try
\let\pgfkeys@orig@unknown=\pgfkeys@unknown

\newif\ifpgfkeysfilteringisactive
\newif\ifpgfkeysfiltercontinue
\let\pgfkeys@key@predicate=\pgfkeys@empty
\let\pgfkeys@filtered@handler=\pgfkeys@empty
\newtoks\pgfkeys@tmptoks

% Performs 'filtered' key settings.
%
% For every option for which the path prefixing has already been done,
% the current key filter predicate will be invoked. If the predicate
% returns true, pgfkeys will process this key in the normal manner.
% If not, a key filter handler will be invoked.
%
% The *predicate* and *handler* semantics are as follows:
% PRECONDITION:
%         1. The variables
%             \pgfkeyscurrentkey (full path including name)
%             \pgfkeyscurrentkeyRAW (the current key as it has been
%                                    found in the key=value list
%                                    without path modification)
%             \pgfkeyscurrentvalue
%             are all set. If the current key is a handler variable,
%                 \pgfkeyscurrentname
%             and
%                 \pgfkeyscurrentpath
%             are also set.
%         2. The type of option has already been checked, that means
%             case (1) whether '.@cmd' exists
%             case (2) whether the key as such has its value
%             case (3) it is a handler like '.code', '.cd' or whatever.
%             case (0) it is unknown.
%             The actual case number (0-3) will be provided as contents
%             of the macro
%                 \pgfkeyscasenumber.
%             It is always a one-character token, so it may be compared
%             with both, \ifnum or \if.
%             Please note that unknown options will be processed with
%             the usual '.unknown' handlers unless the key filter takes
%             control over unknown options as well.
%
% POSTCONDITION:
%         the predicate sets
%             \pgfkeysfiltercontinuetrue
%         or
%             \pgfkeysfiltercontinuefalse
%         (the boolean \ifpgfkeysfiltercontinue).
% Depending on this 'if', option processing will be continued or
% skipped.
%
% The handler can do anything with the option, for example collect
% unmatched ones.
%
% ATTENTION: \pgfkeysfiltered can't be nested (yet). Use the
% \pgfkeyspredicateAND if you need multiple predicates at once.
% Nesting would produce unexpected results because the current filter
% state can't be stored/restored without TeX-groups, therefor it is
% disabled.
%
% ATTENTION: you can't filter error messages.
%
% REMARK: In case (3), the macros \pgfkeyscurrentpath and
% \pgfkeyscurrentname have already been computed, you do not need to
% invoke \pgfkeyssplitpath. In any other case, neither path nor name
% are required for the options processing - if you need them for
% predicates/handlers, you need to compute them by hand.
%
%
% Example:
%   \def\unmatched{}
%   \pgfkeys{/pgf/key filters/is descendant of/.install key filter=/my group}
%   \pgfkeys{/pgf/key filter handlers/append filtered to/.install key filter handler=\unmatched}
%   \pgfkeysfiltered%
%       {/my group/option 1=value 1,/tikz/option 2=value 2}
% ->
%  will set '/my group/option 1' as usual, but '/tikz/option 2' will not
%  be set. Instead, it will be appended to '\unmatched' such that
%  \unmatched = {/tikz/option 2=value2}
%  after the operation.
%
% Arguments:
% #1:  key-value list.
\def\pgfkeysfiltered{%
    % produce
    % '{<default path>}'
    % each expanded exactly one time into the register:
    \expandafter\pgfkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}%
}

% #1: old value of default path.
% #2: key-value-list.
\long\def\pgfkeysfiltered@@install#1#2{%
    \pgfkeys@install@filter@and@invoke{%
        \let\pgfkeysdefaultpath\pgfkeys@root%
        \pgfkeys@parse#2,\pgfkeys@mainstop%
        \def\pgfkeysdefaultpath{#1}%
    }%
}

% Assuming that macro #1 contains a key=value list, this command
% performs an \pgfkeysalso command for the content of macro #1.
%
% It can be used in conjunction with
%   - \pgfkeysfiltered and
%   - \pgfkeysappendfilterednamestomacro:
% the first pass fill only process options matching the filter, then,
% a \pgfkeysalsofrom can be used at a later time to set the remaining
% options.
%
% Example:
% \pgfkeys{/my group/.cd,/utils/exec=\pgfkeysalsofrom\filtered}
\long\def\pgfkeysalsofrom#1{%
    \expandafter\pgfkeysalso\expandafter{#1}%
}

% The same as \pgfkeysalsofrom, but it invokes \pgfkeysalsofiltered.
\long\def\pgfkeysalsofilteredfrom#1{%
    \expandafter\pgfkeysalsofiltered\expandafter{#1}%
}

% #1 = options
\long\def\pgfkeysalsofiltered#1{%
    \pgfkeys@install@filter@and@invoke{\pgfkeysalso{#1}}%
}%

% The same like \pgfkeysfiltered, but with quick search path setting.
%
% #1: default path
% #2: key-value-pairs
\long\def\pgfqkeysfiltered#1{%
    \expandafter\pgfqkeysfiltered@@install\expandafter{\pgfkeysdefaultpath}{#1}%
}

% #1: old value of default path.
% #2: default path
% #3: key-value-list.
\long\def\pgfqkeysfiltered@@install#1#2#3{%
    \pgfkeys@install@filter@and@invoke{%
        \def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}%
    }%
}

% Family management
%
% The family code provides the following features:
% 1. every key can be associated with 0 or 1 'family'.
% 2. Families are a loose association which are independent of the key
% hierarchy.
%   For example, /my tree/key1  can belong to family /tikz.
%
% 3. It is possible to "activate" or "deactivate" single families.
%    Furthermore, it is possible to set only keys which belong to
%    active families (using \pgfkeysfiltered).
% 4. Runtime complexities:
%    If you have N options and you only want to process K active
%    families, the runtime is O( N + K ):
%      - activate every family O(K)
%      - use \pgfkeyshasactivefamily as filter predicate O(N)
%      - deactivate every family O(K)


% Activates family #1.
%
% #1 maybe a macro.
\def\pgfkeysactivatefamily#1{%
    \pgfkeysiffamilydefined
        {#1}%
        {\csname pgfk@#1/familyactivetrue\endcsname}%
        {\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[ACTIVATING FAMILY #1]}%
}

% Deactivates family #1.
%
% #1 maybe a macro.
\def\pgfkeysdeactivatefamily#1{%
    \pgfkeysiffamilydefined
        {#1}%
        {\csname pgfk@#1/familyactivefalse\endcsname}%
        {\pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov}%
%\message{[DEACTIVATING FAMILY #1]}%
}

% Activates all families in the comma separated list #1.
%
% It will also generate code for deactivation of all those families
% into the command #2.
%
% #1: a comma-separated list of fully qualified family names.
% #2: a command which will be filled with a deactivate-all command.
\def\pgfkeysactivatefamilies#1#2{%
    \pgfkeyssavekeyfilterstateto\pgfkeys@cur@state
    \expandafter\pgfkeysactivatefamilies@impl\expandafter{\pgfkeys@cur@state}{#1}{#2}%
}
% #1: commands needed to restore the old filtering state
% #2: family name list
% #3: macro name for de-activate command
\def\pgfkeysactivatefamilies@impl#1#2#3{%
    \pgfkeysinstallkeyfilter{/pgf/key filters/false}{}%
    \let#3=\pgfkeys@empty%
    \def\pgfkeys@filtered@handler{\pgfkeys@family@activate@handler{#3}}%
    \pgfkeysalsofiltered{#2}%
    #1%
}

\def\pgfkeys@family@activate@handler#1{%
    \pgfkeysactivatefamily{\pgfkeyscurrentkey}%
    % produce
    %   <old list> '\pgfkeysdeactivatefamily{' <current key> '}'
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter\pgfkeysdeactivatefamily\expandafter{\pgfkeyscurrentkey}}%
    \edef#1{\the\pgfkeys@tmptoks}%
}

% If for testing whether a family exists.
%
% #1 = fully qualified family name
% #2 = if-case
% #3 = else-case
%
% Description:
%
% If the family exists, #2 will be executed. Otherwise, #3 will be
% called.
\long\def\pgfkeysiffamilydefined#1#2#3{\ifcsname ifpgfk@#1/familyactive\endcsname#2\else#3\fi}

% Sets the TeX boolean
%   \ifpgfkeysfiltercontinue := ( family #1 is active )
%
% Argument:
% #1 the family name. Maybe a macro.
\def\pgfkeysisfamilyactive#1{%
    \pgfkeysiffamilydefined{#1}{%
        \expandafter\let\expandafter\ifpgfkeysfiltercontinue\csname ifpgfk@#1/familyactive\endcsname
    }{%
        \pgfkeysvalueof{/errors/family unknown/.@cmd}{#1}\pgfeov%
        \expandafter\expandafter\expandafter\let\csname ifpgfkeysfiltercontinue\endcsname\csname iffalse\endcsname
    }%
}%

% Retrieve the family of full key #1 into macro #2.
%
% Will set the TeX boolean \ifpgfkeyssuccess to whether the full key
% really has a family.
%
% The family for any key is stored in the sub-key #1/family.
%
% Parameters:
% #1:  the full key name for which the family is requested. Maybe a
%      macro.
% #2:  a macro name which will be filled with the result.
\def\pgfkeysgetfamily#1#2{%
    \pgfkeysifdefined{#1/family}{\pgfkeysgetvalue{#1/family}{#2}\pgfkeyssuccesstrue}{\pgfkeyssuccessfalse}%
}

% Equivalent to \pgfkeys{#1/.belongs to family=#2}
\def\pgfkeyssetfamily#1#2{%
    \pgfkeysiffamilydefined{#2}{%
        \pgfkeyssetvalue{#1/family}{#2}%
    }{%
        \pgfkeysalso{/errors/family unknown=#2}%
    }%
}%


% Sets \ifpgfkeysfiltercontinue to true iff the current key belongs to
% the /errors tree.
\long\def\pgfkeys@cur@is@descendant@of@errors{%
    \expandafter\pgfkeys@cur@is@descendant@of@errors@impl\pgfkeyscurrentkey/errors\pgf@@eov
}%
\long\def\pgfkeys@cur@is@descendant@of@errors@impl#1/errors#2\pgf@@eov{%
    \def\pgfkeyspred@TMP{#1}%
    \ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': TRUE.}%
        \pgfkeysfiltercontinuetrue
    \else
%\message{[SPECIAL CHECK] '\pgfkeyscurrentkey' is descendant of '/errors': FALSE.}%
        \pgfkeysfiltercontinuefalse
    \fi
}%

% \pgfkeysinterruptkeyfilter
% ...
% \endpgfkeysinterruptkeyfilter
% temporarily interrupts key filtering and enables it in
% \endpgfkeysinterruptkeyfilter.
%
% If key filtering it not active, this has no effect at all.
%
% REMARK:
% \pgfkeysinterruptkeyfilter...\endpgfkeysinterruptkeyfilter does NOT
% introduce a \TeX-group.
\def\pgfkeysinterruptkeyfilter{%
    \ifpgfkeysfilteringisactive
        \let\pgfkeys@case@one=\pgfkeys@orig@case@one
        \let\pgfkeys@try=\pgfkeys@orig@try
        \let\pgfkeys@unknown=\pgfkeys@orig@unknown
    \fi
}

\def\endpgfkeysinterruptkeyfilter{%
    \ifpgfkeysfilteringisactive
        \let\pgfkeys@case@one=\pgfkeys@case@one@filtered
        \let\pgfkeys@try=\pgfkeys@try@filtered
        \let\pgfkeys@unknown=\pgfkeys@unknown@filtered
    \fi
}

% Activates families #1, calls \pgfkeysfiltered and deactivates the
% families afterwards.
%
% REMARK: you need to install a family-based key filter predicate
% manually to benefit from the activated families!
%
% #1: comma separated family list
% #2: key-value pairs
%
% @see \pgfkeysactivatefamiliesandfilteroptions
\def\pgfkeysactivatefamiliesandfilteroptions#1#2{%
    \pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
    \pgfkeysfiltered{#2}%
    \pgfkeys@family@deactivation
}

% The "quick" variant of \pgfkeysactivatefamiliesandfilteroptions: it
% also assigns a default path.
%
% #1: comma separated family list
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatefamiliesandfilteroptions#1#2#3{%
    \pgfkeysactivatefamilies{#1}{\pgfkeys@family@deactivation}%
    \pgfqkeysfiltered{#2}{#3}%
    \pgfkeys@family@deactivation
}

% Public version of split path:
\def\pgfkeyssplitpath{\pgfkeys@split@path}%


% The same as \pgfkeysactivatefamiliesandfilteroptions but just for
% ONE family.
%
% #1: family (maybe a macro)
% #2: key-value pairs
\def\pgfkeysactivatesinglefamilyandfilteroptions#1#2{%
    \pgfkeysactivatefamily{#1}%
    \pgfkeysfiltered{#2}%
    \pgfkeysdeactivatefamily{#1}%
}

% The "quick" variant of \pgfkeysactivatesinglefamilyandfilteroptions
%
% #1: family (maybe a macro)
% #2: default path
% #3: key-value pairs
\def\pgfqkeysactivatesinglefamilyandfilteroptions#1#2#3{%
    \pgfkeysactivatefamily{#1}%
    \pgfqkeysfiltered{#2}{#3}%
    \pgfkeysdeactivatefamily{#1}%
}

% Installs the key filter '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter=#2}
%
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilter
% and
% \pgfkeyscurrentkeyfilterargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the key. If the key expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilter#1#2{%
    \pgfkeysifdefined{#1/.@cmd}{%
        \edef\pgfkeyscurrentkeyfilter{#1}%
        \def\pgfkeyscurrentkeyfilterargs{#2}%
        \pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@key@predicate@}%
        \def\pgfkeys@key@predicate{\pgfkeys@key@predicate@#2\pgfeov}%
    }{%
        \pgfkeysvalueof{/errors/no such key filter/.@cmd}{#1}{#2}\pgfeov%
    }%
}

% Installs the key filter handler '#1' with argument '#2'.
% This is equivalent to
%    \pgfkeys{#1/.install key filter handler=#2}
%
% The current values of the key filter handler is stored into the public
% macros
% \pgfkeyscurrentkeyfilterhandler
% and
% \pgfkeyscurrentkeyfilterhandlerargs
%
% #1: a full key name; may be a macro
% #2: optional arguments for the handler. If the handler expects more than one
% argument, supply '{{first}{second}}'
\def\pgfkeysinstallkeyfilterhandler#1#2{%
    \pgfkeysifdefined{#1/.@cmd}{%
        \edef\pgfkeyscurrentkeyfilterhandler{#1}%
        \def\pgfkeyscurrentkeyfilterhandlerargs{#2}%
        \pgfkeysgetvalue{#1/.@cmd}{\pgfkeys@filtered@handler@}%
        \def\pgfkeys@filtered@handler{\pgfkeys@filtered@handler@#2\pgfeov}%
    }{%
        \pgfkeysvalueof{/errors/no such key filter handler/.@cmd}{#1}{#2}\pgfeov%
    }%
}

% Creates a macro which contains commands to re-activate the current
% key filter and key filter handler. It can be used to temporarily
% switch the key filter.
\def\pgfkeyssavekeyfilterstateto#1{%
    % produce the string
    % \pgfkeysinstallkeyfilter{...}{...}
    % \pgfkeysinstallkeyfilterhandler{...}{...}
    % where each argument is expanded once
    % FIXME: Do the same with less overhead!
    \pgfkeys@tmptoks={\pgfkeysinstallkeyfilter}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilter}}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterargs}\pgfkeysinstallkeyfilterhandler}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandler}}%
    \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfkeys@tmptoks\expandafter{\pgfkeyscurrentkeyfilterhandlerargs}}%
    \edef#1{%
        \the\pgfkeys@tmptoks
    }%
}


\pgfkeys{%
    /errors/family unknown/.code=\pgfkeys@error{%
        Sorry, I do not know family '#1' and can't work with any assoicated family handling. Perhaps you misspelled it?},
    /errors/no such key filter/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter '#1'.},
    /errors/no such key filter handler/.code 2 args=\pgfkeys@error{Sorry, there is no such key filter handler '#1'.},
    % HANDLERS:
    %
    % .is family should
    %  1. '.cd' into the families' path,
    %  2. define booleans to activate/deactive the family
    %     (see \pgfkeysisfamilyactive)
    %  3. make sure that \pgfkeyshasactivefamily returns true for
    %     the family itself.
    /handlers/.is family/.append code={%
        %\newif is an \outer macro in plain tex, so this here is not portable:
        %\expandafter\newif\csname if\pgfkeyscurrentpath/familyactive\endcsname
        \edef\pgfkeyspred@TMP{pgfk@\pgfkeyscurrentpath/familyactive}%
        \expandafter\pgfkeys@non@outer@newif\expandafter{\pgfkeyspred@TMP}%
        \edef\pgfkeyspred@TMP{\pgfkeyscurrentpath/.belongs to family=\pgfkeyscurrentpath}%
        \expandafter\pgfkeysalso\expandafter{\pgfkeyspred@TMP}%
    },%
    /handlers/.activate family/.code=\pgfkeysactivatefamily{\pgfkeyscurrentpath},
    /handlers/.deactivate family/.code=\pgfkeysdeactivatefamily{\pgfkeyscurrentpath},
    /handlers/.belongs to family/.code={\pgfkeyssetfamily{\pgfkeyscurrentpath}{#1}},%
    %
    %
    % An addition to the '.try' and '.retry' handlers:
    %
    % It is the same as '.retry', but if the option is still unknown, the
    % usual handlers for unknown keys will be invoked.
    /handlers/.lastretry/.code={%
        \ifpgfkeyssuccess\else
            \pgfkeys@try
            \ifpgfkeyssuccess\else
                \pgfkeys@split@path%
                \pgfkeys@unknown
            \fi
        \fi
    },
    %
    %
    /handlers/.install key filter/.code={%
        \pgfkeysinstallkeyfilter{\pgfkeyscurrentpath}{#1}%
    },%
    /handlers/.install key filter handler/.code={%
        \pgfkeysinstallkeyfilterhandler{\pgfkeyscurrentpath}{#1}%
    },%
    %
    %
    % KEY FILTER HANDLERS:
    %
    /pgf/key filter handlers/append filtered to/.code={%
        % Produce
        %  <orig key> '={' <value> '}'
        % where both, the key and the value are expanded just ONCE:
        \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter\pgfkeyscurrentkeyRAW\expandafter=\expandafter{\pgfkeyscurrentvalue}}%
        \ifx#1\pgfkeys@empty
        \else
            % Produce <old list> ','  <orig key> '={' <value> '}'
            \pgfkeys@tmptoks=\expandafter\expandafter\expandafter{\expandafter#1\expandafter,\the\pgfkeys@tmptoks}%
        \fi
        \edef#1{\the\pgfkeys@tmptoks}%
    },%
    /pgf/key filter handlers/ignore/.code={},
    /pgf/key filter handlers/ignore/.install key filter handler,
    /pgf/key filter handlers/log/.code={%
        \pgf@typeout{LOG: the option '\pgfkeyscurrentkey' (was originally '\pgfkeyscurrentkeyRAW') (case \pgfkeyscasenumber) has not been processed due to pgfkeysfiltered.}%
    },
    %
    %
    % KEY FILTER PREDICATES:
    %
    % Returns true if the currently processed key belongs to an active family.
    % A family is active if it has been activated before.
    /pgf/key filters/active families/.code={%
        \if\pgfkeyscasenumber0%
            % unknown options shall be processed with the
            % unknown-handlers.
            \pgfkeysfiltercontinuetrue
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },%
    %
    %
    %
    % This filter works as follows:
    % 1. if the current key belongs to a family:
    %    return whether its family is active,
    % 2. if the current key does NOT belong to a family:
    %    return the result of criterion '#1',
    % 3. the current key is unknown:
    %    return the result of criterion '#2'.
    %
    % Arguments:
    % #1: the predicate which will be invoked in case 2.
    %     It will be invoked with the current case number as argument.
    % #2: the predicate which will be invoked in case 3 with
    %     the current case number as argument.
    /pgf/key filters/active families or no family/.code 2 args={%
        \if\pgfkeyscasenumber0%
            \pgfkeysevalkeyfilterwith{#2}%
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysevalkeyfilterwith{#1}%
            \fi
        \fi
    },
    /pgf/key filters/active families or no family DEBUG/.code 2 args={%
        \if\pgfkeyscasenumber0%
            \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking unknown handler '#2']}%
            \pgfkeysevalkeyfilterwith{#2}%
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
                \ifpgfkeysfiltercontinue
                    \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is ACTIVE]}%
                \else
                    \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) family is NOT active.]}%
                \fi
            \else% Ok, it does not belong to any family.
                \pgf@typeout{[pgfkeyshasactivefamilyornofamily(\pgfkeyscurrentkey, \pgfkeyscasenumber) invoking has-no-family-handler '#1']}%
                \pgfkeysevalkeyfilterwith{#1}%
            \fi
        \fi
    },
    %
    % A (faster) shortcut for
    % /pgf/key filters/active families or no family=
    %   {/pgf/keys filters/false}
    %   {/pgf/keys filters/false}
    /pgf/key filters/active families and known/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },
    % A (faster) shortcut for
    % /pgf/key filters/active families or no family=
    %   {/pgf/key filters/is descendant of=#1}% for keys without family
    %   {/pgf/keys filters/false}
    /pgf/key filters/active families or descendants of/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \if\pgfkeyscasenumber3%
                \pgfkeysgetfamily\pgfkeyscurrentpath\pgfkeyspred@TMP
            \else
                \pgfkeysgetfamily\pgfkeyscurrentkey\pgfkeyspred@TMP
            \fi
            \ifpgfkeyssuccess
                \pgfkeysisfamilyactive{\pgfkeyspred@TMP}%
            \else% Ok, it does not belong to any family.
                % the 'is descendant of' implementation has been
                % COPY PASTED here:
                %
                % string prefix comparison:
                \def\pgfkeysisdescendantof@impl##1#1##2\pgf@@eov{%
                    \def\pgfkeyspred@TMP{##1}%
                    \ifx\pgfkeyspred@TMP\pgfkeys@empty
                        \pgfkeysfiltercontinuetrue
                    \else
                        \pgfkeysfiltercontinuefalse
                    \fi
                }%
                \expandafter\pgfkeysisdescendantof@impl\pgfkeyscurrentkey#1\pgf@@eov
            \fi
        \fi
    },
    %
    % Processes only options which are children of #1.
    % Example:
    %   is descendant of/.install key filter=/foo
    % will be true for
    %   /foo/bar/x=y
    %   /foo/.cd
    %   /foo/bar/.style=...
    % but not for
    %   /bar/foo/...
    /pgf/key filters/is descendant of/.code={%
        \if\pgfkeyscasenumber0%
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is UNKNOWN. Calling unknown handler.}%
            % unknown options shall be processed with the
            % unknown-handlers.
            \pgfkeysfiltercontinuetrue
        \else
            % string prefix comparison:
            % [ note : this has been COPY-PASTED to
            %   |active families or descendants of| ]
            \def\pgfkeysisdescendantof@impl##1#1##2\pgf@@eov{%
                \def\pgfkeyspred@TMP{##1}%
                \ifx\pgfkeyspred@TMP\pgfkeys@empty
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': TRUE.}%
                    \pgfkeysfiltercontinuetrue
                \else
%\message{'\pgfkeyscurrentkey' (case \pgfkeyscasenumber) is descendant of '#1': FALSE.}%
                    \pgfkeysfiltercontinuefalse
                \fi
            }%
            \expandafter\pgfkeysisdescendantof@impl\pgfkeyscurrentkey#1\pgf@@eov
        \fi
    },%
    %
    %
    %
    % Returns true if the currently processed full key equals #2.
    /pgf/key filters/equals/.code={%
        \if\pgfkeyscasenumber0%
            % Unknown option:
            \pgfkeysfiltercontinuetrue
        \else
            \def\pgfkeyspred@TMP{#1}%
            \ifx\pgfkeyscurrentkey\pgfkeyspred@TMP
                \pgfkeysfiltercontinuetrue
            \else
                \pgfkeysfiltercontinuefalse
            \fi
        \fi
    },%
    %
    %
    % Argument #1 can be any other (evaluated) filter predicate, its logical return
    % value will be inverted.
    % Example:
    %   not/.install key filter={is descendant of=/tikz}
    % will install a key filter which evaluates 'is descendant of' with argument
    % '/tikz' and returns the logical negation of the result.
    %
    /pgf/key filters/not/.code={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
            \pgfkeysfiltercontinuefalse
        \else
            \pgfkeysfiltercontinuetrue
        \fi
    },%
    /pgf/key filters/and/.code 2 args={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
            \pgfkeysevalkeyfilterwith{#2}%
        \fi
    },%
    /pgf/key filters/or/.code 2 args={%
        \pgfkeysevalkeyfilterwith{#1}%
        \ifpgfkeysfiltercontinue
        \else
            \pgfkeysevalkeyfilterwith{#2}%
        \fi
    },%
    /pgf/key filters/true/.code={\pgfkeysfiltercontinuetrue},%
    /pgf/key filters/true/.install key filter,
    /pgf/key filters/false/.code={%
        \pgfkeysfiltercontinuefalse
    },%
    %
    % Returns false if the current key is unknown, which avoids calling
    % the unknown handlers.
    /pgf/key filters/defined/.code={%
        \if\pgfkeyscasenumber0%
            \pgfkeysfiltercontinuefalse
        \else
            \pgfkeysfiltercontinuetrue
        \fi
    },
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Private IMPLEMENTATION
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% This command does THE SAME work as \pgfkeys@case@one,
% but it applies filtering whenever it identified the type of an
% option.
\def\pgfkeys@case@one@filtered{%
    \pgfkeys@cur@is@descendant@of@errors
    \ifpgfkeysfiltercontinue
        \pgfkeys@orig@case@one
    \else
        \pgfkeysfiltercontinuetrue
        \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
            % CASE ONE: a command option
            \def\pgfkeyscasenumber{1}%
            \pgfkeys@key@predicate%
            \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
                \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
            \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                \pgfkeys@filtered@handler%
            \fi
        }{%
            % CASE TWO: a normal value option
            \pgfkeysifdefined{\pgfkeyscurrentkey}{%
                \def\pgfkeyscasenumber{2}%
                \pgfkeys@key@predicate%
                \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                    \pgfkeys@case@two@extern
                \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                    \pgfkeys@filtered@handler%
                \fi
            }{%
                \pgfkeys@split@path
                % CASE THREE: a handler
                \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
                    \pgfkeys@ifexecutehandler{%
                        \def\pgfkeyscasenumber{3}%
                        \pgfkeys@key@predicate%
                        \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                            \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
                            \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
                        \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                            \pgfkeys@filtered@handler%
                        \fi
                    }{%
                        \pgfkeys@unknown
                    }%
                }{%
                    \pgfkeys@unknown
                }%
            }%
        }%
    \fi
}%

\def\pgfkeys@unknown@filtered{%
    % CASE ZERO: an unknown option.
    \def\pgfkeyscasenumber{0}%
    \pgfkeys@key@predicate%
    \ifpgfkeysfiltercontinue
%\message{PROCESSING  KEY \pgfkeyscurrentkey!}%
        % start normal 'unknown' handlers:
        \pgfkeys@orig@unknown
    \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
        \pgfkeys@filtered@handler%
    \fi
}

% Does the same as \pgfkeys@try, but it also invokes the key filters.
\def\pgfkeys@try@filtered{%
    \ifpgfkeysfiltercontinue
        \pgfkeys@orig@try
    \else
        \pgfkeysfiltercontinuetrue
        \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}% make sure that \pgfkeys@code doesn't know about 'try'. Important for .is choice
        \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
            \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
            {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
            {}% no default, so leave it
        \fi%
        \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
        {%
            % CASE ONE: a command option
            \def\pgfkeyscasenumber{1}%
            \pgfkeys@key@predicate%
            \ifpgfkeysfiltercontinue
                \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
                \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
            \else
                \pgfkeys@filtered@handler%
            \fi
            \pgfkeyssuccesstrue%
        }%
        {%
            \pgfkeysifdefined{\pgfkeyscurrentpath}%
            {% CASE TWO: a normal value option
                \def\pgfkeyscasenumber{2}%
                \pgfkeys@key@predicate%
                \ifpgfkeysfiltercontinue
                    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
                        \pgfkeysvalueof{\pgfkeyscurrentpath}%
                    \else%
                        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
                    \fi%
                \else
                    \pgfkeys@filtered@handler%
                \fi
                \pgfkeyssuccesstrue%
            }%
            {%
                \pgfkeys@split@path%
                \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}{%
                    % CASE THREE: a handled key
                    %
                    % in the standard configuration, this check here is redundant
                    % because pgfkeys@ifexecutehandler === true.
                    % It is only interesting for 'handle only existing'.
                    \pgfkeys@ifexecutehandler{%
                        \def\pgfkeyscasenumber{3}%
                        \pgfkeys@key@predicate%
                        \ifpgfkeysfiltercontinue
%\message{PROCESSING KEY \pgfkeyscurrentkey!}%
                            \pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
                            \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov
                        \else
%\message{FILTERED OUT  KEY \pgfkeyscurrentkey!}%
                            \pgfkeys@filtered@handler%
                        \fi
                        \pgfkeyssuccesstrue%
                    }{%
                        \pgfkeyssuccessfalse
                    }%
                }{%
                    \pgfkeyssuccessfalse
                }%
            }%
        }%
    \fi
}


% #1 the code to invoke after init and before cleanup
\long\def\pgfkeys@install@filter@and@invoke#1{%
    \ifpgfkeysfilteringisactive
        \pgfkeys@error{Sorry, nested calls to key filtering routines are not allowed. (reason: It is not possible to properly restore the previous filtering state after returning from the nested call)}%
    \fi
    \pgfkeysfilteringisactivetrue
    \let\pgfkeys@case@one=\pgfkeys@case@one@filtered
    \let\pgfkeys@try=\pgfkeys@try@filtered
    \let\pgfkeys@unknown=\pgfkeys@unknown@filtered
    #1%
    \let\pgfkeys@case@one=\pgfkeys@orig@case@one
    \let\pgfkeys@try=\pgfkeys@orig@try
    \let\pgfkeys@unknown=\pgfkeys@orig@unknown
    \pgfkeysfilteringisactivefalse
}


%--------------------------------------------------
% \def\pgfkeys@eval@key@filter@subroutine@case@one{%
%     \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}{%
%         \pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
%         \let\pgfkeyspred@TMP=\pgfkeyscurrentvalue
%         \pgfkeys@eval@key@filter@subroutine@restorestate
%         \expandafter\pgfkeys@code\pgfkeyspred@TMP\pgfeov
%     }{%
%         \pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyscurrentkey\pgfkeyscurrentvalue\pgfeov%
%     }%
% }
% % THIS VERSION IS TOO SLOW. See below.
% \def\pgfkeysevalkeyfilterwith#1{%
%     \edef\pgfkeys@eval@key@filter@subroutine@restorestate{%
%         \noexpand\def\noexpand\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
%         \noexpand\def\noexpand\pgfkeyscurrentkeyRAW{\pgfkeyscurrentkeyRAW}%
%         \noexpand\def\noexpand\pgfkeyscurrentname{\pgfkeyscurrentname}%
%         \noexpand\def\noexpand\pgfkeyscurrentvalue{\pgfkeyscurrentvalue}%
%         \noexpand\pgfkeys@pathtoks={\pgfkeyscurrentpath}%
%     }%
%     \pgfkeysinterruptkeyfilter
%     \let\pgfkeys@case@one=\pgfkeys@eval@key@filter@subroutine@case@one
%     \pgfkeysalso{#1}%
%     \endpgfkeysinterruptkeyfilter% this here also restored \pgfkeys@case@one.
%     \pgfkeys@eval@key@filter@subroutine@restorestate
% }%
%--------------------------------------------------


% Evaluates a key filter '#1'. Example:
% \pgfkeysevalkeyfilterwith{/pgf/key filters/equals=/tikz}
%
% \pgfkeysevalkeyfilterwith works only if key filtering is
% active.
%
% The argument '#1' MUST be a FULL KEY.
%
% The implementation employs a subset of the \pgfkeysalso code.
\long\def\pgfkeysevalkeyfilterwith#1{%
    \pgfkeys@eval@key@filter@subroutine@unpack#1=\pgfkeysnovalue=\pgfkeys@stop
}%
\long\def\pgfkeys@eval@key@filter@subroutine@unpack#1=#2=#3\pgfkeys@stop{%
    \pgfkeys@spdef\pgfkeyspred@TMP{#1}%
    \edef\pgfkeyspred@TMP{\pgfkeyspred@TMP}%
    \pgfkeys@spdef\pgfkeyspred@TMPB{#2}% TMPB=value
    \ifx\pgfkeyspred@TMPB\pgfkeysnovalue@text% Hmm... no value
        \pgfkeysifdefined{\pgfkeyspred@TMP/.@def}%
        {\pgfkeysgetvalue{\pgfkeyspred@TMP/.@def}{\pgfkeyspred@TMPB}}
        {}% no default, so leave it
    \fi%
    \ifx\pgfkeyspred@TMPB\pgfkeysvaluerequired%
        \pgfkeysvalueof{/errors/value required/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
    \else%
        \pgfkeysifdefined{\pgfkeyspred@TMP/.@cmd}{%
            \pgfkeysgetvalue{\pgfkeyspred@TMP/.@cmd}{\pgfkeys@code}%
            \expandafter\pgfkeys@code\pgfkeyspred@TMPB\pgfeov
        }{%
            \pgfkeysvalueof{/errors/no such key filter/.@cmd}\pgfkeyspred@TMP\pgfkeyspred@TMPB\pgfeov%
        }%
    \fi%
}


\def\pgfkeys@non@outer@newif@#1#2{%
    \expandafter\edef\csname #2true\endcsname{\noexpand\let\noexpand#1=\noexpand\iftrue}%
    \expandafter\edef\csname #2false\endcsname{\noexpand\let\noexpand#1=\noexpand\iffalse}%
    \csname #2false\endcsname
}%

% For latex and context, this here has the same effect as a \newif
% applied to 'if#1'. For plain tex, it has also the same effect, but
% it is not an \outer macro as the plain-tex \newif.
\def\pgfkeys@non@outer@newif#1{%
    \expandafter\pgfkeys@non@outer@newif@\csname if#1\endcsname{#1}%
}
\endinput


==> pgfmath.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% Guard against reading twice
\ifx\pgfmathloaded\pgfutil@undefined
  \let\pgfmathloaded=\relax
\else
  \expandafter\endinput
\fi

% We need keys:
\ifx\pgfkeysloaded\pgfutil@undefined
  \input pgfkeys.code.tex
\fi

\input pgfmathcalc.code.tex
\input pgfmathfloat.code.tex

\endinput


==> pgfmathcalc.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file loads all the parsing, functions and operator stuff
%
% Version 1.414213 29/9/2007

\input pgfmathutil.code.tex
\input pgfmathparser.code.tex
\input pgfmathfunctions.code.tex
%\input pgfmathbase.code.tex

% \pgfmathsetlength, \pgfmathaddtolength
%
% #1 = dimension register
% #2 = expression
%
% Description:
%
% These functions work similar to \setlength and \addtolength. Only,
% they allow #2 to contain an expression, which is evaluated before
% assignment. Furthermore, the font is setup before the assignment is
% done, so that dimensions like 1em are evaluated correctly.
%
% If #2 starts with "+", then a simple assignment is done (but the
% font is still setup). This is orders of magnitude faster than a
% parsed assignment.

\def\pgfmathsetlength#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    % Ok, quick version:
    \begingroup%
      \pgfmath@selectfont%
      #1#2\unskip%
    \expandafter\endgroup%
    \expandafter#1\the#1\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \ifpgfmathmathunitsdeclared%
      #1\pgfmathresult mu\relax%
    \else%
      #1\pgfmathresult pt\relax%
    \fi%
  }%
  \ignorespaces%
}

% \pgfmathaddtolength
%
% Add to #1 the result of evaluating #2.
%
% #1 - a dimension register
% #2 - an expression
%
\def\pgfmathaddtolength#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \begingroup%
      \pgfmath@selectfont%
      \advance#1#2\unskip%
      \expandafter%
    \endgroup%
    \expandafter#1\the#1\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \ifpgfmathmathunitsdeclared%
      \advance#1\pgfmathresult mu\relax%
    \else%
      \advance#1\pgfmathresult pt\relax%
    \fi%
  }%
  \ignorespaces%
}

% \pgfmathsetcount
%
% Assign #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathsetcount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1#2\relax\pgfmath@%
  }%
  {%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
  }%
  \ignorespaces%
}

% \pgfmathaddtocount
%
% Add to #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathaddtocount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1#2\relax\pgfmath@%
    \advance#1\pgfmath@addtocounttemp\relax%
  }%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
    \advance#1\pgfmath@addtocounttemp\relax%
  }%
  \ignorespaces%
}

% \pgfmathnewcounter
%
% LaTeX style counter which also works in plain TeX. Defines
% \c@<name> as a count register and also defines \the<name>.
%
% #1 the name of the counter.
%
% Example:
%
% \pgfmathnewcounter{counter}
% \pgfmathsetcounter{counter}{12}
% \thecounter  (same as \the\c@counter)
%
\def\pgfmathnewcounter#1{%
  \expandafter\ifx\csname c@#1\endcsname\relax%
    \def\pgfmath@marshal{\csname newcount\endcsname}% Ha! Who cares about \outer?
    \expandafter\pgfmath@marshal\csname c@#1\endcsname%
    \expandafter\def\csname the#1\endcsname{\expandafter\the\csname c@#1\endcsname}%
  \fi%
}

% \pgfmathsetcounter
%
% Set the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathsetcounter#1#2{%
   \expandafter\pgfmathsetcount\csname c@#1\endcsname{#2}%
}

% \pgfmathaddtocounter
%
% Add the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathaddtocounter#1#2{%
  \expandafter\pgfmathaddtocount\csname c@#1\endcsname{#2}%
}

% \pgfmathmakecounterglobal
%
% Make the current value of a counter globally defined.
%
% #1 - a (valid) counter name.
%
\def\pgfmath@pgftext{pgf}
\def\pgfmath@tikztext{tikz}
\def\pgfmathmakecounterglobal#1{%
  \pgfmath@ifundefined{c@#1}{}{%
    \expandafter\pgfmath@in@\expandafter{\pgfmath@pgftext}{#1}%
    \ifpgfmath@in@%
    \else%
      \expandafter\pgfmath@in@\expandafter{\pgfmath@tikztext}{#1}%
      \ifpgfmath@in@%
      \else%
        \expandafter\global\csname c@#1\endcsname\csname c@#1\endcsname\relax%
      \fi%
    \fi%
  }%
}

% \pgfmathsetmacro
%
% \edef#1 as the result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetmacro#1#2{%
  \begingroup%
    \pgfmathparse{#2}%
    \let#1=\pgfmathresult
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% \pgfmathsetlengthmacro
%
% \edef#1 as the result of evaluating #2 with pt.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetlengthmacro#1#2{%
  \begingroup%
    \pgfmathsetlength\pgfmath@x{#2}%
    \edef#1{\the\pgfmath@x}%
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% \pgfmathtruncatemacro
%
% \edef#1 as the truncated result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathtruncatemacro#1#2{%
  \begingroup%
    \pgfmathsetcount\c@pgfmath@counta{#2}%
    \edef#1{\the\c@pgfmath@counta}%
    \pgfmath@smuggleone{#1}%
  \endgroup%
}

% Check whether a given parameter starts with quick.
%
% The command should be followed by nonempty text, ending with
% \pgfmath@ as a stop-token. Then should follow
%
% #1 - code to execute if text starts with +
% #2 - code to execute if text does not
%
% Example:
%
% \pgfmath@onquick+0pt\pgfmath@{is quick}{is slow}

\def\pgfmath@onquick{%
  \futurelet\pgfmath@next%
  \pgfmath@@onquick}
\def\pgfmath@@onquick#1\pgfmath@{%
  \ifx\pgfmath@next+%
    \let\pgfmath@next=\pgfmath@firstoftwo%
  \else%
    \let\pgfmath@next=\pgfmath@secondoftwo%
  \fi%
  \pgfmath@next%
}

% *** The following commands DO NOT WORK without the rest of PGF ***
%
% (a dumping ground for stuff that doesn't really belong anywhere else)

% \pgfmathanglebetweenpoints
%
% Define \pgfmathresult as the angle between points #1 and #2
% Should get the quadrants right as well.
%
\def\pgfmathanglebetweenpoints#1#2{%
  \begingroup%
    \pgf@process{\pgfpointdiff{#1}{#2}}%
    \edef\pgf@marshall{\expandafter\noexpand\csname pgfmathatan2@\endcsname{\expandafter\Pgf@geT\the\pgf@y}{\expandafter\Pgf@geT\the\pgf@x}}%
    \pgf@marshall%
    \ifdim\pgfmathresult pt<0pt%
      \pgfmathparse{\pgfmathresult+360}%
    \fi%
    \expandafter%
  \endgroup\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult}%
}

%
% \pgfmathrotatepointaround
%
% Rotate point #1 about point #2 by #3 degrees.
%
\def\pgfmathrotatepointaround#1#2#3{%
  \pgf@process{%
    \pgf@process{#1}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@process{#2}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \advance\pgf@x-\pgf@xa%
    \advance\pgf@y-\pgf@ya%
    \pgfmathsetmacro\angle{#3}%
    \pgfmathsin@{\angle}%
    \let\sineangle\pgfmathresult%
    \pgfmathcos@{\angle}%
    \let\cosineangle\pgfmathresult%
    \pgf@xa\cosineangle\pgf@x%
    \advance\pgf@xa-\sineangle\pgf@y%
    \pgf@ya\sineangle\pgf@x%
    \advance\pgf@ya\cosineangle\pgf@y%
    \pgf@x\pgf@xb%
    \pgf@y\pgf@yb%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
  }%
}

% \pgfmathanglebetweenlines
%
% Calculate the clockwise angle between a line from point #1
% to point #2 and a line from #3 to point #4.
%
\def\pgfmathanglebetweenlines#1#2#3#4{%
  \begingroup%
    \pgfmathanglebetweenpoints{#1}{#2}%
    \let\firstangle\pgfmathresult%
    \pgfmathanglebetweenpoints{#3}{#4}%
    \let\secondangle\pgfmathresult%
    \ifdim\firstangle pt>\secondangle pt\relax%
      \pgfmathadd@{\secondangle}{360}%
      \let\secondangle\pgfmathresult%
    \fi%
    \pgfmathsubtract@{\secondangle}{\firstangle}%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup%
}

% \pgfmathpointreflectalongaxis
%
% Reflects point #1 around an axis centered on #2 at an angle #3.
%
\def\pgfmathreflectpointalongaxis#1#2#3{%
  \pgf@process{%
    \pgfmathanglebetweenpoints{#2}{#1}%
    \pgfmath@tempdima\pgfmathresult pt\relax%
    \pgfmathparse{#3}%
    \advance\pgfmath@tempdima-\pgfmathresult pt\relax%
    \pgfmath@tempdima-2.0\pgfmath@tempdima%
    \pgfmathrotatepointaround{#1}{#2}{\pgfmath@tonumber{\pgfmath@tempdima}}%
  }%
}



% \pgfmathpointintersectionoflineandarc
%
% A bit experimental at the moment:
%
% Locates the point where a line crosses an eliptical arc. If the line
% does not cross the arc, a meaningless point will result.
%
% #1 the point of the line on the "convex" side of the arc.
% #2 the point of the line on the "concave" side of the arc.
% #3 the center of the eliptical arc.
% #4 start angle of the arc.
% #5 end angle of the arc.
% #6 radii of the arc.
%
\def\pgfmathpointintersectionoflineandarc#1#2#3#4#5#6{%
  \pgf@process{%
    %
    % Get the required angle.
    %
    \pgfmathanglebetweenpoints{#2}{#1}%
    \let\x\pgfmathresult%
    %
    % Get the radii of the arc.
    %
    \pgfmath@in@{and }{#6}%
    \ifpgfmath@in@%
      \pgf@polar@#6\@@%
    \else%
      \pgf@polar@#6 and #6\@@%
    \fi%
    \edef\xarcradius{\the\pgf@x}%
    \edef\yarcradius{\the\pgf@y}%
     %
    % Get the start and end angles of the arc...
    %
    \pgfmathsetmacro\s{#4}%
    \pgfmathsetmacro\e{#5}%
    %
    % ...and also with rounding.
    %
    \pgfmathmod@{\s}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\ss\pgfmathresult%
    \pgfmathmod@{\e}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi%
    \let\ee\pgfmathresult%
    %
    % Hackery for when arc straddles zero.
    %
    \ifdim\ee pt<\ss pt\relax%
      \pgfmathadd@{\x}{180}%
      \pgfmathmod@{\pgfmathresult}{360}%
      \let\x\pgfmathresult%
    \fi%
    \def\m{360}% Measure of nearness.
    \pgfmathadd@{\s}{\e}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\n\pgfmathresult% The best estimate (default to middle of arc).
    \pgfmathloop%
      \pgfmathadd@{\s}{\e}%
      \pgfmathdivide@{\pgfmathresult}{2}%
      \let\p\pgfmathresult%
      \ifdim\p pt=\s pt\relax%
      \else%
        \pgfmathanglebetweenpoints{#2}{%
          \pgfpointadd{#3}{%
            \pgf@x\xarcradius\relax%
            \pgfmathcos@{\p}%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y\yarcradius\relax%
            \pgfmathsin@{\p}%
            \pgf@y\pgfmathresult\pgf@y%
          }%
        }%
        %
        % Hackery for when arc straddles zero.
        %
        \ifdim\ee pt<\ss pt\relax%
          \pgfmathadd@{\pgfmathresult}{180}%
          \pgfmathmod@{\pgfmathresult}{360}%
        \fi%
        \let\q\pgfmathresult%
        %
        % More hackery...
        %
        \ifdim\x pt>335pt\relax%
          \ifdim\q pt<45pt\relax%
            \pgfmathadd@{\q}{360}%
            \let\q\pgfmathresult%
          \fi%
        \fi%
        \ifdim\x pt=\q pt% Found it!
            \pgfmathbreakloop% Breaks after current iteration is complete.
          \else
            \ifdim\x pt<\q pt\relax%
              \let\e\p%
            \else%
              \let\s\p%
            \fi%
          \fi%
          \pgfmathsubtract@{\x}{\q}%
          \pgfmathabs@{\pgfmathresult}%
          %
          % Save the estimate if it is better than any previous estimate.
          %
          \ifdim\pgfmathresult pt<\m pt\relax%
            \let\m\pgfmathresult%
            \let\n\p%
          \fi%
    \repeatpgfmathloop%
    \pgfpointadd{#3}{\pgfpointpolar{\n}{\xarcradius and \yarcradius}}%
  }%
}

% \pgfmathangleonellipse
%
% Find the angle corresponding to a point on the border of an ellispe.
%
% #1 - the point on the border.
% #2 - the radii of the ellipse.
%
\def\pgfmathangleonellipse#1#2{%
  \begingroup%
    \pgfmath@in@{and }{#2}%
    \ifpgfmath@in@%
      \pgf@polar@#2\@@%
    \else%
      \pgf@polar@#2 and #2\@@%
    \fi%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@process{#1}%
    \ifdim\pgf@x=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else%
      \pgfutil@tempdima\pgf@x%
      \pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgfutil@tempdima}}%
      \pgfutil@tempdima\pgfmathresult pt\relax%
    \fi%
    \ifdim\pgf@y=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else%
      \pgfmathdivide@{\pgfmath@tonumber{\pgf@y}}{\pgfmath@tonumber{\pgf@ya}}%
      \pgfutil@tempdima\pgfmathresult\pgfutil@tempdima%
      \pgfmathatan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
    \fi%
    %
    \pgfutil@tempdima\pgfmathresult pt\relax%
    \ifdim\pgfutil@tempdima<0pt\relax%
      \advance\pgfutil@tempdima360pt\relax%
    \fi%
    \ifdim\pgf@x<0pt\relax%
      \ifdim\pgf@y=0pt\relax%
        \pgfutil@tempdima180pt\relax%
      \else%
        \ifdim\pgf@y<0pt\relax%
          \advance\pgfutil@tempdima180pt\relax%
        \else%
          \advance\pgfutil@tempdima-180pt\relax%
        \fi%
      \fi%
    \else%
      \ifdim\pgf@x=0pt\relax%
        \ifdim\pgf@y<0pt\relax%
          \pgfutil@tempdima270pt\relax%
        \else%
          \pgfutil@tempdima90pt\relax%
        \fi%
      \else%
        \ifdim\pgf@y=0pt\relax%
          \pgfutil@tempdima0pt\relax%
        \fi%
      \fi%
    \fi%
    \pgfmath@returnone\pgfutil@tempdima%
  \endgroup%
}


% Local Variables:
% tab-width: 2
% End:


==> pgfmathfloat.code.tex <==
% Copyright 2019 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file contains methods for basic floating point arithmetics, rounding
% to arbitrary precision and number pretty printing.
%


\pgfkeys{
    % The bug 3430171 (wrong minus sign spacing in pgfmathprintnumber)
    % has been fixed in 2.10 CVS. Since it changes the spacing, its
    % effects can be undone with this compatibility switch.
    /pgf/compat/number printer/.is choice,
    /pgf/compat/number printer/2.10/.code={%
        \def\pgfmathprintnumber@begingroup{\bgroup}%
        \def\pgfmathprintnumber@endgroup{\egroup}%
    },
    % I do not know the version number of the next release at this
    % time. Please be so kind and KEEP THIS NAME INTACT. Add an alias
    % if needed.
    /pgf/compat/number printer/next after 2.10/.code={%
        \def\pgfmathprintnumber@begingroup{\begingroup}%
        \def\pgfmathprintnumber@endgroup{\endgroup}%
    },
    % activate the fix by default.
    /pgf/compat/number printer/next after 2.10,%
}


\global\newif\ifpgfmathfloatcomparison
\newif\ifpgfmathfloatroundhasperiod
\newif\ifpgfmathprintnumberskipzeroperiod


% used internally in grouped macros:
\toksdef\pgfmathfloat@tmptoks=1
\newif\ifpgfmathfloat@fixed@digits@after@period
\newif\ifpgfmathfloatroundmayneedrenormalize
\toksdef\pgfmathfloat@a@Mtok=0

%% WARNING: avoid conflicting register names!
\let\pgfmathfloat@a@S=\c@pgf@counta
\let\pgfmathfloat@a@M=\pgf@xa
\let\pgfmathfloat@a@E=\c@pgf@countb
\let\pgfmathfloat@b@S=\c@pgf@countc
\let\pgfmathfloat@b@M=\pgf@xb
\let\pgfmathfloat@b@E=\c@pgf@countd

% can be changed with options.
\def\pgfmathfloat@round@precision{2}

% I introduced this to access the "original" precision in case a
% formatted changes it locally... in this case, the formatter may
% overwrite \pgfmathfloat@round@precision@orig to provide the original
% one.
% The default implementation here does nothing:
\def\pgfmathfloat@round@precision@orig{\pgfmathfloat@round@precision}%

\gdef\pgfmathfloat@glob@TMP{}


% Computes a normalised floating point representation for #1 of the
% form
%   [FLAGS] MANTISSE EXPONENT
% meaning
%   [+-]X.XXXXXXX*10^C
% where
%   X.XXXXXX is a mantissa with first number != 0, C is an integer and
% FLAGS contains the sign and some other special cases.
%
% This method does NOT use TeX Registers to represent the numbers! The
% computation is COMPLETELY STRING BASED.
% This allows numbers such at 10000000 or 5.23e-10 to be represented
% properly, although TeX-registers would produce overflow/underflow
% errors in these cases.
%
% It is to be used to compute logs, because log(X*10^Y) = log(X) + log(10)*Y
%
% Arguments:
% #1:  an arbitrary number which shall be parsed. Maybe a macro.
%     Examples:
%     [+-]XXXXX.XXXXXX
%     [+-]XXXXX.XXXXXXeXXXX
%     [+-]0.0000XXXXXX
%     [+-]0.0000XXXXXXeXXXX
%     [+-]inf
%     nan
%    Maybe a macro containing such a number.
%
% Return value:
% \pgfmathresult will be \def'ed to
%  FLAGS MANTISSE 'e' EXPONENT
% where
% FLAGS is a number in [0-5] where
%     0 == '0' (the number is +- 0.0),
%     1 == '+',
%     2 == '-',
%     3 == 'not a number'
%     4 == '+ infinity'
%     5 == '- infinity'
%
% MANTISSE is a normalised number 1 <= M < 10. It always contains a
% period and at least one digit after the period.
%
% EXPONENT is an integer value.
%
% Example:
% \pgfmathfloatparsenumber{1}
% -> \pgfmathresult = 11.0e0
% \pgfmathfloatparsenumber{141.212}
% -> \pgfmathresult = 11.41212e2
\def\pgfmathfloatparsenumber#1{%
    \begingroup
    \edef\pgfmathresult{#1}%
    \expandafter\pgfflt@impl\pgfmathresult\pgfflt@EOI
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.0}%
    \fi
    \pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% The same as \pgfmathfloatparsenumber, but does not perform sanity checking.
% FIXME: there is no longer any difference here.
\let\pgfmathfloatqparsenumber=\pgfmathfloatparsenumber

% Takes a floating point number #1 as input and writes flags to count
% register #2, mantissa to dimen register #3 and exponent to count
% register #4.
\def\pgfmathfloattoregisters#1#2#3#4{%
    \expandafter\pgfmathfloat@decompose#1\relax{#2}{#3}{#4}%
}

% the same, but writes the mantissa into a token register.
\def\pgfmathfloattoregisterstok#1#2#3#4{%
    \expandafter\pgfmathfloat@decompose@tok#1\relax{#2}{#3}{#4}%
}

% Extracts the flags of #1 into the count register #2.
\def\pgfmathfloatgetflags#1#2{%
    \expandafter\pgfmathfloat@decompose@F#1\relax{#2}%
}
% Extracts the flags of #1 into the macro #2.
\def\pgfmathfloatgetflagstomacro#1#2{%
    \expandafter\pgfmathfloat@decompose@Fmacro#1\relax{#2}%
}%

% Extracts the mantissa of #1 into the dimen register #2.
\def\pgfmathfloatgetmantissa#1#2{%
    \expandafter\pgfmathfloat@decompose@M#1\relax{#2}%
}
\let\pgfmathfloatgetmantisse=\pgfmathfloatgetmantissa
% Extracts the mantissa of #1 into the token register #2.
\def\pgfmathfloatgetmantissatok#1#2{%
    \expandafter\pgfmathfloat@decompose@Mtok#1\relax{#2}%
}
\let\pgfmathfloatgetmantissetok=\pgfmathfloatgetmantissatok
% Extracts the exponent of #1 into the count register #2.
\def\pgfmathfloatgetexponent#1#2{%
    \expandafter\pgfmathfloat@decompose@E#1\relax{#2}%
}


% Assigns \pgfmathresult to be a float encoded as
% <FLAGS><MANTISSE>e<EXPONENT>
%
% example:
% \pgfmathfloatcreate{1}{2.0}{10}
% \pgfmathfloat@to@FMeE@style\pgfmathresult
% ->
% \pgfmathresult is now '12.0e10' regardless of the internal float
% format.
\def\pgfmathfloat@to@FMeE@style#1{\expandafter\pgfmathfloat@to@FMeE@style@#1\relax\relax}%
\def\pgfmathfloat@to@FMeE@style@#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@to@FMeE@style@@%
    \else
        \expandafter\pgfmathfloat@to@FMeE@style@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@to@FMeE@style@@#1Y#2e#3]\relax\relax{\def\pgfmathresult{#1#2e#3}}%
\def\pgfmathfloat@to@FMeE@style@error#1\relax\relax{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand\pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%


% decomposes a lowlevel floating point representation into flags,
% mantissa and exponent.
%
% #4: integer register for the flags.
% #5: dimen registers for the mantissa.
% #6: integer register for the exponent.
%
% \expandafter\pgfmathfloat@decompose\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@M\pgfmathfloat@a@E
% -> the three temp registers contain flags, mantissa and exponent
\def\pgfmathfloat@decompose#1#2{% sanitize!
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@%
    \else
        \expandafter\pgfmathfloat@decompose@error%
    \fi
    #1#2%
}
\def\pgfmathfloat@decompose@#1Y#2e#3]\relax#4#5#6{%
   #4=#1\relax
   #5=#2pt % keep space here.
   #6=#3\relax%
}

% overloaded, #5 needs to be a token register for the mantissa.
% @see also \pgfmathfloatvalueof  which does also employ the load
% level repr.
% \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
% -> the three temp registers contain flags, mantissa and exponent
\def\pgfmathfloat@decompose@tok#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@tok@%
    \else
        \expandafter\pgfmathfloat@decompose@tok@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@tok@#1Y#2e#3]\relax#4#5#6{%
   #4=#1\relax
   #5={#2}%
   #6=#3\relax%
}
% overloaded, returns only ONE of the three components into #4:
% \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S
% -> \pgfmathfloat@a@S contains the flags field.
\def\pgfmathfloat@decompose@F#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@F@%
    \else
        \expandafter\pgfmathfloat@decompose@F@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@Fmacro#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@Fmacro@%
    \else
        \expandafter\pgfmathfloat@decompose@F@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@M#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@M@%
    \else
        \expandafter\pgfmathfloat@decompose@M@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@E#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@E@%
    \else
        \expandafter\pgfmathfloat@decompose@E@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@Mtok#1#2{%
    \ifx#2Y%
        \expandafter\pgfmathfloat@decompose@Mtok@%
    \else
        \expandafter\pgfmathfloat@decompose@Mtok@error%
    \fi
    #1#2%
}%
\def\pgfmathfloat@decompose@F@#1Y#2e#3]\relax#4{#4=#1\relax}%
\def\pgfmathfloat@decompose@Fmacro@#1Y#2e#3]\relax#4{\def#4{#1}}%
\def\pgfmathfloat@decompose@M@#1Y#2e#3]\relax#4{#4=#2pt}%
\def\pgfmathfloat@decompose@Mtok@#1Y#2e#3]\relax#4{#4={#2}}%
\def\pgfmathfloat@decompose@E@#1Y#2e#3]\relax#4{#4=#3\relax}%

\def\pgfmathfloat@decompose@error#1\relax#2#3#4{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand#2=\the\pgfmathfloat@a@S\space
        \noexpand#3=\the\pgfmathfloat@a@Mtok pt
        \noexpand#4=\the\pgfmathfloat@a@E\space
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@tok@error#1\relax#2#3#4{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{%
        \noexpand#2=\the\pgfmathfloat@a@S\space
        \noexpand#3={\the\pgfmathfloat@a@Mtok}%
        \noexpand#4=\the\pgfmathfloat@a@E\space
    }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@F@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@S\space}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@M@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@Mtok pt }%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@Mtok@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2={\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
\def\pgfmathfloat@decompose@E@error#1\relax#2{%
    \begingroup
    \pgfmathfloatparsenumber@handleerror{wrong lowlevel format}{#1}{#1}%
    \xdef\pgfmathfloat@decompose@TMP{\noexpand#2=\the\pgfmathfloat@a@E\space}%
    \endgroup
    \pgfmathfloat@decompose@TMP
}%
% Takes a floating point number #1 as input and writes flags to macro
% #2, mantissa to macro #3 and exponent to macro #4.
\def\pgfmathfloattomacro#1#2#3#4{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\def\noexpand#2{\the\pgfmathfloat@a@S}%
        \noexpand\def\noexpand#3{\the\pgfmathfloat@a@Mtok}%
        \noexpand\def\noexpand#4{\the\pgfmathfloat@a@E}%
    }%
    \endgroup
    \pgfmathfloat@glob@TMP
}


% Defines \pgfmathresult as the floating point number encoded by
% the flags #1, mantissa #2 and exponent #3.
%
% All arguments are characters and will be expanded using '\edef'.
\def\pgfmathfloatcreate#1#2#3{%
    \edef\pgfmathresult{#1Y#2e#3]}%
}%
% This is the character present in any low-level floating point
% number. It is assumed to be the SECOND character of a float (after
% the flags integer).
\def\pgfmathfloat@POSTFLAGSCHAR{Y}



% Converts a composed floating point representation to fixed point.
%
% Example:
% \pgfmathfloattofixed{142e1}
% -> \pgfmathresult = 42.0
\def\pgfmathfloattofixed@#1{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifcase\pgfmathfloat@a@S
        \def\pgfmathresult{0.0}%
    \or
        \expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
    \or
        \expandafter\pgfmathfloattofixed@impl\the\pgfmathfloat@a@Mtok\relax
        \pgfmathfloat@a@Mtok=\expandafter{\pgfmathresult}%
        \edef\pgfmathresult{-\the\pgfmathfloat@a@Mtok}%
    \or\def\pgfmathresult{nan}%
    \or\def\pgfmathresult{inf}%
    \or\def\pgfmathresult{-inf}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\let\pgfmathfloattofixed=\pgfmathfloattofixed@

% Converts a float to an integer (in integer format).
%
% @see \pgfmathfloatint
\def\pgfmathfloattoint#1{%
    \pgfmathfloattofixed{#1}%
    \expandafter\pgfmathfloattoint@@\pgfmathresult\relax
}%
\def\pgfmathfloattoint@@#1.#2\relax{%
    \def\pgfmathresult{#1}%
}%

% Converts a floating point number to scientific format 1.234e5.
%
% This operation is very fast.
\def\pgfmathfloattosci@#1{%
    \begingroup
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifcase\pgfmathfloat@a@S
        \def\pgfmathresult{0.0e0}%
    \or
        \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
    \or
        \edef\pgfmathresult{-\the\pgfmathfloat@a@Mtok e\the\pgfmathfloat@a@E}%
    \or\def\pgfmathresult{nan}%
    \or\def\pgfmathresult{inf}%
    \or\def\pgfmathresult{-inf}%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%
\let\pgfmathfloattosci=\pgfmathfloattosci@

% Expands a floating point number to scientific format 1.234e5.
%
% This operation is very fast.
\def\pgfmathfloatvalueof#1{\expandafter\pgfmathfloatvalueof@@#1@@}%

% Make it fool proof such that the following arguments work:
%     \pgfmathfloatvalueof{1Y1.0e1} -> 1.0e1
%     \pgfmathfloatvalueof{2Y1.0e1} -> -1.0e1
% and wrong arguments as well:
%     \pgfmathfloatvalueof{1} -> 1
%     \pgfmathfloatvalueof{1e2} -> 1e2
\def\pgfmathfloatvalueof@@#1#2{%
    \if#2Y%
        % keep in mind that \pgfmathfloatvalueof should be expandable!
        % We must not use \let here. Let's hope that #1 and #2 are
        % single tokens (not something which was enclosed by curly
        % braces...)
        \expandafter\pgfmathfloatvalueof@@@\expandafter#1\expandafter#2%
    \else
        % Oh - no float!? Ok, we cannot report errors in this context.
        % So: make it a feature and return the input argument as-is.
        % Might be useful, in fact...
        \expandafter\pgfmathfloatvalueof@abort\expandafter#1\expandafter#2%
    \fi
}
\def\pgfmathfloatvalueof@@@#1Y#2e#3]@@{%
    \ifcase#1 %
        0.0e0%
    \or
        #2e#3%
    \or
        -#2e#3%
    \or nan%
    \or inf%
    \or -inf%
    \fi
}%
\def\pgfmathfloatvalueof@abort#1@@{#1}%



% Rounds a fixed point number #1 to \pgfmathfloat@round@precision digits precision and returns
% the result into \pgfmathresult.
%
% Any trailing zeros after the period are discarded.
% See \pgfmathroundtozerofill if you want trailing zeros and fixed
% width.
%
% This method is PURELY text based and can work with arbitrary
% precision (well, limited to TeX's stack size and integer size).
%
% Examples:
% \pgfmathroundto{1}
% -> \pgfmathresult = '1'
%
% \pgfmathroundto{19999.9996}
% -> \pgfmathresult = '20000'
%
% Arguments:
% #1 may be either a number or a macro (\pgfmathresult is allowed) expanding to a number.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundto#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodfalse
    \pgfmathroundto@impl{#1}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}


% Overloaded method.
%
% This variant always uses a FIXED number behind the period and fills
% in zeros if necessary.
% Examples:
% \pgfmathroundtozerofill{1}
% -> \pgfmathresult = '1.00'
%
% \pgfmathroundtozerofill{19999.9996}
% -> \pgfmathresult = '20000.00'
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set.
\def\pgfmathroundtozerofill#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodtrue
    \pgfmathroundto@impl{#1}%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% see \pgfmathprintnumber@fixed@style for docs
\def\pgfmathprintnumber@fixed@styleDEFAULT#1#2#3e#4\relax{%
    \begingroup
    \pgfkeysgetvalue{/pgf/number format/set decimal separator}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP
    \pgfkeysgetvalue{/pgf/number format/@dec sep mark}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK
    \pgfkeysgetvalue{/pgf/number format/set thousands separator}\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP
    \c@pgf@counta=#4\relax % it is the exponent here.
    \ifnum#2=0
        \c@pgf@counta=0
    \fi
    \def\pgfmathresult{}%
    \ifpgfmathfloatroundhasperiod
        \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1\pgfmathfloat@EOI
    \else
        \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI%
        \begingroup
        \toks0=\expandafter{\pgfmathresult}%
        \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
        \endgroup
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@period#1.#2\pgfmathfloat@EOI{%
    \ifpgfmathprintnumberskipzeroperiod
        \def\pgfmathfloat@loc@TMPb{#1}%
        \ifx\pgfmathfloatparsenumber@tok@ZERO\pgfmathfloat@loc@TMPb
        \else
            \def\pgfmathfloat@loc@TMPc{-0}%
            \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
                \def\pgfmathresult{-}%
            \else
                \def\pgfmathfloat@loc@TMPc{+0}%
                \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
                    \def\pgfmathresult{+}%
                \else
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
                \fi
            \fi
        \fi
    \else
        \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
    \fi
    \ifpgfmathprintnumber@thousand@sep@in@fractional
        \let\pgfmathresultfractional\pgfutil@empty%
        \pgfmathprintnumber@thousand@sep@in@fractional#2MMMM\@@
    \else
        \def\pgfmathresultfractional{#2}%
    \fi
    \begingroup
    \toks0=\expandafter{\pgfmathresult}%
    \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
    \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP}%
    \toks3=\expandafter{\pgfmathresultfractional}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 \the\toks3 }%
    \endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}%

% assigns \pgfmathresult such that it contains the formatted result.
% It assumes that none of the following tokens contains a period.
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod{%
    \ifx\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP\pgfutil@empty
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
    \else
        \ifnum\c@pgf@counta<0\relax % exponent of the number in this context
            \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
        \else
            \ifnum\c@pgf@counta<\pgfkeysvalueof{/pgf/number format/min exponent for 1000 sep}\relax
                \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall}%
            \else
                \advance\c@pgf@counta by1 % counta:= total number of digits, N.
                \c@pgf@countb=\c@pgf@counta
                \divide\c@pgf@countb by3 %  countb := N DIV 3
                \c@pgf@countc=\c@pgf@countb
                \multiply\c@pgf@countc by3
                \advance\c@pgf@counta by-\c@pgf@countc% now counta := N MOD 3
                \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
                    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign
                }%
            \fi
        \fi
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printsign#1{%
    \def\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
        \let\pgfmathfloat@loc@TMPb=\pgfutil@empty
    \else
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
            \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
            \let\pgfmathfloat@loc@TMPb=\pgfutil@empty
        \else
            \ifpgfmathprintnumber@showpositive
                \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult +}%
            \fi
        \fi
    \fi
    \ifnum\c@pgf@counta>0 % \c@pgf@counta = N MOD 3 in this context
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits\pgfmathfloat@loc@TMPb
        }%
    \else
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird\pgfmathfloat@loc@TMPb
        }%
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printtrailingdigits#1#2{%
    \ifcase\c@pgf@counta % = N MOD 3 in this context
        % does not happen per construction
    \or
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#2%
        }%
    \or
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2}%
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
        }%
    \fi
    \ifnum\c@pgf@countb>0\relax % \c@pgf@countb = N DIV 3 in this context
        \begingroup
        \toks0=\expandafter{\pgfmathresult}%
        \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
        \endgroup
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird#1#2#3{%
    \ifnum\c@pgf@countb>0\relax
        \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1#2#3}%
        \advance\c@pgf@countb by-1
        \ifnum\c@pgf@countb>0\relax
            \begingroup
            \toks0=\expandafter{\pgfmathresult}%
            \toks1=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
            \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
            \endgroup
            \let\pgfmathresult=\pgfmathfloat@glob@TMP
        \fi
        \def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT{%
            \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@counteverythird%
        }%
    \else
        % in this case, #1#2#3 are expected to be
        % \pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI
        %--------------------------------------------------
        % \def\pgfmathfloat@loc@TMPb{\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI}%
        % \def\pgfmathfloat@loc@TMPc{#1#2#3}%
        % \ifx\pgfmathfloat@loc@TMPc\pgfmathfloat@loc@TMPb
        % \else
        %     \pgfmath@error{INTERNAL ERROR in fixed style - The input sequence did not terminate as expected; which indicates a wrong exponent argument provided to \string\pgfmathprintnumber@fixed@style}{}%
        % \fi
        %--------------------------------------------------
        \let\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT=\relax
    \fi
    \pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@NEXT
}

% \pgfmathprintnumber@thousand@sep@in@fractional 01234525MMMM\@@
% ->
% 012<sep>345<sep>25
\def\pgfmathprintnumber@thousand@sep@in@fractional#1#2#3#4{%
    \if#4M%
        % Ok, no further separator
        \def\pgfmathprint@next{\pgfmathprintnumber@thousand@sep@in@fractional@finish#1#2#3#4}%
    \else
        \begingroup
        \toks0=\expandafter{\pgfmathresultfractional}%
        \toks1={#1#2#3}%
        \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@THOUSAND@SEP}%
        \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 }%
        \endgroup
        \let\pgfmathresultfractional=\pgfmathfloat@glob@TMP
        \def\pgfmathprint@next{\pgfmathprintnumber@thousand@sep@in@fractional#4}%
    \fi
    \pgfmathprint@next
}%
\def\pgfmathprintnumber@thousand@sep@in@fractional@finish#1M{%
    \expandafter\def\expandafter\pgfmathresultfractional\expandafter{\pgfmathresultfractional #1}%
    \pgfmathprintnumber@thousand@sep@in@fractional@finish@
}%
\def\pgfmathprintnumber@thousand@sep@in@fractional@finish@#1\@@{}%

\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall#1{%
    \def\pgfmathfloat@loc@TMPb{#1}%
    \let\pgfmathfloat@loc@TMPc=\pgfutil@empty
    \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@MINUS
    \else
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloatparsenumber@tok@PLUS
        \else
            \ifpgfmathprintnumber@showpositive
                \def\pgfmathfloat@loc@TMPc{+}%
            \fi
        \fi
    \fi
    \expandafter\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@\pgfmathfloat@loc@TMPc#1%
}
\def\pgfmathprintnumber@fixed@styleDEFAULT@impl@noperiod@printall@#1\pgfmathfloat@EOI\pgfmathfloat@EOI\pgfmathfloat@EOI{%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmathresult #1}%
}%

% @deprecated. It has been replaced by \pgfmathprintnumber@fixed@styleDEFAULT
% #1 maybe a macro
\def\pgfmathprintnumber@fixed@stylePERIOD#1#2#3e#4\relax{%
    \def\pgfmathresult{#1}%
}

% @deprecated. It has been replaced by \pgfmathprintnumber@fixed@styleDEFAULT
% #1 maybe a macro
\def\pgfmathprintnumber@fixed@styleCOMMA#1#2#3e#4\relax{%
    \ifpgfmathfloatroundhasperiod
        \expandafter\pgfmathprintnumber@fixed@styleCOMMA@impl#1\pgfmathfloat@EOI
    \else
        \def\pgfmathresult{#1}%
    \fi
}
\def\pgfmathprintnumber@fixed@styleCOMMA@impl#1.#2\pgfmathfloat@EOI{\def\pgfmathresult{#1{,}#2}}

% The default style to display fixed point numbers.
%
% It does not apply numerics, but it is responsible for typesetting the
% rounded number.
% It can access the \ifpgfmathfloatroundhasperiod boolean.
%
% Arguments:
% #1#2#3e#4\relax

% Input:
% #1  the fixed point number to be displayed (maybe a macro).
% #2#3e#4:  the (possibly unformatted) floating point representation
%     which belongs to #1. This format is returned (only!) by
%     \pgfmathfloat@to@FMeE@style.
%     It is used to determine sign and exponent.
\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT


% Rounds a normalized floating point number to \pgfmathfloat@round@precision
% digits precision and writes the result to \pgfmathresult.
%
% This method uses \pgfmathroundto for the mantissa.
%
% @see pgfmathfloatroundzerofill
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantissa #5 has a period or not.
\def\pgfmathfloatround#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodfalse
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \pgfmathfloatround@impl
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% Overload.
%
% This method uses a fixed width for the mantissa and fills in zeros
% if necessary.
%
% This method uses \pgfmathroundtozerofill for the mantissa.
%
% SIDE EFFECT: the global variable \ifpgfmathfloatroundhasperiod will be set to
% whether the final mantissa #5 has a period or not.
\def\pgfmathfloatroundzerofill#1{%
    \pgfmathfloatroundhasperiodtrue
    \begingroup
    \pgfmathfloat@fixed@digits@after@periodtrue
    \expandafter\pgfmathfloat@decompose@tok#1\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \pgfmathfloatround@impl
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\newif\ifpgfmathfloatround@allow@empty@mantissa
\def\pgfmathfloatround@mantissa@ONE{1pt }%

% #1: sign
% #2: mantissa
% #3: exponent
% #4: CODE to display if the mantissa is drawn.
%     This code will be shown just before the exponent.
%     Example: #4=\cdot
% #5: CODE to display if the mantissa is NOT draw. (unused currently)
%     Might be used to display '10^1' instead of '1*10^1'.
% #6: CODE to display the exponent.
\def\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax#4#5#6{%
    \pgfkeysgetvalue{/pgf/number format/@sci exponent mark}\pgfmathfloatrounddisplaystyle@e@mark
    \ifcase#1\relax
        \pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
        \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
    \or
        \def\pgfmathfloat@loc@TMPa{1}% "should draw mantissa=1"
        \ifpgfmathfloatround@allow@empty@mantissa
        \else
            \ifdim#2pt=\pgfmathfloatround@mantissa@ONE
                \def\pgfmathfloat@loc@TMPa{0}% do not draw it.
            \fi
        \fi
        %
        \if1\pgfmathfloat@loc@TMPa
            \pgfmathprintnumber@fixed@style{#2}#1#2e0\relax%
            \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
        \else
            \def\pgfmathfloat@loc@TMPa{0}%
            \pgfmathfloatrounddisplaystyle@shared@impl@{#5}{#6}%
        \fi
    \or
        \def\pgfmathfloat@loc@TMPa{1}% "should draw mantissa=1"
        \ifpgfmathfloatround@allow@empty@mantissa
        \else
            \ifdim#2pt=\pgfmathfloatround@mantissa@ONE
                \def\pgfmathfloat@loc@TMPa{0}% do not draw it.
            \fi
        \fi
        %
        \if1\pgfmathfloat@loc@TMPa
            \pgfmathprintnumber@fixed@style{-#2}#1#2e0\relax%
            \expandafter\pgfmathfloatrounddisplaystyle@shared@impl@\expandafter{\pgfmathresult}{#4#6}%
        \else
            \def\pgfmathfloat@loc@TMPa{0}%
            \pgfmathfloatrounddisplaystyle@shared@impl@{-#5}{#6}%
        \fi
    \or
        \pgfmathfloatrounddisplaystyle@shared@impl@@{\hbox{NaN}}{}%
    \or
        \ifpgfmathprintnumber@showpositive
            \pgfmathfloatrounddisplaystyle@shared@impl@@{+\infty}{}%
        \else
            \pgfmathfloatrounddisplaystyle@shared@impl@@{\infty}{}%
        \fi
    \or
        \pgfmathfloatrounddisplaystyle@shared@impl@@{-\infty}{}%
    \fi
}

% #1: the part before the exponent code
% #2: the part for the exponent code.
\def\pgfmathfloatrounddisplaystyle@shared@impl@#1#2{%
    \pgfmathprintnumber@begingroup
    \toks0={#1}%
    \toks1=\expandafter{\pgfmathfloatrounddisplaystyle@e@mark #2}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 }%
    \pgfmathprintnumber@endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}%
% Same as \pgfmathfloatrounddisplaystyle@shared@impl@, but it also
% inserts the '@dec sep mark' at the end.
\def\pgfmathfloatrounddisplaystyle@shared@impl@@#1#2{%
    \pgfmathprintnumber@begingroup
    \toks0={#1}%
    \toks1=\expandafter{\pgfmathfloatrounddisplaystyle@e@mark #2}%
    \pgfkeysgetvalue{/pgf/number format/@dec sep mark}\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK
    \toks2=\expandafter{\pgfmathprintnumber@fixed@styleDEFAULT@DEC@SEP@MARK}%
    \xdef\pgfmathfloat@glob@TMP{\the\toks0 \the\toks1 \the\toks2 }%
    \pgfmathprintnumber@endgroup
    \let\pgfmathresult=\pgfmathfloat@glob@TMP
}

\def\pgfmathfloatrounddisplaystyle@std#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{\cdot}{}{10^{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@subscript#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}{_{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@superscript#1#2e#3\relax{%
    \pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}{^{#3}}%
}
\def\pgfmathfloatrounddisplaystyle@e#1#2e#3\relax{%
    \ifnum#3<0\relax
        \pgfmathprintnumber@begingroup
        \count0=#3\relax
        \multiply\count0 by-1
        \xdef\pgfmathfloat@glob@TMP{e{-}\the\count0}%
        \pgfmathprintnumber@endgroup%
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \else
        \def\pgfmathresult{e{+}#3}%
    \fi
    \def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
    \expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}
\def\pgfmathfloatrounddisplaystyle@E#1#2e#3\relax{%
    \ifnum#3<0\relax
        \pgfmathprintnumber@begingroup
        \count0=#3\relax
        \multiply\count0 by-1
        \xdef\pgfmathfloat@glob@TMP{E{-}\the\count0}%
        \pgfmathprintnumber@endgroup%
        \let\pgfmathresult=\pgfmathfloat@glob@TMP
    \else
        \def\pgfmathresult{E{+}#3}%
    \fi
    \def\pgfmathfloat@loc@TMPb{\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\relax{}{1}}%
    \expandafter\pgfmathfloat@loc@TMPb\expandafter{\pgfmathresult}%
}

\def\pgfmathfloatrounddisplaystyle@generic#1#2e#3\relax{%
    \begingroup
    \pgfkeysvalueof {/pgf/number format/sci generic/@/.@cmd}{#3}{#1}{#2}\pgfeov
    \pgfkeysgetvalue{/pgf/number format/sci generic/mantissa sep}\pgfmathdisplay@aftermantissa
    \pgfkeysgetvalue{/pgf/number format/sci generic/empty mantissa sep}\pgfmathdisplay@nomantissa
    \pgfkeysgetvalue{/pgf/number format/sci generic/exponent}\pgfmathdisplay@e
    \toks0=\expandafter{\pgfmathdisplay@aftermantissa}%
    \toks1=\expandafter{\pgfmathdisplay@nomantissa}%
    \toks2=\expandafter{\pgfmathdisplay@e}%
    \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfmathfloatrounddisplaystyle@shared@impl#1#2e#3\noexpand\relax{\the\toks0}{\the\toks1}{\the\toks2}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}

% A macro which takes the argument '<SIGN><MANTISSE>e<EXPONENT>' and
% expands to the final TeX-representation for that floating point
% number.
%
% PRECONDITION:
%   the floating point number has already been rounded properly and
%   the mantissa has been rounded correctly.
%
% The argument needs to be in the format returned by
% \pgfmathfloat@to@FMeE@style and terminated by '\relax'.
\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std
\newif\ifpgfmathfloat@usezerofill@sci
\newif\ifpgfmathfloat@usezerofill@fixed
\newif\ifpgfmathprintnumber@assumemathmode
\newif\ifpgfmathprintnumber@showpositive
\newif\ifpgfmathprintnumber@frac@warn
\newif\ifpgfmathprintnumber@frac@whole
\newif\ifpgfmathparsenumber@comma@as@period

\long\def\pgfmathfloatfrac@verbatim#1#2{#1/#2}%

\let\pgfmathround@@orig=\pgfmathround@

% 2 = compatible
% 0 = no
% 1 = yes
\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{2}%

\newif\ifpgfmathprintnumber@thousand@sep@in@fractional
\pgfkeys{%
    /pgf/number format/.is family,
    /pgf/number format,
    fixed/.code=           \pgfmath@set@number@printer{pgfmathprintnumber@FIXED},
    sci/.code=             \pgfmath@set@number@printer{pgfmathprintnumber@SCI},
    std/.code=             {\pgfmath@set@number@printer{pgfmathprintnumber@STD}\pgfmathprintnumber@STD@setparam{#1}},
    std/.default=,%
    relative round mode/.is choice,
    relative round mode/fixed/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{1}},
    relative round mode/mantissa/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{0}},
    relative round mode/compatible/.code={\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed{2}},
    % relative={<exponent base 10>}
    relative/.code={%
        \pgfmath@set@number@printer{pgfmathprintnumber@RELATIVE}%
        \pgfmathround@@orig{#1}%
        \expandafter\pgfmathfloattoint@@\pgfmathresult\relax
        \let\pgfmathprintnumber@RELATIVE@param=\pgfmathresult
    },%
    relative/.value required,
    relative*/.style={/pgf/number format/relative={#1},/pgf/number format/relative round mode=fixed},
    every relative/.style=std,
    relative style/.style={/pgf/number format/every relative/.append style={#1}},
    fixed relative/.code=  \pgfmath@set@number@printer{pgfmathprintnumber@FIXED@RELATIVE},
    int detect/.code=      \pgfmath@set@number@printer{pgfmathprintnumber@INT@DETECT},
    int trunc/.code=       \pgfmath@set@number@printer{pgfmathprintnumber@INT@TRUNC},
    frac/.code=            \pgfmath@set@number@printer{pgfmathprintnumber@frac},%
    frac TeX/.initial=\frac,
    frac whole format/.code={\def\pgfmathresult{#1}},
    frac denom/.initial=,
    frac whole/.is if=pgfmathprintnumber@frac@whole,
    frac whole=true,
    frac shift/.initial=4,
    frac warning/.is if=pgfmathprintnumber@frac@warn,
    frac warning=true,
    assume math mode/.is if=pgfmathprintnumber@assumemathmode,
    assume math mode/.default=true,
    fixed zerofill/.is if= pgfmathfloat@usezerofill@fixed,
    fixed zerofill/.default=true,
    sci zerofill/.is if=   pgfmathfloat@usezerofill@sci,
    sci zerofill/.default=true,
    zerofill/.style=       {/pgf/number format/fixed zerofill=#1,/pgf/number format/sci zerofill=#1},
    zerofill/.default=     true,
    precision/.store in=   \pgfmathfloat@round@precision,
    sci precision/.code={%
        \edef\pgfmathfloat@loc@TMPa{#1}%
        \ifx\pgfmathfloat@loc@TMPa\pgfutil@empty
            \def\pgfmathprintnumber@sci@precision{\pgfmathfloat@round@precision}%
        \else
            \let\pgfmathprintnumber@sci@precision=\pgfmathfloat@loc@TMPa
        \fi
    },%
    sci precision/.default=,
    sci precision=,
    fixed default/.code=   {\let\pgfmathprintnumber@fixed@style=\pgfmathprintnumber@fixed@styleDEFAULT},
    set decimal separator/.initial=,
    dec sep/.style={/pgf/number format/set decimal separator={#1}},
    @dec sep mark/.initial=,
    @sci exponent mark/.initial=,
    set thousands separator/.initial=,
    1000 sep in fractionals/.is if=pgfmathprintnumber@thousand@sep@in@fractional,
    1000 sep in fractionals/.default=true,
    1000 sep/.style={/pgf/number format/set thousands separator={#1}},
    min exponent for 1000 sep/.initial=0,
    use period/.style=     {/pgf/number format/set decimal separator={.},/pgf/number format/set thousands separator={{{,}}}},
    use comma/.style=      {/pgf/number format/set decimal separator={{{,}}},/pgf/number format/set thousands separator={.}},
    showpos/.is if=pgfmathprintnumber@showpositive,
    showpos/.default=true,
    print sign/.is if=pgfmathprintnumber@showpositive,
    print sign/.default=true,
    read comma as period/.is if=pgfmathparsenumber@comma@as@period,
    read comma as period/.default=true,
    skip 0./.is if=pgfmathprintnumberskipzeroperiod,
    skip 0./.default=true,
    skip 0.= false,
    use period,
    sci 10^e/.code=        {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
    sci 10e/.code=         {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@std},
    sci e/.code=           {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@e},
    sci E/.code=           {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@E},
    sci subscript/.code=   {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@subscript},
    sci superscript/.code= {\let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@superscript},
    sci generic/.code=     {%
        \let\pgfmathfloatrounddisplaystyle=\pgfmathfloatrounddisplaystyle@generic
        \pgfkeysdefargs{/pgf/number format/sci generic/@}%
            {##1##2##3}%
            {\pgfqkeys{/pgf/number format/sci generic}{#1}}%
    },
    sci generic/mantissa sep/.initial=,%
    sci generic/empty mantissa sep/.initial=,%
    sci generic/mantisse sep/.style={/pgf/number format/sci generic/mantissa sep={#1}},%
    sci generic/empty mantisse sep/.style={/pgf/number format/sci generic/empty mantissa sep={#1}},%
    sci generic/exponent/.initial=,%
    sci generic/.value required,
    verbatim/.code={%
        \pgfqkeys{/pgf/number format}{%
            sci generic={mantissa sep=,exponent={e##1}},
            1000 sep=,
            skip 0.=false,
            print sign=false,
            dec sep=.,
            assume math mode,
            frac TeX=\pgfmathfloatfrac@verbatim,
            frac whole format/.code={\def\pgfmathresult{##1 }},
            @dec sep mark=,
            @sci exponent mark=,
        }%
    },
    retain unit mantissa/.is if=pgfmathfloatround@allow@empty@mantissa,
    retain unit mantissa/.default=true,
    retain unit mantissa=true,
    %
    % allows to replace the implementation, for example
    % 'implementation=\num'. This is experimental -- it is unclear
    % if all consumers work well since they rely on the keys in
    % /pgf/number format.
    implementation/.code={\def\pgfmathprintnumber@protected{#1}},
}



\def\pgfmathprintnumber@STD#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@STD@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@STD@setparam#1{%
    \edef\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfutil@empty
        % DEFAULT for lower and upper bound.
        \def\pgfmathprintnumber@STD@getlowerbound{%
            \c@pgf@counta=\pgfmathfloat@round@precision@orig\relax
            \divide\c@pgf@counta by-2\relax
        }%
        \def\pgfmathprintnumber@STD@upperbound{4}%
    \else
        \expandafter\pgfutil@in@\expandafter:\expandafter{\pgfmathfloat@loc@TMPb}%
        \ifpgfutil@in@
            % we have -4:5 or something like that.
            % parse both values:
            \def\pgfmathfloat@loc@TMPa##1:##2\relax{%
                \edef\pgfmathprintnumber@STD@getlowerbound{%
                    \noexpand\c@pgf@counta=##1\space
                }%
                \edef\pgfmathprintnumber@STD@upperbound{##2}%
            }%
            \expandafter\pgfmathfloat@loc@TMPa\pgfmathfloat@loc@TMPb\relax
        \else
            % we have just the lower bound:
            \def\pgfmathprintnumber@STD@upperbound{4}%
            \edef\pgfmathprintnumber@STD@getlowerbound{%
                \noexpand\c@pgf@counta=\pgfmathfloat@loc@TMPb\space
            }%
        \fi
    \fi
}%

\def\pgfmathprintnumber@STD@issci#1#2e#3\relax{%
    \expandafter\ifnum#1<3
        \expandafter\ifnum#3>\pgfmathprintnumber@STD@upperbound\relax
            \pgfmathprintnumber@SCI@issci#1#2e#3\relax%
        \else
            \begingroup
            \pgfmathprintnumber@STD@getlowerbound
            \ifnum#3<\c@pgf@counta
                \pgfmathprintnumber@SCI@issci#1#2e#3\relax%
            \else
                \pgfmathprintnumber@FIXED@issci#1#2e#3\relax%
            \fi
            \pgfmath@smuggleone\pgfmathresult
            \endgroup
        \fi
    \else% nan or inf:
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
}

\def\pgfmathprintnumber@RELATIVE#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@RELATIVE@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn{%
    \pgf@typeout{! Package pgf warning: the use of /pgf/number format/relative is discouraged (buggy). Please use 'relative*' instead or type \string\pgfkeys{/pgf/number format/relative round mode=fixed} into your preamble.}%
    \global\let\pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn=\relax
}

\def\pgfmathprintnumber@RELATIVE@issci#1#2e#3\relax{%
    \begingroup
        % format X / 10^{relative}:
        \c@pgf@counta=#3\relax
        \advance\c@pgf@counta by-\pgfmathprintnumber@RELATIVE@param\relax
        \pgfmathfloatcreate{#1}{#2}{\the\c@pgf@counta}%
        % OK, round it to the desired precision:
        \if0\pgfmathprintnumber@RELATIVE@choice@roundtofixed
            % relative round mode=mantissa
            \def\b@round@fixed{0}%
        \else
            \if1\pgfmathprintnumber@RELATIVE@choice@roundtofixed
                % relative round mode=fixed
                \def\b@round@fixed{1}%
            \else
                \pgfmathprintnumber@RELATIVE@choice@roundtofixed@warn
                % relative round mode=compatible
                \ifnum\c@pgf@counta>0
                    % hm. for positive exponents, we should round the
                    % mantissa rather than only the fractional part.
                    \def\b@round@fixed{0}%
                \else
                    % negative exponent -> round fixed representation:
                    \def\b@round@fixed{1}%
                \fi
            \fi
        \fi
        \if1\b@round@fixed
            % round fixed representation:
            \pgfmathfloattofixed\pgfmathresult
            \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
            \pgfmathfloatparsenumber{\pgfmathresult}%
            \pgfmathfloatroundhasperiodtrue% make sure the code below works:
        \else
            % round the mantissa:
            \expandafter\pgfmathfloatround\expandafter{\pgfmathresult}%
        \fi
        % Now, compute result * 10^{relative} and format the result:
        \pgfmathfloattoregisterstok\pgfmathresult\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
        \ifnum\pgfmathfloat@a@S=0
            \pgfmathfloat@a@E=\pgfmathfloat@a@S % avoid 0 * 10^8
        \else
            \advance\pgfmathfloat@a@E by+\pgfmathprintnumber@RELATIVE@param\relax
        \fi
        \edef\pgfmathresultX{%
            \the\pgfmathfloat@a@S
            \the\pgfmathfloat@a@Mtok
            \ifpgfmathfloatroundhasperiod\else.0\fi
            e\the\pgfmathfloat@a@E}%
        % call another formatter for the result (but avoid rounding inside of it):
        \pgfqkeys{/pgf/number format}{/pgf/number format/every relative,
            fixed zerofill=false,% useless here!
            sci zerofill=false}%
        \ifx\pgfmathprintnumber@issci\pgfmathprintnumber@RELATIVE@issci
            \pgfmath@error{The '/pgf/number format/every relative' style should set a valid display style}{}%
        \fi
        \let\pgfmathfloat@round@precision@orig=\pgfmathfloat@round@precision
        \def\pgfmathfloat@round@precision{9999}%
        \expandafter\pgfmathprintnumber@issci\pgfmathresultX\relax%
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@FIXED@RELATIVE#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@FIXED@RELATIVE@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@FIXED@RELATIVE@issci#1#2e#3\relax{%
    \begingroup
    \pgfmathfloatcreate{#1}{#2}{#3}%
    % we want the first <precision> digits - not the first
    % <precision>+1 digits:
    \c@pgf@counta=\pgfmathfloat@round@precision\relax
    \advance\c@pgf@counta by-1
    \edef\pgfmathfloat@round@precision{\the\c@pgf@counta}%
    \pgfmathfloatround{\pgfmathresult}%
    \pgfmathfloattoregisterstok\pgfmathresult\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \ifnum\pgfmathfloat@a@S=0
        \pgfmathfloat@a@E=\pgfmathfloat@a@S % avoid 0 * 10^8
    \fi
    \edef\pgfmathresultX{%
        \the\pgfmathfloat@a@S
        \the\pgfmathfloat@a@Mtok
        \ifpgfmathfloatroundhasperiod\else.0\fi
        e\the\pgfmathfloat@a@E}%
    \let\pgfmathfloat@round@precision@orig=\pgfmathfloat@round@precision
    \pgfmathfloat@usezerofill@fixedfalse
    \def\pgfmathfloat@round@precision{9999}% typeset all remaining digits!
    \expandafter\pgfmathprintnumber@FIXED@issci\pgfmathresultX\relax%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@frac#1{%
    % parse the input:
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloatgetfrac{\pgfmathresult}%
    \expandafter\pgfmathprintnumber@frac@formatresult\pgfmathresult
}
\def\pgfmathprintnumber@frac@issci#1#2e#3\relax{%
    \pgfmathfloatcreate{#1}{#2}{#3}%
    \pgfmathfloatgetfrac{\pgfmathresult}%
    \expandafter\pgfmathprintnumber@frac@formatresult\pgfmathresult
}
\def\pgfmathprintnumber@frac@formatresult#1#2#3{%
    \begingroup
    \pgfkeysgetvalue{/pgf/number format/frac TeX}\pgfmathresult
    \toks0=\expandafter{\pgfmathresult}%
    \def\pgfmathfloat@loc@TMPa{#1}%
    \ifx\pgfmathfloat@loc@TMPa\pgfutil@empty
        \ifpgfmathprintnumber@showpositive
            \def\pgfmathfloat@loc@TMPa{+}%
        \fi
    \else
        \ifx\pgfmathfloat@loc@TMPa-%
        \else
            \ifx\pgfmathfloat@loc@TMPa+%
            \else
                \ifpgfmathprintnumber@showpositive
                    \edef\pgfmathfloat@loc@TMPa{+\pgfmathfloat@loc@TMPa}%
                \fi
                \def\pgfmathfloat@loc@TMPb{\pgfkeysvalueof{/pgf/number format/frac whole format/.@cmd}}%
                \expandafter\pgfmathfloat@loc@TMPb\pgfmathfloat@loc@TMPa\pgfeov
                \let\pgfmathfloat@loc@TMPa=\pgfmathresult
            \fi
        \fi
    \fi
    \toks1=\expandafter{\pgfmathfloat@loc@TMPa}%
    \edef\pgfmathresult{%
        \the\toks1 \ifnum#2=0 \else\the\toks0 {#2}{#3}\fi%
    }%
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%

% Defines \pgfmathresult to contain three sets of braces containing
% the sign (optionally containing any components >1), the numerator and the denominator for #1.
%
% \pgfmathfloatgetfrac{0.5}  -> \pgfmathresult contains {}{1}{2}
% \pgfmathfloatgetfrac{-0.5} -> \pgfmathresult contains {-}{1}{2}
% \pgfmathfloatgetfrac{1.5} ->  \pgfmathresult contains {1}{1}{2}
%
% special cases:
% \pgfmathfloatgetfrac{0}   ->  \pgfmathresult contains {0}{0}{1}
% \pgfmathfloatgetfrac{1}   ->  \pgfmathresult contains {1}{0}{1}
%
% The numerator and denominator is always a number (not empty)
\def\pgfmathfloatgetfrac#1{%
    \pgfutil@ifundefined{pgfmathfloatmultiply@}{%
        \pgfmath@error{Sorry, the number format 'frac' requires '\string\usetikzlibrary{fpu}' (and, optionally, \string\usepackage{fp}) in order to work correctly}{}%
        \edef\pgfmathresult{{#1}{0}{1}}%
    }{%
        \pgfmathfloatgetfrac@{#1}%
    }%
}%
\def\pgfmathfloatgetfrac@#1{%
    \begingroup
        \edef\pgfmathfloat@arg{#1}%
        \expandafter\pgfmathfloat@decompose@tok\pgfmathfloat@arg\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
        \def\pgfmathfloat@loc@TMPa{0}%
        \ifcase\pgfmathfloat@a@S
        % #1 = 0:
            \def\pgfmathresult{{0}{0}{1}}%
        \or% #1 > 0
            \pgfmathfloat@a@S=1
            \def\pgfmathfloat@loc@TMPa{1}%
        \or% #1 < 0
            \pgfmathfloat@a@S=-1
            \def\pgfmathfloat@loc@TMPa{1}%
        \or
            \edef\pgfmathresult{{}{NaN}{1}}%
        \or
            \edef\pgfmathresult{{}{\infty}{1}}%
        \or
            \edef\pgfmathresult{{-}{\infty}{1}}%
        \fi
        \if1\pgfmathfloat@loc@TMPa
            \ifnum\pgfmathfloat@a@E<0
                \def\pgfmathfloat@wholenumber{}%
            \else
                \pgfmathfloatcreate{1}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
                \pgfmathfloattofixed\pgfmathresult%
                \def\pgfmathfloat@loc@TMPa##1.##2\relax{%
                    \def\pgfmathfloat@wholenumber{##1}%
                    \pgfmathfloatparsenumber{0.##2}%
                }%
                \expandafter\pgfmathfloat@loc@TMPa\pgfmathresult\relax
                \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@b@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
            \fi
            %
            \def\pgfmathfloat@loc@TMPa##1.##2\relax{%
                \def\pgfmathfloat@mantissa@first{##1}%
                \def\pgfmathfloat@mantissa@ltone{0.##2}%
            }%
            \expandafter\pgfmathfloat@loc@TMPa\the\pgfmathfloat@a@Mtok\relax
            %
            \def\pgfmathfloat@loc@@to@int##1.##2\relax##3{%
                ##3=##1
                \ifdim0.##2pt>0.5pt
                    \advance##3 by1
                \fi
            }%
            %
            % alias registers names:
            \let\pgfmathresultnumerator=\pgfmathfloat@b@S
            \let\pgfmathresultdenom=\pgfmathfloat@b@E
            %
            \pgfkeysgetvalue{/pgf/number format/frac denom}\pgfmath@target@denominator
            \ifx\pgfmath@target@denominator\pgfutil@empty
            %
                \pgfmathfloat@a@E=-\pgfmathfloat@a@E
                \ifdim\pgfmathfloat@mantissa@ltone pt=0pt
                    \def\pgfmathfloat@factor{1}%
                    \edef\pgfmathfloat@scaled@numerator{\the\pgfmathfloat@a@Mtok}%
                \else
                    % FIXME : this here is numerically instable.
                    %
                    % The errors of 1/r are magnified by 10^k which
                    % doesn't work.
                    \pgfutil@ifundefined{FPdiv}{%
                        \pgfmathfloatparsenumber{\pgfmathfloat@mantissa@ltone}%
                        \pgfmathfloatreciprocal@{\pgfmathresult}%
                    }{%
                        % \usepackage{fp}.
                        % yields higher absolute precision.
                        \FPmessagesfalse%
                        \FPdebugfalse%
                        \FPdiv\pgfmathresult{1}{\pgfmathfloat@mantissa@ltone}%
                        \pgfmathfloatparsenumber{\pgfmathresult}%
                    }%
                    \let\pgfmathfloat@inv=\pgfmathresult
                    \pgfmathfloatcreate{1}{1.0}{\pgfkeysvalueof{/pgf/number format/frac shift}}%
                    \let\pgfmathfloat@scalebaseten=\pgfmathresult
                    \pgfmathfloatmultiply@{\pgfmathfloat@inv}{\pgfmathfloat@scalebaseten}%
                    \let\pgfmathfloat@factor=\pgfmathresult
                    %
                    \expandafter\pgfmathfloatparsenumber\expandafter{\the\pgfmathfloat@a@Mtok}%
                    \let\pgfmathfloat@loc@TMPa=\pgfmathresult
                    \pgfmathfloatmultiply@{\pgfmathfloat@factor}{\pgfmathfloat@loc@TMPa}%
                    \pgfmathfloattofixed\pgfmathresult
                    \let\pgfmathfloat@scaled@numerator=\pgfmathresult
                    %
                    \pgfmathfloattofixed\pgfmathfloat@factor
                    \expandafter\pgfmathfloat@loc@@to@int\pgfmathresult\relax{\pgfmathfloat@b@S}%
                    \edef\pgfmathfloat@factor{\the\pgfmathfloat@b@S}%
                \fi
                %
                %
                \pgfmathresultdenom=\pgfmathfloat@factor\relax
                \pgfmathfloat@multiply@ten@to@the@E\pgfmathresultdenom
                %
                \expandafter\pgfmathfloat@loc@@to@int\pgfmathfloat@scaled@numerator\relax{\pgfmathresultnumerator}%
    %\message{scale = \pgfmathfloat@factor;  Z = \the\pgfmathresultnumerator\space ( von \pgfmathfloat@scaled@numerator), N = \the\pgfmathresultdenom.}%
                %
                \pgfmathgreatestcommondivisor{\pgfmathresultnumerator}{\pgfmathresultdenom}%
                \divide\pgfmathresultnumerator by\pgfmathresult\relax
                \divide\pgfmathresultdenom by\pgfmathresult\relax
                \ifpgfmathprintnumber@frac@warn
                    \ifnum\pgfmathresultdenom>1000
                        \pgfutil@ifundefined{FPdiv}{%
                            \pgfmathfloattosci@\pgfmathfloat@arg
                            \pgf@typeout{! Package pgf /pgf/number format/frac warning=true: /pgf/number format/frac of `\pgfmathresult' = \the\pgfmathresultnumerator\space / \the\pgfmathresultdenom\space might be large due to instabilities. Try \string\usepackage{fp} to improve accuracy.}%
                        }{}%
                    \fi
                \fi
            \else
                % use target denominator:
                \pgfmathresultdenom=\pgfmath@target@denominator\relax
                \pgfmathfloatcreate{1}{\the\pgfmathfloat@a@Mtok}{\the\pgfmathfloat@a@E}%
                \pgfmathfloattofixed\pgfmathresult
                \pgf@xa=\pgfmathresult pt
                \multiply\pgf@xa by\pgfmathresultdenom
                \edef\pgfmathfloat@scaled@numerator{\pgfmath@tonumber\pgf@xa}%
                \expandafter\pgfmathfloat@loc@@to@int\pgfmathfloat@scaled@numerator\relax{\pgfmathresultnumerator}%
            \fi
            \ifpgfmathprintnumber@frac@whole
            \else
                \ifx\pgfmathfloat@wholenumber\pgfutil@empty
                \else
                    \count0=\pgfmathfloat@wholenumber\relax
                    \multiply\count0 by\pgfmathresultdenom
                    \advance\pgfmathresultnumerator by\count0
                    \def\pgfmathfloat@wholenumber{}%
                \fi
            \fi
            \ifnum\pgfmathfloat@a@S<0
                \edef\pgfmathresult{{-\pgfmathfloat@wholenumber}{\the\pgfmathresultnumerator}{\the\pgfmathresultdenom}}%
            \else
                \edef\pgfmathresult{{\pgfmathfloat@wholenumber}{\the\pgfmathresultnumerator}{\the\pgfmathresultdenom}}%
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%
\def\pgfmathfloat@gobble@until@relax#1\relax{}

% computes the greatest common divisor of two integer numbers (in
% integer arithmetics).
\def\pgfmathgreatestcommondivisor#1#2{%
    \begingroup
        \count0=#1\relax
        \count1=#2\relax
        \ifnum\count0=0
            \edef\pgfmathresult{\the\count1}%
        \else
            \pgfmathgreatestcommondivisor@loop
            \edef\pgfmathresult{\the\count0}%
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}
\def\pgfmathgreatestcommondivisor@loop{%
    \ifnum\count1=0
    \else
        \ifnum\count0>\count1
            \advance\count0 by-\count1
        \else
            \advance\count1 by-\count0
        \fi
        \expandafter\pgfmathgreatestcommondivisor@loop
    \fi
}%

% multiplies a TeX register by 10^E where E is stored in the register
% \pgfmathfloat@a@E (and it should be positive!)%
%
% #1 a TeX register
\def\pgfmathfloat@multiply@ten@to@the@E#1{%
    \ifnum\pgfmathfloat@a@E>0
        \multiply#1 by10
        \advance\pgfmathfloat@a@E by-1
        \def\pgfmathfloat@multiply@ten@to@the@E@next{\pgfmathfloat@multiply@ten@to@the@E{#1}}%
    \else
        \let\pgfmathfloat@multiply@ten@to@the@E@next=\relax%
    \fi
    \pgfmathfloat@multiply@ten@to@the@E@next
}%

\def\pgfmathprintnumber@INT@TRUNC#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@INT@TRUNC@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@TRUNC@impl#1.#2\relax#3#4e#5\relax{%
    \pgfmathfloatroundhasperiodfalse
    \pgfmathprintnumber@fixed@style{#1}#3#4e#5\relax%
}
\def\pgfmathprintnumber@INT@TRUNC@issci#1#2e#3\relax{%
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \expandafter\pgfmathprintnumber@INT@TRUNC@impl\pgfmathresult\relax#1#2e#3\relax
    \else
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
}

% Invokes '#2' if '#1' is actually an integer or '#3' if not.
%
% As a side-effect, \pgfretval will be set to the integer value if it
% actually *is* an integer. Otherwise, \pgfretval will contain the
% parsed floating point number.
%
% #1 a number constant (not necessarily a parsed float).
\def\pgfmathifisint#1#2#3{%
    \gdef\pgfmathfloatisint@@{0}%
    \begingroup
    \pgfmathfloatparsenumber{#1}%
    \let\pgfretval\pgfmathresult
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathfloatisint@\pgfmathresult\relax
    \pgfmath@smuggleone\pgfretval
    \endgroup
    \if1\pgfmathfloatisint@@ #2\else #3\fi
}%
\def\pgfmathfloatisint@#1#2e#3\relax{%
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \def\pgfmathfloat@round@precision{6}%
        \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \ifpgfmathfloatroundhasperiod
        \else
            \let\pgfretval\pgfmathresult%
            \gdef\pgfmathfloatisint@@{1}%
        \fi
    \fi
}

\def\pgfmathprintnumber@INT@DETECT#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@INT@DETECT@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@INT@DETECT@issci#1#2e#3\relax{%
    \begingroup
    \ifnum#1<3\relax
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \let\pgfmathfloat@round@precision@=\pgfmathfloat@round@precision
        \def\pgfmathfloat@round@precision{6}%
        \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \let\pgfmathfloat@round@precision=\pgfmathfloat@round@precision@
        \ifpgfmathfloatroundhasperiod
            \pgfmathprintnumber@SCI@issci#1#2e#3\relax
        \else
            \expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax
        \fi
    \else
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\def\pgfmathprintnumber@FIXED#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@FIXED@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@FIXED@issci#1#2e#3\relax{%
    \begingroup
    \ifnum#1<3
        \pgfmathfloatcreate{#1}{#2}{#3}%
        \pgfmathfloattofixed{\pgfmathresult}%
        \ifpgfmathfloat@usezerofill@fixed
            \expandafter\pgfmathroundtozerofill\expandafter{\pgfmathresult}%
        \else
            \expandafter\pgfmathroundto\expandafter{\pgfmathresult}%
        \fi
        \ifpgfmathfloatroundmayneedrenormalize
            \pgfmathfloat@a@E=#3\relax
            \advance\pgfmathfloat@a@E by1
            \edef\pgfmathfloat@loc@TMPb{\noexpand\pgfmathprintnumber@fixed@style{\pgfmathresult}#1#2e\the\pgfmathfloat@a@E}%
            \pgfmathfloat@loc@TMPb\relax%
        \else
            \expandafter\pgfmathprintnumber@fixed@style\expandafter{\pgfmathresult}#1#2e#3\relax%
        \fi
    \else% nan or inf:
        \pgfmathfloatrounddisplaystyle#1#2e#3\relax%
    \fi
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}


\def\pgfmathprintnumber@SCI#1{%
    \pgfmathfloatparsenumber{#1}%
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathprintnumber@SCI@issci\pgfmathresult\relax
}

\def\pgfmathprintnumber@SCI@issci#1#2e#3\relax{%
    \begingroup
    \pgfmathfloatcreate{#1}{#2}{#3}%
    \edef\pgfmathfloat@round@precision{\pgfmathprintnumber@sci@precision}%
    \ifpgfmathfloat@usezerofill@sci
        \pgfmathfloatroundzerofill{\pgfmathresult}%
    \else
        \pgfmathfloatround{\pgfmathresult}%
    \fi
    \pgfmathfloat@to@FMeE@style\pgfmathresult
    \expandafter\pgfmathfloatrounddisplaystyle\pgfmathresult\relax
    \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

% Prints argument #1 using the current pretty printer environment (all
% variables in /pgf/number format).
%
% You may specify optional arguments with \pgfmathprintnumber[...].
\def\pgfmathprintnumber{%
    % \protect allows to supply \pgfmathprintnumber inside of latex
    % captions. The \csname yields \relax in case protect is undefined.
    \pgf@texdist@protect\pgfmathprintnumber@protected
}%
\def\pgfmathprintnumber@protected{%
    \pgfutil@ifnextchar[%
        {\pgfmathprintnumber@OPT}%
        {\pgfmathprintnumber@noopt}%
}

\def\pgfmathprintnumber@noopt#1{%
    \pgfmathprintnumber@{#1}%
    \ifpgfmathprintnumber@assumemathmode
        \pgfmathresult
    \else
        \pgfutilensuremath{\pgfmathresult}%
    \fi
}%
\def\pgfmathprintnumber@OPT[#1]#2{%
    \begingroup
    \pgfqkeys{/pgf/number format}{#1}%
    \pgfmathprintnumber@{#2}%
    \ifpgfmathprintnumber@assumemathmode
        \pgfmathresult
    \else
        \pgfutilensuremath{\pgfmathresult}%
    \fi
    \endgroup
}%

% As \pgfmathprintnumber, but it produces its output into the second
% argument.
\def\pgfmathprintnumberto{%
    \pgfutil@ifnextchar[%
        {\pgfmathprintnumberto@OPT}%
        {\pgfmathprintnumberto@noopt}%
}

\def\pgfmathprintnumberto@noopt#1#2{%
    \begingroup
    \pgfmathprintnumber@{#1}%
    \ifpgfmathprintnumber@assumemathmode
        \global\let\pgfmathfloat@glob@TMP=\pgfmathresult
    \else
        \toks0=\expandafter{\pgfmathresult}%
        \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
    \fi
    \endgroup
    \let#2=\pgfmathfloat@glob@TMP
}%
\def\pgfmathprintnumberto@OPT[#1]#2#3{%
    \begingroup
    \pgfqkeys{/pgf/number format}{#1}%
    \pgfmathprintnumber@{#2}%
    \ifpgfmathprintnumber@assumemathmode
        \global\let\pgfmathfloat@glob@TMP=\pgfmathresult
    \else
        \toks0=\expandafter{\pgfmathresult}%
        \xdef\pgfmathfloat@glob@TMP{\noexpand\pgfutilensuremath{\the\toks0 }}%
    \fi
    \endgroup
    \let#3=\pgfmathfloat@glob@TMP
}%


% Changes the current number pretty printer to #1.
%
% #1 is the macro base name for the pretty print routine, without the
% leading '\'.
\def\pgfmath@set@number@printer#1{%
    \expandafter\let\expandafter\pgfmathprintnumber@\csname #1\endcsname
    \expandafter\let\expandafter\pgfmathprintnumber@issci\csname #1@issci\endcsname
}

\pgfkeys{/pgf/number format/std}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% IMPL
%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% equals only itself when compared with \ifx:
\def\pgfmathfloat@EOI{\pgfmathfloat@EOI}%

% Re-use counters internally.
%
% They are always grouped and only used inside of the rounding
% routines.
\let\c@pgfmathroundto@prec=\pgfmathfloat@b@S% ATTENTION: DOUBLE-USED REGISTERS!
\let\c@pgfmathroundto@offsetbehindperiod=\pgfmathfloat@b@E
\newcount\c@pgfmathroundto@lastzeros

\newif\ifpgfmathround@impl@PREPERIOD@is@negative@zero

% PRECONDITION:
% \ifpgfmathfloatroundhasperiod=\iftrue  holds outside of the current TeX group.
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set correctly AFTER the
%   current TeX group.
%   \ifpgfmathfloatroundmayneedrenormalize will be set globally
\def\pgfmathroundto@impl#1{%
    \edef\pgfmathround@input{#1}%
    \global\pgfmathfloatroundmayneedrenormalizefalse
    \pgfmathfloat@tmptoks={}%
    \let\pgfmathround@next=\pgfutil@empty
    \let\pgfmathround@cur=\pgfutil@empty
    \let\pgfmathresult=\pgfutil@empty
    \expandafter\c@pgfmathroundto@prec\pgfmathfloat@round@precision\relax
    \c@pgfmathroundto@lastzeros=0
    \c@pgfmathroundto@offsetbehindperiod=-1 % means: no period found so far
    \pgfmathround@impl@PREPERIOD@is@negative@zerotrue
    \expandafter\pgfmathroundto@impl@ITERATE@NODOT@firstcall\pgfmathround@input\pgfmathfloat@EOI
}

% \pgfmathroundto implementation in WORDS:
%
% coarse idea:
%     1. collect all digits/sign BEFORE the first period in REVERSE order
%     2. then, collect UP TO \prec digits after the period in REVERSE order
% Steps 1. and 2. lead to the digit [sign] sequence
%     "x_{-p} x_{-p+1} ... x_{-2} x_{-1} '.' x_0 ... x_r"
% where 'r' is the total number of digits. The integer 'p' denotes the
% ACTUALLY collected number of digits behind the period.
%
% Let 'k' be the desired precision.
%
% Please note that pgfmathroundto rounds the mantissa, that means |abs(x)|.
%
% There are exactly TWO cases:
% 1. The case with p<=k and x_{-p-1} = end of input.
% 2. The case with p=k and x_{-p-1} is a further, next character.
%
% Then, for case 1.):
%     discard any unused zeros at the tail of our number (possibly
%     including the period)
%
% and in case 2.)
%   if NEXT DIGIT < 5:
%       do exactly the same as in case 1.) above and discard any
%       following digits.
%   else
%       let q := -p
%       while(x_q = 9 and q<=r )
%           if q>=0
%               set x_q = '0'
%           else
%               discard digit x_q='9'
%           fi
%           ++q
%           if q=0
%               discard the period
%           fi
%       end while
%       if q = r+1
%           insert a '1'
%       else
%           set x_q = x_q + 1
%       fi
%   fi
%
% All these loops have been implemented in spaghetti-code below.
% Sorry, I fear its hard to understand. In principle, everything is
% realised using more or less finite state machines (with some number
% counting logic).
%
% Some comments:
%     - The token register \pgfmathfloat@tmptoks is used to accumulate the REVERSED input number.
%     - \pgfmathfloat@EOI always denotes 'END OF INPUT'.
%     - in the second stage, we need to reverse \pgfmathfloat@tmptoks.
%       This is -- again -- done with \pgfmathfloat@tmptoks.

\def\pgfmathroundto@impl@discard@period#1.#2\pgfmathfloat@EOI{%
    \pgfmathfloatroundhasperiodfalse
    \aftergroup\pgfmathfloatroundhasperiodfalse
    \def\pgfmathresult{#1}%
}

\def\pgfmathroundto@impl@gobble@rest@and@start#1\pgfmathfloat@EOI{%
    \pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble@and@start\pgfmathfloat@EOI{%
    \pgfmathroundto@impl@start
}
\def\pgfmathroundto@impl@gobble\pgfmathfloat@EOI{}%
\def\pgfmathroundto@impl@gobble@rest#1\pgfmathfloat@EOI{}%

% This method will be invoked as soon as the first step, the reverse
% collection of up to PREC digits after the period, has finished.
\def\pgfmathroundto@impl@start{%
    \ifx\pgfmathround@next\pgfutil@empty
        \ifnum\c@pgfmathroundto@offsetbehindperiod<0
            % no period found.
            \ifpgfmathfloat@fixed@digits@after@period
                \ifnum\c@pgfmathroundto@prec=0\relax
                    \pgfmathfloatroundhasperiodfalse
                    \aftergroup\pgfmathfloatroundhasperiodfalse
                    \edef\pgfmathresult{\pgfmathround@input}%
                \else
                    \pgfmathfloat@tmptoks=\expandafter{\pgfmathround@input.}%
                    \c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
                    \pgfmathroundto@impl@append@zeros
                    \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
                \fi
            \else
                \pgfmathfloatroundhasperiodfalse
                \aftergroup\pgfmathfloatroundhasperiodfalse
                \edef\pgfmathresult{\pgfmathround@input}%
            \fi
        \else
            %\ifnum\c@pgfmathroundto@offsetbehindperiod>\c@pgfmathroundto@prec
            %    \pgfmath@error{Internal logic error in pgfmathroundto at [I] - should not have happened!?}{}%
            %\fi
            \pgfmathroundto@impl@finish@with@truncation
        \fi
    \else
        %\ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
        %\else
        %    \pgfmath@error{Internal logic error in pgfmathroundto at [II] - should not have happened!? I have offsetbehindperiod=\the\c@pgfmathroundto@offsetbehindperiod and prec = \the\c@pgfmathroundto@prec}{}%
        %\fi
        \expandafter\ifnum\pgfmathround@next<5\relax
            \pgfmathroundto@impl@finish@with@truncation
        \else
            \multiply\c@pgfmathroundto@offsetbehindperiod by-1
            \expandafter\pgfmathroundto@impl@ADD@ONE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \fi
    \fi
}

% takes the current input and decides whether trailing zeros shall be
% discarded or more zeros need to be filled in.
\def\pgfmathroundto@impl@finish@with@truncation{%
    \ifpgfmathfloat@fixed@digits@after@period
        \expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
            \ifpgfmathround@impl@PREPERIOD@is@negative@zero
                % write '0.0000' instead of '-0.0000':
                \expandafter\pgfmathroundto@impl@discard@minus\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
            \fi
        \fi
        \ifnum\c@pgfmathroundto@prec=0\relax
            \expandafter\pgfmathroundto@impl@discard@period\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \else
            \advance\c@pgfmathroundto@prec by-\c@pgfmathroundto@offsetbehindperiod
            \c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
            \pgfmathroundto@impl@append@zeros
            \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
        \fi
    \else
        \pgfmathroundto@impl@discard@suffix@zeros
    \fi
}

\def\pgfmathroundto@impl@discard@minus-#1\pgfmathfloat@EOI{\pgfmathfloat@tmptoks={#1}}%

% appends \c@pgfmathroundto@offsetbehindperiod zeros at the end of \pgfmathfloat@tmptoks.
\def\pgfmathroundto@impl@append@zeros{%
    \ifnum\c@pgfmathroundto@offsetbehindperiod>0
        \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
        \advance\c@pgfmathroundto@offsetbehindperiod by-1
        \pgfmathroundto@impl@append@zeros
    \fi
}

\def\pgfmathroundto@impl@ADD@ONE{%
    \pgfmathfloat@tmptoks={}% no longer needed because its old value will be read from input
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@ITERATE{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        \global\pgfmathfloatroundmayneedrenormalizetrue
        \edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
        \pgfmathroundto@impl@gobble
    }{%
        \pgfutil@ifnextchar.{%
            \ifnum\c@pgfmathroundto@prec=0
                % silently discard period in special case precision=0
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
            \else
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT}%
            \fi
            \pgfmathround@nextcmd
        }{%
            \pgfutil@ifnextchar+{%
                \global\pgfmathfloatroundmayneedrenormalizetrue
                \edef\pgfmathresult{1\the\pgfmathfloat@tmptoks}%
                \pgfmathroundto@impl@gobble@rest
            }{%
                \pgfutil@ifnextchar-{%
                    \global\pgfmathfloatroundmayneedrenormalizetrue
                    \edef\pgfmathresult{-1\the\pgfmathfloat@tmptoks}%
                    \pgfmathroundto@impl@gobble@rest
                }{%
                    \pgfmathroundto@impl@ADD@ONE@NEXT
                }%
            }%
        }%
    }%
}

\def\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot.{%
    \pgfmathfloatroundhasperiodfalse
    \aftergroup\pgfmathfloatroundhasperiodfalse
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}

\def\pgfmathroundto@impl@ADD@ONE@NEXT@COLLECT#1{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
    \pgfmathroundto@impl@ADD@ONE@ITERATE
}
\def\pgfmathroundto@impl@ADD@ONE@NEXT#1{%
    \ifnum#1=9
        \ifnum\c@pgfmathroundto@offsetbehindperiod<0
            \ifpgfmathfloat@fixed@digits@after@period
                \pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
            \else
                % silently DROP digit
            \fi
        \else
            \pgfmathfloat@tmptoks=\expandafter{\expandafter0\the\pgfmathfloat@tmptoks}%
        \fi
        \advance\c@pgfmathroundto@offsetbehindperiod by1
        \ifnum\c@pgfmathroundto@offsetbehindperiod=0
            \ifpgfmathfloat@fixed@digits@after@period
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
            \else
                \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE@gobble@dot}%
            \fi
        \else
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ADD@ONE@ITERATE}%
        \fi
    \else
        % re-use this counter:
        \c@pgfmathroundto@lastzeros=#1
        \advance\c@pgfmathroundto@lastzeros by1
        \edef\pgfmathresult{\the\c@pgfmathroundto@lastzeros\the\pgfmathfloat@tmptoks}%
        \pgfmathfloat@tmptoks=\expandafter{\pgfmathresult}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE@ITERATE}%
    \fi
    \pgfmathround@nextcmd
}


\def\pgfmathroundto@impl@discard@suffix@zeros{%
    \ifnum\c@pgfmathroundto@lastzeros=\c@pgfmathroundto@offsetbehindperiod
        \ifpgfmathround@impl@PREPERIOD@is@negative@zero
            \pgfmathfloatroundhasperiodfalse
            \aftergroup\pgfmathfloatroundhasperiodfalse
            \def\pgfmathresult{0}% write '0' instead of '-0'
        \else
            \expandafter\pgfmathroundto@impl@discard@period\pgfmathround@input\pgfmathfloat@EOI
        \fi
    \else
        \ifnum\c@pgfmathroundto@lastzeros=0
            \expandafter\pgfmathroundto@impl@REVERSE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \else
            \expandafter\pgfmathroundto@impl@discard@suffix@zeros@ITERATE\the\pgfmathfloat@tmptoks\pgfmathfloat@EOI
        \fi
    \fi
}

% PRECONDITION:
%     \c@pgfmathroundto@lastzeros > 0
\def\pgfmathroundto@impl@discard@suffix@zeros@ITERATE#1{%
    \advance\c@pgfmathroundto@lastzeros by-1
    \ifnum\c@pgfmathroundto@lastzeros=0
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@REVERSE}%
    \else
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@discard@suffix@zeros@ITERATE}%
    \fi
    \pgfmathround@nextcmd
}

% Usage:
% \pgfmathroundto@impl@REVERSE#1\pgfmathfloat@EOI
% -> writes #1 reversed into \pgfmathfloat@tmptoks
\def\pgfmathroundto@impl@REVERSE{%
    \pgfmathfloat@tmptoks={}%
    \pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@REVERSE@ITERATE{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        \edef\pgfmathresult{\the\pgfmathfloat@tmptoks}%
        \pgfmathroundto@impl@gobble
    }{%
        \pgfmathroundto@impl@REVERSE@NEXT
    }%
}

\def\pgfmathroundto@impl@REVERSE@NEXT#1{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
    \pgfmathroundto@impl@REVERSE@ITERATE
}

\def\pgfmathroundto@impl@BEGIN@DOT.{%
    \pgfmathfloat@tmptoks=\expandafter{\expandafter.\the\pgfmathfloat@tmptoks}%
    \c@pgfmathroundto@offsetbehindperiod=0
    \pgfmathroundto@impl@ITERATE@DOT
}
\def\pgfmathroundto@impl@ITERATE@DOT{%
    \pgfutil@ifnextchar\pgfmathfloat@EOI{%
        % finished.
        \pgfmathroundto@impl@gobble@and@start
    }{%
        \pgfmathroundto@impl@NEXT@DOT
    }%
}
\def\pgfmathroundto@impl@NEXT@DOT#1{%
    \ifnum\c@pgfmathroundto@offsetbehindperiod=\c@pgfmathroundto@prec
        \def\pgfmathround@next{#1}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@gobble@rest@and@start}%
    \else
        \advance\c@pgfmathroundto@offsetbehindperiod by1
        \ifnum#1=0
            \advance\c@pgfmathroundto@lastzeros by1
        \else
            \c@pgfmathroundto@lastzeros=0
        \fi
        \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@DOT}%
    \fi
    \pgfmathround@nextcmd
}%

% in contrast to pgfmathroundto@impl@ITERATE@NODOT, this method here
% checks also for signs
\def\pgfmathroundto@impl@ITERATE@NODOT@firstcall#1{%
    \def\pgfmathround@cur{#1}%
    \ifx\pgfmathround@cur\pgfmathfloat@EOI
        \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
    \else
        \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
            \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
        \else
            \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@MINUS
            \else
                \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \fi
            \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
        \fi
    \fi
    \pgfmathround@nextcmd
}

\def\pgfmathroundto@impl@ITERATE@NODOT#1{%
    \def\pgfmathround@cur{#1}%
    \ifx\pgfmathround@cur\pgfmathfloat@EOI
        \def\pgfmathround@nextcmd{\pgfmathroundto@impl@start}%
    \else
        \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@PERIOD
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@BEGIN@DOT.}%
        \else
            \ifx\pgfmathround@cur\pgfmathfloatparsenumber@tok@ZERO
            \else
                \pgfmathround@impl@PREPERIOD@is@negative@zerofalse
            \fi
            \pgfmathfloat@tmptoks=\expandafter{\expandafter#1\the\pgfmathfloat@tmptoks}%
            \def\pgfmathround@nextcmd{\pgfmathroundto@impl@ITERATE@NODOT}%
        \fi
    \fi
    \pgfmathround@nextcmd
}

%--------------------------------------------
% END of pgfmathroundto implementation.
%--------------------------------------------


% flags, mantissa and exponent has already been stored into
% \pgfmathfloat@a@* [using ...@Mtok]
%
% PRECONDITION:
%   \ifpgfmathfloatroundhasperiod = \iftrue outside of the current
%   group
%
% POSTCONDITION:
%   \ifpgfmathfloatroundhasperiod will be set after the current TeX
%   group.
\def\pgfmathfloatround@impl{%
    \expandafter\pgfmathroundto@impl\expandafter{\the\pgfmathfloat@a@Mtok}%
    \ifpgfmathfloatroundmayneedrenormalize
        \ifpgfmathfloatroundhasperiod
            \expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult\pgfmathfloat@EOI%
        \else
            \expandafter\pgfmathfloatround@impl@renormalize\pgfmathresult.\pgfmathfloat@EOI%
        \fi
        \advance\pgfmathfloat@a@E by1
    \fi
    \pgfmathfloatcreate{\the\pgfmathfloat@a@S}{\pgfmathresult}{\the\pgfmathfloat@a@E}%
}

\def\pgfmathfloatround@impl@renormalize#1#2.#3\pgfmathfloat@EOI{%
    \pgfmathroundto@impl{#1.#2#3}%
}





% ATTENTION: this thing REQUIRES a period in the mantissa!
% collects everything into \pgfmathresult
\def\pgfmathfloattofixed@impl#1.#2\relax{%
    \ifnum\pgfmathfloat@a@E<0
        \ifcase-\pgfmathfloat@a@E
        \or%e-1
            \pgfmathfloat@a@Mtok={0.}%
        \or%e-2
            \pgfmathfloat@a@Mtok={0.0}%
        \or%e-3
            \pgfmathfloat@a@Mtok={0.00}%
        \or%e-4
            \pgfmathfloat@a@Mtok={0.000}%
        \or%e-5
            \pgfmathfloat@a@Mtok={0.0000}%
        \or%e-6
            \pgfmathfloat@a@Mtok={0.00000}%
        \or%e-7
            \pgfmathfloat@a@Mtok={0.000000}%
        \or%e-8
            \pgfmathfloat@a@Mtok={0.0000000}%
        \or%e-9
            \pgfmathfloat@a@Mtok={0.00000000}%
        \or%e-10
            \pgfmathfloat@a@Mtok={0.000000000}%
        \else%<= -11
            \pgfmathfloat@a@Mtok={0.0000000000}%
            \advance\pgfmathfloat@a@E by10
            \pgfutil@loop
            \ifnum\pgfmathfloat@a@E<-1
                \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
                \advance\pgfmathfloat@a@E by1
            \pgfutil@repeat
        \fi
        \def\pgfmathfloat@loc@TMPb{#2}%
        \def\pgfmathfloat@loc@TMPc{0}%
        \ifx\pgfmathfloat@loc@TMPb\pgfmathfloat@loc@TMPc
            \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1}%
        \else
            \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok #1#2}%
        \fi
    \else
        %--------------------------------------------------
        % \ifnum\pgfmathfloat@a@E=0%
        %     \edef\pgfmathresult{#1.#2}%
        % \else
        %     \pgfmathfloat@a@Mtok={#1}%
        %     \pgfmathfloattofixed@impl@collectmantissa#2\count\pgfmathfloat@a@E
        %     \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok}%
        % \fi
        %--------------------------------------------------
        \pgfmathfloat@a@Mtok{#1}%
        \pgfmathfloattofixed@impl@pos#2000000000\pgfmathfloat@EOI
        \edef\pgfmathresult{\the\pgfmathfloat@a@Mtok}%
    \fi
}

% FIXME: this implementation here is very fast, but it introduces trailing zeros. Is that acceptable?
\def\pgfmathfloattofixed@impl@pos#1#2#3#4#5#6#7#8#9\pgfmathfloat@EOI{%
    \ifcase\pgfmathfloat@a@E
    % e+0
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok .#1#2#3#4#5#6#7#8#9}%
    \or%e+1
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1.#2#3#4#5#6#7#8#9}%
    \or%e+2
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2.#3#4#5#6#7#8#9}%
    \or%e+3
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3.#4#5#6#7#8#9}%
    \or%e+4
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4.#5#6#7#8#9}%
    \or%e+5
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5.#6#7#8#9}%
    \or%e+6
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6.#7#8#9}%
    \or%e+7
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7.#8#9}%
    \or%e+8
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7#8.#9}%
    \else%>=9
        \pgfmathfloat@a@Mtok\expandafter{\the\pgfmathfloat@a@Mtok #1#2#3#4#5#6#7#8}%
        \advance\pgfmathfloat@a@E by-8
        \pgfmathfloattofixed@impl@collectmantissa#9\count\pgfmathfloat@a@E
    \fi
}%

\def\pgfmathfloattofixed@impl@collectmantissa#1#2\count#3{%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok #1}%
    \advance\pgfmathfloat@a@E by-1%
    \def\pgfmathfloat@loc@TMPb{#2}%
    \ifx\pgfmathfloat@loc@TMPb\pgfutil@empty
        \pgfutil@loop
        \ifnum\pgfmathfloat@a@E>0%
            \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok 0}%
            \advance\pgfmathfloat@a@E by-1%
        \pgfutil@repeat
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .0}%
    \else
        \ifnum\pgfmathfloat@a@E=0
            \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok .#2}%
        \else
            \pgfmathfloattofixed@impl@collectmantissa#2\count#3%
        \fi
    \fi
}


% ============================================
%
%
% \pgfmathfloatparsenumber implementation
%
%
% ============================================

% accepted parser tokens:
\def\pgfmathfloatparsenumber@tok@ZERO{0}
\def\pgfmathfloatparsenumber@tok@PLUS{+}
\def\pgfmathfloatparsenumber@tok@MINUS{-}
\def\pgfmathfloatparsenumber@tok@PERIOD{.}

\newif\ifpgfmathfloatparsenumberpendingperiod

\def\pgfflt@EOI{p@EOI}%
\def\pgfflt@EOI@unexpanded{\pgfflt@EOI}%

% Starts a finite-start-machine parser to read a number.
%
% The machine's state is represented by the macro which is currently
% processed; state transitions are realised using \csname...#1\endcsname
% constructions.
%
% It assigns \pgfmathfloat@a@S, \pgfmathfloat@a@Mtok, \pgfmathfloat@a@E.
\def\pgfflt@impl#1{%
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfmathfloat@tmptoks={}% this register is used to collect PENDING ZEROS
    \pgfmathfloat@a@E=0
    % start parsing: check for sign:
    \expandafter\ifx\csname pgfflt@#1\endcsname\relax
        \pgfmathfloat@a@S=1
        \expandafter\pgfflt@init\expandafter#1%
    \else
        \expandafter\expandafter\csname pgfflt@#1\endcsname
    \fi
}
% State transitions:
\expandafter\def\csname pgfflt@+\endcsname{%
    \pgfmathfloat@a@S=1 %
    \pgfflt@init}%
\expandafter\def\csname pgfflt@-\endcsname{%
    \pgfmathfloat@a@S=2 %
    \pgfflt@init}%
\expandafter\def\csname pgfflt@\pgfflt@EOI\endcsname{%
    \pgfmathfloatparsenumber@handleerror{empty number}{}{}}%

\pgfkeys{
    /pgf/fpu/handlers/empty number/.style 2 args={%
        /pgf/fpu/handlers/invalid number={#1}{#2}%
    },
    /pgf/fpu/empty number is zero/.style={%
        /pgf/fpu/handlers/empty number/.code 2 args={%
            \pgfmathfloatcreate{0}{0.0}{0}%
        }%
    },%
    /pgf/fpu/handlers/invalid separator/.code 2 args={%
        \pgfmath@error{Could not parse input '#1' as a floating point number, sorry. The unreadable part was near the decimal separator '#2'. Do you need the option 'read comma as period'?}{}%
    },
    /pgf/fpu/handlers/invalid number/.code 2 args={%
        \pgfmath@error{Could not parse input '#1' as a floating point number, sorry. The unreadable part was near '#2'.}{}%
    },
    /pgf/fpu/handlers/wrong lowlevel format/.code 2 args={%
        \pgfmath@error{Sorry, an internal routine of the floating point unit got an ill-formatted floating point number `#1'. The unreadable part was near '#2'.}{}%
        \let\pgfmathresult=\pgfutil@empty
    },
}

% #1 the error handler
% #2 the number which was invalid.
% #3 the part which produced the error
%
% POSTCONDITION: the three registers
%     \pgfmathfloat@a@S
%     \pgfmathfloat@a@Mtok
%     \pgfmathfloat@a@E
% will contain the number which results from the error handler.
\def\pgfmathfloatparsenumber@handleerror#1#2#3{%
    \let\pgfmathresult=\pgfutil@empty
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfkeys{/pgf/fpu/handlers/#1={#2}{#3}}%
    \ifx\pgfmathresult\pgfutil@empty
        \pgfmathfloat@a@S=3
        \pgfmathfloat@a@Mtok={0.0}%
        \pgfmathfloat@a@E=0
    \else
        \expandafter\pgfmathfloat@decompose@tok\pgfmathresult\relax\pgfmathfloat@a@S\pgfmathfloat@a@Mtok\pgfmathfloat@a@E
    \fi
}
\def\pgfflt@error#1\pgfflt@EOI{%
    \begingroup
    \pgfmathfloat@a@Mtok={#1}%
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\pgfmathfloatparsenumber@handleerror
            {invalid number}{\pgfmathresult}{\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}%



% FROM: checksign.
%
\def\pgfflt@init#1{%
    \expandafter\ifx\csname pgffltA@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltA@#1\endcsname
    \fi}
% state transitions:
\expandafter\def\csname pgffltA@0\endcsname{\pgfflt@leadingzero}% FIXME: inline optimization!
\expandafter\def\csname pgffltA@1\endcsname{\pgfflt@nonzerodigit1}%
\expandafter\def\csname pgffltA@2\endcsname{\pgfflt@nonzerodigit2}%
\expandafter\def\csname pgffltA@3\endcsname{\pgfflt@nonzerodigit3}%
\expandafter\def\csname pgffltA@4\endcsname{\pgfflt@nonzerodigit4}%
\expandafter\def\csname pgffltA@5\endcsname{\pgfflt@nonzerodigit5}%
\expandafter\def\csname pgffltA@6\endcsname{\pgfflt@nonzerodigit6}%
\expandafter\def\csname pgffltA@7\endcsname{\pgfflt@nonzerodigit7}%
\expandafter\def\csname pgffltA@8\endcsname{\pgfflt@nonzerodigit8}%
\expandafter\def\csname pgffltA@9\endcsname{\pgfflt@nonzerodigit9}%
\def\pgfflt@nonzerodigit#1{%
    \pgfmathfloat@a@Mtok={#1}%
    \pgfmathfloatparsenumberpendingperiodtrue
    \pgfflt@positiveexp}%
\expandafter\def\csname pgffltA@n\endcsname{\pgfflt@readnan}% FIXME: inlining?
\expandafter\def\csname pgffltA@N\endcsname{\pgfflt@readnan}% FIXME: inlining?
\expandafter\def\csname pgffltA@i\endcsname{\pgfflt@readinf}% FIXME: inlining?
\expandafter\def\csname pgffltA@I\endcsname{\pgfflt@readinf}% FIXME: inlining?
\expandafter\def\csname pgffltA@.\endcsname{% read '.9' like '0.9'
    \pgfmathfloat@a@E=-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltA@,\endcsname{% read ',9' like '0,9'
    \pgfmathfloat@frenchinput{%
        \pgfmathfloat@a@E=-1
        \pgfflt@leadingzero@foundperiod
    }%
}%

\def\pgfmathfloat@frenchinput#1{%
    \ifpgfmathparsenumber@comma@as@period
        \def\pgf@marshal{#1}%
        \expandafter\pgf@marshal
    \else
        \expandafter\pgfflt@error@separator\expandafter,%
    \fi
}%
\def\pgfflt@error@separator#1\pgfflt@EOI{%
    \begingroup
    \pgfmathfloat@a@Mtok={#1}%
    \xdef\pgfmathfloat@glob@TMP{%
        \noexpand\pgfmathfloatparsenumber@handleerror
            {invalid separator}{\pgfmathresult}{\the\pgfmathfloat@a@Mtok}}%
    \endgroup
    \pgfmathfloat@glob@TMP
}%

\def\pgfflt@finish#1\pgfflt@EOI{}

\def\pgfflt@readnan #1#2{%
    \def\pgfflt@readnan@ok{1}%
    \if#1a\else\if#1A\else\def\pgfflt@readnan@ok{0}\fi\fi
    \if#2n\else\if#2N\else\def\pgfflt@readnan@ok{0}\fi\fi
    \if\pgfflt@readnan@ok1%
        \pgfmathfloat@a@S=3\relax%
        \pgfmathfloat@a@Mtok={0.0}%
        \pgfmathfloat@a@E=0%
        \expandafter\pgfflt@finish
    \else
        \def\pgfflt@readnan@{\pgfflt@error #1#2}%
        \expandafter\pgfflt@readnan@
    \fi
}
\def\pgfflt@readinf #1#2{%
    \def\pgfflt@readinf@ok{1}%
    \if#1n\else\if#1N\else\def\pgfflt@readinf@ok{0}\fi\fi
    \if#2f\else\if#2F\else\def\pgfflt@readinf@ok{0}\fi\fi
    \if\pgfflt@readinf@ok1%
        \ifnum\pgfmathfloat@a@S=1 %
            \pgfmathfloat@a@S=4 %
            \pgfmathfloat@a@Mtok={0.0}%
        \else
            \pgfmathfloat@a@S=5 %
            \pgfmathfloat@a@Mtok={0.0}%
        \fi
        \pgfmathfloat@a@E=0 %
        \expandafter\pgfflt@finish
    \else
        \def\pgfflt@readinf@{\pgfflt@error #1#2}%
        \expandafter\pgfflt@readinf@
    \fi
}
\def\pgfflt@leadingzero#1{%
    \expandafter\ifx\csname pgffltB@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltB@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltB@0\endcsname{\pgfflt@leadingzero}%
\expandafter\def\csname pgffltB@1\endcsname{\pgfmathfloat@a@Mtok={1}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@2\endcsname{\pgfmathfloat@a@Mtok={2}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@3\endcsname{\pgfmathfloat@a@Mtok={3}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@4\endcsname{\pgfmathfloat@a@Mtok={4}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@5\endcsname{\pgfmathfloat@a@Mtok={5}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@6\endcsname{\pgfmathfloat@a@Mtok={6}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@7\endcsname{\pgfmathfloat@a@Mtok={7}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@8\endcsname{\pgfmathfloat@a@Mtok={8}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@9\endcsname{\pgfmathfloat@a@Mtok={9}\pgfmathfloatparsenumberpendingperiodtrue \pgfflt@positiveexp}
\expandafter\def\csname pgffltB@\pgfmathfloat@POSTFLAGSCHAR\endcsname{\pgfmathfloat@a@Mtok={0}\pgfflt@readlowlevelfloat}%
\expandafter\def\csname pgffltB@.\endcsname{%
    \pgfmathfloat@a@E=-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltB@,\endcsname{%
    \pgfmathfloat@frenchinput{%
        \pgfmathfloat@a@E=-1
        \pgfflt@leadingzero@foundperiod
    }%
}%
\expandafter\def\csname pgffltB@e\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0%
    \pgfflt@readexponent}%
\let\pgffltB@E=\pgffltB@e
\expandafter\def\csname pgffltB@\pgfflt@EOI\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0}%

\def\pgfflt@leadingzero@foundperiod#1{%
    \expandafter\ifx\csname pgffltC@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltC@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltC@0\endcsname{%
    \advance\pgfmathfloat@a@E by-1
    \pgfflt@leadingzero@foundperiod}%
\expandafter\def\csname pgffltC@1\endcsname{\pgfmathfloat@a@Mtok={1}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@2\endcsname{\pgfmathfloat@a@Mtok={2}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@3\endcsname{\pgfmathfloat@a@Mtok={3}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@4\endcsname{\pgfmathfloat@a@Mtok={4}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@5\endcsname{\pgfmathfloat@a@Mtok={5}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@6\endcsname{\pgfmathfloat@a@Mtok={6}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@7\endcsname{\pgfmathfloat@a@Mtok={7}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@8\endcsname{\pgfmathfloat@a@Mtok={8}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@9\endcsname{\pgfmathfloat@a@Mtok={9}\pgfmathfloatparsenumberpendingperiodtrue\pgfflt@finish@number@after@period}%
\expandafter\def\csname pgffltC@e\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0%
    \pgfflt@readexponent}%
\let\pgffltC@E=\pgffltC@e
\expandafter\def\csname pgffltC@\pgfflt@EOI\endcsname{%
    \pgfmathfloat@a@S=0\relax%
    \pgfmathfloat@a@Mtok={0.0}%
    \pgfmathfloat@a@E=0}%


\def\pgfflt@positiveexp#1{%
    \expandafter\ifx\csname pgffltD@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltD@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltD@0\endcsname{%
    \advance\pgfmathfloat@a@E by1
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros@positiveexp}%
\expandafter\def\csname pgffltD@1\endcsname{\pgffltD@nonzerodigit1}%
\expandafter\def\csname pgffltD@2\endcsname{\pgffltD@nonzerodigit2}%
\expandafter\def\csname pgffltD@3\endcsname{\pgffltD@nonzerodigit3}%
\expandafter\def\csname pgffltD@4\endcsname{\pgffltD@nonzerodigit4}%
\expandafter\def\csname pgffltD@5\endcsname{\pgffltD@nonzerodigit5}%
\expandafter\def\csname pgffltD@6\endcsname{\pgffltD@nonzerodigit6}%
\expandafter\def\csname pgffltD@7\endcsname{\pgffltD@nonzerodigit7}%
\expandafter\def\csname pgffltD@8\endcsname{\pgffltD@nonzerodigit8}%
\expandafter\def\csname pgffltD@9\endcsname{\pgffltD@nonzerodigit9}%
\expandafter\def\csname pgffltD@\pgfmathfloat@POSTFLAGSCHAR\endcsname{\pgfflt@readlowlevelfloat}%
\expandafter\def\csname pgffltD@.\endcsname{\pgfflt@finish@number@after@period}% FIXME : inlining?
\expandafter\def\csname pgffltD@,\endcsname{\pgfmathfloat@frenchinput{\pgfflt@finish@number@after@period}}%
\expandafter\def\csname pgffltD@e\endcsname{\pgfflt@readexponent}% FIXME : inlining?
\let\pgffltD@E=\pgffltD@e
\expandafter\def\csname pgffltD@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltD@nonzerodigit#1{%
    \advance\pgfmathfloat@a@E by1
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@positiveexp}%

% Read a low-level floating point.
% Since we are in the second state, \pgfmathfloat@a@Mtok contains the
% FLAGS. The post-flags-char has also been read.
\def\pgfflt@readlowlevelfloat#1e#2]\pgfflt@EOI{%
    \pgfmathfloatparsenumberpendingperiodfalse
    \pgfmathfloat@a@S=\the\pgfmathfloat@a@Mtok\relax
    \pgfmathfloat@a@Mtok={#1}%
    \pgfmathfloat@a@E=#2
}%

\def\pgfflt@readexponent#1\pgfflt@EOI{%
    \afterassignment\pgfflt@readexponent@
    \pgfmathfloat@b@E=#1 \pgfflt@EOI% the white space is important, otherwise \pgfflt@EOI will be expanded.
}
\def\pgfflt@readexponent@#1{%
    \advance\pgfmathfloat@a@E by\pgfmathfloat@b@E\relax
    %
    % sanity checking:
    \def\pgfmathfloat@loc@TMPb{#1}%
    \ifx\pgfmathfloat@loc@TMPb\pgfflt@EOI@unexpanded
    \else
        \def\pgfmathfloat@loc@TMPb{\pgfflt@error#1}%
        \expandafter\pgfmathfloat@loc@TMPb
    \fi
}

\def\pgfflt@pendingzeros@positiveexp#1{%
    \expandafter\ifx\csname pgffltE@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltE@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltE@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \advance\pgfmathfloat@a@E by1
    \pgfflt@pendingzeros@positiveexp}%
\expandafter\def\csname pgffltE@1\endcsname{\pgffltE@nonzerodigit1}%
\expandafter\def\csname pgffltE@2\endcsname{\pgffltE@nonzerodigit2}%
\expandafter\def\csname pgffltE@3\endcsname{\pgffltE@nonzerodigit3}%
\expandafter\def\csname pgffltE@4\endcsname{\pgffltE@nonzerodigit4}%
\expandafter\def\csname pgffltE@5\endcsname{\pgffltE@nonzerodigit5}%
\expandafter\def\csname pgffltE@6\endcsname{\pgffltE@nonzerodigit6}%
\expandafter\def\csname pgffltE@7\endcsname{\pgffltE@nonzerodigit7}%
\expandafter\def\csname pgffltE@8\endcsname{\pgffltE@nonzerodigit8}%
\expandafter\def\csname pgffltE@9\endcsname{\pgffltE@nonzerodigit9}%
\expandafter\def\csname pgffltE@.\endcsname{\pgfflt@finish@number@after@period}% FIXME : inlining?
\expandafter\def\csname pgffltE@,\endcsname{\pgfmathfloat@frenchinput{\pgfflt@finish@number@after@period}}% FIXME : inlining?
\def\pgffltE@e{\pgfflt@readexponent}% FIXME : inlining?
\let\pgffltE@E=\pgffltE@e
\expandafter\def\csname pgffltE@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltE@nonzerodigit#1{%
    \advance\pgfmathfloat@a@E by1
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@positiveexp}%

\def\pgfflt@finish@number@after@period#1{%
    \expandafter\ifx\csname pgffltF@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltF@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltF@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros}%
\expandafter\def\csname pgffltF@1\endcsname{\pgffltF@nonzerodigit1}%
\expandafter\def\csname pgffltF@2\endcsname{\pgffltF@nonzerodigit2}%
\expandafter\def\csname pgffltF@3\endcsname{\pgffltF@nonzerodigit3}%
\expandafter\def\csname pgffltF@4\endcsname{\pgffltF@nonzerodigit4}%
\expandafter\def\csname pgffltF@5\endcsname{\pgffltF@nonzerodigit5}%
\expandafter\def\csname pgffltF@6\endcsname{\pgffltF@nonzerodigit6}%
\expandafter\def\csname pgffltF@7\endcsname{\pgffltF@nonzerodigit7}%
\expandafter\def\csname pgffltF@8\endcsname{\pgffltF@nonzerodigit8}%
\expandafter\def\csname pgffltF@9\endcsname{\pgffltF@nonzerodigit9}%
\def\pgffltF@e{\pgfflt@readexponent}%
\let\pgffltF@E=\pgffltF@e
\expandafter\def\csname pgffltF@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltF@nonzerodigit#1{%
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@finish@number@after@period}%


\def\pgfflt@pendingzeros#1{%
    \expandafter\ifx\csname pgffltG@#1\endcsname\relax
        \expandafter\pgfflt@error\expandafter#1%
    \else
        \expandafter\expandafter\csname pgffltG@#1\endcsname
    \fi}
% State transitions:
\expandafter\def\csname pgffltG@0\endcsname{%
    \pgfmathfloat@tmptoks=\expandafter{\the\pgfmathfloat@tmptoks0}%
    \pgfflt@pendingzeros}%
\expandafter\def\csname pgffltG@1\endcsname{\pgffltG@nonzerodigit1}%
\expandafter\def\csname pgffltG@2\endcsname{\pgffltG@nonzerodigit2}%
\expandafter\def\csname pgffltG@3\endcsname{\pgffltG@nonzerodigit3}%
\expandafter\def\csname pgffltG@4\endcsname{\pgffltG@nonzerodigit4}%
\expandafter\def\csname pgffltG@5\endcsname{\pgffltG@nonzerodigit5}%
\expandafter\def\csname pgffltG@6\endcsname{\pgffltG@nonzerodigit6}%
\expandafter\def\csname pgffltG@7\endcsname{\pgffltG@nonzerodigit7}%
\expandafter\def\csname pgffltG@8\endcsname{\pgffltG@nonzerodigit8}%
\expandafter\def\csname pgffltG@9\endcsname{\pgffltG@nonzerodigit9}%
\def\pgffltG@e{\pgfflt@readexponent}% FIXME: inlining?
\let\pgffltG@E=\pgffltG@e
\expandafter\def\csname pgffltG@\pgfflt@EOI\endcsname{}% NOP
\def\pgffltG@nonzerodigit#1{%
    \ifpgfmathfloatparsenumberpendingperiod
        \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok.}%
        \pgfmathfloatparsenumberpendingperiodfalse
    \fi
    \pgfmathfloat@a@Mtok=\expandafter\expandafter\expandafter{\expandafter\the\expandafter\pgfmathfloat@a@Mtok\the\pgfmathfloat@tmptoks}%
    \pgfmathfloat@tmptoks={}%
    \pgfmathfloat@a@Mtok=\expandafter{\the\pgfmathfloat@a@Mtok#1}%
    \pgfflt@finish@number@after@period}%

\endinput


==> pgfmathfunctions.code.tex <==
% Copyright 2019 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% Declare a function for the parser.
%
% #1 - the name of the function.
% #2 - arity (or ... for variable arguments).
% #3 - the code for the function.
%
% Use \pgfmathdeclarefunction* to force a redefinition if the function exists already.
\def\pgfmathdeclarefunction{\pgfmath@ifnextchar*\pgfmathdeclarefunction@force\pgfmathdeclarefunction@check}
\def\pgfmathdeclarefunction@check#1{%
    \expandafter\ifx\csname pgfmath@function@#1\endcsname\relax\else%
        \pgfmath@error{The function `#1' already exists}{}%
    \fi%
    \pgfmath@declarefunction{#1}%
}
\def\pgfmathdeclarefunction@force*{\pgfmath@declarefunction}%

\def\pgfmathredeclarefunction#1#2{%
    \expandafter\ifx\csname pgfmath@function@#1\endcsname\relax%
        \pgfmath@error{The function `#1' does not exist}{}%
    \else%
    % was: \pgfmath@namedef{pgfmath#1@}{#2}% TT
    \edef\pgf@marshal{\noexpand\pgfmathdeclarefunction*{#1}{\csname    pgfmath@operation@#1@arity\endcsname}}%
    \pgf@marshal{#2}%
    \fi%
}

\def\pgfmath@declarefunction#1#2{%
    \pgfmath@namedef{pgfmath@function@#1}{#1}%
    \pgfmath@namedef{pgfmath@operation@#1@type}{function}%
    \pgfmath@namedef{pgfmath@operation@#1@arity}{#2}%
    \pgfmath@namedef{pgfmath@operation@#1@infix}{#1}%
    \pgfmath@namedef{pgfmath@operation@#1@precedence}{1000}%
    \expandafter\ifx\csname pgfmath@operation@#1@arity\endcsname\pgfmath@dots%
        \pgfmath@namedef{pgfmath@operation@#1@arity}{1}%
    \else%
        \ifnum\csname pgfmath@operation@#1@arity\endcsname>9\relax%
                \pgfmath@namedef{pgfmath@operation@#1@arity}{1}%
        \fi%
    \fi%
    \edef\pgfmath@marshal{%
        \noexpand\pgfmath@@declarefunction%
        {\expandafter\noexpand\csname pgfmath#1\endcsname}%
        {\expandafter\noexpand\csname pgfmath#1@\endcsname}%
        {\csname pgfmath@operation@#1@arity\endcsname}%
    }%
    \pgfkeysvalueof{/pgf/declare function/execute at begin function}%
    \pgfmath@marshal%
}

% #1 - \pgfmath<name>.
% #2 - \pgfmath<name>@.
% #3 - arity.
% #4 - code for function <name>.
%
\def\pgfmath@@declarefunction#1#2#3#4{% Function of arity 0 - 9.
    \pgfkeysvalueof{/pgf/declare function/execute at end function}%
    \ifcase#3\relax%
        \def#1{#2}%
        \def\pgfmath@@head{\def#2}%
    \or
        \def#1##1{\pgfmathparse{##1}\expandafter#2\expandafter{\pgfmathresult}}%
        \def\pgfmath@@head{\def#2####1}%
    \else%
        \pgfmath@toks={}%
        \pgfmathloop%
        \ifnum\pgfmathcounter>#3\relax%
        \else%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@char@hash}%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmathcounter}%
        \repeatpgfmathloop%
        \edef\pgfmath@head{\noexpand\def\noexpand#1\the\pgfmath@toks}%
        \edef\pgfmath@@head{\noexpand\def\noexpand#2\the\pgfmath@toks}%
        \pgfmath@toks={}%
        \def\pgfmath@arguments{}%
        \pgfmathloop%
        \ifnum\pgfmathcounter>#3\relax%
        \else%
            \pgfmath@addto@toks{\pgfmathparse}%
            \expandafter\expandafter\expandafter\pgfmath@addto@toks%
                \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
                    {\expandafter\pgfmath@char@hash\pgfmathcounter}}%
            \pgfmath@addto@toks{\let}%
            \expandafter\pgfmath@addto@toks\expandafter{%
                \csname pgfmath@argument@\pgfmathcounter\endcsname=\pgfmathresult}%
            \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
                \pgfmath@arguments\expandafter\expandafter\expandafter{\expandafter%
                    \pgfmath@arguments\expandafter{\csname pgfmath@argument@\pgfmathcounter\endcsname}}%
        \repeatpgfmathloop%
        \expandafter\pgfmath@addto@toks\expandafter{\expandafter#2\pgfmath@arguments}%
        \edef\pgfmath@body{{\the\pgfmath@toks}}%
        \expandafter\pgfmath@head\pgfmath@body%
    \fi%
    \pgfmath@@head{#4}%
}

\def\pgfmath@addto@toks#1{%
    \edef\pgfmath@toks@expanded{\the\pgfmath@toks}%
    \expandafter\pgfmath@toks\expandafter{\pgfmath@toks@expanded#1}}

% Key for declaring local functions.
%
\pgfkeys{%
    /pgf/declare function/.code={%
        \pgfmath@local@functions#1@=@;%
    },
    /pgf/declare function/execute at begin function/.initial={},
    /pgf/declare function/execute at end function/.initial={},
    /pgf/declare function/ignore spaces/.is choice,
    /pgf/declare function/ignore spaces/.default=true,
    /pgf/declare function/ignore spaces/true/.style={%
        /pgf/declare function/execute at begin function={%
            \begingroup
            \catcode`\^^I=9\relax
            \catcode`\ =9\relax
            \catcode`\~=10\relax
            \endlinechar=`\ \relax
        },
        /pgf/declare function/execute at end function={%
            \endgroup
        },
    },
    /pgf/declare function/ignore spaces/false/.style={%
        /pgf/declare function/execute at begin function={},
        /pgf/declare function/execute at end function={},
    },
}

\def\pgfmath@local@gobbleone#1{}
\def\pgfmath@local@at{@}%

\def\pgfmath@local@functions{%
    \pgfutil@ifnextchar x{\pgfmath@local@@functions}{\pgfmath@local@@functions}%
}

\def\pgfmath@local@@functions#1=#2;{%
    \def\pgfmath@local@temp{#1}%
    \ifx\pgfmath@local@temp\pgfmath@local@at%
        \let\pgfmath@local@next=\relax%
    \else%
        \pgfmath@local@function#1=#2;%
        \let\pgfmath@local@next=\pgfmath@local@functions%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function{%
    \let\pgfmath@local@name=\pgfutil@empty%
    \let\pgfmath@local@args=\pgfutil@empty%
    \let\pgfmath@local@body=\pgfutil@empty%
    \pgfmath@local@@function}

\def\pgfmath@local@@function#1{%
    \if#1=%
        \let\pgfmath@local@next=\pgfmath@local@function@body%
    \else%
        \if#1(%
            \let\pgfmath@local@next=\pgfmath@local@function@args%
        \else%
            \expandafter\def\expandafter\pgfmath@local@name\expandafter{\pgfmath@local@name#1}%
            \let\pgfmath@local@next=\pgfmath@local@@function%
        \fi%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function@args#1){%
    \def\pgfmath@local@args{#1}%
    \pgfmath@local@@function}

\def\pgfmath@local@function@body#1;{%
    \def\pgfmath@local@body{#1}%
    \begingroup%
        \c@pgf@counta=0\relax%
        \ifx\pgfmath@local@args\pgfmath@empty%
            \expandafter\pgfmath@toks\expandafter=\expandafter{\pgfmath@local@body}%
        \else%
            \pgfmath@toks={}%
            \expandafter\pgfmath@local@function@@body\pgfmath@local@args,,%
        \fi%
        \xdef\pgfmath@local@temp{%
            \noexpand\pgfmathnotifynewdeclarefunction{\pgfmath@local@name}{\the\c@pgf@counta}%
                {\the\pgfmath@toks}%
        }%
    \endgroup%
    \pgfmath@local@temp%
}

% #1: the name
% #2: the number of arguments <n>
% #3: a math expression containing '#1', '#2', ... ,'#'<n>
% This callback is overwritten by pgflibraryluamath.
\def\pgfmathnotifynewdeclarefunction#1#2#3{%
    \pgfmathdeclarefunction{#1}{#2}{\pgfmathparse{#3}}%
}%

\def\pgfmath@local@function@@body#1,{%
    \def\pgfmath@local@test{#1}%
    \ifx\pgfmath@local@test\pgfutil@empty%
        \let\pgfmath@local@next=\relax%
    \else%
        \edef\pgfmath@local@var@string{@\expandafter\pgfmath@local@gobbleone\string#1}%
        \advance\c@pgf@counta by1\relax%
        \expandafter\expandafter\expandafter\pgfmath@toks\expandafter\expandafter\expandafter=%
            \expandafter\expandafter\expandafter{\expandafter\pgfmath@char@hash\the\c@pgf@counta}%
        \edef#1{\the\pgfmath@toks}%
        \pgfmath@toks={}%
        \expandafter\pgfmath@local@function@@@body\pgfmath@local@body @%
        \edef\pgfmath@local@body{\the\pgfmath@toks}%
        \let\pgfmath@local@next=\pgfmath@local@function@@body%
    \fi%
    \pgfmath@local@next%
}

\def\pgfmath@local@function@@@body{%
    \pgfutil@ifnextchar\bgroup{\pgfmath@local@function@@@body@bgroup}%
        {\pgfmath@local@function@@@body@nobgroup}}%

\def\pgfmath@local@function@@@body@bgroup#1{%
    \begingroup%
        \pgfmath@toks={}%
        \pgfmath@local@function@@@body#1 @%
        \xdef\pgfmath@local@temp{{\the\pgfmath@toks}}%
    \endgroup%
    \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@local@temp}%
    \pgfmath@local@function@@@body%
}

\def\pgfmath@local@function@@@body@nobgroup#1{%
    \ifx#1@%
        \let\pgfmath@local@next=\relax%
    \else%
        \let\pgfmath@local@next=\pgfmath@local@function@@@body%
        \edef\pgfmath@local@var@@string{@\expandafter\pgfmath@local@gobbleone\string#1}%
        \ifx\pgfmath@local@var@@string\pgfmath@local@var@string%
            \expandafter\pgfmath@addto@toks\expandafter{#1}%
        \else%
            \edef\pgfmath@local@temp{\the\pgfmath@toks}%
            \pgfmath@toks={#1}%
            \edef\pgfmath@local@@temp{\the\pgfmath@toks}%
            \expandafter\pgfmath@toks\expandafter=\expandafter{\pgfmath@local@temp}%
            \expandafter\pgfmath@addto@toks\expandafter{\pgfmath@local@@temp}%
        \fi%
    \fi%
    \pgfmath@local@next%
}

% Allows to define 'x' as some \TeX command '#2'.
\def\pgfmathdeclarepseudoconstant#1#2{%
    \pgfmathdeclarefunction*{#1}{0}{#2}%
}%
% Redefines a pseudo constant '#1'.
\def\pgfmathredeclarepseudoconstant#1#2{%
    \pgfmathredeclarefunction{#1}{#2}%
}%

\input pgfmathfunctions.basic.code.tex
\input pgfmathfunctions.trigonometric.code.tex
\input pgfmathfunctions.random.code.tex
\input pgfmathfunctions.comparison.code.tex
\input pgfmathfunctions.base.code.tex
\input pgfmathfunctions.round.code.tex
\input pgfmathfunctions.misc.code.tex
\input pgfmathfunctions.integerarithmetics.code.tex



% Local Variables:
% tab-width: 2
% End:


==> pgfmathparser.code.tex <==

\newdimen\pgfmath@dimen
\newcount\pgfmath@count
\newbox\pgfmath@box
\newtoks\pgfmath@toks

\newif\ifpgfmath@quickparse
\newif\ifpgfmathfloat
\newif\ifpgfmathunitsdeclared
\newif\ifpgfmathmathunitsdeclared
\newif\ifpgfmathignoreunitscale

\let\pgfmath@protected@edef=\edef
\ifcsname protected@edef\endcsname
  \let\pgfmath@protected@edef=\protected@edef
\fi

\def\pgfmathprint#1{\pgfmathparse{#1}\pgfmathresult}

\def\pgfmathparse{%
  \begingroup
    \pgfmath@catcodes
    \pgfmath@quickparsefalse
    % Test for the fpu library
    \ifpgfmathfloat
      \let\pgfmath@parse@next=\pgfmathfloatparsenumber
    \else
      \let\pgfmath@parse@next=\pgfmathparse@
    \fi
    \pgfmath@parse@next}

\def\pgfmath@catcodes{% Maybe unnecessary.
  \catcode`\==12 %
  \catcode`\,=12 %
  \catcode`\|=12 %
  \catcode`\&=12 %
}

\def\pgfmathqparse{%
  \begingroup
    \pgfmath@catcodes
    \pgfmath@quickparsetrue
    \pgfmathparse@}

\def\pgfmathparse@#1{%
    % No (math) units yet.
    \global\pgfmathunitsdeclaredfalse
    \global\pgfmathmathunitsdeclaredfalse
    % Expand expression so any remaining CSs are registers
    % or box dimensions (i.e. |\wd|, |\ht|, |\dp|).
    \pgfmath@protected@edef\pgfmath@expression{#1}%
    %
    \expandafter\pgfmathparse@trynumber@loop\pgfmath@expression\pgfmath@parse@stop
    %
    % this here is the _real_ parser. it is invoked by
    % \pgfmathparse@trynumber@loop if that says "this is no number"
    %\pgfmathparse@@\pgfmath@parse@stop%
}

\def\pgfmath@parse@stop{\pgfmath@parse@stop}% equals only itself

\def\pgfmathparse@trynumber@token{numeric}
\begingroup
\def\\{\global\let\pgf@let@space@token= } \\ % now, \pgf@let@space@token is a space token
\endgroup

% This a "fast-lane": if the expressions consist merely of number
% tokens, we can simply return the number as-is.
%
% This is significantly faster and should resemble the 80% use-case.
%
% #1 a single token
\def\pgfmathparse@trynumber@loop{%
    \futurelet\pgfmath@token@let\pgfmathparse@trynumber@loop@
}%
\def\pgfmathparse@trynumber@loop@#1{%
    \ifx\pgfmath@token@let\pgf@let@space@token
        % Hm. we found a white space... and we have no support for
        % trimming. That means we have to assume that the white space
        % occurred somewhere in the middle - and fall back to the
        % expensive method.
        \def\pgfmath@parse@next{\pgfmathparse@@#1}%
    \else
        \ifx\pgfmath@token@let\bgroup%
            % oh! We found '{' #1.
            % Well, these braces appear to be special; fall back to
            % the complicated routine...
            \let\pgfmath@parse@next=\pgfmathparse@@
        \else
            \ifx\pgfmath@token@let\pgfmath@parse@stop
                % Ah: we have passed the check! The expression consists only
                % of 0123456789. , so do not parse anything and return it
                % as-is!
                \let\pgfmath@parse@next=\pgfmathparse@expression@is@number
            \else
                \expandafter\ifx\csname pgfmath@token@\pgfmathparse@trynumber@token @\string#1\endcsname\relax%
                    % hm. It is none of 0123456789.
                    \let\pgfmath@parse@next=\pgfmathparse@@
                \else
                    % continue... we only found one of 0123456789. so
                    % far...
                    \let\pgfmath@parse@next=\pgfmathparse@trynumber@loop
                \fi
            \fi
        \fi
    \fi
    \pgfmath@parse@next
}%

\def\pgfmathparse@expression@is@number{%
    \let\pgfmathresult=\pgfmath@expression
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup
  \ignorespaces
}%
\def\pgfmathparse@@#1\pgfmath@parse@stop{%
    % We are inside a group (opened in |\pgfmathparse| or
    % |\pgfmathqparse|).
    % Stuff for calc compatibility.
    \let\real=\pgfmath@calc@real
    \let\minof=\pgfmath@calc@minof
    \let\maxof=\pgfmath@calc@maxof
    \let\ratio=\pgfmath@calc@ratio
    \let\widthof=\pgfmath@calc@widthof
    \let\heightof=\pgfmath@calc@heightof
    \let\depthof=\pgfmath@calc@depthof
    % Restore font (defined in pgfmathutil.code.tex)
    \pgfmath@selectfont
    % Set up stack.
    \pgfmath@stack@operation={{}{}{}}%
    \pgfmath@stack@operand={{}{}{}}%
    \let\pgfmath@stack@operation@top=\pgfmath@stack@empty
    \let\pgfmath@stack@operand@top=\pgfmath@stack@empty
    % An expression always begins with an operand.
    \expandafter\pgfmath@bgroup@strip\expandafter{\pgfmath@expression}%
    % |\pgfmath@bgroup@stripped| is the result of
    % |\pgfmath@bgroup@strip|
    \expandafter\pgfmath@parse@@operand\pgfmath@bgroup@stripped @@@@\pgfmath@parse@stop%
}

\def\pgfmath@parse@end#1\pgfmath@parse@stop{%
    \pgfmathpostparse
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup
  \ignorespaces}

\let\pgfmathpostparse=\relax

% For compatibility with older version.
%
\def\pgfmathscaleresult{%
  \ifpgfmathunitsdeclared
  \else
    \ifpgfmathignoreunitscale
    \else
       \afterassignment\pgfmath@gobbletilpgfmath@%
      \pgfmath@x\pgfmathresultunitscale pt\relax\pgfmath@%
      \expandafter\pgfmath@x\pgfmathresult\pgfmath@x%
      \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
    \fi
  \fi
}

\def\pgfmathsetresultunitscale#1{\def\pgfmathresultunitscale{#1}}

\def\pgfmathresultunitscale{1}


% A utility function which evaluates expression '#1' and invokes '#2'
% if the expression is true and '#3' if it is false.
\def\pgfmathifexpression#1#2#3{%
    \pgfmathparse{#1}%
    \pgfmath@iftrue{#2}{#3}%
}%
% Executes '#1' if \pgfmathresult is 'true', '#2' otherwise.
% WARNING : overwritten in fpu lib!
\def\pgfmath@iftrue{%
    \ifdim\pgfmathresult pt=1.0pt %
        \let\pgfmath@next=\pgfutil@firstoftwo
    \else
        \let\pgfmath@next=\pgfutil@secondoftwo
    \fi
    \pgfmath@next%
}%

% Stuff for computability with the calc package.
%
\def\pgfmath@calc@real#1{#1}
\def\pgfmath@calc@minof#1#2{min(#1,#2)}
\def\pgfmath@calc@maxof#1#2{max(#1,#2)}
\def\pgfmath@calc@ratio#1#2{#1/#2}
\def\pgfmath@calc@widthof#1{width("#1")}
\def\pgfmath@calc@heightof#1{height("#1")}
\def\pgfmath@calc@depthof#1{depth("#1")}

\def\pgfmath@bgroup{\string\pgfmath@bgroup}
\def\pgfmath@egroup{\string\pgfmath@egroup}
\def\pgfmath@egroup@token{\pgfmath@egroup}

\def\pgfmath@text@@{@}
\def\pgfmath@text@operator{operator}
\def\pgfmath@text@function{function}
\def\pgfmath@dots{...}
\def\pgfmath@char@zero{0}
\def\pgfmath@char@quote{"}
\def\pgfmath@char@exclamation{!}
\def\pgfmath@char@plus{+}
\def\pgfmath@char@minus{-}
\def\pgfmath@char@period{.}
\def\pgfmath@char@leftangle{<}
\def\pgfmath@char@leftbracket{[}
\pgfmath@toks={#}
\edef\pgfmath@char@hash{\the\pgfmath@toks}

\def\pgfmath@tokens@make#1#2{%
  % Defines for each token or balanced text in |#2| a control sequence
  % |\pgfmath@token@<#1>@\string<one token from #2>| and stores |#2|
  % in it.
  \def\pgfmath@prefix{#1}%
  % Note the empty group |{}| at the end that ends the loop in
  % |\pgfmath@token@@make|.
  \expandafter\pgfmath@tokens@@make#2{}}

\def\pgfmath@tokens@@make#1{%
  \def\pgfmath@token{#1}%
  \ifx\pgfmath@token\pgfmath@empty
    % End of loop: all tokens or balanced texts were parsed.
  \else
    \pgfmath@namedef{pgfmath@token@\pgfmath@prefix @\string#1}{#1}%
    \expandafter\pgfmath@tokens@@make%
  \fi}

\pgfmath@tokens@make{box}{\wd\ht\dp}
\ifx\dimexpr\@undefined\else % needed for classic tex
  \pgfmath@tokens@make{dimexpr}{\dimexpr\glueexpr}
\fi
\pgfmath@tokens@make{unit}{{bp}{cc}{cm}{dd}{em}{ex}{in}{mm}{pc}{pt}{sp}}
\ifx\pdftexversion\@undefined\else % for pdfTeX
  \pgfmath@tokens@make{unit}{{nc}{nd}{px}}
\fi
\ifx\directlua\@undefined\else % for LuaTeX
  \pgfmath@tokens@make{unit}{{nc}{nd}{px}}
\fi
\ifx\kanjiskip\@undefined\else % for pTeX, upTeX
  \pgfmath@tokens@make{unit}{{H}{Q}{zh}{zw}}
\fi
%
\pgfmath@tokens@make{mathunit}{{mu}}
\pgfmath@tokens@make{numeric}{.0123456789}
\pgfmath@tokens@make{number}{0123456789}
\pgfmath@tokens@make{functional}{_abcdefghijklmnopqrstuvwxyzABCDEFGHIJKLMNOPQRSTUVWXYZ}
\pgfmath@tokens@make{exponent}{eE}
\pgfmath@tokens@make{group}{{()}{[]}{\pgfmath@bgroup\pgfmath@egroup}}
\pgfmath@tokens@make{specials}{@)]\pgfmath@egroup}
\pgfmath@tokens@make{hexadecimal}{0123456789ABCDEFabcdef}
\pgfmath@tokens@make{octal}{01234567}
\pgfmath@tokens@make{binary}{01}

\pgfmath@namedef{pgfmath@base@0x}{16}
\pgfmath@namedef{pgfmath@base@0X}{16}
\pgfmath@namedef{pgfmath@base@0b}{2}
\pgfmath@namedef{pgfmath@base@0B}{2}

% Determine if a register is a count or a dimension/skip register.
\newif\ifpgfmath@dimen@
\def\pgfmath@dimen@#1{%
  \begingroup
    \afterassignment\pgfmath@dimen@@%
    #1=0.0pt\relax\pgfmath@}
\def\pgfmath@dimen@@#1#2\pgfmath@{%
  \endgroup
  \ifx#1.%
    \pgfmath@dimen@false
  \else
    \pgfmath@dimen@true
  \fi}

\def\pgfmath@parse@ifbgroup#1#2{%
  \let\pgfmath@parse@bgroup@after=#1%
  \let\pgfmath@parse@nobgroup@after=#2%
  \futurelet\pgfmath@token@let%
  \pgfmath@parse@@ifbgroup}

\def\pgfmath@parse@@ifbgroup{%
  \ifx\pgfmath@token@let\bgroup
    \let\pgfmath@parse@next=\pgfmath@parse@@@ifbgroup
  \else
    % |\pgfmath@sptoken| defined in \file{pgfmathutil.code.tex}.
    \ifx\pgfmath@token@let\pgfmath@sptoken
      \let\pgfmath@parse@next=\pgfmath@parse@@@@ifbgroup
    \else
      \let\pgfmath@parse@next=\pgfmath@parse@nobgroup@after
    \fi
  \fi
  \pgfmath@parse@next}

% TT: If false, octal parsing is switched off (needed for time parsing)
\newif\ifpgfmath@octalparsing
\pgfmath@octalparsingtrue

% I (CJ) *think* it replaces |{| and |}| by |\pgfmath@bgroup| and
% |\pgfmath@egroup|?
\def\pgfmath@parse@@@ifbgroup#1{%
  \pgfmath@parse@bgroup@after\pgfmath@bgroup#1\pgfmath@egroup}

{
\def\:{\pgfmath@parse@@@@ifbgroup}
\expandafter\gdef\: {\futurelet\pgfmath@token@let\pgfmath@parse@@ifbgroup}
}

% Parse an operand.
\def\pgfmath@parse@operand{%
  \expandafter\pgfmath@parse@@operand\pgfmath@token@next}

% This is the entry point for the parser. It is called at the end of
% |\pgfmathparse@| with the following syntax
% |\expandafter\pgfmath@parse@@operand\pgfmath@bgroup@stripped
% @@@@\pgfmath@parse@stop|.
% Note: we are inside a group.
\def\pgfmath@parse@@operand{%
  \pgfmath@parse@ifbgroup{\pgfmath@parse@@operand}{\pgfmath@parse@@operand@}}

% An operand is
% * |+| (unary plus),
% * |-| (unary minus),
% * a prefix operator
\def\pgfmath@parse@@operand@#1{%
  \def\pgfmath@token{#1}%
  \ifx\pgfmath@token\pgfmath@char@plus
    % Unary (prefix) plus
    \let\pgfmath@parse@next=\pgfmath@parse@@operand%
  \else
    \ifx\pgfmath@token\pgfmath@char@minus
      % Unary (prefix) minus
      \pgfmath@stack@push@operation{neg}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand
    \else
      % See |\pgfmathdeclareoperator| (below). Note that |+| and |-|
      % that are also declared as operators have been tested before so
      % they should never be parsed as binary (infix) operator at this stage.
      \expandafter\ifx\csname pgfmath@operation@\expandafter\string\pgfmath@token @prefix\endcsname\pgfmath@token
        \let\pgfmath@parse@next=\pgfmath@parse@prefix@operator
      \else
        \ifpgfmath@quickparse
          \let\pgfmath@parse@next=\pgfmath@qparse@operand
        \else
          \let\pgfmath@number=\pgfmath@empty
          \expandafter\ifx\csname pgfmath@token@functional@\string#1\endcsname\relax%
            \let\pgfmath@base=\pgfmath@empty%
            \let\pgfmath@token@next=\pgfmath@token%
            \if#10% Check for octal prefix.
              \ifpgfmath@octalparsing%
                \def\pgfmath@base{8}%
              \fi%
            \fi%
            \let\pgfmath@parse@next=\pgfmath@parse@number%
          \else%
            \let\pgfmath@function=\pgfmath@token%
            \let\pgfmath@parse@next=\pgfmath@parse@function%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}

% Parse prefix operators.
%
\def\pgfmath@parse@prefix@operator{%
  \ifx\pgfmath@token\pgfmath@char@quote% Quote character.
    \let\pgfmath@parse@next=\pgfmath@parse@operand@quote%
  \else%
    \ifx\pgfmath@token\pgfmath@char@exclamation% Prefix !.
      \pgfmath@stack@push@operation{not}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \else% Anything else, just push and hope.
      \expandafter\pgfmath@stack@push@operation\expandafter{\pgfmath@token}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \fi%
  \fi%
  \pgfmath@parse@next%
}%


% Quote part of an expression.
%
\def\pgfmath@parse@operand@quote#1"{%
  \def\pgfmathresult{#1}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Quick operand parsing. Should always have units.
% No functions, base conversion, quoting or scientific notation
% are permitted.
\def\pgfmath@qparse@operand{%
  \afterassignment\pgfmath@qparse@@operand%
  \pgfmath@dimen\pgfmath@token}
\def\pgfmath@qparse@@operand{%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Parse a number, which can take the form:
%
% 1. An integer, or a decimal, with or without units.
% 2. A dimension/skip or a count register.
% 3. A dimension register preceded by a number or count register.
% 4. A box dimension (e.g., \wd\mybox).
% 5. A box dimension preceded by a number or a count register.
% 6. Scientific notation (e.g., 1.234567e-10).
% 7. A binary, hexadecimal, or octal number.
%
\def\pgfmath@parse@number{\pgfmath@parse@ifbgroup{\pgfmath@parse@number}{\pgfmath@parse@number@}}
\def\pgfmath@parse@number@#1{%
  \let\pgfmath@token=\pgfmath@token@next%
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@number}

\def\pgfmath@parse@@number{%
  \ifx\pgfmath@token\pgfmath@egroup@token%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmath@number}%
    \let\pgfmath@parse@next=\pgfmath@parse@@@operator%
  \else%
    \expandafter\ifcat\pgfmath@token\relax% A CS?
      \expandafter\ifx\csname pgfmath@token@dimexpr@\expandafter\string\pgfmath@token\endcsname\relax%
        \expandafter\ifx\pgfmath@token\numexpr%
          \let\pgfmath@parse@next=\pgfmath@parse@numexpr%
        \else%
          \expandafter\ifx\pgfmath@token\muexpr%
            \let\pgfmath@parse@next=\pgfmath@parse@muexpr%
          \else%
            \expandafter\ifx\csname pgfmath@token@box@\expandafter\string\pgfmath@token\endcsname\relax%
              % So, is the CS is a dimension or a count register?
              \expandafter\pgfmath@dimen@\pgfmath@token%
              \ifpgfmath@dimen@% A dimension register.
                \global\pgfmathunitsdeclaredtrue%
                \pgfmath@dimen=\pgfmath@number\pgfmath@token%
                \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
                \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                \let\pgfmath@parse@next=\pgfmath@parse@operator%
              \else% A count register.
                \pgfmath@count=\pgfmath@token%
                \expandafter\def\expandafter\pgfmath@number\expandafter{\the\pgfmath@count}%
                \expandafter\ifcat\pgfmath@token@next\relax%
                  % A CS following a count register should be \wd, \ht or \dp.
                  \let\pgfmath@parse@next=\pgfmath@parse@number%
                \else%
                  \let\pgfmathresult=\pgfmath@number%
                  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                  \let\pgfmath@parse@next=\pgfmath@parse@operator%
                \fi%
              \fi%
            \else%
              % This should be a box specification, for example, 0.5\wd\mybox.
              \global\pgfmathunitsdeclaredtrue%
              \pgfmath@dimen=\pgfmath@number\pgfmath@token\pgfmath@token@next%
              \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
              \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
              \let\pgfmath@parse@next=\pgfmath@parse@@operator%
            \fi%
          \fi%
        \fi%
      \else%
        \global\pgfmathunitsdeclaredtrue%
        \let\pgfmath@parse@next=\pgfmath@parse@dimexpr%
      \fi%
    \else%
      \expandafter\ifx\csname pgfmath@token@numeric@\expandafter\string\pgfmath@token\endcsname\relax%
        % It isn't numeric (i.e., 012345679.), so it might be units...
        % first double-character units...
        \expandafter\ifx\csname pgfmath@token@unit@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
        % then single-character units...
        \expandafter\ifx\csname pgfmath@token@unit@\pgfmath@token\endcsname\relax%
          % ...or the exponent characters...
          \expandafter\ifx\csname pgfmath@token@exponent@\pgfmath@token\endcsname\relax%
            % ...or a base prefix...
            \expandafter\ifx\csname pgfmath@base@\pgfmath@number\pgfmath@token\endcsname\relax%
              % ...or a math unit...
              \expandafter\ifx\csname pgfmath@token@mathunit@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
                % ...none of the above...
                  \ifx\pgfmath@base\pgfmath@empty%
                    \let\pgfmathresult=\pgfmath@number%
                  \else%
                    \ifx\pgfmath@number\pgfmath@char@zero%
                      \let\pgfmathresult=\pgfmath@number%
                    \else%
                      % Convert from octal.
                      \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{8}{10}%
                    \fi%
                  \fi%
                  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                  \let\pgfmath@parse@next=\pgfmath@parse@@@operator%
              \else%
                % ...here, it is a math unit (mu). Treat it as a pt.
                \global\pgfmathunitsdeclaredtrue%
                \global\pgfmathmathunitsdeclaredtrue%
                \pgfmath@dimen=\pgfmath@number pt\relax%
                \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
                \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
                \let\pgfmath@parse@next=\pgfmath@parse@@operator%
              \fi%
            \else%
              % ...here, it is a base prefix 0x, 0X, 0b or 0B
              \expandafter\let\expandafter\pgfmath@base\expandafter=%
                \csname pgfmath@base@\pgfmath@number\pgfmath@token\endcsname%
              \let\pgfmath@parse@next=\pgfmath@parse@base%
            \fi%
          \else% ... and here, it is the exponent characters.
            \let\pgfmath@parse@next=\pgfmath@parse@exponent%
          \fi%
        \else% ...but here it is single-character units.
          \global\pgfmathunitsdeclaredtrue%
          \pgfmath@dimen=\pgfmath@number\pgfmath@token\relax%
          \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
          \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
          \let\pgfmath@parse@next=\pgfmath@parse@@operator%
        \fi%
        \else% ...but here it is double-character units.
          \global\pgfmathunitsdeclaredtrue%
          \pgfmath@dimen=\pgfmath@number\pgfmath@token\pgfmath@token@next\relax%
          \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
          \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
          \let\pgfmath@parse@next=\pgfmath@parse@@operator%
        \fi%
      \else% It is numeric.
        \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgfmath@number%
          \expandafter\expandafter\expandafter{\expandafter\pgfmath@number\pgfmath@token}%
        \ifx\pgfmath@token\pgfmath@char@period%
          \let\pgfmath@base=\pgfmath@empty%
        \fi%
        \let\pgfmath@parse@next=\pgfmath@parse@number%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}


% Parse a \dimexpr
\def\pgfmath@parse@dimexpr{%
  \afterassignment\pgfmath@parse@dimexpr@%
  \expandafter\expandafter\expandafter\pgfmath@dimen\expandafter\pgfmath@token\pgfmath@token@next%
}
\def\pgfmath@parse@dimexpr@{%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@dimen}}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}


% Parse a \muexpr
\def\pgfmath@parse@muexpr{%
  \begingroup%
    \afterassignment\pgfmath@parse@muexpr@%
    \expandafter\expandafter\expandafter\muskip\expandafter\expandafter\expandafter0\expandafter\pgfmath@token\expandafter\pgfmath@token@next%
}
\def\pgfmath@parse@muexpr@{%
  \expandafter\endgroup%
  \expandafter\edef\expandafter\pgfmathresult\expandafter{\expandafter\pgfMATH@STRIPMU\the\muskip0}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

{
\catcode`\m=12
\catcode`\u=12
\gdef\pgfMATH@STRIPMU#1mu{#1}
}


% Parse a \numexpr
\def\pgfmath@parse@numexpr{%
  \afterassignment\pgfmath@parse@numexpr@%
  \expandafter\expandafter\expandafter\pgfmath@count\expandafter\pgfmath@token\pgfmath@token@next%
}
\def\pgfmath@parse@numexpr@#1{%
  \expandafter\def\expandafter\pgfmath@number\expandafter{\the\pgfmath@count}%
  \def\pgfmath@token@next{#1}%
  \expandafter\ifcat\pgfmath@token@next\relax%
    % A CS following a count register should be \wd, \ht or \dp.
    \let\pgfmath@parse@next=\pgfmath@parse@number%
  \else%
    \let\pgfmathresult=\pgfmath@number%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \fi%
  \pgfmath@parse@next%
}


% Parse the exponent of a number.
%
% REMARK: this method will be overwritten by the FPU library. Please
% keep changes consistent...
\def\pgfmath@parse@exponent{%
  \afterassignment\pgfmath@parse@@exponent%
  \pgfmath@count\pgfmath@token@next}
\def\pgfmath@parse@@exponent{%
  \pgfmathscientific{\pgfmath@number}{\the\pgfmath@count}%
  \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
  \pgfmath@parse@@operator%
}

% Parse binary or hexadecimal numbers (octal numbers done elsewhere).
%
\def\pgfmath@parse@base{%
  \ifnum\pgfmath@base=2\relax%
    \let\pgfmath@parse@next=\pgfmath@parse@binary%
  \else%
    \ifnum\pgfmath@base=16\relax%
      \let\pgfmath@parse@next=\pgfmath@parse@hexadecimal%
    \else%
      \pgfmath@error{Unexpected numerical base `\pgfmath@base'}{}%
      \def\pgfmathresult{0}%
      \let\pgfmath@parse@next=\pgfmath@parse@end%
    \fi%
  \fi%
  \let\pgfmath@number=\pgfmath@empty%
  \expandafter\pgfmath@parse@next\pgfmath@token@next%
}

\def\pgfmath@parse@binary#1{%
  \expandafter\ifx\csname pgfmath@token@binary@#1\endcsname\relax%
    \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{2}{10}%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \def\pgfmath@token@next{#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \else%
    \expandafter\def\expandafter\pgfmath@number\expandafter{\pgfmath@number#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@binary%
  \fi%
  \pgfmath@parse@next%
}

\def\pgfmath@parse@hexadecimal#1{%
  \expandafter\ifx\csname pgfmath@token@hexadecimal@#1\endcsname\relax%
    \expandafter\pgfmathbasetobase\expandafter\pgfmathresult\expandafter{\pgfmath@number}{16}{10}%
    \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
    \def\pgfmath@token@next{#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@operator%
  \else%
    \expandafter\def\expandafter\pgfmath@number\expandafter{\pgfmath@number#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@hexadecimal%
  \fi%
  \pgfmath@parse@next%
}

% Parse a function.
%
\def\pgfmath@parse@function{\pgfmath@parse@ifbgroup{\pgfmath@parse@function}{\pgfmath@parse@@function}}
\def\pgfmath@parse@function@{\futurelet\pgfmath@token@let\pgfmath@parse@@function}
\def\pgfmath@parse@@function{%
  \ifx\pgfmath@token@let\pgfmath@sptoken%
    \let\pgfmath@token=\pgfmath@empty%
    \let\pgfmath@parse@next=\pgfmath@parse@@@@function%
  \else%
    \let\pgfmath@parse@next=\pgfmath@parse@@@function%
  \fi%
  \pgfmath@parse@next}

\def\pgfmath@parse@@@function#1{%
  \expandafter\ifx\csname pgfmath@token@functional@\expandafter\string#1\endcsname\relax%
    \expandafter\ifx\csname pgfmath@token@number@\expandafter\string#1\endcsname\relax%
      \def\pgfmath@token{#1}% Not from A-Z, a-z, 0-9, or _.
      \let\pgfmath@parse@next=\pgfmath@parse@@@@function%
    \else% It is from 0-9.
      \expandafter\def\expandafter\pgfmath@function\expandafter{\pgfmath@function#1}%
      \let\pgfmath@parse@next=\pgfmath@parse@function@%
    \fi%
  \else% It is from  A-Z, a-z, or _.
    \edef\pgfmath@function{\pgfmath@function#1}%
    \let\pgfmath@parse@next=\pgfmath@parse@function@%
  \fi%
  \pgfmath@parse@next}

\def\pgfmath@parse@@@@function{%
  \expandafter\ifx\csname pgfmath@function@\pgfmath@function\endcsname\relax%
    \pgfmath@error{Unknown function `\pgfmath@function'}{}%
    \def\pgfmathresult{0}%
    \let\pgfmath@parse@next=\pgfmath@parse@end%
  \else%
    \expandafter\ifnum\csname pgfmath@operation@\pgfmath@function @arity\endcsname=0\relax%
     % Functions with zero arity are called directly.
      \csname pgfmath\pgfmath@function @\endcsname%
      \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operator%
    \else% Otherwise, they are pushed onto the operator stack
      \expandafter\pgfmath@stack@push@operation\expandafter{\pgfmath@function}%
      \let\pgfmath@parse@next=\pgfmath@parse@@operand%
    \fi%
  \fi%
  \expandafter\pgfmath@parse@next\pgfmath@token}

% Parse an operator.
%
\def\pgfmath@parse@operator{\pgfmath@parse@ifbgroup{\pgfmath@parse@operator}{\pgfmath@parse@operator@}}%
\def\pgfmath@parse@operator@#1{% Get one token.
  \let\pgfmath@token=\pgfmath@token@next%
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@@operator}

\def\pgfmath@parse@@operator{\pgfmath@parse@ifbgroup{\pgfmath@parse@@operator}{\pgfmath@parse@@operator@}}%
\def\pgfmath@parse@@operator@#1{% Get first token...
  \def\pgfmath@token{#1}%
  \pgfmath@parse@ifbgroup{\pgfmath@parse@@operator@@}{\pgfmath@parse@@operator@@}}%
\def\pgfmath@parse@@operator@@#1{% ...and second token.
  \def\pgfmath@token@next{#1}%
  \pgfmath@parse@@@operator}

\def\pgfmath@parse@@@operator{%
  \expandafter\ifx\csname pgfmath@operator@\pgfmath@token\expandafter\string\pgfmath@token@next\endcsname\relax%
    % Not a double character operator.
    \expandafter\ifx\csname pgfmath@operator@\pgfmath@token\endcsname\relax%
      % Not a single character operator.
      \pgfmath@error{Unknown operator `\pgfmath@token' or `\pgfmath@token\pgfmath@token@next'}{}%
      \def\pgfmathresult{0}%
    \let\pgfmath@parse@next=\pgfmath@parse@end%
    \else%
      \expandafter\pgfmath@operation@process\expandafter{\pgfmath@token}%
      \ifx\pgfmath@token\pgfmath@text@@%
        \let\pgfmath@parse@next=\pgfmath@parse@end%
      \else%
        \expandafter\ifx\csname pgfmath@operation@\pgfmath@token @postfix\endcsname\pgfmath@token%
          % Postfix operators are followed by an operator.
          \ifx\pgfmath@token@next\pgfmath@char@leftbracket% Except [.
            \let\pgfmath@parse@next=\pgfmath@parse@operand%
          \else%
            \let\pgfmath@parse@next=\pgfmath@parse@operator%
          \fi%
        \else%
          % Any other operator is followed by an operand.
          \let\pgfmath@parse@next=\pgfmath@parse@operand%
        \fi%
      \fi%
    \fi%
  \else%
    % A double character operator...
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
      \pgfmath@token\expandafter\expandafter\expandafter%
        {\expandafter\pgfmath@token\pgfmath@token@next}%
    \expandafter\pgfmath@operation@process\expandafter{\pgfmath@token}%
    % ...is always followed by an operand.
    \let\pgfmath@parse@next=\pgfmath@parse@@operand%
  \fi%
  \pgfmath@parse@next%
}


% Process an operation.
%
\def\pgfmath@operation@process#1{%
  \def\pgfmath@operator{#1}%
  \ifx\pgfmath@stack@operation@top\pgfmath@stack@empty%
  \else%
    \pgfmath@operation@@process%
  \fi%
  \expandafter\ifx\csname pgfmath@token@specials@#1\endcsname\relax%
    \pgfmath@stack@push@operation{#1}%
  \fi%
}

% Process the operation stack.
%
\def\pgfmath@operation@@process{%
  \ifx\pgfmath@stack@operation@top\pgfmath@stack@empty%
    \let\pgfmath@parse@next=\relax%
  \else%
    \ifnum\csname pgfmath@operation@\pgfmath@operator @precedence\endcsname>%
      \csname pgfmath@operation@\pgfmath@stack@operation@top @precedence\endcsname\relax%
      % If the precedence of the scanned operator is greater than the
      % precedence of the operator at the top of the stack, do nothing.
      \let\pgfmath@parse@next=\relax%
    \else%
      \let\pgfmath@stack@operation@last=\pgfmath@stack@operation@top%
      \expandafter\ifx\csname pgfmath@operator@\pgfmath@stack@operation@top\endcsname\relax%
        \pgfmath@function@@@process%
      \else%
        \pgfmath@operator@@@process%
      \fi%
      \expandafter\pgfmath@stack@push@operand\expandafter{\pgfmathresult}%
      \expandafter\ifx\csname pgfmath@token@group@\pgfmath@stack@operation@last\pgfmath@operator\endcsname\relax%
        \let\pgfmath@parse@next=\pgfmath@operation@@process%
      \else%
        \let\pgfmath@parse@next=\relax%
      \fi%
    \fi%
  \fi%
  \pgfmath@parse@next%
}

% Process an operator.
%
\def\pgfmath@operator@@@process{% Process an operator.
  \pgfmath@stack@pop@operation\pgfmath@@operator%
  \pgfmath@stack@pop@operand\pgfmath@operand@a%
  \ifcase\csname pgfmath@operation@\pgfmath@@operator @arity\endcsname\relax%
    % Zero arity operators (!).
  \or%
    \pgfmath@operator@@@@process{\pgfmath@operand@a}%
  \or%
    \pgfmath@stack@pop@operand\pgfmath@operand@b%
    \pgfmath@operator@@@@process{\pgfmath@operand@b}{\pgfmath@operand@a}%
  \or%
    \pgfmath@stack@pop@operand\pgfmath@operand@b%
    \expandafter\pgfmath@operator@@@@process\expandafter%
      {\expandafter\pgfmath@operand@b\expandafter}\pgfmath@operand@a%
  \else%
    % No operators with more than tenary arity.
  \fi%
}

\def\pgfmath@operator@@@@process{%
  \csname pgfmath%
    \csname pgfmath@operation@\pgfmath@@operator @name\endcsname%
  @\endcsname}

% Process a function.
%
\def\pgfmath@function@@@process{% Process a function.
  \ifnum\csname pgfmath@operation@\pgfmath@stack@operation@top @arity\endcsname>0\relax%
    \pgfmath@stack@pop@operation\pgfmath@@function%
    \pgfmath@stack@pop@operand\pgfmath@@operand%
    \ifnum\csname pgfmath@operation@\pgfmath@@function @arity\endcsname>1\relax%
      \ifnum\csname pgfmath@operation@\pgfmath@@function @arity\endcsname>9\relax%
        \csname pgfmath\pgfmath@@function @\endcsname{\pgfmath@@operand}%
      \else%
        \expandafter\pgfmath@function@@@@process\pgfmath@@operand%
      \fi
    \else%
      \expandafter\pgfmath@function@@@@process\expandafter{\pgfmath@@operand}%
    \fi%
  \fi%
}

\def\pgfmath@function@@@@process{\csname pgfmath\pgfmath@@function @\endcsname}

% Stack.
%
\newtoks\pgfmath@stack@operand
\newtoks\pgfmath@stack@operation
\let\pgfmath@stack@empty=\pgfmath@empty

\def\pgfmath@stack@push#1#2{%
  \def\pgfmath@stack@top{#2}%
  \expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
      {\expandafter\pgfmath@stack@top\expandafter}\the#1}}%

\def\pgfmath@stack@pop#1#2{\expandafter\pgfmath@stack@@pop\the#1\pgfmath@stack@stop{#1}{#2}}
\def\pgfmath@stack@@pop#1#2#3\pgfmath@stack@stop#4#5{\def#5{#1}#4={{#2}#3}\def\pgfmath@stack@top{#2}}

\def\pgfmath@stack@push@operation#1{%
  \pgfmath@stack@push\pgfmath@stack@operation{#1}%
  \let\pgfmath@stack@operation@top=\pgfmath@stack@top}

\def\pgfmath@stack@pop@operation#1{%
  \pgfmath@stack@pop\pgfmath@stack@operation{#1}%
  \let\pgfmath@stack@operation@top=\pgfmath@stack@top}

% REMARK: This method will be overwritten by the FPU library. Please
% keep any changes consistent.
\def\pgfmath@stack@push@operand#1{%
  \pgfmath@stack@push\pgfmath@stack@operand{#1}%
  \let\pgfmath@stack@operand@top=\pgfmath@stack@top}

\def\pgfmath@stack@pop@operand#1{%
  \pgfmath@stack@pop\pgfmath@stack@operand{#1}%
  \let\pgfmath@stack@operand@top=\pgfmath@stack@top}


% Declare an operator for the parser.
%
% It is not recommended that new operators be created as
% the parser is not fully robust for arbitrary operators.
%
\def\pgfmathdeclareoperator#1#2#3#4#5{%
  \ifx\pgfmath@operatorlist\pgfutil@empty
    \edef\pgfmath@operatorlist{{\string#1}}%
  \else
    \edef\pgfmath@operatorlist{\pgfmath@operatorlist,{\string#1}}%
  \fi
  \pgfmath@namedef{pgfmath@operator@\string#1}{#1}%
  \pgfmath@namedef{pgfmath@operation@\string#1@name}{#2}%
  \pgfmath@namedef{pgfmath@operation@\string#1@arity}{#3}%
  \pgfmath@namedef{pgfmath@operation@\string#1@#4}{#1}%
  \pgfmath@namedef{pgfmath@operation@\string#1@precedence}{#5}%
}

\def\pgfmath@operatorlist{}

\pgfmathdeclareoperator{+}{add}     {2}{infix}{500}
\pgfmathdeclareoperator{-}{subtract}{2}{infix}{500}
\pgfmathdeclareoperator{*}{multiply}{2}{infix}{700}
\pgfmathdeclareoperator{/}{divide}  {2}{infix}{700}
\pgfmathdeclareoperator{^}{pow}     {2}{infix}{900}

\pgfmathdeclareoperator{<} {}       {1}{prefix} {1}

\pgfmathdeclareoperator{>} {greater}   {2}{infix} {250}
\pgfmathdeclareoperator{<} {less}      {2}{infix} {250}
\pgfmathdeclareoperator{==}{equal}     {2}{infix} {250}
\pgfmathdeclareoperator{>=}{notless}   {2}{infix} {250}
\pgfmathdeclareoperator{<=}{notgreater}{2}{infix} {250}
\pgfmathdeclareoperator{&&}{and}       {2}{infix} {200}
\pgfmathdeclareoperator{||}{or}        {2}{infix} {200}
\pgfmathdeclareoperator{!=}{notequal}  {2}{infix} {250}
\pgfmathdeclareoperator{!} {not}       {1}{prefix}{975}
\pgfmathdeclareoperator{?} {ifthenelse}{3}{infix} {100}
\pgfmathdeclareoperator{:} {@@collect}  {2}{infix}{101}

\pgfmathdeclareoperator{!}{factorial}{1}{postfix}{800}% Must be defined after prefix ! operator.
\pgfmathdeclareoperator{r}{deg}      {1}{postfix}{600}

\pgfmathdeclareoperator{,}{@collect}   {2}{infix}  {10}
\pgfmathdeclareoperator{[}{@startindex}{2}{prefix} {7}
\pgfmathdeclareoperator{]}{@endindex}  {0}{postfix}{6}
\pgfmathdeclareoperator{(}{@startgroup}{1}{prefix} {5}
\pgfmathdeclareoperator{)}{@endgroup}  {0}{postfix}{4}

\pgfmathdeclareoperator{\pgfmath@bgroup}{@startarray}{1}{prefix} {3}
\pgfmathdeclareoperator{\pgfmath@egroup}{@endarray}  {1}{postfix}{2}%

% Special operators.
\pgfmathdeclareoperator{"}{}{1}{prefix}{1}
\pgfmathdeclareoperator{@}{}{0}{postfix}{0}

% Internal functions.

% Begin and end parenthesis ().
%
\def\pgfmath@startgroup@#1{\pgfmath@protected@edef\pgfmathresult{#1}}
\def\pgfmath@endgroup@{}% Never actually called.

% Begin and end array access [].
%
\def\pgfmath@startindex@#1#2{%
  \expandafter\pgfmatharray@#1{#2}%
  \expandafter\pgfmath@bgroup@strip\expandafter{\pgfmathresult}%
  \ifx\pgfmath@token@let\bgroup%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmathresult}}%
  \fi}
\def\pgfmath@endindex@{}% Never actually called.

% Begin and end array {}.
%
\def\pgfmath@startarray@#1{\expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{#1}}}
\def\pgfmath@endarray@#1{\expandafter\def\expandafter\pgfmathresult\expandafter{#1}}% Never actually called.


\def\pgfmath@@collect@#1#2{%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgfmathresult\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter%
      {\expandafter#1\expandafter}\expandafter{#2}}%
}
% Collect items separated by ,.
%
\def\pgfmath@collect@#1#2{%
  \expandafter\def\expandafter\pgfmath@collect@original\expandafter{#1}%
  \expandafter\pgfmath@bgroup@strip\expandafter{#1}%
  \ifx\pgfmath@token@let\bgroup%
    \ifx\pgfmath@collect@original\pgfmath@bgroup@stripped%
      \expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmath@bgroup@stripped}%
    \else%
      \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmath@bgroup@stripped}}%
    \fi%
  \else%
    \expandafter\def\expandafter\pgfmathresult\expandafter{\expandafter{\pgfmath@bgroup@stripped}}%
  \fi%
  \expandafter\pgfmath@bgroup@strip\expandafter{#2}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter%
    \pgfmathresult\expandafter\expandafter\expandafter%
      {\expandafter\pgfmathresult\expandafter{\pgfmath@bgroup@stripped}}%
}

% Strip braces from a token sequence.
%
\def\pgfmath@bgroup@strip#1{%
  \def\pgfmath@bgroup@strip@last{#1}%
  \pgfmath@bgroup@@strip{#1}\pgfmath@\pgfmath@@\pgfmath@@@}

\def\pgfmath@bgroup@strip@#1{%
  \def\pgfmath@bgroup@strip@last{#1}%
  \pgfmath@bgroup@@strip#1\pgfmath@\pgfmath@@\pgfmath@@@}

\def\pgfmath@bgroup@pgfmath@{\pgfmath@}

\def\pgfmath@bgroup@@strip{%
  \futurelet\pgfmath@token@let\pgfmath@bgroup@@@strip}

\def\pgfmath@bgroup@@@strip#1#2#3\pgfmath@@@{%
  \ifx\pgfmath@token@let\bgroup
    \def\pgfmath@bgroup@test{#2}%
    \ifx\pgfmath@bgroup@test\pgfmath@bgroup@pgfmath@
      \def\pgfmath@next{\pgfmath@bgroup@strip@{#1}}%
    \else
      \let\pgfmath@bgroup@stripped=\pgfmath@bgroup@strip@last
      \let\pgfmath@next=\relax
    \fi
  \else
    \pgfmath@bgroup@@@@strip#1#2#3%
    \let\pgfmath@next=\relax
  \fi
  \pgfmath@next}

\def\pgfmath@bgroup@@@@strip#1\pgfmath@\pgfmath@@{%
  \def\pgfmath@bgroup@stripped{#1}}

% Local Variables:
% tab-width: 2
% End:


==> pgfmathutil.code.tex <==
% Copyright 2019 Mark Wibrow
%
% but subject to the LaTeX Project Public License
% (http://www.latex-project.org/lppl.txt)
%
% and the GNU Public License
% (http://www.gnu.org/licenses/gpl.txt)
%

% This file defines utilities common to the \pgfmath files.
%
% Version 1.414213 29/9/2007

\def\pgfmathincluded{}

% Helper macros for \pgfmath@ifregister
%
\def\pgfmath@grabv#1#2#3#4#5#6#7\pgfmath@grabv{#2#3#4#5\ifx#6!!\fi}
\def\pgfmath@ifskip@extract#1{\expandafter\pgfmath@grabv\meaning#1!!!!!!\pgfmath@grabv}
\def\pgfmath@iftoks@extract#1{\expandafter\pgfmath@grabv\meaning#1!!!!!!\pgfmath@grabv}

\def\pgfmath@grabvi#1#2#3#4#5#6#7#8\pgfmath@grabvi{#2#3#4#5#6\ifx#7!!\fi}
\def\pgfmath@ifdimen@extract#1{\expandafter\pgfmath@grabvi\meaning#1!!!!!!\pgfmath@grabvi}
\def\pgfmath@ifcount@extract#1{\expandafter\pgfmath@grabvi\meaning#1!!!!!!\pgfmath@grabvi}

\def\pgfmath@grabvii#1#2#3#4#5#6#7#8#9\pgfmath@grabvii{#2#3#4#5#6#7\ifx#8!!\fi}
\def\pgfmath@ifmuskip@extract#1{\expandafter\pgfmath@grabvii\meaning#1!!!!!!\pgfmath@grabvii}

% \pgfmath@ifdimen@unguarded
%
% Check if #2 is a register of type #1.
% Credits to Frank: https://tex.stackexchange.com/a/56905
%
% #1 register type (count, dimen, skip, muskip, toks)
% #2 single token
%
\def\pgfmath@ifregister@unguarded#1#2{%
    \expandafter\ifx\csname\csname pgfmath@if#1@extract\endcsname{#2}\expandafter\endcsname\csname #1\endcsname
        \expandafter\pgfutil@firstoftwo
    \else
        \expandafter\pgfutil@secondoftwo
    \fi}

% \pgfmath@ifregister
%
% Checks if a token is a a certain type of register
%
% #1 register type (count, dimen, skip, muskip, toks)
% #2 single token
%
\def\pgfmath@ifregister#1#2{%
    \pgfutil@IfUndefined{pgfmath@if#1@extract}%
        {\errmessage{Package PGF Math Error: Cannot test for #1 register}}%
        {\pgfutil@IfUndefined{\csname pgfmath@if#1@extract\endcsname{#2}}%
            {\pgfutil@secondoftwo}}%
            {\pgfmath@ifregister@unguarded{#1}{#2}}}

% \pgfmath@ensureregister
%
% Ensure a control sequence exists as a TeX count/dimen register.
%
% #1 - count or dimen.
% #2 - a control sequence.
%
\def\pgfmath@ensureregister#1#2{%
    \pgfmath@ifregister{#1}{#2}%
        {}%
        {\csname new#1\endcsname#2}%
}

% Check registers exist. If not, create them.
%
\pgfmath@ensureregister{dimen}{\pgf@x}
\pgfmath@ensureregister{dimen}{\pgf@xa}
\pgfmath@ensureregister{dimen}{\pgf@xb}
\pgfmath@ensureregister{dimen}{\pgf@xc}

\pgfmath@ensureregister{dimen}{\pgf@y}
\pgfmath@ensureregister{dimen}{\pgf@ya}
\pgfmath@ensureregister{dimen}{\pgf@yb}
\pgfmath@ensureregister{dimen}{\pgf@yc}

\pgfmath@ensureregister{dimen}{\pgfutil@tempdima}
\pgfmath@ensureregister{dimen}{\pgfutil@tempdimb}

\pgfmath@ensureregister{count}{\c@pgf@counta}
\pgfmath@ensureregister{count}{\c@pgf@countb}
\pgfmath@ensureregister{count}{\c@pgf@countc}
\pgfmath@ensureregister{count}{\c@pgf@countd}

\pgfmath@ensureregister{count}{\pgfutil@tempcnta}
\pgfmath@ensureregister{count}{\pgfutil@tempcntb}

% Alias for \pgfmath.
%
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\pgfmath@tempdima\pgfutil@tempdima
\let\pgfmath@tempdimb\pgfutil@tempdimb

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc
\let\c@pgfmath@countd\c@pgf@countd

\let\pgfmath@tempcnta\pgfutil@tempcnta
\let\pgfmath@tempcntb\pgfutil@tempcntb

% Now check if pgfutil and pgf@sys stuff exists. If it does, fine.
% Just \let pgfmath versions. If not, define pgfmath versions (Arghhh).
%

% \...ifnextchar
%
\ifx\pgfutil@ifnextchar\pgfmath@undefined%
    \long\def\pgfmath@ifnextchar#1#2#3{%
  \let\pgfmath@reserved@d#1%
  \def\pgfmath@reserved@a{#2}%
  \def\pgfmath@reserved@b{#3}%
  \futurelet\pgfmath@let@token\pgfmath@ifnch}
    \def\pgfmath@ifnch{%
      \ifx\pgfmath@let@token\pgfmath@sptoken%
        \let\pgfmath@reserved@c\pgfmath@xifnch%
      \else%
        \ifx\pgfmath@let@token\pgfmath@reserved@d%
          \let\pgfmath@reserved@c\pgfmath@reserved@a%
        \else%
          \let\pgfmath@reserved@c\pgfmath@reserved@b%
        \fi%
      \fi%
      \pgfmath@reserved@c}
    {%
      \def\:{\global\let\pgfmath@sptoken= } \:
      \def\:{\pgfmath@xifnch} \expandafter\gdef\: {\futurelet\pgfmath@let@token\pgfmath@ifnch}
    }%
\else%
    \let\pgfmath@ifnextchar\pgfutil@ifnextchar%
    % Still need to define \pgfmath@sptoken (cannot \let).
    {%
        \def\:{\global\let\pgfmath@sptoken= } \:
    }%
\fi%

% \...ifundefined
%
\ifx\pgfutil@ifundefined\pgfmath@undefined%
    \long\def\pgfmath@ifundefined#1{%
      \expandafter\ifx\csname#1\endcsname\relax%
        \expandafter\pgfmath@firstoftwo%
      \else%
        \expandafter\pgfmath@secondoftwo%
      \fi}%
\else%
    \let\pgfmath@ifundefined\pgfutil@ifundefined%
\fi%

% \...selectfont
%
\ifx\pgfutil@selectfont\pgfmath@undefined%
    \ifx\selectfont\pgfmath@undefined%
        \let\pgfmath@selectfont\rm% Plain TeX and ConTeXt.
    \else%
        \let\pgfmath@selectfont\selectfont% LaTeX.
    \fi%
\else%
    \let\pgfmath@selectfont\pgfutil@selectfont%
\fi%

% New definition easier than fussing around with let.
%
\newif\ifpgfmath@in@
\def\pgfmath@in@#1#2{%
 \def\pgfmath@in@@##1#1##2##3\pgfmath@in@@{%
  \ifx\pgfmath@in@##2\pgfmath@in@false\else\pgfmath@in@true\fi}%
 \pgfmath@in@@#2#1\pgfmath@in@\pgfmath@in@@}


% \...tonumber
%
\ifx\pgf@sys@tonumber\pgfmath@undefined%
  {\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}
    \def\pgfmath@tonumber#1{\expandafter\Pgf@geT\the#1}
\else%
    \let\pgfmath@tonumber\pgf@sys@tonumber%
\fi%


% \PackageWarning and \PackageError
%
\ifx\PackageWarning\pgfmath@undefined
    \def\pgfmath@PackageWarning#1#2{\immediate\write-1{Package #1: Warning! #2.}}%
\else%
    \let\pgfmath@PackageWarning\PackageWarning%
\fi%
\ifx\PackageError\pgfmath@undefined
    \def\pgfmath@PackageError#1#2#3{\errmessage{Package #1 Error: #2.}}%
\else%
    \let\pgfmath@PackageError\PackageError%
\fi%

\def\pgfmath@error#1#2{%
    \pgfmath@PackageError{PGF Math}{%
        #1%
        \pgfutil@ifundefined{pgfmath@expression}{}{ (in '\pgfmath@expression')}%
    }{#2}%
}
\def\pgfmath@warning#1{%
    \pgfmath@PackageWarning{PGF Math}{%
        #1%
        \pgfutil@ifundefined{pgfmath@expression}{}{ (in '\pgfmath@expression')}%
    }%
}

% \pgfmath@pt
%
% Needed to test for 'pt' resulting from expansion using \the.
%
{\catcode`\p=12\catcode`\t=12\gdef\PgfmaTh@PT{pt}}
\edef\pgfmath@pt{\PgfmaTh@PT}%

% \pgfmath@empty
%
% A handy macro.
%
\def\pgfmath@empty{}

\def\pgfmath@firstoftwo#1#2{#1}
\def\pgfmath@secondoftwo#1#2{#2}

% \pgfmath@gobbletilpgfmath@
%
% Gobble stream until \pgfmath@ {which is undefined}.
%
\def\pgfmath@gobbletilpgfmath@#1\pgfmath@{}
\def\pgfmath@gobbleone#1{}%


\def\pgfmath@namedef#1{\expandafter\def\csname#1\endcsname}
\def\pgfmath@nameedef#1{\expandafter\edef\csname#1\endcsname}

% \pgfmathloop
%
% A version of the standard TeX and LaTeX
% \loop, with an additional macro \pgfmathcounter
% (which is *not* a TeX counter) which keeps
% track of the iterations.
%
\newif\ifpgfmathcontinueloop
\def\pgfmathloop#1\repeatpgfmathloop{%
    \def\pgfmathcounter{1}%
    \def\pgfmath@iterate{%
        #1\relax%
        {% Do this inside a group, just in case...
            \c@pgfmath@counta\pgfmathcounter%
            \advance\c@pgfmath@counta1\relax%
            \xdef\pgfmathloop@temp{\the\c@pgfmath@counta}%
        }%
        \edef\pgfmathcounter{\pgfmathloop@temp}%
        \expandafter\pgfmath@iterate\fi}%
    \pgfmath@iterate\let\pgfmath@iterate\relax}
\let\repeatpgfmathloop\fi
\def\pgfmathbreakloop{\let\pgfmath@iterate\relax}%

% \pgfmath@returnone
%
% #1 - a dimension representing a number or dimension.
%
% Changed by TT: made faster and simpler since it is used
% *heavily*. #1 must be something that can be assigned to a
% dimension.
%
\def\pgfmath@returnone#1\endgroup{%
  \pgfmath@x#1%
  \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
  \expandafter\endgroup\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmath@temp}%
}

\let\pgfmathreturn=\pgfmath@returnone

% \pgfmath@smuggleone
%
% Smuggle a macro outside a group.
%
% Changed by TT: Speedup by insisting, that smuggleone is directly
% followed by \endgroup
%
\def\pgfmath@smuggleone#1\endgroup{%
  \expandafter\endgroup\expandafter\def\expandafter#1\expandafter{#1}}

\let\pgfmathsmuggle=\pgfmath@smuggleone


==> pgfmodulematrix.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmodulematrix.code.tex}

\usepgfmodule{shapes}%

\newif\ifpgfmatrix
\newif\ifpgf@matrix@correct@call

\newif\ifpgf@matrix@fixed

\newcount\pgfmatrixcurrentrow

\newcount\pgfmatrixcurrentcolumn
\newcount\pgf@matrix@numberofcolumns

\let\pgf@matrix@cell=\pgfnodeparttextbox % alias
\let\pgf@matrix@box=\pgf@matrix@cell % alias

\long\def\pgfmatrixbeforeassemblenode#1{%
  \long\def\pgf@matrix@before@assemnble@node{#1}}
\pgfmatrixbeforeassemblenode{}

% Sets the default row or column sep
%
% #1 = default row or column sep list
%
% Description:
%
% Sets the macro \pgfmatrixrowsep or \pgfmatrixcolumnsep to #1.
%
% Example:
%
% \pgfsetmatrixrowsep{5pt}

\def\pgfsetmatrixrowsep#1{\def\pgfmatrixrowsep{#1}}%
\def\pgfsetmatrixcolumnsep#1{\def\pgfmatrixcolumnsep{#1}}%

\def\pgfmatrixrowsep{0pt}%
\def\pgfmatrixcolumnsep{0pt}%



% The pgfmatrix command creates a node that contains a matrix. Like
% the \pgfnode command, it is to be used inside a pgfpicture
% environment.
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
% #5 = inner shift
% #6 = startup code
% #7 = the matrix code (may contain verbatim stuff)
%
% Description:
%
% This command creates a node that contains a matrix. For
% each cell of the matrix, drawing commands may be given. These
% commands will create a cell picture and a bounding box is computed
% for each cell picture. The cell picture is then placed inside the
% cell. The position inside the cell is computed according to the
% following rules:
%
% 1. In each column, the origins of the cell pictures are all on a
%    vertical line.
% 2. In each row, the origins of the cell pictures are all on a
%    horizontal line.
% 3. All cells in the same row have the same height and depth.
% 4. All cells in the same column have the same width.
% 5. The size of cells are chosen minimal such that the boxes fit into
%    the cells and still meet the above requirement.
%
% Next, the whole resulting matrix, which is given as #7, is placed
% inside a node whose name is given as #3, whose shape is #1, and
% whose anchor is #2. This means that the resulting node is shifted
% such that the given anchor lies at the origin. Then, as for a normal
% node, the #4 path usage command is used for the node.
%
% The parameter #5 is an additional negative shift for the node. Normally, such
% a shift could be given beforehand (that is, the shift could be
% preapplied to the current transformation matrix). However, when #5
% is evaluated, you can refer to temporary positions of nodes inside
% the matrix. In detail, the following happens: When the matrix has
% been typeset, all nodes in the matrix temporarily get assigned their
% positions in the matrix box. The origin of this coordinate system is
% at the left baseline end of the matrix box, which corresponds to the
% text anchor. The position #5 is then interpreted inside this
% coordinate system and then used for shifting.
%
% The idea behind using the parameter #5 is the following: If you
% specify "text" as anchor #2 and specify \pgfpointanchor{inner
% node}{some anchor} for parameter #5, where inner node is a node that
% is created in the matrix, then the whole matrix will be shifted such
% that inner node.some anchor lies at the origin of the whole picture.
%
% At the beginning and at the end of each cell, the macros
% \pgfmatrixbegincode and \pgfmatrixendcode are called. Inside these
% macros you can use \pgfmatrixcurrentcolumn and \pgfmatrixcurrentrow
% to access the current row and column.
%
% Before each column except for the first, an extra space given by the
% macro \pgfmatrixcolumnsep is added. Additionally, an extra space
% given by the optional argument of the \pgfmatrixnextcell commands in
% the first line are added, which may vary between columns. Between
% rows, an extra space given by the macro \pgfmatrixrowsep is
% added. You can also change this value for each row by using a \gdef.
%
%
% Lines are ended using the command \pgfmatrixendrow. The command \\
% is \let to be the same, but \\ is sometimes overridden by, say,
% minipage, so it's good to have \pgfmatrixendrow as a "fallback".
%
% Inside the matrix, \\ must be used to end every line ***including
% the last***. You can pass an optional parameter to \\ as in \\[2pt]
% to give an additional space after this particular line.
%
% The usage of \\ at the end of the matrix is important since this
% command is used to find the end of the matrix. What happens is that
% \\ followed by a closing brace ends the matrix.
%
% Inside the matrix, you must use \pgfmatrixnextcell to separate
% columns. The reason is that two columns are used internally for
% every single column shown. The macro \pgfmatrixnextcell is yields
% (more or less) two && (and some further trickery).
%
% The parameter #6 is executed at the beginning of the matrix
% group. It is inside the protecting group of the matrix, but outside
% the matrix itself. It can be used for different purposes: 1) It can be
% used to simplify the next cell macro. 2) It can be used to issue an
% \aftergroup command. 3) It can be used to setup local settings. For
% example, by setting #6 to \let\&=\pgfmatrixnextcell you can use \&
% instead of \pgfmatrixnextcell. You can also set the catcode of & to
% active.
%
%
% Example:
%
% \begin{tikzpicture}
%
%   \draw (0,0) circle (1mm);  % b.north will lie on the center of this circle
%
%   \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{\let\&=\pgfmatrixnextcell}
%   {
%     \draw (0,0) circle (1cm); \& \node (a) [draw] {Hallo}; \\
%     \node (b) [draw] {Welt};  \& \draw (0,0) circle (5mm); \\
%   }
%
%   \draw [->] (a) -- (b);
%
% \end{tikzpicture}

\def\pgfmatrix#1#2#3#4#5#6{%
  \ifpgfmatrix%
    \pgferror{You cannot nest pgfmatrix environments, yet}
  \fi%
  \bgroup%
    \everycr{}%
    #6%
    \def\pgf@matrix@par@shape{#1}%
    \def\pgf@matrix@par@anchor{#2}%
    \def\pgf@matrix@par@name{#3}%
    \def\pgf@matrix@par@usage{#4}%
    \def\pgf@matrix@par@shift{#5}%
    % the matrix must have a name:
    \ifx\pgf@matrix@par@name\pgfutil@empty%
      \def\pgf@matrix@par@name{pgf@matrix@internal}%
    \fi%
    \pgfmatrixcurrentrow=0\relax%
    \pgfmatrixcurrentcolumn=0\relax%
    \pgf@matrix@numberofcolumns=0\relax%
    \let\\=\pgfmatrixendrow%
    \tabskip=0pt%
    \offinterlineskip%
    \pgfmatrixtrue%
    \let\pgf@matrix@node@list=\pgfutil@empty%
    \expandafter\let\csname pgf@matrix@column@finish@1\endcsname=\pgfutil@empty%
    \let\pgf@matrix@row@finish=\pgfutil@empty%
    %
    % Get rid of bgroup
    %
    \afterassignment\pgf@matrix@cont\let\pgf@next=%
}%
\def\pgf@matrix@cont{%
    \setbox\pgf@matrix@box=\hbox\bgroup\vbox\bgroup%
    \halign\bgroup%
    \pgf@matrix@init@row%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }%
    &%
    ##\pgf@matrix@padding&&%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }&%
    ##\pgf@matrix@padding%
    \cr%
}%

\def\pgf@end@matrix{%
      \egroup\egroup%
    \egroup%
    %
    % Inject custom tokens before assembling the node holding the matrix.  Can
    % be used to apply additional settings.
    %
    \pgf@matrix@before@assemnble@node
    %
    % If there are named nodes, we must adjust their coordinates.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      % Ok, this means we got a lot of work to do...
      \pgf@matrix@compute@origin%
      \pgf@matrix@shift@nodes@initial%
    \fi%
    %
    % Compute additional shift
    %
    \pgftransformresetnontranslations%
    \pgftransformshift{\pgf@process{\pgftransformreset\pgf@matrix@par@shift\pgf@x=-\pgf@x\pgf@y=-\pgf@y}}%
    %
    % Create node
    %
    \pgfmultipartnode{\pgf@matrix@par@shape}{\pgf@matrix@par@anchor}{\pgf@matrix@par@name}{\pgf@matrix@par@usage}%
    %
    % If there are named nodes, we must adjust their coordinates, again.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      {%
        \pgftransformreset%
        \pgf@process{\pgfpointanchor{\pgf@matrix@par@name}{text}}%
        \xdef\pgf@matrix@offset{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \pgf@matrix@shift@nodes@secondary{\pgf@matrix@offset}%
      }%
    \fi%
}%




% Ending a cell
%
% #1 = (optional) spacing between previous and next column. This
%      parameter only has an effect in the first row.
%
% Description:
%
% This command ends a cell of a matrix.
%
% Example:
%
% \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{}
% {
%   \draw (0,0) circle (1cm); \pgfmatrixnextcell[1cm] \node (a) [draw] {Hallo}; \\
%   \node (b) [draw] {Welt};  \pgfmatrixnextcell \draw (0,0) circle (5mm); \\
% }

\def\pgfmatrixnextcell{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  \pgfutil@ifnextchar[{\pgf@matrix@cell@cont}{\pgf@matrix@cell@cont[0pt]}}%}%

\def\pgf@matrix@cell@cont[#1]{%
  \xdef\pgf@matrix@last@nextcell@options{#1}%
  &\pgf@matrix@correct@calltrue&%
}%


\def\pgf@matrix@fixed@text{between origins}%
\def\pgf@matrix@natural@text{between borders}%

\def\pgf@matrix@addtolength#1#2{\edef\pgf@temp{#2}\expandafter\pgf@matrix@addtolength@\expandafter#1#2,\pgf@stop}%
\def\pgf@matrix@addtolength@#1#2,#3\pgf@stop{%
  \def\pgf@temp{#2}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \ifx\pgf@temp\pgf@matrix@fixed@text%
      \global\pgf@matrix@fixedtrue%
    \else%
      \ifx\pgf@temp\pgf@matrix@natural@text%
        \global\pgf@matrix@fixedfalse%
      \else%
        \pgfmathaddtolength{#1}{#2}%
      \fi%
    \fi%
  \fi%
  \def\pgf@temp{#3}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgf@matrix@addtolength@#1#3\pgf@stop%
  \fi%
}%



% Init a line

\def\pgf@matrix@init@row{%
  \relax%
  \global\advance\pgfmatrixcurrentrow by 1\relax%
  \global\pgfmatrixcurrentcolumn=0\relax%
  \expandafter\gdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{0pt}%
  \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
}%



% Step the row column number

\def\pgf@matrix@step@column{%
  \relax%
  \global\advance\pgfmatrixcurrentcolumn by1\relax%
}%



% Start a cell

\def\pgf@matrix@startcell{%
  %
  % Step 1: Init the list of nodes for this cell
  %
  \let\pgf@nodecallback=\pgf@matrix@nodecallback%
  %
  % Step 2: Setup the bounding box
  %
  \pgfinterruptboundingbox%
  %
  % Step 3: Reset the transformation matrix
  %
  \pgftransformreset%
  %
  % Step 4: Collect everything in a cell box
  %
  \setbox\pgf@matrix@cell=\hbox\bgroup\bgroup%
    % make sure that cell pictures are not affected if matrices have
    % 'overlay' option on:
    \pgf@relevantforpicturesizetrue
    \pgfsys@beginpicture%
    \normalbaselines%
    % Find out whether the cell is empty:
    \pgfutil@ifnextchar\let%
    {% ok, candidate, check following symbol
      \afterassignment\pgf@matrix@empty@check\let\pgf@matrix@temp=% get rid of \let
    }%
    {% no, not empty
      \pgf@matrix@empty@cell@false%
      \pgfmatrixbegincode%
    }%
}%

\def\pgf@matrix@empty@check{\futurelet\pgf@matrix@check@token\pgf@matrix@empty@check@cont}%
\def\pgf@matrix@empty@check@cont{%
  \ifx\pgf@matrix@check@token\pgf@matrix@signal@cell@end%
    \pgf@matrix@empty@cell@true%
    \expandafter%
    \pgfmatrixemptycode%
    \expandafter%
    \let% reinserted
  \else%
    \pgf@matrix@empty@cell@false%
    \expandafter%
    \pgfmatrixbegincode%
    \expandafter
    \let% reinserted
  \fi%
}%

\newif\ifpgf@matrix@empty@cell@


% End a  cell

\def\pgf@matrix@endcell{%
    \ifpgf@matrix@empty@cell@%
    \else%
      \expandafter\expandafter\expandafter\pgfmatrixendcode%
      \expandafter\ifpgf@matrix@last@cell@in@row\expandafter\pgf@matrix@last@cell@in@rowtrue\expandafter\fi%
    \fi%
    \pgfsys@endpicture%
    \ifnum\pgfmatrixcurrentcolumn<\pgf@matrix@numberofcolumns%
    \else%
    \ifpgf@matrix@last@cell@in@row\else%
    {%
      \global\pgf@matrix@fixedfalse%
      \pgf@x=0pt%
      \pgf@matrix@addtolength{\pgf@x}{\pgfmatrixcolumnsep}%
      \pgf@matrix@addtolength{\pgf@x}{\pgf@matrix@last@nextcell@options}%
      \ifpgf@matrix@fixed%
        \expandafter\pgfutil@g@addto@macro\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
          {\global\pgf@picmaxx=0pt}%
      \fi%
      \advance\pgfmatrixcurrentcolumn by1\relax % only temporary for the following:
      \expandafter\xdef\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@x}%
      \ifpgf@matrix@fixed%
        \expandafter\gdef\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname{\global\pgf@picminx=0pt}%
      \else%
        \expandafter\global\expandafter\let\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname=\pgfutil@empty%
      \fi%
    }%
    \fi\fi%
    % Special case of the empty picture
    \ifdim\pgf@picmaxx=-16000pt\relax%
      \global\pgf@picmaxx=0pt\relax%
      \global\pgf@picminx=0pt\relax%
      \global\pgf@picmaxy=0pt\relax%
      \global\pgf@picminy=0pt\relax%
    \fi%
    \csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
    \pgf@matrix@row@finish%
  \egroup\egroup%
  %
  % Step 5: Horizontal gap
  %
  \ifnum\pgfmatrixcurrentcolumn>1\relax%
    \pgf@y=\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname\relax%
    \advance\pgf@picminx by-\pgf@y%
  \fi%
  %
  % Step 6: Protocol and adjust height and depth
  %
  % Step 6.1: Protocol...
  %
  \ifdim\pgf@picmaxy>\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picmaxy}%
  \fi%
  \ifdim\pgf@picminy<\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picminy}%
  \fi%
  %
  % Step 6.2: and setup.
  %
  \ht\pgf@matrix@cell=\pgf@picmaxy%
  \dp\pgf@matrix@cell=-\pgf@picminy%
  %
  % Step 7: Protocol and adjust left and right width
  %
  % Step 7.1: Protocol...
  %
  \ifnum\pgfmatrixcurrentcolumn>\pgf@matrix@numberofcolumns\relax%
    \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \global\pgf@matrix@numberofcolumns=\pgfmatrixcurrentcolumn\relax%
  \else%
    \ifdim\pgf@picmaxx>\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \fi%
    \ifdim\pgf@picminx<\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \fi%
  \fi%
  %
  % Step 7.2: and setup.
  %
  \xdef\pgf@matrix@paddingskip{\the\pgf@picmaxx}%
  %
  % Step 8: Put in the box now
  %
  \hfil\hskip-\pgf@picminx%
  \wd\pgf@matrix@cell=0pt%
  \box\pgf@matrix@cell%
  %
  % Step 9: End bounding box
  \endpgfinterruptboundingbox%
}%

% Default code for the start and end code
\let\pgfmatrixbegincode=\relax
\let\pgfmatrixendcode=\relax
\let\pgfmatrixemptycode=\relax


% The following callback is called for every node that is produced
% inside a cell

\def\pgf@matrix@nodecallback#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \xdef\pgf@matrix@node@list{\pgf@matrix@node@list,{#1}}%
    \expandafter\xdef\csname pgf@matrix@node@location@#1\endcsname{{\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  \fi%
}%



% Padding code

\def\pgf@matrix@padding{%
  \ifpgf@matrix@correct@call%
  \else%
    \pgferror{Single ampersand used with wrong catcode}%
  \fi%
  \hskip\pgf@matrix@paddingskip\hfil%
}%


% Compute the real positions of the origins

% We must now compute the real positions of the origins of all the
% small pictures. To this end, we need to compute prefix sums. After
% the procedure is done, the minx and the maxy will contain the origin
% positions.

\def\pgf@matrix@compute@origin{%
  %
  % Inverse prefix sum on the vertical positions
  %
  {%
    \ifnum\pgfmatrixcurrentrow>0\relax%
      \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
    \fi
    \c@pgf@counta=\pgfmatrixcurrentrow\relax%
    \loop%
    \ifnum\c@pgf@counta>1\relax%
      \pgf@y=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by\csname pgf@matrix@maxy\the\c@pgf@counta\endcsname\relax
      \advance\c@pgf@counta by-1\relax%
      \pgf@ya=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by-\pgf@ya\relax%
      \expandafter\xdef\csname pgf@matrix@miny\the\c@pgf@counta\endcsname{\the\pgf@y}%
    \repeat%
  }%
  %
  % Prefix sum on the horizontal positions
  %
  {%
    \ifnum\pgf@matrix@numberofcolumns>0\relax%
      \pgf@x=\csname pgf@matrix@minx1\endcsname\relax%
      \pgf@x=-\pgf@x%
      \expandafter\xdef\csname pgf@matrix@minx1\endcsname{\the\pgf@x}%
    \fi
    \c@pgf@counta=1\relax%
    \loop%
    \ifnum\c@pgf@counta<\pgf@matrix@numberofcolumns\relax%
      \pgf@x=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by\csname pgf@matrix@maxx\the\c@pgf@counta\endcsname\relax%
      \advance\c@pgf@counta by1\relax%
      \pgf@xa=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by-\pgf@xa\relax%
      \expandafter\xdef\csname pgf@matrix@minx\the\c@pgf@counta\endcsname{\the\pgf@x}%
    \repeat%
  }%
}%


% Shift the nodes to their origins

% The following procedure shifts all nodes in
% \pgf@matrix@node@list to their location inside a temporary
% picture. This picture will later be shifted again to its final
% position in the real picture.

\def\pgf@matrix@shift@nodes@initial{%
  {%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{%
          \pgf@x=\csname pgf@matrix@minx%
            \expandafter\expandafter\expandafter\pgfutil@secondoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          \pgf@y=\csname pgf@matrix@miny%
            \expandafter\expandafter\expandafter\pgfutil@firstoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          }%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
  }%
}%


% The second shifting, done in the following procedure, shifts all
% nodes to their real positions inside the real picture.

\def\pgf@matrix@shift@nodes@secondary#1{%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{#1}%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
}%


% End of line
\def\pgfmatrixendrow{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end
  \pgf@matrix@last@cell@in@rowtrue%
  \xdef\pgf@matrix@rowsep{\pgfmatrixrowsep}%
  &\pgf@matrix@correct@calltrue%
  \global\pgf@matrix@fixedfalse%
  \pgf@y=0pt%
  \pgf@matrix@addtolength\pgf@y{\pgf@matrix@rowsep}%
  \pgfutil@ifnextchar[{\pgfmatrixendrow@skip}{\pgf@matrix@finish@line}%
}%
\newif\ifpgf@matrix@last@cell@in@row

\def\pgf@matrix@signal@cell@end{\pgf@matrix@signal@cell@end}%
% exact definition does not matter, only needs to be unique.

\def\pgfmatrixendrow@skip[#1]{%
  \pgf@matrix@addtolength\pgf@y{#1}%
  \pgf@matrix@finish@line%
}%

\def\pgf@matrix@finish@line{%
  \global\pgf@y=\pgf@y%
  \pgf@ya=-\pgf@y%
  \global\advance\pgf@ya by\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
  \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@ya}%
  \pgfutil@ifnextchar\egroup{\cr\pgf@end@matrix}{\pgf@matrix@no@eom@found}%
}%

\def\pgf@matrix@eom@found{%
  \cr%
  \pgf@end@matrix%
}%

\def\pgf@matrix@no@eom@found{%
  \cr%
  \noalign{\vskip\pgf@y%
  \ifpgf@matrix@fixed%
    \vskip\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname% unskip
    \vskip\pgf@y%
    \pgf@y=-\pgf@y%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
    \gdef\pgf@matrix@row@finish{\global\pgf@picmaxy=0pt}%
  \else%
    \global\let\pgf@matrix@row@finish=\pgfutil@empty%
  \fi%
  }%
}%


\endinput


==> pgfmoduleplot.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmoduleplot.code.tex}


% PGF's plotting interface works as follows:
%
% In order to plot something, two things need to be done. First, you
% need to provide the coordinates (obviously) of the points that
% should be plotted. The coordinates are given via a long stream of
% commands. These commands are \pgfplotstreamstart, which is
% given exactly once at the beginning, the commands
% \pgfplotstreampoint, \pgfplotstreampointoutlier,
% \pgfplotstreampointundefined, \pgfplotstreamnewdataset, of which
% there are numerous in the middle, the special \pgfplotstreamspecial,
% of which there may be numerous in the middle, and \pgfplotstreamend,
% which must be given at the end. Between these commands arbitrary
% other commands may be given. Here is an example:
%
% ...
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreamnewdataset
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampointoutlier{\pgfpointxy{3}{9}}
% \pgfplotstreamspecial{some handler-dependent special stuff}
% \pgfplotstreamend
%
% By themselves, the \pgfplotstreamxxxx commands do not do anything by
% default. Rather, to ``use'' such a stream, you must first install a
% stream handler. For example, the ``lineto'' handler will simply
% basically every \pgfplotstreampoint into a \pgfpathlineto.
%
% One special things is the handling of "jumps" in a stream. For
% instance, when a lineto handler encounters an "outlier" or a new
% data set, the current line should end and a new subpath should start
% (unless configured otherwise). For this, the special jump handler is
% important.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
%
% \pgfplothandlerlineto
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamend


% The stream commands actually call their ``internal'' versions, which
% are set by the handlers:
\def\pgfplotstreamstart{\pgf@plotstreamstart}%
\def\pgfplotstreampoint#1{\gdef\pgfplotlastpoint{#1}\pgf@plotstreampoint{#1}}%
\def\pgfplotstreampointoutlier#1{\pgfplot@outliers{}{\pgf@plotstreamjump}{\pgfplotstreampoint{#1}}}%
\def\pgfplotstreampointundefined{\pgfplot@outliers{}{\pgf@plotstreamjump}{}}%
\def\pgfplotstreamnewdataset{\pgfplot@outliers{}{\pgf@plotstreamjump}{}}%
\def\pgfplotstreamspecial{\pgf@plotstreamspecial}%
\def\pgfplotstreamend{\pgf@plotstreamend}%

\def\pgfplot@ignorer#1#2#3{#1}%
\def\pgfplot@jumper#1#2#3{#2}%
\def\pgfplot@plotter#1#2#3{#3}%

\let\pgfplot@outliers\pgfplot@jumper
\let\pgfplot@undefined\pgfplot@jumper
\let\pgfplot@newdata\pgfplot@jumper

\pgfset{
  handle outlier points in plots/.is choice,
  handle outlier points in plots/ignore/.code=\let\pgfplot@outliers\pgfplot@ignorer,
  handle outlier points in plots/jump/.code=\let\pgfplot@outliers\pgfplot@jumper,
  handle outlier points in plots/plot/.code=\let\pgfplot@outliers\pgfplot@plotter,
  handle undefined points in plots/.is choice,
  handle undefined points in plots/ignore/.code=\let\pgfplot@undefined\pgfplot@ignorer,
  handle undefined points in plots/jump/.code=\let\pgfplot@undefined\pgfplot@jumper,
  handle new data sets in plots/.is choice,
  handle new data sets in plots/ignore/.code=\let\pgfplot@newdata\pgfplot@ignorer,
  handle new data sets in plots/jump/.code=\let\pgfplot@newdata\pgfplot@jumper,
}%


% Declares a new plot handler
%
% #1 = macro that should install the stream handler subsequently
% #2 = parameter list of said macro.
% #3 = keys as described below
%
% Description:
%
% When you declare a new plot handler, you provide, through keys,
% different "actions" that should be taken when the different stream
% commands are used:
%
% start       = some code to be executed when \pgfplotstreamstart is called
%               for this plothandler
% end         = same for the end of the stream
% point       = code to be executed for a point of the stream
% jump        = code to be executed for a "jump" in the stream
% special     = code to be executed for \pgfplotstreamspecial
% start macro   = here and for the following keys, the to-be-executed
%                 code is stored in the given macro
% end macro     = see above
% jump macro    = see above
% point macro   = see above
% special macro = see above
%
% Example:
%
% \pgfdeclareplothandler{\ultrasimplehandler}{}{
%   point=\pgfpathlineto{##1}
% }

\def\pgfdeclareplothandler#1#2#3{%
  \def#1#2{%
    \pgfkeys{%
      /pgf/plots/@handler options/.cd,
      start=\relax,
      end macro=\relax,
      point macro=\pgfutil@gobble,
      jump macro=\relax,
      special macro=\pgfutil@gobble,%
      #3%
    }%
  }%
}%

\pgfkeys{%
  /pgf/plots/@handler options/.cd,
  start/.code=%
    \gdef\pgf@plotstreamstart{%
      \global\pgf@plot@startedfalse%
      \global\let\pgf@plotstreamend\pgf@plotstreamend@init%
      \global\let\pgf@plotstreampoint\pgf@plotstreampoint@init%
      \global\let\pgf@plotstreamjump\pgf@plotstreamjump@init%
      \global\let\pgf@plotstreamspecial\pgf@plotstreamspecial@init%
      #1%
    },%
  start macro/.code=%
    \gdef\pgf@plotstreamstart{%
      \global\pgf@plot@startedfalse%
      \global\let\pgf@plotstreamend\pgf@plotstreamend@init%
      \global\let\pgf@plotstreampoint\pgf@plotstreampoint@init%
      \global\let\pgf@plotstreamjump\pgf@plotstreamjump@init%
      \global\let\pgf@plotstreamspecial\pgf@plotstreamspecial@init%
      #1%
    },%
  end/.code=\gdef\pgf@plotstreamend@init{#1},
  end macro/.code=\global\let\pgf@plotstreamend@init#1,
  point/.code=\gdef\pgf@plotstreampoint@init##1{#1},
  point macro/.code=\global\let\pgf@plotstreampoint@init#1,
  jump/.code=\gdef\pgf@plotstreamjump@init{#1},
  jump macro/.code=\global\let\pgf@plotstreamjump@init#1,
  special/.code=\gdef\pgf@plotstreamspecial@init##1{#1},
  special macro/.code=\global\let\pgf@plotstreamspecial@init#1,
}%

\newif\ifpgf@plot@started




% Sets the action taken for the first point of a plot to a lineto.
%
% Description:
%
% For certain handlers it makes sense either the start a plot by
% moving to the first point of the plot or to do a lineto to that
% first point. Using this command this action can be set to a lineto.
%
% Example:
%
% \pgfsetlinetofirstplotpoint

\def\pgfsetlinetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathlineto}%


% Sets the action taken for the first point of a plot to a moveto.
%
% Example:
%
% \pgfsetmovetofirstplotpoint

\def\pgfsetmovetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathmoveto}%

\let\pgf@plot@first@action=\pgfpathmoveto




%
% Handlers
%


% This handler converts each plot stream command into a lineto
% command, except for the first, which is converted to the action that
% has previously been specified using \pgfsetlinetofirstplotpoint or
% \pgfsetmovetofirstplotpoint.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerlineto}{}{
  point macro=\pgf@plot@line@handler,
  jump=\global\let\pgf@plotstreampoint\pgf@plot@line@handler@move%
}%

\def\pgf@plot@line@handler#1{%
  \pgf@plot@first@action{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%

\def\pgf@plot@line@handler@move#1{%
  \pgfpathmoveto{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%



% This handler turns creates a series of lineto commands, with the
% last command being a closepath, resulting in a closed path. If a
% jump is encountered, the current subpath is closed and a new subpath
% is started.
%
% Example:
%
% \pgfplothandlerpolygon
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerpolygon}{}{%
  point macro=\pgf@plot@line@handler@close,
  jump macro=\pgf@plot@next@close@and@moveto,
  end macro=\pgf@plot@polygon@stop
}%

\def\pgf@plot@line@handler@close#1{%
  \pgfpathmoveto{#1}%
  \global\pgf@plot@startedtrue%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}%

\def\pgf@plot@polygon@stop{%
  \ifpgf@plot@started%
    \pgfpathclose%
  \fi%
  \global\pgf@plot@startedfalse%
}%

\def\pgf@plot@next@close@and@moveto{%
  \ifpgf@plot@started%
    \pgfpathclose%
  \fi%
  \global\let\pgf@plotstreampoint\pgf@plot@line@handler@close%
}%


% More handlers are defined in pgflibraryplothandlers





% This handler discards the plot.
%
% Example:
%
% \pgfplothandlerdiscard
% \pgfplotxyfile{mytable}

\pgfdeclareplothandler{\pgfplothandlerdiscard}{}{}%



% This handler records each plot stream command to a macro. This is
% useful if plot commands are difficult to generate and need to be
% ``recycled'' later on.
%
% Example:
%
% \pgfplothandlerrecord{\myplot}
% \pgfplotxyfile{mytable}  % stored in \myplot now
% \pgfplothandlerline
% \myplot
% \pgftransformxshift{1cm}
% \myplot

\pgfdeclareplothandler{\pgfplothandlerrecord}{#1}{%
  start=\gdef#1{\pgfplotstreamstart},
  point=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreampoint{##1}},
  jump=\expandafter\gdef\expandafter#1\expandafter{#1\pgf@plotstreamjump},
  special=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamspecial{##1}},
  end=\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend},
}%



% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Each line of the file should begin with two numbers separated by a
% space. Such a line with number #1 and #2 is converted to a
% \pgfplotstreampoint{\pgfpointxy{#1}{#2}}. Extra characters following
% on the line are ignored.
%
% Lines starting with ``%'' and ``#'' are ignored.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyfile#1{%
  \begingroup%
    \def\b@pgfplotsxyfile@scanning@for@first{1}%
    \pgfplotstreamstart%
    \openin\r@pgf@reada=#1
    \ifeof\r@pgf@reada
      \pgfwarning{Plot data file `#1' not found.}
     \else
      \catcode`\#=14
      \catcode`\^^M=5
      \pgf@readxyfile%
    \fi
    \pgfplotstreamend%
  \endgroup%
}%

\let\pgf@savedpar=\par
\def\pgf@partext{\par}%
\def\pgf@readxyfile{%
  \pgfutil@read\r@pgf@reada to \pgf@temp%
  \let\par=\pgf@savedpar%
  \edef\pgf@temp{\pgf@temp}%
  \ifx\pgf@temp\pgfutil@empty%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else\ifx\pgf@temp\pgf@partext%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else%
    \expandafter\pgf@parsexyline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof\r@pgf@reada\else\expandafter\pgf@readxyfile\fi%
}%

\def\pgf@parsexyline#1 #2 #3\pgf@stop{%
  \def\b@pgfplotsxyfile@scanning@for@first{0}%
  \edef\pgf@xyline@flag@val{#3}%
  \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
    \pgfplotstreampointundefined%
  \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
    \pgfplotstreampointoutlier{\pgfpointxy{#1}{#2}}%
  \else%
    \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
  \fi\fi%
}%

\edef\pgf@xyline@flag@out{o\space}%
\edef\pgf@xyline@flag@undef{u\space}%




% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Like xy, except that each line contains three numbers, which are
% converted to xyz coordinates.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyzfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin\r@pgf@reada=#1
    \ifeof\r@pgf@reada
      \pgfwarning{Plot data file `#1' not found.}
    \else
      \catcode`\#=14
      \catcode`\^^M=5
      \pgf@readxyzfile%
    \fi
    \pgfplotstreamend%
  \endgroup%
}%

\def\pgf@readxyzfile{%
  \pgfutil@read\r@pgf@reada to \pgf@temp%
  \ifx\pgf@temp\pgfutil@empty%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else\ifx\pgf@temp\pgf@partext%
    \if1\b@pgfplotsxyfile@scanning@for@first
    \else
        \ifeof\r@pgf@reada\else\pgfplotstreamnewdataset\fi%
    \fi
  \else%
    \expandafter\pgf@parsexyzline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof\r@pgf@reada\else\expandafter\pgf@readxyzfile\fi%
}%

\def\pgf@parsexyzline#1 #2 #3 #4\pgf@stop{%
  \def\b@pgfplotsxyfile@scanning@for@first{0}%
  \edef\pgf@xyline@flag@val{#4}%
  \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
    \pgfplotstreampointundefined%
  \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
    \pgfplotstreampointoutlier{\pgfpointxyz{#1}{#2}{#3}}%
  \else%
    \pgfplotstreampoint{\pgfpointxyz{#1}{#2}{#3}}%
  \fi\fi%
}%




% Render a function using gnuplot.
%
% #1 = filename prefix for .gnuplot and .table files (optional,
%      default is \jobname)
% #2 = gnuplot function text
%
% Description:
%
% This command will write a file called #1.gnuplot that sets up
% some gnuplot commands to write output to a file called
% #1.table. Then it calls gnuplot (using the \write18 mechanism)
% to execute the file. Then it reads #2.table using \pgfplotxyfile.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotgnuplot[\jobname]{plot [x=0:5] x*sin(x)}

{%
  \catcode`\%=12
  \catcode`\"=12
  \xdef\pgf@gnuplot@head{set table \noexpand\pgf@plottablefile@quoted; set format "%.5f"}
}%

\let\pgf@plotwrite=\w@pgf@writea
\newif\ifpgf@resample@plot

\pgfkeys{%
  /pgf/plot/gnuplot call/.initial={gnuplot}}%

\def\pgfplotgnuplot{\pgfutil@ifnextchar[{\pgf@plotgnuplot}{\pgf@plotgnuplot[\jobname]}}%}%
\def\pgf@plotgnuplot[#1]#2{%
  \pgf@resample@plottrue%
  \pgfutilpreparefilename{#1.gnuplot}%
  \let\pgf@plotgnuplotfile=\pgfretval
  \pgfutilpreparefilename{#1.table}%
  \let\pgf@plottablefile=\pgfretval
  \let\pgf@plottablefile@quoted=\pgfretvalquoted
  % Check, whether it is up-to-date
  \openin\pgfutil@inputcheck=\pgf@plotgnuplotfile\relax
  \ifeof\pgfutil@inputcheck%
  \else%
    \pgfutil@read\pgfutil@inputcheck to\pgf@temp% ignored
    \pgfutil@read\pgfutil@inputcheck to\pgf@plot@line%
    \closein\pgfutil@inputcheck
    \edef\pgf@plot@code{#2\space}%
    \ifx\pgf@plot@code\pgf@plot@line%
      \openin\pgfutil@inputcheck=\pgfretval\relax
      \ifeof\pgfutil@inputcheck%
      \else%
        \closein\pgfutil@inputcheck
        \pgf@resample@plotfalse%
      \fi%
    \fi%
  \fi
  \ifpgf@resample@plot%
    \immediate\openout\pgf@plotwrite=\pgf@plotgnuplotfile\relax
    \immediate\pgfutil@write\pgf@plotwrite{\pgf@gnuplot@head}%
    \immediate\pgfutil@write\pgf@plotwrite{#2}%
    \immediate\closeout\pgf@plotwrite%
    \pgfutil@shellescape{%
      \pgfkeysvalueof{/pgf/plot/gnuplot call} \pgf@plotgnuplotfile}%
  \fi%
%  \let\pgf@savedparsexyline=\pgf@parsexyline%
%  \let\pgf@parsexyline=\pgf@parsegnuplotxyline%
  \pgfplotxyfile{\pgf@plottablefile}%
%  \let\pgf@parsexyline=\pgf@savedparsexyline%
}%

% \def\pgf@parsegnuplotxyline#1 #2 #3\pgf@stop{%
%   \edef\pgf@xyline@flag@val{#3}%
%   \edef\pgf@xyline@flag@out{o\space}%
%   \edef\pgf@xyline@flag@undef{u\space}%
%   \ifx\pgf@xyline@flag@val\pgf@xyline@flag@undef%
%     \pgfplotstreampointundefined%
%   \else\ifx\pgf@xyline@flag@val\pgf@xyline@flag@out%
%     \pgfplotstreampointoutlier{\pgfpointxy{#1}{#2}}%
%   \else%
%     \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
%   \fi\fi%
% }%

% This producer handler plots a function using pgf's mathematical engine.
%
% #1 = variable
% #2 = domain for the variable
% #3 = point, typically defined in terms of the value of the variable
%
% Description:
%
% This producer will iterate the variable #1 over all variables in #2
% (using the \foreach statement). For each value, a plot coordinate
% #3  is created.
%
% Note that this command is pretty slow.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotfunction{\x}{0,0.1,...,3.141}{\pgfpointxy{\x}{sin(\x)}}

\def\pgfplotfunction#1#2#3{%
  \pgfplotstreamstart%
  \foreach#1in{#2}%
  {%
    \pgf@process{#3}%
    \edef\pgf@marshal{\noexpand\pgfplotstreampoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
    \pgf@marshal%
  }
  \pgfplotstreamend%
}%




\endinput


==> pgfmoduleshapes.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS{pgfmoduleshapes.code.tex}



\newbox\pgfnodeparttextbox


% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% When this command is called, the shape-specific TeX boxes of the
% node must have been setup correctly.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfmultipartnode{rectangle}{center}{hellonode}{\pgfusepath{stroke}}

\def\pgfmultipartnode#1#2#3#4{%
  \pgfutil@ifundefined{pgf@sh@s@#1}%
  {\pgferror{Unknown shape ``#1''}}%
  {%
    {%
      \ifpgflatenodepositioning%
        \pgfsys@beginscope%
      \fi%
      \pgf@outer@adjust@hook%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \def\pgf@sm@shape@name{#1}% CJ % TT added prefix!
      \csname pgf@sh@s@#1\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{#1}{#2}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@#3\endcsname{%
        \pgf@sh@reanchor{#1}{#2}% FIXME : this is double work!
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@node@name{#3}%
      \ifpgflatenodepositioning%
        \pgf@shapes@late@pos@begin%
      \fi%
      \ifx\pgf@node@name\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@\pgf@node@name\endcsname{#1}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@\pgf@node@name\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@\pgf@node@name\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp%
        \expandafter\xdef\csname pgf@sh@nt@\pgf@node@name\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@\pgf@node@name\endcsname{\pgfpictureid}%
      \fi%
      \pgfutil@ifundefined{pgf@sh@bbg@#1}{}
      {{\pgfusetype{.behind background}\pgfidscope\pgfscope\csname pgf@sh@bbg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \pgfutil@ifundefined{pgf@sh@bg@#1}{%
        \global\let\pgfpositionnodelaterpath\pgfutil@empty%
      }%
      {\pgfpushtype%
       \pgfusetype{.background}\csname pgf@sh@bg@#1\endcsname%
        \ifpgflatenodepositioning%
          \pgfsyssoftpath@getcurrentpath\pgfpositionnodelaterpath%
          \pgfprocessround{\pgfpositionnodelaterpath}{\pgfpositionnodelaterpath}%
          \global\let\pgfpositionnodelaterpath\pgfpositionnodelaterpath%
        \fi%
        #4\pgfpoptype}%
      \pgfutil@ifundefined{pgf@sh@fbg@#1}{}
      {{\pgfusetype{.before background}\pgfidscope\pgfscope\csname pgf@sh@fbg@#1\endcsname\endpgfscope\endpgfidscope}}%
      {%
        \expandafter\pgfutil@for\expandafter\pgf@shape@com\expandafter:\expandafter=\csname pgf@sh@boxes@#1\endcsname\do{%
          {%
            \pgfusetype{.\pgf@shape@com}%
            \pgftransformshift{\pgf@sh@reanchor{#1}{\pgf@shape@com}}%
            \pgfapproximatenonlineartransformation%
            \expandafter\pgfqboxsynced\expandafter{\csname pgfnodepart\pgf@shape@com box\endcsname}%
          }%
        }%
      }%
      \pgfutil@ifundefined{pgf@sh@bfg@#1}{}%
      {{\pgfusetype{.behind foreground}\pgfidscope\pgfscope\csname pgf@sh@bfg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \pgfutil@ifundefined{pgf@sh@fg@#1}{}%
      {\pgfpushtype\pgfusetype{.foreground}\csname pgf@sh@fg@#1\endcsname#4\pgfpoptype}%
      \pgfutil@ifundefined{pgf@sh@ffg@#1}{}%
      {{\pgfusetype{.before foreground}\pgfidscope\pgfscope\csname pgf@sh@ffg@#1\endcsname\endpgfscope\endpgfidscope}}%
      \ifpgflatenodepositioning%
        \pgf@shapes@late@pos@end%
        \pgfsys@endscope%
      \else%
        \expandafter\pgf@nodecallback\expandafter{\pgf@node@name}%
      \fi%
    }%
  }%
}%
\let\pgf@outer@adjust@hook\relax

\def\pgf@shapes@late@pos@begin{%
  % Rename node
  \edef\pgf@node@name{not yet positionedPGFINTERNAL\pgf@node@name}%
  % Interrupt bounding box!
  \pgfinterruptboundingbox%
    % Put everything in our box:
    \pgf@relevantforpicturesizetrue%
    \setbox\pgfpositionnodelaterbox=\hbox%
      \bgroup%
        \pgfsys@beginscope%
}%

\def\pgf@shapes@late@pos@end{%
       \pgfsys@endscope%
      \egroup% Close box
    \ifdim\pgf@picminx>\pgf@picmaxx\relax% happens for empty nodes
      \def\pgfpositionnodelaterminx{0.0pt}%
      \let\pgfpositionnodelaterminy\pgfpositionnodelaterminx%
      \let\pgfpositionnodelatermaxx\pgfpositionnodelaterminx%
      \let\pgfpositionnodelatermaxy\pgfpositionnodelaterminx%
    \else%
      \edef\pgfpositionnodelaterminx{\the\pgf@picminx}%
      \edef\pgfpositionnodelaterminy{\the\pgf@picminy}%
      \edef\pgfpositionnodelatermaxx{\the\pgf@picmaxx}%
      \edef\pgfpositionnodelatermaxy{\the\pgf@picmaxy}%
    \fi%
    \let\pgfpositionnodelatername=\pgf@node@name%
    \pgf@positionnodelater@macro%
  \endpgfinterruptboundingbox%
}%

\def\pgf@shift@node#1#2{%
  % This internal command shifts the recorded coordinates for node #1
  % by the vector #2. It is used to
  % correct the position of the node if the recorded coordinate
  % happens to be wrong
  {%
    \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
    \pgf@process{#2}%
    \advance\pgf@pt@x by\pgf@x%
    \advance\pgf@pt@y by\pgf@y%
    \pgfgettransform{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  }%
}%



% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = normal TeX text
% #4 = name for later reference
% #5 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfnode{rectangle}{center}{Hello}{hellonode}{\pgfusepath{stroke}}

\def\pgfnode#1#2#3#4#5{%
  {%
    \setbox\pgfnodeparttextbox=\hbox%
    {%
      \pgfinterruptpicture%
        {#3}%
      \endpgfinterruptpicture%
    }%
    \pgfmultipartnode{#1}{#2}{#4}{#5}%
  }
}%



% Create a node that is positioned later
%
% #1 = macro to be called after the next node has been created
%
% Description:
%
% You can use this command to create a node that is "positioned
% later". The idea is the following: Normally, when a node is created
% using a command like \pgfnode, the node is immediately inserted into
% the current picture. In particular, you have no chance to change the
% position of a created node after it has been create.
%
% Using \pgfpositionnodelater, you can change the default
% behaviour. This command is not a replacement for \pgfnode, but is
% called before such a command and will cause the following to happen:
% The node is created, but not inserted into the picture. Instead, it
% is stored in the box \pgfpositionnodelaterbox. Furthermore, the node
% is not relevant for the picture's bounding box, but a bounding box
% for the node is computed and stored in the macros
% \pgfpositionnodelaterboundboxminx to
% \pgfpositionnodelaterboundboxmaxy. Finally, the
% macro #1 is called with the following macros setup:
%
%   \pgfpositionnodelaterbox
%   A box register (box 0 by default) that stores the node's paths and
%   texts. You should move the contents of this box to a box of your
%   choice.
%
%   \pgfpositionnodelatername
%   The name of the just-created-node. This name will be the
%   originally "desired" name of the box plus the prefix "not yet
%   positioned boxPGFINTERNAL".
%
%   \pgfpositionnodelaterminx
%   \pgfpositionnodelatermaxx
%   \pgfpositionnodelaterminy
%   \pgfpositionnodelatermaxy
%   These four macros store the bounding box as dimensions that are
%   guarenteed to end with "pt".
%
% By setting #1 to \relax (which is the default), you can switch off
% the whole mechanism
%
% Once a late node has been created, you can add arbitrary code in the
% same picture. Then, at some later point, you call
% \pgfpositionnodenow to finally position the node at a given position.
%
% When \pgfpositionnodenow is called, the macros mentioned above
% should have the exact same values they had when #1 is called.

\def\pgfpositionnodelater#1{%
  \let\pgf@positionnodelater@macro=#1%
  \ifx\pgf@positionnodelater@macro\relax%
    \pgflatenodepositioningfalse%
  \else%
    \pgflatenodepositioningtrue%
  \fi%
}%
\newif\ifpgflatenodepositioning
\pgfpositionnodelater{\relax}%
\def\pgfpositionnodelaterbox{0}%




% Position a node that has been scheduled for later insertion
%
% #1 = position in the picture, where the original anchor should go,
%      now
%
% Description:
%
% This command works in concert with \pgfpositionnodelater, see the
% description there. When \pgfpositionnodenow is called, the macros
% \pgfpositionnodelaterbox and so on should be set to the values they
% had when the macro given to \pgfpositionnodelater was called. Then,
% the box described by these macros will be inserted into the picture
% at the position given #1. More precisely, the original node will
% have been positioned such that the anchor given upon invocation is
% at (0,0) and the node is now shifted by #1 before being inserted
% into the actual picture.

\def\pgfpositionnodenow#1{%
  \pgfinterruptpath%
  {%
    \pgfpointtransformed{#1}%
    \edef\pgf@temp@shift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
    \pgftransformreset%
    \pgftransformshift{\pgf@temp@shift}%
    \pgfsys@pictureboxsynced\pgfpositionnodelaterbox%
    \pgf@shift@node{\pgfpositionnodelatername}{\pgf@temp@shift}%
    % Bounding box update...
    \pgfpointtransformed{\pgfqpoint{\pgfpositionnodelaterminx}{\pgfpositionnodelaterminy}}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}
    \pgfpointtransformed{\pgfqpoint{\pgfpositionnodelatermaxx}{\pgfpositionnodelatermaxy}}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}
    % Naming and callbacks
    \expandafter\pgfpositionnodenow@rename\pgfpositionnodelatername\relax%
  }%
  % Late setup%
  {%
    \csname pgf@lns@\pgfpositionnodelatername\endcsname%
    \expandafter\global\expandafter\let\csname pgf@lns@\pgfpositionnodelatername\endcsname\relax%
  }%
  \endpgfinterruptpath%
}%

\def\pgfpositionnodenow@rename not yet positionedPGFINTERNAL#1\relax{%
  \pgfnoderename{#1}{not yet positionedPGFINTERNAL#1}
}%



% "Fake" a node
%
% #1 = node name
%
% Description:
%
% This command will setup things so that it "looks like" a node named
% #1 has been created, but, in reality, no node is created. The idea
% is that a node created in this way can be referenced by systems
% using the late positioning, which will only create the node later
% on.
%
\def\pgffakenode#1{%
  \edef\pgf@temp{\ifpgflatenodepositioning not yet positionedPGFINTERNAL\fi#1}%
  \expandafter\gdef\csname pgf@sh@ns@\pgf@temp\endcsname{coordinate}%
  \expandafter\gdef\csname pgf@sh@np@\pgf@temp\endcsname{\def\centerpoint{\pgfpointorigin}}%
  \expandafter\gdef\csname pgf@sh@nt@\pgf@temp\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
  \expandafter\global\expandafter\let\csname pgf@sh@ma@\pgf@temp\endcsname\pgfutil@empty%
  \expandafter\xdef\csname pgf@sh@pi@\pgf@temp\endcsname{\pgfpictureid}%
}%



% Specify code that should be executed after a node has been created
%
% #1 = node name
% #2 = later code
%
% Description:
%
% This macro allows you to provide some code #2 that will be executed
% right after a node has been positioned using \pgfpositionnodenow. If
% the node has already been positioned (if the late positioning is not
% switched on), nothing happens.

\def\pgfnodepostsetupcode#1#2{%
  \ifpgflatenodepositioning%
    \expandafter\ifx\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname\relax%
      \expandafter\gdef\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname{#2}%
    \else%
      \expandafter\pgfutil@g@addto@macro\csname pgf@lns@not yet positionedPGFINTERNAL#1\endcsname{#2}%
    \fi%
  \fi%
}%



% Alias a node
%
% #1 = new node name
% #2 = existing node name
%
% Description:
%
% This command allows you to subsequently access the node #2 using the
% name #1.
%
% Example:
%
% \pgfnode{rectangle}{center}{Hallo}{hellonode}{}
% \pgfnodealias{mynode}{hellonode}

\def\pgfnodealias#1#2{%
  \pgf@node@gnamelet{pgf@sh@ns@#1}{pgf@sh@ns@#2}%
  \pgf@node@gnamelet{pgf@sh@np@#1}{pgf@sh@np@#2}%
  \pgf@node@gnamelet{pgf@sh@nt@#1}{pgf@sh@nt@#2}%
  \pgf@node@gnamelet{pgf@sh@pi@#1}{pgf@sh@pi@#2}%
  \pgf@node@gnamelet{pgf@sh@ma@#1}{pgf@sh@ma@#2}%
  \pgf@nodecallback{#1}%
}%
\def\pgf@node@gnamelet#1#2{%
  \expandafter\let\expandafter\pgf@temp\csname #2\endcsname%
  \expandafter\global\expandafter\let\csname #1\endcsname=\pgf@temp%
}%

% Rename a node
%
% #1 = new name
% #2 = old name
%
% Description:
%
% Renames a node. This is like an alias, only the memory used for the
% old name is freed.

\def\pgfnoderename#1#2{%
  \pgfnodealias{#1}{#2}%
  \expandafter\global\expandafter\let\csname pgf@sh@ns@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@np@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@nt@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@pi@#2\endcsname\relax
  \expandafter\global\expandafter\let\csname pgf@sh@ma@#2\endcsname\relax
}%




% Quickly create a coordinate node
%
% #1 = name
% #2 = coordinate
%
% Description:
%
% Creates a node of shape coordinate. The following have the same
% effect, only the second is much faster:
%
% { \pgftransformshift{\pgfpoint{1cm}{2cm} \pgfnode{coordinate}{center}{}{foo}{} }
% \pgfcoordinate{foo}{\pgfpoint{1cm}{2cm}}

\def\pgfcoordinate#1#2{%
  \edef\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty% do nothing
  \else%
    \ifpgflatenodepositioning%
      {\pgftransformshift{#2}\pgfnode{coordinate}{center}{}{#1}{}}%
    \else%
      \pgf@process{\pgfpointtransformed{#2}}%
      \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{coordinate}%
      \expandafter\xdef\csname pgf@sh@np@#1\endcsname{%
        \noexpand\def\noexpand\centerpoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      }
      \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
      \expandafter\global\expandafter\let\csname pgf@sh@ma@#1\endcsname\pgfutil@empty%
      \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
    \fi%
  \fi%
}%

\def\pgf@sh@redeferredanchor#1#2{% CJ
  \expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @#1\endcsname{#2}}% CJ






\def\pgf@sh@resavedanchor#1#2{%
  \pgf@process{#2}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    }}%
  \pgf@sh@marshal%
}%


\def\pgf@sh@resaveddimen#1#2{%
  {#2\global\pgf@x=\pgf@x}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\the\pgf@x}%
    }}%
  \pgf@sh@marshal%
}%

\def\pgf@sh@resavedmacro#1#2{%
    \let#1\pgfutil@empty%
    \def\addtosavedmacro##1{%
        \expandafter\def\expandafter\pgf@sh@addtomacro@temp\expandafter{#1\noexpand\def\noexpand##1{##1}}%
        {\expandafter\pgfutil@toks@\expandafter{\pgf@sh@addtomacro@temp}\expandafter}%
        \expandafter\def\expandafter#1\expandafter{\the\pgfutil@toks@}%
    }%
  #2\relax%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedmacros{%
      \noexpand\def\noexpand#1{#1}%
    }}%
  \pgf@sh@marshal%
}%

% Invoke an anchor
\def\pgf@sh@reanchor#1#2{%
  \pgfutil@ifundefined{pgf@anchor@#1@#2}%
  {%
    \pgfutil@ifundefined{pgf@anchor@generic@#2}{%
        \pgfmathsetcounter{pgf@counta}{#2}%
        \csname pgf@anchor@#1@border\endcsname{\pgfqpointpolar{\the\c@pgf@counta}{1pt}}%
    }{%
        \csname pgf@anchor@generic@#2\endcsname{#1}%
    }%
  }%
  {\csname pgf@anchor@#1@#2\endcsname}%
}%

% Defines a generic anchor, i.e. one which gets the associated shape
% as first argument.
%
% #1: the anchor name.
% #2: the code of the anchor. It may depend upon '##1', the shape's
% name.
%
% The anchor will be defined locally in the current TeX scope.
%
% If the anchor will be referenced later by \pgfpointanchor, the macro \pgfreferencednodename
% can be used to query the referenced node's name.
% This macro is not defined during node creation.
\def\pgfdeclaregenericanchor#1#2{%
  \expandafter\def\csname pgf@anchor@generic@#1\endcsname##1{#2}%
}%


% Retrieves an anchor of a shape
%
% #1 = name
% #2 = anchor or a number (corresponding to a degree)
%
% Description:
%
% This command yields a point at the anchor of the given named shape.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointanchor{hellonode}{center}}

\def\pgfpointanchor#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\pgfutil@ifundefined{pgf@sh@ns@not yet positionedPGFINTERNAL#1}{%
      \pgferror{No shape named `#1' is known}}{
      % else, fail silently
    }%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      \edef\pgfreferencednodename{#1}% for use inside of anchors.
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname
      \pgf@sh@reanchor{\csname pgf@sh@ns@#1\endcsname}{#2}%
      {%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform@glob%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform@glob%
    }%
  }%
}%

\def\pgf@shape@interpictureshift#1{%
  \expandafter\ifx\csname pgf@sh@pi@#1\endcsname\pgfpictureid%
  \else%
    \pgfsys@getposition{\csname pgf@sh@pi@#1\endcsname}\pgf@shape@original@pos%
    \pgfsys@getposition{\pgfpictureid}\pgf@shape@current@pos%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@current@pos}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@original@pos}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
  \fi%
}%



% Retrieves a border point of a shape
%
% #1 = name
% #2 = another point
%
% Description:
%
% This command yields a point on the border of the shape that is on a
% straight line from the center to the point #2.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointshapeborder{hellonode}{\pgfpoint{2cm}{1cm}}
% \pgfpathlineto{\pgfpoint{2cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfpointshapeborder#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\pgferror{No shape named `#1' is known}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      \edef\pgfreferencednodename{#1}% for use inside of anchors.
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname%
      {%
        \pgf@process{\pgfpointtransformed{#2}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgftransforminvert%
        \pgf@pos@transform@glob%
        \pgf@xa=\pgf@x%
        \pgf@ya=\pgf@y%
        \pgf@process{\csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @center\endcsname}%
        \pgf@process{\pgf@shape@interpictureshift{#1}}%%
        \advance\pgf@xa by-\pgf@x%
        \advance\pgf@ya by-\pgf@y%
        % Now (\pgf@xa, \pgf@ya) is a coord in shape's coord system, and
        % relative to the anchor "center". If (xa, ya) is almost identical to
        % the node center, which is determined by sqrt(xa^2+ya^2) < 0.02pt,
        % just return the node center.
        %
        % \pgf@xb = 10*\pgf@xa if -1pt<\pgf@xa<1pt else 10pt
        %  - "10*\pgf@xa": reduce ruonding errors when \pgf@xa is small
        %  - "-1pt<\pgf@xa<1pt": guard against error "Dimension too large"
        \pgf@xb=10pt
        \ifdim\pgf@xa<1pt\ifdim\pgf@xa>-1pt
          \pgf@xb=10\pgf@xa
        \fi\fi
        % \pgf@yb = 10*\pgf@ya if -1pt<\pgf@ya<1pt else 10pt
        \pgf@yb=10pt
        \ifdim\pgf@ya<1pt\ifdim\pgf@ya>-1pt
          \pgf@yb=10\pgf@ya
        \fi\fi
        % if xb^2+yb^2 < 0.04pt, which means sqrt(xa^2+ya^2) < 0.02pt,
        % return node center
        \ifdim\dimexpr\expandafter\Pgf@geT\the\pgf@xb\pgf@xb
                     +\expandafter\Pgf@geT\the\pgf@yb\pgf@yb\relax<0.04pt
          \expandafter\pgfutil@firstoftwo
        \else
          \expandafter\pgfutil@secondoftwo
        \fi
        {% return coord of "center"
          \pgfwarning
            {Returning node center instead of a point on node border. Did you
            specify a point identical to the center of node
            ``\pgfreferencednodename''?}%
          \pgf@sh@reanchor{\csname pgf@sh@ns@#1\endcsname}{center}%
        }
        {% this calls the corresponding \anchorborder in shape declaration
          \csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @border\endcsname
            {\pgfqpoint{\pgf@xa}{\pgf@ya}}%
        }%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform@glob%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform@glob%
    }%
  }%
}%


% Retrieve the list of node parts of a shape
%
% #1 = a macro
% #2 = a shape name
%
% Description:
%
% Stores the list of node parts of a shape #2 in the macro #1.
%
% Example:
%
% \pgfgetnodeparts\mylist{circle split}
%
% This will set \mylist\ to "text,lower"

\def\pgfgetnodeparts#1#2{%
  \expandafter\let\expandafter#1\csname pgf@sh@boxes@#2\endcsname%
}%


% Declares a shape type
%
% #1 = shape type
% #2 = shape specification
%
% Description:
%
% This command declares a new shape type. The shape specification
% should contain the following commands:
%
% - \savedanchor
%   This command takes two arguments: a name and some code. The point
%   specified by the code (the \pgf@x and \pgf@y values resulting from
%   executing the code, to be precise), will be stored under the given
%   name. Whenever, later on, an anchor is invoked these stored points
%   will be available. The \saveddimen works like \savedanchor, only a
%   single dimension is stored (taken from \pgf@x).
%   When a savedanchor is calculated, the height/width/depth of the
%   boxes mentioned in \nodeparts can be used.
%
% - \anchor
%   Specifies an anchor. This command takes two arguments: an anchor
%   name and some code for computing the anchor. When the anchor
%   computation starts, all shape points and shape dimension will be
%   setup.
%
% - \anchorborder
%   This command should compute a point on the border of the
%   shape. When the code is called, \pgf@x and \pgf@y will have been
%   preinitialised with a direction.
%
% - \behindbackgroundpath
%   Some things to be draw behind everything.
%
% - \backgroundpath
%   A path that is drawn behind the main box. How this path is used
%   depends on how \pgfshape is called.
%
% - \beforebackgroundpath
%   Some things to be draw before the background path, but behind the
%   main box.
%
% - \behindforegroundpath
%   Some things to be draw on top of the main box.
%
% - \foregroundpath
%   A path that is drawn on top of all of the above. How this path is
%   used depends on how \pgfshape is called.
%
% - \beforeforegroundpath
%   Some things to be draw before everything.
%
% - \nodeparts
%   List of node parts that make up the shape. For each entry XYZ in
%   the list there must be a box named \pgfnodepartXYZbox (possibly
%   ``redirected'' to some different box using \let). Each such box
%   will be placed at the anchor XYZ.
%   By default, \nodeparts is just {text}. Thus, there will be one
%   node part box named \pgfnodeparttextbox and this node will be
%   placed at the anchor text.
%
%
% Example:
%
% See the definition of rectangle, below.

\long\def\pgfdeclareshape#1#2{%
  {%
    \def\pgf@sm@shape@name{#1}%
    \let\savedanchor=\pgf@sh@savedanchor
    \let\saveddimen=\pgf@sh@saveddimen
    \let\savedmacro=\pgf@sh@savedmacro% MW
    \let\deferredanchor=\pgf@sh@deferredanchor% CJ
    \let\anchor=\pgf@sh@anchor
    \let\anchorborder=\pgf@sh@anchorborder
    \let\behindbackgroundpath=\pgf@sh@behindbgpath
    \let\backgroundpath=\pgf@sh@bgpath
    \let\beforebackgroundpath=\pgf@sh@beforebgpath
    \let\behindforegroundpath=\pgf@sh@behindfgpath
    \let\foregroundpath=\pgf@sh@fgpath
    \let\beforeforegroundpath=\pgf@sh@beforefgpath
    \let\nodeparts=\pgf@sh@boxes
    \let\inheritsavedanchors=\pgf@sh@inheritsavedanchors
    \let\inheritanchor=\pgf@sh@inheritanchor
    \let\inheritanchorborder=\pgf@sh@inheritanchorborder
    \let\inheritbehindbackgroundpath=\pgf@sh@inheritbehindbgpath
    \let\inheritbackgroundpath=\pgf@sh@inheritbgpath
    \let\inheritbeforebackgroundpath=\pgf@sh@inheritbeforebgpath
    \let\inheritbehindforegroundpath=\pgf@sh@inheritbehindfgpath
    \let\inheritforegroundpath=\pgf@sh@inheritfgpath
    \let\inheritbeforeforegroundpath=\pgf@sh@inheritbeforefgpath
    \let\inheritnodeparts=\pgf@sh@inheritboxes
    \anchorborder{\csname pgf@anchor@#1@center\endcsname}%
    \anchor{text}{\pgfpointorigin}%
    \nodeparts{text}%
    \expandafter\global\expandafter\let\csname pgf@sh@s@\pgf@sm@shape@name\endcsname=\pgfutil@empty%
    #2%
  }%
}%

\def\pgf@sh@savedanchor#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resavedanchor{#1}{#2}}}%
\def\pgf@sh@saveddimen#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resaveddimen{#1}{#2}}}%
 \def\pgf@sh@savedmacro#1#2{% MW
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@resavedmacro{#1}{#2}}}% MW
\def\pgf@sh@anchor#1#2{\expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @#1\endcsname{#2}}%
\def\pgf@sh@deferredanchor#1#2{% CJ
  \expandafter\pgfutil@g@addto@macro
    \csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\pgf@sh@redeferredanchor{#1}{#2}}}% CJ
\def\pgf@sh@anchorborder#1{\expandafter\gdef\csname pgf@anchor@\pgf@sm@shape@name @border\endcsname##1{\pgf@process{##1}#1}}%
\long\def\pgf@sh@behindbgpath#1{\expandafter\gdef\csname pgf@sh@bbg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@bgpath#1{\expandafter\gdef\csname pgf@sh@bg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@beforebgpath#1{\expandafter\gdef\csname pgf@sh@fbg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@behindfgpath#1{\expandafter\gdef\csname pgf@sh@bfg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@fgpath#1{\expandafter\gdef\csname pgf@sh@fg@\pgf@sm@shape@name\endcsname{#1}}%
\long\def\pgf@sh@beforefgpath#1{\expandafter\gdef\csname pgf@sh@ffg@\pgf@sm@shape@name\endcsname{#1}}%
\def\pgf@sh@boxes#1{\expandafter\gdef\csname pgf@sh@boxes@\pgf@sm@shape@name\endcsname{#1}}%

\def\pgf@sh@inheritsavedanchors[from=#1]{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\pgf@sm@shape@name\endcsname{\csname pgf@sh@s@#1\endcsname}}%

\def\pgf@sh@inheritanchor[from=#1]#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\pgf@sm@shape@name @#2\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@#2\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritanchorborder[from=#1]{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\pgf@sm@shape@name @border\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@border\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritor#1#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@sh@#1@\pgf@sm@shape@name\endcsname=\expandafter\noexpand\csname
    pgf@sh@#1@#2\endcsname}%
  \pgf@marshal%
}%
\def\pgf@sh@inheritbehindbgpath[from=#1]{\pgf@sh@inheritor{bbg}{#1}}%
\def\pgf@sh@inheritbgpath[from=#1]{\pgf@sh@inheritor{bg}{#1}}%
\def\pgf@sh@inheritbeforebgpath[from=#1]{\pgf@sh@inheritor{fbg}{#1}}%
\def\pgf@sh@inheritbehindfgpath[from=#1]{\pgf@sh@inheritor{bfg}{#1}}%
\def\pgf@sh@inheritfgpath[from=#1]{\pgf@sh@inheritor{fg}{#1}}%
\def\pgf@sh@inheritbeforefgpath[from=#1]{\pgf@sh@inheritor{ffg}{#1}}%
\def\pgf@sh@inheritboxes[from=#1]{\pgf@sh@inheritor{boxes}{#1}}%



%
% Coordinate. This shape is special: It is only used to reference a
% point for later usage. Nothing is drawn, all anchors are identical
% to the center.
%

\pgfdeclareshape{coordinate}
{%
  \savedanchor\centerpoint{%
    % x
    \pgf@x=.5\wd\pgfnodeparttextbox%
    % y
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by -.5\dp\pgfnodeparttextbox%
  }%

  \anchor{center}{\centerpoint}%
  \anchor{north}{\centerpoint}%
  \anchor{north west}{\centerpoint}%
  \anchor{north east}{\centerpoint}%
  \anchor{west}{\centerpoint}%
  \anchor{east}{\centerpoint}%
  \anchor{mid}{\centerpoint}%
  \anchor{mid west}{\centerpoint}%
  \anchor{mid east}{\centerpoint}%
  \anchor{base}{\centerpoint}%
  \anchor{base west}{\centerpoint}%
  \anchor{base east}{\centerpoint}%
  \anchor{south}{\centerpoint}%
  \anchor{south west}{\centerpoint}%
  \anchor{south east}{\centerpoint}%
  \anchorborder{\centerpoint}%

  \nodeparts{}% no text
}%


% Value keys for shapes:
%
% /pgf/inner xsep     : recommended inner x separation
% /pgf/inner ysep     : recommended inner y separation
% /pgf/outer xsep     : recommended outer x separation
% /pgf/outer ysep     : recommended outer y separation
% /pgf/minimum width  : recommended minimum width
% /pgf/minimum height : recommended minimum height

\pgfset{
  inner xsep/.initial     =.3333em,
  inner ysep/.initial     =.3333em,
  inner sep/.style        ={/pgf/inner xsep=#1,/pgf/inner ysep=#1},
  outer xsep/.initial     =.5\pgflinewidth,
  outer ysep/.initial     =.5\pgflinewidth,
  outer sep/.code         =\pgf@handle@outer@sep{#1},
  minimum width/.initial  =1pt,
  minimum height/.initial =1pt,
  minimum size/.style     ={/pgf/minimum width=#1,/pgf/minimum height=#1},
}%



\def\pgf@handle@outer@sep#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgf@auto@text%
    \def\pgf@outer@adjust@hook{%
      \pgftransformationadjustments%
      \pgfkeyssetvalue{/pgf/outer xsep}{.5\pgflinewidth*\pgfhorizontaltransformationadjustment}%
      \pgfkeyssetvalue{/pgf/outer ysep}{.5\pgflinewidth*\pgfverticaltransformationadjustment}%
      \pgf@outer@auto@adjust@hook%
    }%
  \else%
    \pgfkeyssetvalue{/pgf/outer xsep}{#1}%
    \pgfkeyssetvalue{/pgf/outer ysep}{#1}%
  \fi%
}%
\def\pgf@auto@text{auto}%

\let\pgf@outer@auto@adjust@hook\relax


% Keys for rotating the shape border.
% (may not be supported by all shapes)
%
% /pgf/shape border uses incircle : Calculate the shape border using the incircle
%                                   around the node contents (+inner sep).
%
% /pgf/shape border rotate        : Angle of independent border rotation.

\newif\ifpgfshapeborderusesincircle
\pgfkeys{/pgf/shape border uses incircle/.is if=pgfshapeborderusesincircle}%
\pgfkeys{/pgf/shape border rotate/.initial=0}%

%
% Rectangle
%

\pgfdeclareshape{rectangle}
{%
  \savedanchor\northeast{%
    % Calculate x
    %
    % First, is width < minimum width?
    \pgf@x=\the\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by 2\pgf@xc%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    % Now, calculate right border: .5\wd\pgfnodeparttextbox + .5 \pgf@x + outer sep
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    % Calculate y
    %
    % First, is height+depth < minimum height?
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by 2\pgf@yc%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    % Now, calculate upper border: .5\ht-.5\dp + .5 \pgf@y + outer sep
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    \advance\pgf@y by.5\ht\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }%

  \savedanchor\southwest{%
      % Calculate x
      %
      % First, is width < minimum width?
      \pgf@x=\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
      \advance\pgf@x by 2\pgf@xc%
      \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
      \ifdim\pgf@x<\pgf@xb%
        % yes, too small. Enlarge...
        \pgf@x=\pgf@xb%
      \fi%
      % Now, calculate left border: .5\wd\pgfnodeparttextbox - .5 \pgf@x - outer sep
      \pgf@x=-.5\pgf@x%
      \advance\pgf@x by.5\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
      \advance\pgf@x by-\pgf@xa%
      % Calculate y
      %
      % First, is height+depth < minimum height?
      \pgf@y=\ht\pgfnodeparttextbox%
      \advance\pgf@y by\dp\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
      \advance\pgf@y by 2\pgf@yc%
      \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
      \ifdim\pgf@y<\pgf@yb%
        % yes, too small. Enlarge...
        \pgf@y=\pgf@yb%
      \fi%
       % Now, calculate upper border: .5\ht-.5\dp - .5 \pgf@y - outer sep
      \pgf@y=-.5\pgf@y%
      \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
      \advance\pgf@y by.5\ht\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
      \advance\pgf@y by-\pgf@ya%
  }%

  %
  % Anchors
  %
  \anchor{center}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \pgf@y=.5\pgf@y%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base}{\pgf@anchor@rectangle@center\pgf@y=0pt}%
  \anchor{north}{
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }%
  \anchor{south}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }%
  \anchor{west}{
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid west}{\southwest\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base west}{\southwest\pgf@y=0pt}%
  \anchor{north west}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa}%
  \anchor{south west}{\southwest}%
  \anchor{east}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }%
  \anchor{mid east}{\northeast\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base east}{\northeast\pgf@y=0pt}%
  \anchor{north east}{\northeast}%
  \anchor{south east}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
  }%
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%

  %
  % Background path
  %
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  }%
}%


% Special current path start coordinate:
\expandafter\def\csname pgf@sh@ns@current subpath start\endcsname{coordinate}%
\expandafter\def\csname pgf@sh@np@current subpath start\endcsname{%
  \def\centerpoint{\expandafter\pgfqpoint\pgfsyssoftpath@lastmoveto}%
}%
\expandafter\def\csname pgf@sh@nt@current subpath start\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current subpath start\endcsname{\pgfpictureid}%



% Special  current bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current bounding box\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
  \def\northeast{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
}%
\expandafter\def\csname pgf@sh@nt@current bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current bounding box\endcsname{\pgfpictureid}%


% Special  current path bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current path bounding box\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current path bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@pathminx}{\pgf@pathminy}}%
  \def\northeast{\pgfqpoint{\pgf@pathmaxx}{\pgf@pathmaxy}}%
}%
\expandafter\def\csname pgf@sh@nt@current path bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current path bounding box\endcsname{\pgfpictureid}%


% Special  current page bounding box rectangle:
\expandafter\def\csname pgf@sh@ns@current page\endcsname{rectangle}%
\expandafter\def\csname pgf@sh@np@current page\endcsname{%
  \def\southwest{\pgfpointorigin}%
  \def\northeast{\pgfpoint{\pgfsys@thepagewidth}{\pgfsys@thepageheight}}%
}%
\expandafter\def\csname pgf@sh@nt@current page\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
\expandafter\def\csname pgf@sh@pi@current page\endcsname{pgfpageorigin}%


% Special scope bounding box rectangle:
\pgfkeys{/pgf/local bounding box/.code={%
    \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
    \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
      \def\southwest{\pgfqpoint{\csname pgf@lbb@minx@#1\endcsname}{\csname pgf@lbb@miny@#1\endcsname}}%
      \def\northeast{\pgfqpoint{\csname pgf@lbb@maxx@#1\endcsname}{\csname pgf@lbb@maxy@#1\endcsname}}%
    }
    \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
    \expandafter\gdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}
    \expandafter\gdef\csname pgf@lbb@maxx@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@minx@#1\endcsname{16000pt}%
    \expandafter\gdef\csname pgf@lbb@maxy@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@miny@#1\endcsname{16000pt}%
    \pgf@size@hookedtrue%
    \expandafter\def\expandafter\pgf@path@size@hook\expandafter{\pgf@path@size@hook\pgf@lbb@do{#1}}
  },
  /pgf/freeze local bounding box/.code={%
    {%
      \csname pgf@sh@np@#1\endcsname%
      \southwest%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \northeast%
      \expandafter\xdef\csname pgf@sh@np@#1\endcsname{%
        \noexpand\def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
        \noexpand\def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      }%
    }%
  },
}%
\def\pgf@lbb@do#1{%
  \ifdim\pgf@size@hook@x<\csname pgf@lbb@minx@#1\endcsname\expandafter\xdef\csname pgf@lbb@minx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@x>\csname pgf@lbb@maxx@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@y<\csname pgf@lbb@miny@#1\endcsname\expandafter\xdef\csname pgf@lbb@miny@#1\endcsname{\the\pgf@size@hook@y}\fi%
  \ifdim\pgf@size@hook@y>\csname pgf@lbb@maxy@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxy@#1\endcsname{\the\pgf@size@hook@y}\fi%
}%

%
% Circle
%

\pgfdeclareshape{circle}
%
% Draws a circle around the text
%
{%
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }%

  \saveddimen\radius{%
    %
    % Calculate ``height radius''
    %
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yb%
    %
    % Calculate ``width radius''
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    %
    % Calculate length of radius vector:
    %
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    %
    % If necessary, adjust radius so that the size requirements are
    % met:
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    %
    % Now, add larger of outer separations.
    %
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }%

  %
  % Anchors
  %
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base}{\centerpoint\pgf@y=0pt}%
  \anchor{north}{\centerpoint\advance\pgf@y by\radius}%
  \anchor{south}{\centerpoint\advance\pgf@y by-\radius}%
  \anchor{west}{\centerpoint\advance\pgf@x by-\radius}%
  \anchor{east}{\centerpoint\advance\pgf@x by\radius}%
  \anchor{mid west}{\centerpoint\advance\pgf@x by-\radius\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{mid east}{\centerpoint\advance\pgf@x by\radius\pgfmathsetlength\pgf@y{.5ex}}%
  \anchor{base west}{\centerpoint\advance\pgf@x by-\radius\pgf@y=0pt}%
  \anchor{base east}{\centerpoint\advance\pgf@x by\radius\pgf@y=0pt}%
  \anchor{north west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }%
  \anchor{south west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }%
  \anchor{north east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }%
  \anchor{south east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }%
  \anchorborder{%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\radius}{\radius}}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }%

  %
  % Background path
  %
  \backgroundpath{%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
  }%
}%





\endinput


==> pgfrcs.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ifx\eTeXrevision\undefined%
  \pgfutil@packageerror{PGF}{PGF requires etex in extended mode}{}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

\ifnum\eTeXversion<2
  \pgfutil@packageerror{PGF}{PGF requires etex version 2}{}%
  \csname @@end\expandafter\endcsname\expandafter\end%
\fi

% The purpose of this file is to define the command
% \ProvidesPackageRCS, which should be followed by an RCS id
% string. This command will also be available in plain TeX, where it
% prints out a message to the log.

\pgfutil@IfFileExists{pgf.revision.tex}{\input pgf.revision.tex } {%
    \def\pgfrevision{0}%
    \def\pgfversion{0.0}%
    \def\pgfversiondatetime{2014-07-01 00:00:00 +100}%
    \def\pgfrevisiondatetime{2014-07-01 00:00:00 +100}%
    \def\pgfversiondate{2014/07/01}%
    \def\pgfrevisiondate{2014/07/01}%
}

\begingroup
\catcode`\"=12
\pgfutil@IfUndefined{directlua}{}{%
    \directlua{pgf = {}; pgf.pgfversion = "\pgfversion"}%
}%
\endgroup

% \def\pgftypesetversion{\oldstylenums{3}.\oldstylenums{0}.\oldstylenums{1}}
% XXX : implement pretty-printing:
% which is better? 'version' is something like 3.0.1 . revision is
% 3.0.1-151-g62184b3 which might be better for instable builds
%\let\pgftypesetversion=\pgfversion
\let\pgftypesetversion=\pgfrevision


\ifx\pgfrcsloaded\undefined
\def\pgfrcsloaded{}

\edef\pgfrcsatcode{\the\catcode`\@}
\catcode`\@=11

% not used in PGF, deprecated
\def\ProvidesFileRCS{%
    \let\pgfrcs@final=\ProvidesFileRCS@
	\pgfrcs@parseinput
}
\def\ProvidesFileRCS@#1{%
    \ProvidesFile{#1}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]%
}

\def\pgf@remove@ext#1.#2\relax{%
    \def\pgfretval{#1}%
}%

\def\ProvidesPackageRCS{%
	\let\pgfrcs@final=\ProvidesPackageRCS@
	\pgfrcs@parseinput
}
\def\ProvidesPackageRCS@#1{%
    \pgf@remove@ext#1.\relax
    \edef\pgfrcs@marshal{{\pgfretval}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]}%
    \expandafter\ProvidesPackage\pgfrcs@marshal
}

% not used in PGF, deprecated
\def\ProvidesClassRCS{%
	\let\pgfrcs@final=\ProvidesClassRCS@
	\pgfrcs@parseinput
}
\def\ProvidesClassRCS@#1{%
    \pgf@remove@ext#1.\relax
    \edef\pgfrcs@marshal{{\pgfretval}[\pgfversiondate\space v\pgfversion\space(\pgfrevision)]}%
    \expandafter\ProvidesClass\pgfrcs@marshal
}

\def\pgfrcs@parseinput@bracket{[}%
\def\pgfrcs@parseinput@dollarsign{$}%

\def\pgfrcs@parseinput#1{%
	\def\pgfrcs@parseinput@{#1}%
	\ifx\pgfrcs@parseinput@\pgfrcs@parseinput@bracket%
		% still accept it if someone has written his own pgfrcs files with headers of sorts
		% \ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.7 2010/04/11 07:09:19 username Exp $
		\let\next=\pgfrcs@parseinput@opt
	\else
		\ifx\pgfrcs@parseinput@\pgfrcs@parseinput@dollarsign
			% still accept it if someone has written his own pgfrcs files with headers of sorts
			% \ProvidesPackageRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.7 2010/04/11 07:09:19 username Exp $
			\let\next\pgfrcs@parseinput@dollar
		\else
			% the new, normal pgf-way is \ProvidesPackageRCS{pgfcore.code.tex}
			\def\next{\pgfrcs@final{#1}}%
		\fi
	\fi
	\next
}
\def\pgfrcs@parseinput@opt#1] ${%
	% just backwards compatibility -- ignore the information, but parse the input tokens:
	\pgfrcs@parseinput@dollar
}%
\def\pgfrcs@parseinput@dollar#1${%
	\pgf@parseid $#1$%
	% we ignore pretty much everything except for the file name:
	\edef\pgfrcs@parseinput@{\pgf@rcsfile.\pgf@rcssuffix}%
	\expandafter\pgfrcs@final\expandafter{\pgfrcs@parseinput@}%
}%
% Get date and version from RCS Ids
\def\pgf@parseid $#1: #2.#3,v #4 #5/#6/#7 #8${%
  \pgf@parsercsfile$#2/$
  \def\pgf@rcssuffix{#3}
  \def\pgf@rcsrevision{#4}
  \def\pgf@rcsdate{#5/#6/#7}
}
\def\pgf@parsercsfile$#1/#2${
  \def\pgf@temp{#2}
  \ifx\pgf@temp\pgfutil@empty
    \def\pgf@rcsfile{#1}
  \else
    \pgf@parsercsfile$#2$
  \fi}


\ifx\ProvidesPackage\@undefined
    % plain tex
    \def\ProvidesPackage#1[#2]{\wlog{Loading package #1 version #2.}}
\fi

\ifx\ProvidesFile\@undefined
    % plain tex
    \def\ProvidesFile#1[#2]{\wlog{Loading file #1 version #2.}}
\fi

\ProvidesPackageRCS{pgfrcs.code.tex}

\catcode`\@=\pgfrcsatcode

\fi


% Local Variables:
% coding: undecided-unix
% End:


==> pgfsys.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{pgfsys.code.tex}


% Load key mechanism
\input pgfkeys.code.tex

% "pgf" is a family
\pgfkeys{/pgf/.is family}
\def\pgfset{\pgfqkeys{/pgf}}

% This if is needed *very* early
\newif\ifpgfpicture


%
% The following conversion functions are used to convert from TeX
% dimensions to postscript/pdf points.
%
{\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}

\def\pgf@sys@tonumber#1{\expandafter\Pgf@geT\the#1}

\def\pgf@sys@bp@correct#1{#1=0.99627#1}

\def\pgf@sys@bp#1{%
  {%
    \pgf@x=#1\relax%
    \pgf@x=0.99627\pgf@x%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \pgfutil@toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\pgfutil@toks@}%
  }%
}
\def\pgf@sys@pt#1{%
  {%
    \pgf@x=#1\relax%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \pgfutil@toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\pgfutil@toks@}%
  }%
}


% internal dimensions that are always present when pgsys is loaded.
\newdimen\pgf@x
\newdimen\pgf@y
\newdimen\pgf@xa
\newdimen\pgf@ya
\newdimen\pgf@xb
\newdimen\pgf@yb
\newdimen\pgf@xc
\newdimen\pgf@yc
\newdimen\pgf@xd
\newdimen\pgf@yd

\newwrite\w@pgf@writea
\newread\r@pgf@reada
\let\pgfutil@inputcheck=\r@pgf@reada

% internal counters that are always present when pgfsys is loaded
\newcount\c@pgf@counta
\newcount\c@pgf@countb
\newcount\c@pgf@countc
\newcount\c@pgf@countd

\newtoks\t@pgf@toka
\newtoks\t@pgf@tokb
\newtoks\t@pgf@tokc

% Ensure that math registers are the same (math is broken in case it
% is loaded first)
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc
\let\c@pgfmath@countd\c@pgf@countd





% In the following dummy definitions of the pgf system commands are
% given. The individual drivers must overwrite these definitions,
% preferably all of them. If some system command is used that has not
% been overwritten, the command fails with a warning.
%
% In some cases, some pgf system commands are just shorthands for a
% series of more complicated commands. In this case, a default
% implementation is given in this file, but a driver may choose to
% overwrite this default implementation with a more efficient
% version. For example, a closestroke is the same as a closepath
% followed by a stroking, but in pdf there is a special shorthand for
% this. So, the pdf driver overwrites \pgfsys@closestroke, while the
% postscript driver does not.
%
% The commands for which default implementations are available are
% given at the end.

\def\pgf@sys@fail#1{%
  \expandafter\ifx\csname pgf@sys@fail@#1\endcsname\pgfutil@empty%
  \else%
    \expandafter\global\expandafter\let\csname pgf@sys@fail@#1\endcsname=\pgfutil@empty%
    \pgfwarning{Your graphic driver \pgfsysdriver\space does not support #1. This warning is given only once}%
  \fi%
}



%
% Invocation commands
%

\def\pgfsys@invoke{\pgf@sys@fail{invoking specials}}
% This command is used whenever some literal text needs to be inserted
% into the resulting .pdf, .ps, or .dvi file. Note that most
% \pgfsys@xxxx commands will not directly call this command, but,
% rather, use the protocolling mechanism to record their literal
% text. It is then left to the discretion of the protocolling
% mechanism to insert the literal text at some appropriate, later
% time.
%
% This command should only be called when \pgfsys@beginpicture has
% been called previously and when the picture has not been suspended
% using \pgfsys@beginhbox.

\def\pgfsys@outerinvoke{\pgfsys@invoke}
% This command can be used to insert protocolled graphic commands
% outside any picture. This is extremely dangerous, but sometimes
% useful. By default, this command does the same as inside pictures.



%
%
% Path construction commands
%
%

\def\pgfsys@moveto#1#2{\pgf@sys@fail{path constructions}}
% This command is used to start a path at a specific point (#1,#2)
% or to move the current point of the current path to (#1,#2)
% without drawing anything upon stroking (the current path is
% `interrupted').
%
% The arguments must be dimensions (like |10pt|).
%
% Example:
%
% \pgfsys@moveto{10pt}{10pt}
% \pgfsys@lineto{0pt}{0pt}
% \pgfsys@stroke
%
% This will draw a line from (10pt,10pt) to the origin of the picture.

\def\pgfsys@lineto#1#2{\pgf@sys@fail{path constructions}}
% Continue the current path to (#1,#2) with a line.

\def\pgfsys@curveto#1#2#3#4#5#6{\pgf@sys@fail{path constructions}}
% Continue the current path with a bezier curve to (#5,#6). The
% control points of the curve are at (#1,#2) and (#3,#4).

\def\pgfsys@rect#1#2#3#4{\pgf@sys@fail{path constructions}}
% Append a rectangle to the current path whose lower left corner is at
% (#1,#2) and whose width/height is given by (#3,#4).
%
% This command can be `mapped back' to moveto and lineto commands, but
% it is included since pdf has a special, quick version of this command.

\def\pgfsys@closepath{\pgf@sys@fail{path constructions}}
% Close the current path. This results in joining the current point of
% the path with the point specified by the last moveto
% operation. Typically, this is preferable over using lineto to the
% last point specified by a moveto, since the line starting at this
% point and the line ending at this point will be smoothly joined by
% closepath.
%
% Example:
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@closepath
% \pgfsys@stroke
%
% versus
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
%
% The difference between the above will be that in the second triangle
% the corner at the origin will be wrong; it will just be the overlay
% of two lines going in different directions, not a sharp pointed
% corner.






%
%
% Stroking and filling commands
%
%

\def\pgfsys@stroke{\pgf@sys@fail{path usage}}
% Stroke the current path (as if it were drawn with a pen). A number
% of so-called graphic state parameters influence this, which can be
% set in different ways:
%
% - linewidth
%   The `thickness' of the line. A width of 0 is the thinnest width
%   renderable on the device. On a high-resolution printer this may
%   become invisible and should be avoided. A good choice is 0.4pt,
%   which is the default.
%
% - stroke color
%   This special color is used for stroking. If it is not set, the
%   current color is used.
%
% - cap
%   The cap describes how the endings of lines a drawn. A round cap
%   adds a little half circle to these endings. A butt cap ends the
%   lines exactly at the end (or start) point without anything
%   added. A rectangular cap ends the lines like the butt cap, but the
%   lines protrude over the endpoint by the line thickness. (See also
%   the pdf or postscript manual). If the path has been closed, no cap
%   is drawn.
%
% - join
%   This describes how a bend (a join) in a path is rendered. A round
%   join draws bends using small arcs. A bevel join just draws the two
%   lines and then fills the join minimally so that it becomes
%   convex. A miter join extends the lines so that they form a single
%   sharp corner, but only up to a certain miter limit. (See the pdf
%   or postscript manual once more).
%
% - dash
%   The line may be dashed according to a dashing pattern.
%
% - clipping area
%   If a clipping area is established, only those parts of the path
%   that are inside the clipping area will be drawn.
%
% In addition to stroking a path, the path may also be used for
% clipping after it has been stroked. This will happen if the
% \pgfsys@clipnext is used prior to this command, see there for
% details.

\def\pgfsys@fill{\pgf@sys@fail{path usage}}
% This command fills the area surrounded by the current path. If the
% path has not yet been closed, it is closed prior to filling. The
% path itself is not stroked. For self-intersecting paths or paths
% consisting of multiple parts, the nonzero winding number rule is
% used to determine whether a point is inside or outside the
% path, except if \ifpgfsys@eorule holds -- in which case the even-odd
% rule should be used. (See the pdf or postscript manual for details.)
%
% The following graphic state parameters influence the filling:
%
% - fill color
%   If the fill color is not especially set, the current color is
%   used.
%
% - clipping area
%   If a clipping area is established, only those parts of the filling
%   area that are inside the clipping area will be drawn.
%
% In addition to filling the path, the path will also be used for
% clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@fillstroke{\pgf@sys@fail{path usage}}
% First, the path is filled, then the path is stroked. If the fill and
% stroke colors are the same (or if they are not specified and the
% current color is used), this yields almost the same as a
% \pgfsys@fill. However, due to the line thickness of the stroked
% path, the fillstroked area will be slightly larger.
%
% In addition to stroking and filling the path, the path will also be
% used for clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@clipnext{\pgf@sys@fail{path usage}}
% This command should be issued after a path has been constructed, but
% before it has been stroked and/or filled or discarded. When the
% command is used, the next stroking/filling/discarding command will
% first be executed normally. Then, afterwards, the just-used path
% will be used for subsequent clipping. If there has already been a
% clipping region, this region is intersected with the new clipping
% path (the clipping cannot get bigger). The nonzero winding number
% rule is used to determine whether a point is inside or outside the
% clipping area or the even-odd rule, depending on whether
% \ifpgfsys@eorule holds.

\def\pgfsys@discardpath{\pgf@sys@fail{path usage}}
% Normally, this command should `throw away' the current path.
% However, after \pgfsys@clipnext has been called, the current path
% should subsequently be used for clipping. See \pgfsys@clipnext for
% details.

\def\pgfsys@closestroke{\pgfsys@closepath\pgfsys@stroke}
% This command should have the same effect as first closing the path
% and then stroking it.

\newif\ifpgfsys@eorule
% Decides, whether even-odd filling and clipping is
% to be used or normal the non-zero winding number rule. See the
% pdf-documentation for details on what these rules are.




%
%
% Stroking options
%
%
\def\pgfsys@setlinewidth#1{\pgf@sys@fail{setting the line width}}
% Sets the width of lines, when stroked, to #1, which must be a TeX
% dimension (as text).

\def\pgfsys@buttcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a butt cap. See \pgfsys@stroke.

\def\pgfsys@roundcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a round cap. See \pgfsys@stroke.

\def\pgfsys@rectcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a rectangular cap. See \pgfsys@stroke.

\def\pgfsys@miterjoin{\pgf@sys@fail{setting the line join}}
% Sets the join to a miter join. See \pgfsys@stroke.

\def\pgfsys@setmiterlimit#1{\pgf@sys@fail{setting the line cap}}
% Sets the miter limit of lines to #1. See the pdf or postscript
% documentation.

\def\pgfsys@roundjoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a round join. See \pgfsys@stroke.

\def\pgfsys@beveljoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a bevel join. See \pgfsys@stroke.

\def\pgfsys@setdash#1#2{\pgf@sys@fail{setting the dashing pattern}}
% Sets the dashing patter. #1 should be a list of lengths separated by
% commas. #2 should be a single dimension.
%
% The list of values in #1 is used to determine the lengths of the
% `on' phases of the dashing and of the `off' phases. For example, if
% #1 is `3pt,4pt', then the dashing pattern is `3pt on followed by 4pt
% off, followed by 3pt on, followed by 4pt off, and so on'. A pattern
% of `.5pt,4pt,3pt,1.5pt' means `.5pt on, 4pt off, 3pt on, 1.5pt off, .5pt on,
% ...'. If the number of entries is odd, the last one is used twice,
% so `3pt' means `3pt on, 3pt off, 3pt on, 3pt off,...'. An empty list
% means `always on'.
%
% The second argument determines the `phase' of the pattern. For
% example, for a pattern of `3pt,4pt' and a phase of `1pt', the pattern
% would start: `2pt on, 4pt off, 3pt on, 4pt off, 3pt on, 4pt off...'.





%
%
% Color stuff
%
%

\def\pgfsys@color@rgb@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given rgb tuple
% (numbers between 0 and 1).
%
% Example: Make stroked text dark red: \pgfsys@color@rgb@stroke{0.5}{0}{0}
%
% The special stroking color is only used if the stroking color has
% been set since the last \pgfutil@color command. Thus, each \pgfutil@color command
% should reset both the stroking and filling colors.

\def\pgfsys@color@rgb@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given rgb tuple
% (numbers between 0 and 1). This color may be different from the
% stroking color.

\def\pgfsys@color@rgb#1#2#3{\pgfsys@color@rgb@stroke{#1}{#2}{#3}\pgfsys@color@rgb@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations. This is a
% ``low-level'' version of the \pgfutil@color command. It is currently only
% used by the plain tex version to support colors.

\def\pgfsys@color@cmyk@stroke#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cymk tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmyk@fill#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cymk tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmyk#1#2#3#4{\pgfsys@color@cmyk@stroke{#1}{#2}{#3}{#4}\pgfsys@color@cmyk@fill{#1}{#2}{#3}{#4}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@cmy@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cym tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmy@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cym tuple
% (numbers between 0 and 1).

\def\pgfsys@color@cmy#1#2#3{\pgfsys@color@cmy@stroke{#1}{#2}{#3}\pgfsys@color@cmy@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@gray@stroke#1{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given gray level
% (number between 0 and 1).

\def\pgfsys@color@gray@fill#1{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given gray level
% (number between 0 and 1).

\def\pgfsys@color@gray#1{\pgfsys@color@gray@stroke{#1}\pgfsys@color@gray@fill{#1}}
% Sets the color used for filling and stroking operations.

\newif\ifpgfsys@color@reset@inorder
% This if decides whether the color resetting of the
% \pgfsys@color@reset command may assume that all color commands are
% given ``in order.'' This means that this command will not be called,
% say, at the beginning of a box that is later inserted at a point
% where a fill color was actively set. This may allow the command to
% produce more compact code when it ``knows'' that no special fill or
% stroke color has been set.
\pgfsys@color@reset@inordertrue


\def\pgfsys@color@reset{}
% This command will be called when the \pgfutil@color command is used. It
% should purge any internal settings of stroking and filling
% color. After this call, till the next use of a command like
% \pgfsys@color@rgb@fill, the current color installed by the \pgfutil@color
% command should be used.

\def\pgfsys@color@unstacked#1{}
% This slightly obscure command causes the color stack to be
% tricked. When called, this command should set the current color to
% #1 without causing any change in the color stack.

\def\pgfsys@text@to@black@hook{}
% Another slightly obscure command that allows tikz to hack into
% dvisvgm's color management inside text nodes. The problem is that
% the color "black" is special for dvisvgm.



%
%
% Coordinate system transformations
%
%

\def\pgfsys@transformcm#1#2#3#4#5#6{\pgf@sys@fail{transformations}}
% Perform a concatenation of the low-level current transformation
% matrix with the matrix given by the values #1 to #6. The
% transformation matrix is a transformation on a homogeneous
% 2D-coordinate system. See the pdf or postscript manual for details.

\def\pgfsys@transformshift#1#2{\pgfsys@transformcm{1}{0}{0}{1}{#1}{#2}}
% This command will change the origin of the low-level coordinate
% system to (#1,#2).

\def\pgfsys@transformxyscale#1#2{\pgfsys@transformcm{#1}{0}{0}{#2}{0bp}{0bp}}
% This command will scale the low-level coordinate system (and
% everything that is drawn) by a factor of #1 in x-directed and #2 in
% y-direction. Note that this applies to everything, including
% lines. So a scaled line will have a different width and may even
% have a different width when going along the x-axis and when going
% along the y-axis, if the scaling is different in these directions.

\def\pgfsys@viewboxmeet#1#2#3#4#5#6#7#8{\pgfsys@beginscope\pgf@sys@default@viewbox@impl{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{<}}
% Consider the two rectangles R with lower left corner
% (#5,#6) and upper right (#7,#8) and S with lower left corner
% (#1,#2) and upper right (#3,#4). Now, consider the transformation
% that scales and translates R so that the result T has the same
% center as S and has maximal size while still being inside S. This
% transformation gets installed in a new graphics group, which must be
% ended with a corresponding \pgfsys@endviewbox.

\def\pgfsys@viewboxslice#1#2#3#4#5#6#7#8{\pgfsys@beginscope\pgf@sys@default@viewbox@impl{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{>}}
% Works like \pgfsys@viewboxmeet, but R3 will have minimal size so
% that in contains all of R2.

\def\pgfsys@endviewbox{\pgfsys@endscope}
% Ends a viewbox scope started by either of the previous two commands.


\def\pgf@sys@default@viewbox@impl#1#2#3#4#5#6#7#8#9{{%
    \pgf@x#1%
    \pgf@y#2%
    \pgf@xa#3%
    \pgf@ya#4%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgfmathdivide@\pgf@xa\pgf@ya%
    \let\aspectr\pgfmathresult%
    \pgf@xb#5%
    \pgf@yb#6%
    \pgf@xc#7%
    \pgf@yc#8%
    \advance\pgf@xc by-\pgf@xb%
    \advance\pgf@yc by-\pgf@yb%
    \pgfmathdivide@\pgf@xc\pgf@yc%
    \let\aspects\pgfmathresult%
    \ifdim\aspectr pt#9\aspects pt%
      \pgfmathdivide@\pgf@xa\pgf@xc%
    \else%
      \pgfmathdivide@\pgf@ya\pgf@yc%
    \fi%
    \advance\pgf@x by.5\pgf@xa%
    \advance\pgf@xb by.5\pgf@xc%
    \advance\pgf@y by.5\pgf@ya%
    \advance\pgf@yb by.5\pgf@yc%
    \pgfsys@transformcm{\pgfmathresult}{0}{0}{\pgfmathresult}{\pgf@x}{\pgf@y}%
    \pgfsys@transformcm{1}{0}{0}{1}{-\pgf@xb}{-\pgf@yb}%
  }%
}




%
%
% Graphic state saving and restoring.
%
%

\def\pgfsys@beginscope{\pgf@sys@fail{scoping}}
% Saves the current graphic state on a graphic state stack. All
% changes to the graphic state parameters mentioned for \pgfsys@stroke
% and \pgfsys@fill will be local to the current graphic state and will
% the old values will be restored after endscope is used.
%
% WARNING: pdf and postscript differ with respect to the question of
% whether the current path is part of the graphic state or not. For
% this reason, you should never use this command unless the path is
% currently empty. For example, it might be a good idea to use
% discardpath prior to calling this command.

\def\pgfsys@endscope{\pgf@sys@fail{scoping}}
% Restores the last saved graphic state.

\def\pgfsys@begin@idscope{%
  \begingroup%
    \edef\pgf@sys@cacheref{\pgfsys@id@refcurrent}%
    \expandafter\let\expandafter\pgfsys@beg@save\csname pgf@sys@att@beg@\pgf@sys@cacheref\endcsname%
    \expandafter\let\expandafter\pgfsys@end@save\csname pgf@sys@att@end@\pgf@sys@cacheref\endcsname%
    \ifx\pgfsys@beg@save\relax%
      \ifx\pgfsys@end@save\relax%
      \else%
        \pgfsys@call@save%
      \fi%
    \else%
      \pgfsys@call@save%
    \fi%
    \pgfsys@invalidate@currentid%
      \begingroup%
}
% Starts an "id scope" where the current value of \pgfsys@use@id and
% \pgfsys@use@type is used. If the combination has been used before,
% nothing happens. Otherwise, depending of the driver, a graphic
% scope may or may not be created. To ensure that a graphic scope is
% created, use \pgfsys@beginscope additionally.

\def\pgfsys@call@save{%
  \pgfsys@beginscope%
  \pgfsys@beg@save%
  \expandafter\global\expandafter\let\csname pgf@sys@att@beg@\pgfsys@id@refcurrent\endcsname\relax%
  \expandafter\global\expandafter\let\csname pgf@sys@att@end@\pgfsys@id@refcurrent\endcsname\relax%
}

\def\pgfsys@end@idscope{
      \endgroup%
    \ifx\pgfsys@beg@save\relax%
      \ifx\pgfsys@end@save\relax%
      \else%
        \pgfsys@call@end%
      \fi%
    \else%
      \pgfsys@call@end%
    \fi%
  \endgroup
}
% Ends an id scope.

\def\pgfsys@call@end{%
  \pgfsys@end@save%
  \pgfsys@endscope%
}


\def\pgfsys@begin@text{}
% Inside a text box you should not use graphics command. However, TikZ
% needs to insert some color commands at the beginnings of text
% boxes. For most drivers, this is not a problem; except for SVG,
% where every change of the graphics state opens a scope and needs a
% closing scope. This command should be used at the beginning of text
% boxes containing such color commands and the matching
% \pgfsys@end@text at the end. If the box does not contain commands
% that change the graphics state, this command is not needed.

\def\pgfsys@end@text{}
% Closes a \pgfsys@begin@text.



%
%
% Id management (all of these commands have a default implementation
% any typically need not be redefined by a driver)
%
%

% The id count
\newcount\pgf@sys@id@count

\def\pgfsys@new@id#1{%
  \edef#1{pgf\the\pgf@sys@id@count}%
  \global\advance\pgf@sys@id@count by1\relax%
}
% Creates a new id and stores it in the macro #1.

\def\pgfsys@use@id#1{%
  \edef\pgf@sys@id@current@id{#1}%
  \let\pgfsys@current@type\pgfutil@empty%
}
\let\pgf@sys@id@current@id\pgfutil@empty
% Sets the id to be used for the next graphic object (group, box, or
% path). The type is reset to be empty. #1 must be a macro name that
% has previously been set using \pgfsys@new@id.
%
% Each combination of id and type can be used only once, on a second
% use nothing happens.

\def\pgfsys@clear@id{%
  \let\pgf@sys@id@current@id\pgfutil@empty%
}
% Clears the current id, so nothing can be referenced.

\def\pgfsys@use@type#1{%
  \edef\pgfsys@current@type{#1}%
  \pgfsys@register@type\pgfsys@current@type%
}
\let\pgfsys@current@type\pgfutil@empty
% Sets the type to be used for the next graphic object.

\def\pgfsys@append@type#1{%
  \ifx\pgfsys@current@type\pgfutil@empty%
    \pgfsys@use@type{#1}%
  \else%
    \pgfsys@use@type{\pgfsys@current@type.#1}%
  \fi%
}
% Appends something to the current type

\def\pgfsys@register@type#1{%
  \expandafter\let\expandafter\pgf@sys@temp\csname pgf@sys@reg@type@#1\endcsname%
  \ifx\pgf@sys@temp\relax%
    {%
      \c@pgf@counta\pgf@sys@type@count\relax%
      \global\advance\c@pgf@counta by1\relax%
      \edef\pgf@sys@type@count{\the\c@pgf@counta}%
      \expandafter\xdef\csname pgf@sys@reg@type@#1\endcsname{y\the\c@pgf@counta}%
    }%
  \fi%
}
% Registers a type with the system. Must be called before any use of
% the type
\def\pgf@sys@reg@type@{}
\def\pgf@sys@reg@type@background{b}
\def\pgf@sys@reg@type@path{p}
\def\pgf@sys@reg@type@text{t}
\expandafter\def\csname pgf@sys@reg@type@background.path\endcsname{bp}
\def\pgf@sys@type@count{0}

\def\pgfsys@push@type{%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgf@sys@typestack%
  \expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\pgfsys@current@type%
    \expandafter\expandafter\expandafter{\expandafter\pgfsys@current@type\expandafter}%
    \expandafter\def\expandafter\pgf@sys@typestack\expandafter{\pgf@sys@typestack}}%
}
\let\pgf@sys@typestack\pgfutil@empty
% Pushes the current type onto a global stack. This is useful for
% temporarily changing the type without creating \TeX scopes.

\def\pgfsys@pop@type{\pgf@sys@typestack}
% Pops the last id from the stack.

\def\pgfsys@id@ref#1#2{#1\csname pgf@sys@reg@type@#2\endcsname}
% Expands to a text that can be inserted as a reference. #1 must be a
% reference created \pgfsys@new@id, #2 must be a type that has been
% registered using \pgfsys@id@register@type.

\def\pgfsys@id@refcurrent{\pgfsys@id@ref{\pgf@sys@id@current@id}{\pgfsys@current@type}}
% Expands to a text that can be inserted as a reference to the current
% id-type pair in use.

\def\pgfsys@invalidate@currentid{%
  \expandafter\global\expandafter\let\csname pgf@sys@id@keylist@\pgfsys@id@refcurrent\endcsname\pgfutil@empty%
}
% Mark the current id-type pair as used.

\def\pgfsys@attach@to@id#1#2#3#4{%
  \pgfsys@register@type{#2}%
  \expandafter\def\expandafter\pgf@sys@tempbeg\expandafter{\csname pgf@sys@att@beg@\pgfsys@id@ref{#1}{#2}\endcsname}%
  \expandafter\def\expandafter\pgf@sys@tempend\expandafter{\csname pgf@sys@att@end@\pgfsys@id@ref{#1}{#2}\endcsname}%
  \expandafter\ifx\pgf@sys@tempbeg\relax%
    \expandafter\let\pgf@sys@tempbeg\pgfutil@empty%
  \fi%
  \expandafter\ifx\pgf@sys@tempend\relax%
    \expandafter\let\pgf@sys@tempend\pgfutil@empty%
  \fi%
  \expandafter\let\expandafter\pgf@sys@tempbeg@cont\pgf@sys@tempbeg%
  \expandafter\let\expandafter\pgf@sys@tempend@cont\pgf@sys@tempend%
  \expandafter\expandafter\expandafter\gdef\expandafter\pgf@sys@tempbeg\expandafter{\pgf@sys@tempbeg@cont#3}%
  \def\pgf@sys@temp{#4}%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\pgf@sys@tempend\expandafter\expandafter\expandafter{\expandafter\pgf@sys@temp\pgf@sys@tempend@cont}%
}
% Attaches some code to an id-type pair so that when the id's scope
% gets created, #3 is added at the beginning and #4 is added at the
% end.

\def\pgfsys@if@fresh@id#1#2#3#4{%
  \edef\pgf@sys@temp{#1}%
  \ifx\pgf@sys@temp\pgfutil@empty% empty id always counts as "has been used"
    #4%
  \else%
    \pgfsys@register@type{#2}%
    \expandafter\ifx\csname pgf@sys@id@keylist@\pgfsys@id@ref{#1}{#2}\endcsname\pgfutil@empty%
      % has already been used!
      #4%
    \else%
      #3%
    \fi%
  \fi%
}
% Checks whether a given id-type pair #1-#2 has not been used, yet. If
% so, #3 is executed, otherwise #4.

\def\pgfsys@if@fresh@currentid#1#2{%
  \ifx\pgf@sys@id@current@id\pgfutil@empty% empty id always counts as "has been used"
    #2%
  \else%
    \expandafter\ifx\csname pgf@sys@id@keylist@\pgfsys@id@refcurrent\endcsname\pgfutil@empty%
      % has already been used!
      #2%
    \else%
      #1%
    \fi%
  \fi%
}
% Checks whether the current id-type pair in use has not been used,
% yet. If so, #1 is executed, otherwise #2.




%
%
% Special commands
%
%

\def\pgfsys@imagesuffixlist{}
% A list of suffixes, separated by `:', that will be tried when
% searching for an image.



%
%
% Transparency
%
%

\def\pgfsys@opacity#1{\pgfsys@stroke@opacity{#1}\pgfsys@fill@opacity{#1}}
% Ideally, this should sets the opacity of all operations, treating
% the group as a transparency group with 1 meaning fully opaque, 0
% meaning fully transparent. Since most drivers do not support this,
% the fallback is to set the stroke and fill opacity at the same
% time. This is not quite the same, however.

\def\pgfsys@stroke@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of stroking operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@fill@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of filling operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@transparencygroupfrombox#1{\pgf@sys@fail{transparency groups}}
% This takes a TeX box and converts it into a transparency
% group. This means that any transparency settings apply to the box as
% a whole. For instance, if a box contains two overlapping black
% circles and you draw them normally with 50% transparency, then the
% overlap will be darker than the rest. By comparison, if the circles
% are part of a transparency group, the overlap will get the same
% color as the rest.
%
% The following settings modify the behaviour of a transparency group:

\newif\ifpgfsys@transparency@group@isolated
\newif\ifpgfsys@transparency@group@knockout


\def\pgfsys@blend@mode#1{\pgf@sys@fail{blend mode}}
% Sets the current blend mode. See the PDF specification for details
% on blend modes.


\def\pgfsys@definemask{\pgf@sys@fail{image masks}}
% This command declares a mask for usage with images. It works similar
% to \pgfsys@defineimage: Certain macros are set when the command is
% called. The result should be to set the macro \pgf@mask to a pdf
% object count that can subsequently be used as a soft mask. The
% following macros will be set when this command is invoked:
%
% - \pgf@filename
%   File name of the mask to be defined.
%
% - \pgf@maskmatte
%   The so-called matte of the mask (see the pdf documentation for
%   details). The matte is a color specification consisting of 1, 3 or
%   4 numbers between 0 and 1. The number of numbers depends on the
%   number of color channels in the image (not in the mask!). It will
%   be assumed that the image has been preblended with this color.

\def\pgfsys@fadingfrombox#1#2{\pgf@sys@fail{fadings}}
% Declares an fading named #1. The parameter #2 must be a
% box. Its contents luminosity determines the opacity of the resulting
% mask.

\def\pgfsys@usefading#1#2#3#4#5#6#7{\pgf@sys@fail{fadings}}
% Installs a previously declared fading #1 in the current graphics
% state. Parameters #2 to #7 specify a transformation cm that should
% be applied to the mask before it is used.

\def\pgfsys@clipfading{}
% This default implementation is a no-op for all drivers except `dvips'
% where we have to set the clipping path _before_ installing the fading (used in
% \pgfsetfadingforcurrentpath, \pgfsetfadingforcurrentpathstroked commands of
% the basic layer)


%
%
% Shading commands
%
%

\def\pgfsys@horishading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a horizontal shading for later use. The effect of this
% command should be the definition of a macro called `@pgfshading#1!'
% (or \csname @pdfshading#1!\endcsname, to be precise). When invoked,
% this new macro should insert a shading at the current position.
%
% #1 is the name of the shading, which is also used in the output
% macro name. #2 is the height of the shading and must be given as a
% TeX dimension like `2cm' or `10pt'. #3 is a shading color
% specification as specified in the pgfuserguide. The shading
% specification implicitly fixes the width of the shading.
%
% When `@pgfshading#1!' is invoked, it should insert a box of height
% #2 and the width implicit in the shading declaration.

\def\pgfsys@vertshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Like horishading, only for vertical shadings. This time, the height
% of the shading is implicit in #3 and the width is given as #2.

\def\pgfsys@radialshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a radial shading. Like the previous macros, this command
% should setup the macro `@pgfshading#1!', which upon invocation
% should insert a radial shading whose size is implicit in #3.
%
% The parameter #2 is a pgf point specification if the starting point
% of the shading. See the pgfuserguide for details.

\def\pgfsys@functionalshading#1#2#3#4{\pgf@sys@fail{shadings (functional)}\pgf@sys@noshading{#1}}
% Declares a shading using a PostScript-like function that provides a
% color for each point. Like the previous macros, this command
% should setup the macro `@pgfshading#1!' so that it will produce a
% box containing the desired shading.
%
% Parameter #1 is the name of the shading. Parameter #4 is a
% Postscript-like function (type 4 function of the PDF specification)
% as described in Section 3.9.4 of the PDF Specification version 1.7.
% Parameter #2 and #3 are pgf point specifications that specifies the
% lower left and upper right coordinate.
%
% When function #4 is evaluated, the coordinate of the current
% point will be on the (virtual) PostScript stack in bp units. After
% the function has been evaluated, the stack should consist of three
% numbers (not integers! - the Apple PDF renderer is broken in this
% regard, so add cvr's at the end if needed) that represent the red,
% green, and blue components of the color.
%
% A buggy #4 will result is *totally unpredictable chaos* during
% rendering.

\def\pgf@sys@noshading#1{\expandafter\global\expandafter\let\csname @pgfshading#1!\endcsname=\pgfutil@empty}




%
%
% Pattern stuff
%
%

\def\pgfsys@declarepattern#1#2#3#4#5#6#7#8#9{\pgf@sys@fail{patterns}}
% This command declares a new colored or uncolored pattern. Uncolored
% patterns have no inherent color, the color is provided when they are
% set. Colored patters have an inherent color.
% #1       = name of the pattern (must be a plain suffix for use in
%            postscript/pdf/etc.)
% #2 to #5 = four coordinates describing the corners of a bounding box
%            of pattern cells
% #6       = x-step
% #7       = y-step
% #8       = pattern code
% #9       = 0 if uncolored patter, 1 if colored pattern.

\def\pgfsys@setpatternuncolored#1#2#3#4{\pgf@sys@fail{patterns}}
% Sets an uncolored pattern #1 as filling color. The numbers #2, #3,
% #4 must be an rgb-value to be used as the color of the pattern.

\def\pgfsys@setpatterncolored#1{\pgf@sys@fail{patterns}}
% Sets an colored pattern #1 as filling color.





%
%
% Animations
%
%


\newif\ifpgfsysanimationsupported
% Will be set to true by a driver when animations are supported. Note
% that snapshots are always supported.


\def\pgfsys@animate#1{\pgf@sys@fail{animations}}
% Adds an animation of the attribute #1 to the current scope.
% The configuration of the animation (like start times, etc.) is taken
% from the current values of the animation keys, which are configured
% using calls to \pgfsys@animation@..., which setup an animation
% key for the local scope. This means that you typically setup these
% keys in a scope and at the end of the scope call \pgfsys@animate.
%
% Some keys accumulate (like begin or keytime), most do not. In those
% cases, the last call overrides the previous one.
%
% Not all value types make sense or are allowed, it depends on the
% specific \pgfsys@animate call.
%
% Example:
%
% {
%   \pgfsys@animation@offset{10}{begin}%
%   \pgfsys@animation@event{}{click}{1}{begin}%
%   \pgfsys@animation@time{5}{1}{1}{0}{0}
%   \pgfsys@animation@val@scalar{1}
%   \pgfsys@animation@time{8}{1}{1}{0}{0}
%   \pgfsys@animation@val@scalar{0.5}
%   \pgfsys@animation@sum%
%   \pgfsys@animate{fillopacity}%
% }
%
% When a driver does not support a specific attribute #1, it should
% issue a \pgf@sys@fail. Typical attributes are things like "opacity"
% or "linewidth" or "dash".
%
% The following values are permissible for "#1":
%
% "opacity" adds an animation of the opacity.
% Type: scalar
%
% "fillopacity" adds an animation of the fill opacity.
% Type: scalar
%
% "strokeopacity" adds an animation of the stroke opacity.
% Type: scalar
%
% "visibility" adds an animation of the visibility.
% Type: text ("visible" or "hidden")
%
% "linewidth" adds an animation of the line width.
% Type: dimension
%
% "dash" adds an animation of the dash.
% Type: dash
%
% "translate" adds an animation of the transformation.
% Type: translate
%
% "scale" adds an animation of the transformation.
% Type: scale
%
% "rotate" adds an animation of the transformation.
% Type: scalar
%
% "skewx" adds an animation of the transformation.
% Type: scalar
%
% "skewy" adds an animation of the transformation.
% Type: scalar
%
% "motion" adds a movement along a path.
% Type: motion
%
% "strokecolor" adds an animation of the stroke color.
% Type: color
%
% "fillcolor" adds an animation of the fill color.
% Type: color
%
% "viewbox" adds an animation of the view box.
% Type: view box
%
% "path" adds an animation of the path to the path specified by
% \pgfsys@animation@whom
% Type: path
%
% "syncbase" adds a sync base to the animation. A sync base does not animate
% anything by itself, but other animations can begin and end relative
% to it.
%
% "none" suppresses the animation
% Type: any




% Animation timing :
%
% You specify an animation using a timeline. A timeline consists of a
% sequence of times together with values for these times. The times
% must be given in increasing order. You use the command
% \pgfsys@animation@time to specify a time and
% \pgfsys@animation@val@... to specify a value. The time must be
% specified first, the time--value is created when the value command is
% used.
%
% Times are given in seconds (so 0.01 is one hundredth of a second).
%
% The animation's timeline will start with the first time mentioned
% (not necessarily zero and not necessarily a positive value) and ends
% with the last value. The duration is the difference between these
% two values.

\def\pgfsys@animation@restart@always{}
% Specifies that the animation can always restart

\def\pgfsys@animation@restart@never{}
% Specifies that the animation should never restart

\def\pgfsys@animation@restart@whennotactive{}
% Specifies that the animation should only restart when it is not active

\def\pgfsys@animation@repeat#1{}
% #1 must be a number

\def\pgfsys@animation@repeat@indefinite{}
% Repeats forever

\def\pgfsys@animation@repeat@dur#1{}
% #1 must be a clock value

\def\pgfsys@animation@freezeatend{}
% Specifies that the last value of the animation remains in force at
% the end

\def\pgfsys@animation@removeatend{}
% Specifies that the effect of the animation is removed at the end

\def\pgfsys@animation@time#1#2#3#4#5{}
% Specifies a time together with spline control points for the entry
% and the exit to this time. The value #1 is a time in seconds (so 60
% means 1 minute, 0.001 means one millisecond). The values #2 and #3
% specify the control point of the spline *entering* the time point,
% while the values #4 and #5 specify the control point of the spline
% *leaving* the time point. They are all dimensionless values between
% 0 and 1. For a linear animation, set the first two to 1 and the last
% two to 0.
%
% Example:
% \pgfsys@animation@time{5}{1}{1}{0.25}{0.1}
% \pgfsys@animation@val@scalar{80}
% \pgfsys@animation@time{8}{.75}{1}{0}{0}
% \pgfsys@animation@val@scalar{90}
%
% In SVG, this will create the following entries:
% begin     = +5s
% duration  = 3s
% keyTimes  = 0;1
% values    = 80;90
% keySpline = 0.25 0.1 0.75 1
%
% For the key spline, note that the entry spline controls of the first
% time and the exit spline controls of the last point are dropped.
%
%
% When the exit spline takes the special values #4="stay" and #5="0",
% the attribute's value "stays" until the next value for the next time
% (it "jumps" to the next value then). This corresponds, roughly, to
% an "infinite" #4.
%
% Similarly, when the entry spline takes the special value #2="jump"
% and #3="1", the value immediately jumps from the previous value to
% the next value when the previous value was "created".

\def\pgfsys@stay@text{{stay}{0}}
\def\pgfsys@jump@text{{jump}{1}}

\def\pgfsys@animation@base{}
% Think of this command as setting the value of the attribute in the
% timeline before the timeline starts. Normally, an animation only
% influences the timeline while the animation is running (which may be
% forever) and before and after the animation is running, the
% attribute's value is not modified by the animation (so, it is just
% inherited from the surrounding scope). When a base value is set,
% while the animation is not running, this value is used. For most
% attributes you can achieve the same effect by surrounding the
% to-be-animated object by a scope and setting the value there, but
% using bases is often more convenient and, for instance for the
% visibility attribute, it is necessary to use a base.
%
% Note that when a backend driver does not support animations, base
% values will not be depicted unless a snapshot is used explicitly.

\def\pgfsys@animation@offset#1#2{}
% #1 must be a value in seconds, #2 is the target "begin" or "end" to
% which this offset is appended.

\def\pgfsys@animation@syncbegin#1#2#3#4{}
% #1 is the id of a sync base (obtained by
% \pgfsys@new@id), #2 is the id type (or empty), #3 is an optional
% offset, #4 is the target.

\def\pgfsys@animation@syncend#1#2#3#4{}
% Like the previous command.

\def\pgfsys@animation@event#1#2#3#4#5{}
% #1 is the optional id of another element (obtained by
% \pgfsys@new@id), #2 is the optional type of the id, #3 is an event
% name, #4 is an optional offset, #5 is the target.

\def\pgfsys@animation@repeat@event#1#2#3#4#5{}
% #1 is the optional id of another element, #2 is the type, #3 is a
% repeat count, and #4 is an optional offset, #5 is the target.

\def\pgfsys@animation@accesskey#1#2#3{}
% #1 is a character, #2 is an optional offset, #3 is the target.

\def\pgf@sys@begin@text{begin}


% Accumulation

\def\pgfsys@animation@accumulate{}
% Corresponds to accumulate="sum" in SVG

\def\pgfsys@animation@noaccumulate{}
% Corresponds to accumulate="none" in SVG


% Targeting

\def\pgfsys@animation@whom#1#2{}
% Sets the target of the animation. #1 must be an id previously
% created using \pgfsys@new@id and #2 must be empty or a type
% previously created using \pgfsys@new@id@type


% Attribute definitions

\def\pgfsys@animation@rotatealong{}
% Applicable only to motion animations. Indicates that the
% to-be-animated group should be rotated automatically so that it
% points along the path as time progresses.

\def\pgfsys@animation@norotatealong{}
% Corresponds to rotate="0"

\def\pgfsys@animation@movealong#1{}
% Applicable only to motion animations. #1 is a softpath along which
% the movement will be done.

\def\pgfsys@animation@tip@markers#1#2{}
% Applicable only to path animations. #1 and #2 are markers (declared
% using \pgfsys@marker@declare) that store marker symbols to be added
% at the start and at the end of the to-be-animated path. If empty, no
% markers are added.

\def\pgfsys@animation@canvas@transform#1#2{}
% #1 is some code that may call \pgfsys@transformcm at most once. It
% will be executed when a canvas transformation animation is
% installed for a scope id. #2 is some further codes that may also
% call \pgfsys@transformcm at most once. It will be installed right
% after the animation.
%
% Typically, #1 is some pgf coordinate shift followed by
% {\pgflowlevelsynccm} and #2 is \pgftransforminvert followed by
% \pgflowlevelsynccm.



% Values

\def\pgfsys@animation@val@current{}
% The current value of the attribute. At least with SVG, this can only
% be used for the first value and, then, only if there is only one
% other value.

\def\pgfsys@animation@val@text#1{}
% #1 should be some text.

\def\pgfsys@animation@val@scalar#1{}
% #1 should be a single value.

\def\pgfsys@animation@val@dimension#1{}
% #1 must be a dimension.

\def\pgfsys@animation@val@color@rgb#1#2#3{}
% #1,#2,#3 must be an rgb tuple

\def\pgfsys@animation@val@color@cmyk#1#2#3#4{}
% #1,#2,#3,#4 must be an cmyk tuple

\def\pgfsys@animation@val@color@cmy#1#2#3{}
% #1,#2,#3 must be an cmy tuple

\def\pgfsys@animation@val@color@gray#1{}
% #1 must be a gray value

\def\pgfsys@animation@val@path#1{}
% #1 must consist of path-construction tokens (as returned by the
% softpath layer)

\def\pgfsys@animation@val@translate#1#2{}
% #1,#2 must be dimensions

\def\pgfsys@animation@val@scale#1#2{}
% #1,#2 must be dimensionless

\def\pgfsys@animation@val@viewbox#1#2#3#4{}
% #1,#2 describe the lower left, #3,#4 the upper right corner of the
% view box.

\def\pgfsys@animation@val@dash#1#2{}
% #1,#2 have the syntax of \pgfsys@setdash.



%
%
% Markers
%
%

\def\pgfsys@marker@declare#1#2{%
  {%
    \pgfpicturetrue%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@marker@temp%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    \pgfsys@beginscope%
    #2%
    \pgfsys@endscope%
    \xdef#1{\the\pgf@sys@id@count}%
    \expandafter\expandafter\expandafter\global\expandafter\pgfsysprotocol@getcurrentprotocol\csname pgf@sys@marker@prot@#1\endcsname%
    \pgfsys@marker@declare@% curtesy hook
    \pgfsysprotocol@setcurrentprotocol\pgfsys@marker@temp%
    \global\advance\pgf@sys@id@count by1\relax%
  }%
}
\let\pgfsys@marker@declare@\relax
% Declares a new marker symbol whose code is in #2. #1 should be a
% macro name, which will be set to a unique
% value by which the marker can be referenced later on. #2 should be
% code that, when executed, produces recordable code.

\def\pgfsys@marker@use#1{%
  \pgfsysprotocol@literal{\csname pgf@sys@marker@prot@#1\endcsname}%
}
% Draws the marker symbol not at the end of a path, but simply with
% the current transformation matrix






%
%
% RDF
%
%

\def\pgfsys@rdf@about#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute "about" with value #1 to the next
% idscope. The RDF-spec says: "a SafeCURIEorCURIEorIRI, used for
% stating what the data is about (a 'subject' in RDF terminology);"

\def\pgfsys@rdf@content#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute content with value #1 to the next
% idscope. The RDF-spec says: "a CDATA string, for supplying
% machine-readable content for a literal (a 'literal object', in RDF
% terminology);"

\def\pgfsys@rdf@datatype#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute datatype with value #1 to the next
% idscope. The RDF-spec says: "a TERMorCURIEorAbsIRI representing a
% datatype, to express the datatype of a literal;"

\def\pgfsys@rdf@href#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute href with value #1 to the next idscope
% The RDF-spec says: "a traditionally navigable IRI for
% expressing the partner resource of a relationship (a 'resource
% object', in RDF terminology);"

\def\pgfsys@rdf@inlist{\pgf@sys@fail{rdf}}
% Adds the rdf attribute inlist to the next idscope. The
% RDF-spec says: "An attribute used to indicate that the object
% associated with a rel or property attribute on the same element is
% to be added to the list for that predicate. The value of this
% attribute must be ignored. Presence of this attribute causes a list
% to be created if it does not already exist."

\def\pgfsys@rdf@prefix#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf prefix attribute to the next
% idscope. Can be called several times, in which case all values of #1
% are concatenated with whitespaces. The RDF-spec says: "a white space
% separated list of prefix-name IRI pairs of the form NCName ':' ' '+
% xsd:anyURI"

\def\pgfsys@rdf@property#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf property attribute to the next
% idscope. Can be called repeatedly. The RDF-spec says: "a white space
% separated list of TERMorCURIEorAbsIRIs, used for expressing
% relationships between a subject and either a resource object if
% given or some literal text (also a 'predicate');"

\def\pgfsys@rdf@rel#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf rel attribute to the next
% next idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of
% TERMorCURIEorAbsIRIs, used for expressing relationships between two
% resources ('predicates' in RDF terminology);"

\def\pgfsys@rdf@resource#1{\pgf@sys@fail{rdf}}
% Adds the rdf attribute resource with value #1 to the next idscope. The
% RDF-spec says: "a SafeCURIEorCURIEorIRI for expressing the partner
% resource of a relationship that is not intended to be navigable
% (e.g., a 'clickable' link) (also an 'object');"

\def\pgfsys@rdf@rev#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf rev attribute to the next
% idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of
% TERMorCURIEorAbsIRIs, used for expressing reverse relationships
% between two resources (also 'predicates');

\def\pgfsys@rdf@src#1{\pgf@sys@fail{rdf}}
% Adds an rdf attribute src with value #1 to the next idscope. The
% RDF-spec says: "an IRI for expressing the partner resource of a
% relationship when the resource is embedded (also a 'resource
% object');"

\def\pgfsys@rdf@typeof#1{\pgf@sys@fail{rdf}}
% Adds #1 to the list of the rdf typeof attribute to the next
% idscope. Can be called repeatedly. The
% RDF-spec says: "a white space separated list of TERMorCURIEorAbsIRIs
% that indicate the RDF type(s) to associate with a subject;"

\def\pgfsys@rdf@vocab#1{\pgf@sys@fail{rdf}}
% Adds an rdf attribute vocab with value #1 to the next idscope. The
% RDF-spec says: "an IRI that defines the mapping to use when a TERM
% is referenced in an attribute value. See General Use of Terms in
% Attributes and the section on Vocabulary Expansion."



%
%
% Page size stuff
%
%

\def\pgfsys@papersize#1#2{\pgf@sys@fail{papersize}}
% This command sets the paper size in a portable way. It tries to do
% so "locally" for the current page, but what really happens depends
% strongly on the driver. For instance, dvips will use whatever is
% used with the first call to this command that is part of the
% shipped-out document and will ignore all other uses. In contrast,
% pdftex will use the current value of the papersize for each page
% and, additionally, setting the papersize is local to the current TeX
% group.
% #1 = width
% #2 = height

\def\pgfsys@global@papersize#1#2{\pgfsys@papersize{#1}{#2}}
% This command does the same as the papersize command, only for
% drivers that support this, \global is used to set the papersize.
% #1 = width
% #2 = height

\def\pgfsys@prepare@papersize#1#2{\pgfsys@papersize{#1}{#2}}
% Like \pgfsys@papersize, this prepares the paper size in a portable
% way -- but it is supposed to be a preparation step before the
% document has started. Drivers may decide to postpone the action
% until the document has started.
%
% The root cause why I added this method is that image externalization
% seems to suffer from the fact that some drivers need a "prepared"
% routine whereas others must not have a prepared routine and have to
% apply the action right-away. This method is the solution for image
% externalization.
% #1 = width
% #2 = height

\ifx\paperheight\@undefined
  \def\pgfsys@thepageheight{\the\vsize} % this is wrong, but I do not
                                % know how to compute the page height
                                % in plain tex.
  \def\pgfsys@thepagewidth{\the\hsize}
\else
  \def\pgfsys@thepageheight{\paperheight}
  \def\pgfsys@thepagewidth{\paperwidth}
\fi


%
%
% Position tracking commands
%
%

% Marks the current position on the page. This position can later be
% referenced using \pgfsys@getposition
\def\pgfsys@markposition#1{\pgf@sys@fail{marking the current position}}

% Sets #2 to a pgfpoint macro that returns the position #1 is
% returned in a coordinate system where the x-axis goes right and the
% y-axis goes up. The origin of this coordinate system may or may not
% lie in the lower left corner; you should shift the coordinate system
% to the position "pgfpageorigin" to make sure that the origin is at
% the lower left corner. Typically, getting this position
% requires two runs of TeX. On the first run, the macro will be set to
% \relax, indicating that the position is not available.
%
% If #1 is set to the special position "pgfpageorigin", the position
% of the the lower left page corner is returned.

\def\pgfsys@getposition#1#2{\let#2=\relax}



%
%
% Commands having a default implementation. These commands only need
% not be implemented by drivers if this results in a better
% performance.
%
%


\def\pgfsys@shadingoutsidepgfpicture#1{%
  #1%
}
% This command gets the definition of a shading (@pgfshadingxxxx!) as
% an argument and should insert this shading into the normal text.
%
% This command has a default implementation.


\def\pgfsys@shadinginsidepgfpicture#1{%
  \pgf@makehbox{#1}%
  \setbox\pgf@hbox=\hbox{\hskip-.5\wd\pgf@hbox\lower.5\ht\pgf@hbox\hbox{\box\pgf@hbox}}%
  \pgfqbox{\pgf@hbox}%
}
% This command works like \pgfsys@shadingoutsidepgfpicture, only it is
% called when a shading should be inserted inside a picture. This
% command should insert the shading centered on the origin (which will
% typically have been low-level translated somewhere else.)
%
% This command has a default implementation.


\def\pgfsys@hbox#1{%
  \pgfsys@begin@idscope%
  \pgfsys@beginscope%
    \setbox#1=\hbox{\box#1}%
    \wd#1=0pt%
    \ht#1=0pt%
    \dp#1=0pt%
    \box#1%
  \pgfsys@endscope%
  \pgfsys@end@idscope%
}
% Called to insert a TeX hbox into a pgfpicture.

\def\pgfsys@hboxsynced#1{%
  \pgfsys@beginscope\pgflowlevelsynccm\pgfsys@hbox#1\pgfsys@endscope%
}%
% Called to insert box #1 into a pgfpicture, but with the current
% coordinate transformation matrix synced with the canvas
% transformation matrix and surrounded by a scope.
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfsys@hbox#1. However, a
% ``TeX-translation'' is used for the translation part of the
% transformation cm. This will ensure that hyperlinks ``survive'' at
% least translations.

\def\pgfsys@pictureboxsynced#1{%
  {%
    \setbox0=\hbox{\pgfsys@beginpicture\box#1\pgfsys@endpicture}%
    \pgfsys@hboxsynced0%
  }%
}
% Basically, this should do the same as doing a (scoped) low level sync
% followed by inserting the box #1 directly into the output
% stream. However, the default implementation uses \pgfsys@hboxsynced
% in conjunction with \pgfsys@beginpicture to ensure that, if
% possible, hyperlinks survive in pdfs. Drivers that are sensitive to
% picture-in-picture scopes should replace this implementation by
% \pgfsys@beginscope\pgflowlevelsynccm\box#1\pgfsys@endscope

\def\pgfsys@beginpicture{}
% Called at the beginning of a pgfpicture. Used to setup things.

\def\pgfsys@endpicture{}
% Called at the end of a pgfpicture.

\def\pgfsys@typesetpicturebox#1{%
  \pgf@ya=\pgf@shift@baseline\relax%
  \advance\pgf@ya by-\pgf@picminy\relax%
  %
  %
  \advance\pgf@picmaxy by-\pgf@picminy\relax% maxy is now the height
  \advance\pgf@picmaxx by-\pgf@picminx\relax% maxx is now the width
  \setbox#1=\hbox{\hskip-\pgf@picminx\lower\pgf@picminy\box#1}%
  \ht#1=\pgf@picmaxy%
  \wd#1=\pgf@picmaxx%
  \dp#1=0pt%
  \leavevmode%
  \pgf@xa=\pgf@trimleft@final\relax  \ifdim\pgf@xa=0pt \else\kern\pgf@xa\fi
  \raise-\pgf@ya\box#1%
  \pgf@xa=\pgf@trimright@final\relax \ifdim\pgf@xa=0pt \else\kern\pgf@xa\fi
}
% Called after a picture has been typeset in box #1. This
% command should insert the box into the normal TeX code. The box #1
% will still be a ``raw'' box that contains only the \special's. The
% job of this command is to resize and shift this box according to the
% baseline shift and the size of the box.
%
% This command has a default implementation.

\def\pgfsys@beginpurepicture{\pgfsys@beginpicture}
% This version of the beginpicture command can be used for pictures
% that are guaranteed not to contain any hboxes. In this case, a
% driver might provide a more compact version of the command.

\def\pgfsys@endpurepicture{\pgfsys@endpicture}
% Called at the end of a ``pure'' pgfpicture.

\def\pgfsys@defineimage{%
  \ifx\pgf@imagewidth\pgfutil@empty\else\edef\pgf@imagewidth{width=\pgf@imagewidth,}\fi%
  \ifx\pgf@imageheight\pgfutil@empty\else\edef\pgf@imageheight{height=\pgf@imageheight,}\fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepage{page=\pgf@imagepage,}\fi%
  \edef\pgf@image{\noexpand\includegraphics[\pgf@imageheight\pgf@imagewidth]{\pgf@filename}}%
}
% Called, when an image should be defined.
%
% This command does not take any parameters. Instead, certain macros
% will be preinstalled with appropriate values when this command is
% invoked. These are:
%
% - \pgf@filename
%   File name of the image to be defined.
%
% - \pgf@imagewidth
%   Will be set to the desired (scaled) width of the image.
%
% - \pgf@imageheight
%   Will be set to the desired (scaled) height of the image.
%
%   If this macro and also the height macro are empty, the image
%   should have its `natural' size.
%
%   If exactly only of them is specified, the undefined value the
%   image is scaled so that the aspect ratio is kept.
%
%   If both are set, the image is scaled in both directions
%   independently, possibly changing the aspect ratio.
%
%
% The following macros presumable mostly make sense for drivers that
% can handle pdf:
%
% - \pgf@imagepage
%   The desired page number to be extracted from a multi-page
%   `image'.
%
% - \pgf@imagemask
%   If set, it will be set to `/SMask x 0 R', where x is the pdf
%   object number of a soft mask to be applied to the image.
%
% - \pgf@imageinterpolate
%   If set, it will be set to `/Interpolate true' or  `/Interpolate
%   false', indicating whether the image should be interpolated in
%   pdf.
%
%
% The command should now setup the macro \pgf@image such that calling
% this macro will result in typesetting the image. Thus, \pgf@image is
% the `return value' of the command.


\def\pgfsys@defobject#1#2#3#4{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfpicturetrue%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    \pgfsys@beginscope%
    #4%
    \pgfsys@endscope%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@@temp%
    \expandafter\global\expandafter\let\csname #1\endcsname=\pgfsys@@temp%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Declares an object for later use. The idea is that the object can be
% precached in some way and then be rendered more quickly when used
% several times. For example, an arrow head might be defined and
% prerendered in this way.
%
% The parameter #1 is the name for later use. #2 and #3 are pgf points
% specifying a bounding box for the object. #4 is the code for the
% object. The code may only contain protocolable code.


\def\pgfsys@useobject#1#2{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedfalse%
    #2%
    \expandafter\pgfsysprotocol@setcurrentprotocol\csname #1\endcsname%
    \pgfsysprotocol@invokecurrentprotocol%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Renders a previously declared object. The first parameter is the
% name of the object. The second parameter is extra code that
% should be executed right *before* the object is rendered. Typically,
% this will be some transformation code.


\def\pgfsys@begininvisible{\pgfsys@transformcm{1}{0}{0}{1}{2000bp}{2000bp}}
% Between this command and the closing endinvisible, all output should
% be suppressed. Nothing should be drawn at all, which includes all
% paths, images and shadings. This command typically should not open a
% graphic scope.

\def\pgfsys@endinvisible{\pgfsys@transformcm{1}{0}{0}{1}{-2000bp}{-2000bp}}
% Ends the invisibility section, unless invisibility blocks have been
% nested. In this case, only the `last' one restores visibility.

\def\pgfsys@begininvisiblescope{\pgfsys@beginscope\pgfsys@begininvisible}
% Works like pgfsys@begininvisible, but it may open a graphics scope.

\def\pgfsys@endinvisiblescope{\pgfsys@endinvisible\pgfsys@endscope}
% Closes the invisibility scope.


\def\pgfsys@atbegindocument{}
% This command will be executed at the begin of the document. If for
% whatever reason this is not done, you may wish to execute this
% command yourself. It will setup certain specials that need to be
% inserted into the resulting .pdf/.ps/.xxx file.


% String comparison
\ifdefined\pdfstrcmp
  \let\pgfsys@strcmp\pdfstrcmp
\else\ifdefined\strcmp
  \let\pgfsys@strcmp\strcmp
\else\ifdefined\directlua
  \directlua{
  local lft = lua.get_functions_table()
  lft[\string#lft+1] = function()
      local lhs = token.scan_string()
      local rhs = token.scan_string()
      if lhs < rhs then
          tex.sprint(-2, "-1")
      elseif lhs == rhs then
          tex.sprint(-2, "0")
      else
          tex.sprint(-2, "1")
      end
  end
  token.set_lua("pgfsys@strcmp", \string#lft, "global")
  }
\else
  \def\pgfsys@strcmp#1#2{\pgf@sys@fail{string comparison}}%
\fi\fi\fi


% Discern the driver:

% Default driver:
\ifx\pgfsysdriver\@undefined
  \pgfutil@guessdriver
\fi

\input pgf.cfg

\immediate\write-1{Driver file for pgf: \pgfsysdriver}
\pgfutil@InputIfFileExists{\pgfsysdriver}{}{%
  \pgferror{Driver file ``\pgfsysdriver'' not found.}}



% This will insert always-present-specials at the beginning of the
% code.
\AtBeginDocument{
  \pgfsys@atbegindocument
  \let\pgfsys@atbegindocument=\pgfutil@empty
}



% Read aux file in plain and context mode:

\pgfutil@aux@read@hook


\endinput


==> pgfutil-common.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


%
% This file provides utility commands that are used throughout pgf.
%
% For most commands, the definition of these commands is just given
% below. We cannot use the LaTeX definition of these commands since
% LaTeX may not be the current format and since LaTeX packages tend to
% redefine these commands.
%
% For some commands the actual definition of the format (like latex or
% context) is to be preferred over the generic definition below. In
% this case, the definition of the format is installed when the file
% pgfutil-XXXX.tex is read, where XXXX is the format name (latex,
% plain, or context).



\catcode`\@=11\relax


% Which format is loaded?
\newif\ifpgfutil@format@is@latex
\newif\ifpgfutil@format@is@plain
\newif\ifpgfutil@format@is@context

% Aliases

\let\pgfutil@exp\romannumeral
\chardef\pgfutil@exp@end=0

% Simple stuff

% \pgfutil@trimspaces{<token list>}
%
% Removes spaces on both sides of <token list>.  Same as trimspaces.sty
\catcode`\Q=3
\def\pgfutil@trimspaces#1{%
  \romannumeral-`0\pgfutil@trimspaces@\noexpand#1Q Q}
\def\pgfutil@trimspaces@#1 Q{\pgfutil@trimspaces@@#1Q}
\def\pgfutil@trimspaces@@#1Q#2{#1}
\catcode`\Q=11

% \pgfutil@ifx{<token 1>}{<token 2>}{<true code>}{<false code>}
%
% This macro is expandable.
\long\def\pgfutil@ifx#1#2{%
  \ifx#1#2%
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

% \pgfutil@ifstrequal{<lhs>}{<rhs>}{<true code>}{<false code>}
%
% Check if <lhs> and <rhs> are equal by string comparison
%
% This macro is expandable.
\long\def\pgfutil@ifstrequal#1#2{%
  \ifnum\pgfsys@strcmp{\pgfutil@unexpanded{#1}}{\pgfutil@unexpanded{#2}}=0
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi
}

% \pgfutil@ifxempty{<token 1>}{<true code>}{<false code>}
%
% Shortcut for \pgfutil@ifx\pgfutil@empty{<token 1>}{<true code>}{<false code>}
%
% This macro is expandable.
\def\pgfutil@ifxempty{\pgfutil@ifx\pgfutil@empty}

% pgfutil@ifempty
%
% Check if #1 is empty. No expansion is performed on #1.
%
% This macro is expandable.
\long\def\pgfutil@ifempty#1{%
  \if\relax\detokenize{#1}\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

% \pgfutil@ifundefined{<macro name with backslash>}
%  {<is undefined code>}{<is defined code>}
%
% This will let #1 to \relax if it undefined.
%
% This macro is expandable.
\def\pgfutil@ifundefined#1{%
  \expandafter\pgfutil@ifx\csname#1\endcsname\relax}

% A variant of \pgfutil@ifundefined which will NOT let #1 to \relax it
% is undefined.
\def\pgfutil@IfUndefined#1{%
  \ifcsname#1\endcsname
    \expandafter\pgfutil@secondoftwo
  \else
    \expandafter\pgfutil@firstoftwo
  \fi
}

\long\def\pgfutil@firstofone#1{#1}
\long\def\pgfutil@firstoftwo#1#2{#1}
\long\def\pgfutil@secondoftwo#1#2{#2}
\def\pgfutil@empty{}
\long\def\pgfutil@gobble@until@relax#1\relax{}
\long\def\pgfutil@gobble#1{}
\long\def\pgfutil@gobbletwo#1#2{}
\def\pgfutil@namedef#1{\expandafter\def\csname #1\endcsname}
\def\pgfutil@namelet#1{\expandafter\pgfutil@@namelet\csname#1\endcsname}
\def\pgfutil@@namelet#1#2{\expandafter\let\expandafter#1\csname#2\endcsname}
\long\def\pgfutil@g@addto@macro#1#2{%
  \begingroup
    \pgfutil@toks@\expandafter{#1#2}%
    \xdef#1{\the\pgfutil@toks@}%
 \endgroup}
\newif\ifpgfutil@tempswa
\newif\ifpgfutil@tempswb

% \pgfutil@pushmacro
% \pgfutil@popmacro
%
% Macro stack.  Allows pushing a macro over \egroup.  Taken from ConTeXt

\let\pgfutil@pushmacro@string\pgfutil@empty

\def\pgfutil@pushmacro#1{%
    \xdef\pgfutil@pushmacro@string{\string#1}%
    \ifcsname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\else
        % \newcount is \outer in Plain
        \csname newcount\expandafter\endcsname\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname
    \fi
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname 1\relax
    \global\expandafter\let\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname#1%
}

\def\pgfutil@popmacro#1{%
    \xdef\pgfutil@pushmacro@string{\string#1}%
    \expandafter\let\expandafter#1\csname\the\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname\pgfutil@pushmacro@string\endcsname
    \global\advance\csname pgfutil@pushedmacro@\pgfutil@pushmacro@string\endcsname -1\relax
}

% pgfutil@ifnextchar

\long\def\pgfutil@ifnextchar#1#2#3{%
  \let\pgfutil@reserved@d=#1%
  \def\pgfutil@reserved@a{#2}%
  \def\pgfutil@reserved@b{#3}%
  \futurelet\pgfutil@let@token\pgfutil@ifnch}
\def\pgfutil@ifnch{%
  \ifx\pgfutil@let@token\pgfutil@sptoken
    \let\pgfutil@reserved@c\pgfutil@xifnch
  \else
    \ifx\pgfutil@let@token\pgfutil@reserved@d
      \let\pgfutil@reserved@c\pgfutil@reserved@a
    \else
      \let\pgfutil@reserved@c\pgfutil@reserved@b
    \fi
  \fi
  \pgfutil@reserved@c}
{%
  \def\:{\global\let\pgfutil@sptoken= } \:
  \def\:{\pgfutil@xifnch} \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ifnch}
}

% pgfutil@ignorespaces

\def\pgfutil@ignorespaces
  {\ifx\pgfutil@let@token\pgfutil@sptoken
     \expandafter\pgfutil@ignorespaces@helper
   \else
     \expandafter\pgfutil@next
   \fi}

{
  \def\:{\pgfutil@ignorespaces@helper}
  \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ignorespaces}
}

% pgfutil@in@

\newif\ifpgfutil@in@

% Usage:
% \pgfutil@in@{one}{three two one}
% \ifpgfutil@in@
%     -> will be true!
% \else
% \fi
%
% \pgfutil@in@{,}{1234,456567}
% \ifpgfutil@in@
%     -> will be true!
% \else
% \fi
\def\pgfutil@in@#1#2{%
 \def\pgfutil@in@@##1#1##2##3\pgfutil@in@@{%
  \ifx\pgfutil@in@##2\pgfutil@in@false\else\pgfutil@in@true\fi}%
 \pgfutil@in@@#2#1\pgfutil@in@\pgfutil@in@@}


% pgfutil@for

\def\pgfutil@nnil{\pgfutil@nil}
\def\pgfutil@fornoop#1\@@#2#3{}
\long\def\pgfutil@for#1:=#2\do#3{%
  \expandafter\def\expandafter\pgfutil@fortmp\expandafter{#2}%
  \ifx\pgfutil@fortmp\pgfutil@empty \else
    \expandafter\pgfutil@forloop#2,\pgfutil@nil,\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\pgfutil@nnil \else
       #5\def#4{#2}\ifx #4\pgfutil@nnil \else#5\pgfutil@iforloop #3\@@#4{#5}\fi\fi}
\long\def\pgfutil@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@iforloop\fi#2\@@#3{#4}}
\def\pgfutil@tfor#1:={\pgfutil@tf@r#1 }
\long\def\pgfutil@tf@r#1#2\do#3{\def\pgfutil@fortmp{#2}\ifx\pgfutil@fortmp\pgfutil@space\else
    \pgfutil@tforloop#2\pgfutil@nil\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@tforloop\fi#2\@@#3{#4}}

\def\pgfutil@space{ }

% pgfutil@IfFileExists

\chardef\pgfutil@inputcheck0
\def\pgfutil@IfFileExists#1#2#3{%
  \openin\pgfutil@inputcheck=#1 %
  \ifeof\pgfutil@inputcheck
     #3\relax
  \else
    #2\relax
  \fi
  \closein\pgfutil@inputcheck}

\def\pgfutil@InputIfFileExists#1#2#3{\pgfutil@IfFileExists{#1}{\input #1\relax#2}{#3}}%


% pgfutil@loop (from plain.tex)

\def\pgfutil@loop#1\pgfutil@repeat{\def\pgfutil@body{#1}\pgfutil@iterate}
\def\pgfutil@iterate{\pgfutil@body \let\pgfutil@next\pgfutil@iterate \else\let\pgfutil@next\relax\fi \pgfutil@next}
\let\pgfutil@repeat=\fi % this makes \loop...\if...\repeat skippable

% \pgfutil@switch
%
% #1: comparison function of the form
%     \comp{<lhs>}{<rhs>}{<true code>}{<false code>}
%     Has to be expandable!
% #2: lhs
% #3: sequence of rhs-value pairs
% #4: default statement in case of match
% #5: default statement in case of no match
%
% Example:
%
% \pgfutil@switch\pgfutil@ifx\pgf@let@token{%
%   {(}{\tikz@movetoabs}%)
%   {+}{\tikz@movetorel}%
%   {-}{\tikz@lineto}%
% }{}{\tikz@expand}

\let\pgfutil@scan@mark\relax
\let\pgfutil@scan@stop\relax

\long\def\pgfutil@switch#1#2#3#4#5{%
  \pgfutil@exp
  \pgfutil@switch@@{#1}%
  {#2}#3% user-defined cases
  {#2}{}% default case
  \pgfutil@scan@mark{#4}% true code
  \pgfutil@scan@mark{#5}% false code
  \pgfutil@scan@stop
}
\long\def\pgfutil@switch@@#1#2#3#4{%
  #1{#2}{#3}%
    {\pgfutil@switch@end{#4}}%
    {\pgfutil@switch@@{#1}{#2}}%
}
\long\def\pgfutil@switch@end#1#2#3\pgfutil@scan@mark#4#5\pgfutil@scan@stop{\pgfutil@exp@end#1#4}

% aux-read-hook

\let\pgfutil@aux@read@hook=\relax


% Tokens for the end of the typesetting -- they will be added at the
% end of every job (hopefully...).

\newtoks\pgfutil@everybye


%
% PDF-Resource management -- might seem strange that this is here, but
% it turns out to be the correct place since latex and context handle
% this stuff quite differently
%

% Adding something to the pdf-resources:

\def\pgfutil@addpdfresource@extgs#1{\pgf@sys@addpdfresource@extgs@plain{#1}}
\def\pgfutil@addpdfresource@colorspaces#1{\pgf@sys@addpdfresource@colorspaces@plain{#1}}
\def\pgfutil@addpdfresource@patterns#1{\pgf@sys@addpdfresource@patterns@plain{#1}}
\def\pgfutil@setuppdfresources{\pgf@sys@setuppdfresources@plain}


% Inserts the argument at the begin of the current page (hopefully)

\let\pgfutil@insertatbegincurrentpage=\relax


% Ragged left and ragged right

\def\pgfutil@raggedright{\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}
\def\pgfutil@raggedleft{\leftskip\z@ plus2em \rightskip\z@ \spaceskip.3333em \xspaceskip.5em\parfillskip0pt\relax}


% Error Messages
\def\pgfutil@packageerror#1#2#3{\errhelp{#3}\errmessage{Package #1 Error: #2}}
\def\pgfutil@packagewarning#1#2{\immediate\write17{Package #1: Warning! #2.}}
\def\pgferror#1{\pgfutil@packageerror{pgf}{#1}{}}
\def\pgfwarning#1{\pgfutil@packagewarning{pgf}{#1}}


% Library files inclusion


% Include a library file.
%
% #1 = List of names of library file.
%
% Description:
%
% This command includes a list of library files. For each file X in the
% list, the file pgflibraryX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgflibrary{arrows}
% \usepgflibrary[patterns,snakes]

\def\usepgflibrary{\pgfutil@ifnextchar[{\use@pgflibrary}{\use@@pgflibrary}}%}
\def\use@pgflibrary[#1]{\use@@pgflibrary{#1}}
\def\use@@pgflibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname pgf@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@library@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@library@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \pgfutil@InputIfFileExists{pgflibrary\pgf@temp.code.tex}{}{%
          \pgferror{I did not find the pgf library
            '\pgf@temp'. I looked for the file named
            pgflibrary\pgf@temp.code.tex, but could not find it in in
            the current texmf trees.}
        }%
      \catcode`\@=\csname pgf@library@#1@atcode\endcsname
      \catcode`\|=\csname pgf@library@#1@barcode\endcsname
      \catcode`\$=\csname pgf@library@#1@dollarcode\endcsname
      \fi%
    \fi
  }%
}


% Include a module file.
%
% #1 = List of names of module files.
%
% Description:
%
% This command includes a list of module files. For each file X in the
% list, the file pgfmoduleX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgfmodule{matrix}

\def\usepgfmodule{\pgfutil@ifnextchar[{\use@pgfmodule}{\use@@pgfmodule}}%}
\def\use@pgfmodule[#1]{\use@@pgfmodule{#1}}
\def\use@@pgfmodule#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@module@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@module@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@module@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@module@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@module@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \input pgfmodule\pgf@temp.code.tex
      \catcode`\@=\csname pgf@module@#1@atcode\endcsname
      \catcode`\|=\csname pgf@module@#1@barcode\endcsname
      \catcode`\$=\csname pgf@module@#1@dollarcode\endcsname
    \fi%
  }%
}

\def\pgfutilensuremath#1{%
  \ifmmode#1\else$#1$\fi
}


%
% Guess the driver:
%

\begingroup
    \catcode`\"=12
    \edef\pgf@loc@TMPa{"}%
    %
    % prepares file names by checking for double colons.
    %
    % If '#1' is a usual file name without anything fancy, \pgfretval
    % will simply contain it. However, if '#1' contains double colons
    % (introduces, for example, by pdftex because there are white
    % spaces in '#1'), the routine
    % - removes the double colons,
    % - re-inserts them outside of the string.
    %
    % \pgfutilpreparefilename{file.tex} -> file.tex
    % \pgfutilpreparefilename{"A file name".file} -> "A file name.file"
    %
    % The resulting file name is returned in '\pgfretval',
    % furthermore, a *quoted* version of the file name is returned in
    % \pgfretvalquoted. The latter result is to have some sort of
    % output normalisation: if the file name as such contains double
    % quotes, we don't want to insert another set of them.
    %
    % This special handling has the following purposes:
    % 1. Both, treatment of white spaces and double colons is not
    % properly defined in TeX. Thus, we should only work with them if
    % necessary and maintain backwards compatibility as far as
    % possible.
    % 2. It *should* work if there are spaces.
    %
    \gdef\pgfutilpreparefilename#1{%
        \begingroup
            \ifnum\the\catcode`\"=13
                \pgfutilconvertdcolon
            \fi
            \xdef\pgf@temp{#1}%
        \endgroup
        \expandafter\pgfutil@in@\expandafter"\expandafter{\pgf@temp}%
        \ifpgfutil@in@
            \def\pgf@loc@TMPa{\pgfutilstrreplace{"}{}}%
            \expandafter\pgf@loc@TMPa\expandafter{\pgf@temp}%
            \edef\pgfretval{"\pgfretval"}% re-insert quotes! Otherwise, TeX can't use the file name.
            \let\pgfretvalquoted=\pgfretval
        \else
            \let\pgfretval=\pgf@temp
            \edef\pgfretvalquoted{"\pgfretval"}%
        \fi
    }%
    \catcode`\"=13
    \xdef\pgfutilconvertdcolon{%
        \noexpand\def\noexpand"{\pgf@loc@TMPa}%
    }%
\endgroup

% Converts an arbitrary command (without arguments) to a string in which all characters
% have category 12.
%
% #1: a macro name (which takes no arguments)
% #2: a macro name which will be assigned to '#1' converted to string.
%
% This uses '\meaning#1' hackery.
\def\pgfutil@command@to@string#1#2{%
    \expandafter\pgfutil@command@to@string@@\meaning#1\pgfutil@EOI{#2}%
}%
\xdef\pgfutil@glob@TMPa{\meaning\pgfutil@empty}%
\expandafter\def\expandafter\pgfutil@command@to@string@@\pgfutil@glob@TMPa#1\pgfutil@EOI#2{%
    \def#2{#1}%
}%
\begingroup
\catcode`\|=0
\catcode`\\=12
|gdef|pgfutil@backslash@as@other{\}%
|endgroup

% Checks if the token sequence #1 (unexpanded) contains a macro and
% invokes #2 if so and #3 if not.
\def\pgfutilifcontainsmacro#1#2#3{%
    \def\pgf@marshal{#1}%
    \pgfutil@command@to@string\pgf@marshal\pgf@marshal
    \edef\pgf@marshal{\noexpand\pgfutil@in@{\pgfutil@backslash@as@other}{\pgf@marshal}}%
    \pgf@marshal
    \ifpgfutil@in@
        \def\pgf@marshal{#2}%
    \else
        \def\pgf@marshal{#3}%
    \fi
    \pgf@marshal
}%

% Tests if string '#2' starts with pattern '#1'.
%
% If so, it executes #3 and defines \pgfretval to contain the
% suffix which is not equal to #1. Otherwise it executes #4.
\def\pgfutilifstartswith#1#2#3#4{%
    \def\pgfutilifstartswith@ ##1#1##2\pgf@EOI{%
        \def\pgfutil@tmp{##1}%
        \ifx\pgfutil@tmp\pgfutil@empty
            % Ah - a hit!
            %
            % define \pgfretval to be the suffix...
            \def\pgfutil@tmp#1####1\pgf@EOI{%
                \def\pgfretval{####1}%
            }%
            \pgfutil@tmp#2\pgf@EOI%
            %
            % ... and execute the <true> code:
            #3\relax%
        \else
            % hm. No such prefix.
            #4\relax%
        \fi
    }%
    \pgfutilifstartswith@#2--#1\pgf@EOI%
}%

% Usage:
% \pgfutilstrreplace{<token>}{<replacement>}{<string>}
%
% -> will assign the modified string into \pgfretval.
%
% #1: the string to search (one or more tokens)
% #2: zero, one or more tokens which will be inserted instead of '#1'.
% #3: the string to search in
\long\def\pgfutilstrreplace#1#2#3{%
    \def\pgfretval{}%
    \long\def\pgfutil@search@and@replace@@##1#1##2\pgf@EOI{%
        \expandafter\def\expandafter\pgfretval\expandafter{\pgfretval ##1#2}%
        \pgfutil@search@and@replace@loop{#1}{##2}%
    }%
    \pgfutil@search@and@replace@loop{#1}{#3}%
}
\long\def\pgfutil@search@and@replace@loop#1#2{%
    \pgfutil@in@{#1}{#2}%
    \ifpgfutil@in@
        \def\pgf@loc@TMPa{\pgfutil@search@and@replace@@ #2\pgf@EOI}%
    \else
        \expandafter\def\expandafter\pgfretval\expandafter{\pgfretval #2}%
        \let\pgf@loc@TMPa=\relax
    \fi
    \pgf@loc@TMPa
}%

% Solves a linear equation system of size 2x2 using gauss elimination.
%
% It employs TeX register arithmetics to do so.
% #1: should contain 4 sets of braces with matrix entries,
%     {<a11>}{<a12>}
%     {<a21>}{<a22>}
%     where each entry should be a number without unit.
%     It is acceptable if '#1' is a macro which expands to the expected
%     format.
% #2: should contain 2 sets of braces with the right-hand-side,
%     {<r1>}{<r2>}
%     where each entry should be a number without unit.
%     It is acceptable if '#2' is a macro which expands to the expected
%     format.
%
% It will assign \pgfmathresult to contain two sets of braces with the
% result.
%
% Example:
% \pgfutilsolvetwotwoleq{
%     {0.24}{1}
%     {-0.97}{0}
% }{
%     {-7}
%     {18}
% }
% -> yields \pgfmathresult={−18.55618}{−2.54642}
%
% The algorithm employs column pivotisation.
%
% If the matrix is singular, the routine will return {}.
\def\pgfutilsolvetwotwoleq#1#2{%
    \begingroup
        \dimendef\aa=0
        \dimendef\ab=1
        \dimendef\ba=2
        \dimendef\bb=3
        \dimendef\ra=4
        \dimendef\rb=5
        \dimendef\tmpa=6
        \dimendef\tmpb=7
        \edef\pgf@temp{#1}%
        \expandafter\pgfutilsolvetwotwoleq@A\pgf@temp
        \edef\pgf@temp{#2}%
        \expandafter\pgfutilsolvetwotwoleq@r\pgf@temp
        %
        \pgfutilsolvetwotwoleq@ifislarger\aa\ba{%
            % identity "permutation":
            \def\Pa{a}%
            \def\Pb{b}%
        }{%
            % permutation matrix: switch rows!
            \def\Pa{b}%
            \def\Pb{a}%
        }%
        % \pivot := 1/aa
        \tmpa=\csname m\Pa a\endcsname pt %
        \ifdim\tmpa<0pt \tmpa=-\tmpa\fi
        \ifdim\tmpa<0.0001pt
            % singular matrix!
            \let\pgfmathresult=\pgfutil@empty
        \else
            \pgfmathreciprocal@
                {\csname m\Pa a\endcsname}%
            \let\pivot=\pgfmathresult
            %
            % \factor := 1/aa * ba
            \csname \Pb a\endcsname=\pivot\csname \Pb a\endcsname
            \edef\factor{\expandafter\pgf@sys@tonumber\csname \Pb a\endcsname}%
            %
            % bb -= ba/aa * ab
            \tmpa=-\factor\csname \Pa b\endcsname
            \advance\csname \Pb b\endcsname by\tmpa
            %
            % rb -= ba/aa * ra
            \tmpa=-\factor\csname r\Pa\endcsname
            \advance\csname r\Pb\endcsname by\tmpa
            %
            \tmpa=\csname \Pb b\endcsname%
            \ifdim\tmpa<0pt \tmpa=-\tmpa\fi
            \ifdim\tmpa<0.0001pt
                % singular matrix!
                \let\pgfmathresult=\pgfutil@empty
            \else
                % xb := rb / bb (the modified rb and modified bb!)
                \pgfmathdivide@
                    {\expandafter\pgf@sys@tonumber\csname r\Pb\endcsname}
                    {\expandafter\pgf@sys@tonumber\csname \Pb b\endcsname}%
                \expandafter\let\csname pgfmathresult\Pb\endcsname=\pgfmathresult
                %
                % ra := ra - xb * ab
                \tmpa=\csname pgfmathresult\Pb\endcsname\csname \Pa b\endcsname
                \advance\csname r\Pa\endcsname by-\tmpa
                %
                % xa := 1/aa * ra  (the modified ra!)
                \tmpa=\pivot\csname r\Pa\endcsname
                \expandafter\edef\csname pgfmathresult\Pa\endcsname{\pgf@sys@tonumber\tmpa}%
                %
                \edef\pgfmathresult{%
                    {\csname pgfmathresult\Pa\endcsname}%
                    {\csname pgfmathresult\Pb\endcsname}%
                }%
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%

\def\pgfutilsolvetwotwoleq@ifislarger#1#2#3#4{%
    \tmpa=#1
    \ifdim\tmpa<0pt
        \multiply\tmpa by-1
    \fi
    \tmpb=#2
    \ifdim\tmpb<0pt
        \multiply\tmpb by-1
    \fi
    \ifdim\tmpa>\tmpb
        #3%
    \else
        #4%
    \fi
}%

\def\pgfutilsolvetwotwoleqfloat@ifislarger#1#2#3#4{%
    \pgfmathfloatabs@{#1}\let\tmpa=\pgfmathresult
    \pgfmathfloatabs@{#2}\let\tmpb=\pgfmathresult
    \pgfmathfloatlessthan@{\tmpb}{\tmpa}%
    \ifpgfmathfloatcomparison
        #3%
    \else
        #4%
    \fi
}%
\def\pgfutilsolvetwotwoleq@A#1#2#3#4{%
    \def\maa{#1}\def\mab{#2}%
    \def\mba{#3}\def\mbb{#3}%
    \aa=#1pt \ab=#2pt
    \ba=#3pt \bb=#4pt
}
\def\pgfutilsolvetwotwoleq@r#1#2{%
    \ra=#1pt \rb=#2pt
}%
\def\pgfutilsolvetwotwoleqfloat@A#1#2#3#4{%
    \pgfmathfloatparsenumber{#1}\let\maa=\pgfmathresult
    \pgfmathfloatparsenumber{#2}\let\mab=\pgfmathresult
    \pgfmathfloatparsenumber{#3}\let\mba=\pgfmathresult
    \pgfmathfloatparsenumber{#4}\let\mbb=\pgfmathresult
}
\def\pgfutilsolvetwotwoleqfloat@r#1#2{%
    \pgfmathfloatparsenumber{#1}\let\ra=\pgfmathresult
    \pgfmathfloatparsenumber{#2}\let\rb=\pgfmathresult
}%

% Same as \pgfutilsolvetwotwoleq, but using floating point
% arithmetics. The return value is still in fixed point.
\def\pgfutilsolvetwotwoleqfloat#1#2{%
    \begingroup
        \pgfmathfloatcreate{1}{1.0}{-4}% FIXME : use a smaller threshold for FPU?
        \let\thresh=\pgfmathresult
        %
        \edef\pgf@temp{#1}%
        \expandafter\pgfutilsolvetwotwoleqfloat@A\pgf@temp
        \edef\pgf@temp{#2}%
        \expandafter\pgfutilsolvetwotwoleqfloat@r\pgf@temp
        %
        \pgfutilsolvetwotwoleqfloat@ifislarger\maa\mba{%
            % identity "permutation":
            \def\Pa{a}%
            \def\Pb{b}%
        }{%
            % permutation matrix: switch rows!
            \def\Pa{b}%
            \def\Pb{a}%
        }%
        % \pivot := 1/aa
        \expandafter\pgfmathfloatabs@\expandafter{\csname m\Pa a\endcsname}%
        \let\tmpa=\pgfmathresult
        \pgfmathfloatlessthan@{\tmpa}{\thresh}%
        \ifpgfmathfloatcomparison
            % singular matrix!
            \let\pgfmathresult=\pgfutil@empty
        \else
            \expandafter\pgfmathfloatreciprocal@\expandafter{\csname m\Pa a\endcsname}%
            \let\pivot=\pgfmathresult
            %
            % \factor := 1/aa * ba
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pb a\endcsname}{\pivot}%
            \let\factor=\pgfmathresult
            \expandafter\let\csname m\Pb a\endcsname=\factor
            %
            % bb -= ba/aa * ab
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pa b\endcsname}{\factor}%
            \let\tmpa=\pgfmathresult
            \expandafter\pgfmathfloatsubtract@\expandafter{\csname m\Pb b\endcsname}{\tmpa}%
            \expandafter\let\csname m\Pb b\endcsname=\pgfmathresult
            %
            % rb -= ba/aa * ra
            \expandafter\pgfmathfloatmultiply@\expandafter{\csname r\Pa\endcsname}{\factor}%
            \let\tmpa=\pgfmathresult
            \expandafter\pgfmathfloatsubtract@\expandafter{\csname r\Pb\endcsname}{\tmpa}%
            \expandafter\let\csname r\Pb\endcsname=\pgfmathresult
            %
            \expandafter\pgfmathfloatabs@\expandafter{\csname m\Pb b\endcsname}%
            \let\tmpa=\pgfmathresult
            \pgfmathfloatlessthan@{\tmpa}{\thresh}%
            \ifpgfmathfloatcomparison
                % singular matrix!
                \let\pgfmathresult=\pgfutil@empty
            \else
                % xb := rb / bb (the modified rb and modified bb!)
                \edef\pgf@marshal{%
                    \noexpand\pgfmathfloatdivide@
                        {\csname r\Pb\endcsname}
                        {\csname m\Pb b\endcsname}%
                }%
                \pgf@marshal
                \expandafter\let\csname pgfmathresult\Pb\endcsname=\pgfmathresult
                \let\tmpa=\pgfmathresult
                %
                % ra := ra - xb * ab
                \expandafter\pgfmathfloatmultiply@\expandafter{\csname m\Pa b\endcsname}{\tmpa}%
                \let\tmpa=\pgfmathresult
                \expandafter\pgfmathfloatsubtract@\expandafter{\csname r\Pa\endcsname}{\tmpa}%
                \expandafter\let\csname r\Pa\endcsname=\pgfmathresult
                %
                % xa := 1/aa * ra  (the modified ra!)
                \expandafter\pgfmathfloatmultiply@\expandafter{\csname r\Pa\endcsname}{\pivot}%
                \expandafter\let\csname pgfmathresult\Pa\endcsname=\pgfmathresult
                %
                \edef\pgfmathresult{%
                    {\csname pgfmathresult\Pa\endcsname}%
                    {\csname pgfmathresult\Pb\endcsname}%
                }%
                \expandafter\pgfutilsolvetwotwoleqfloat@to@pgf@range\pgfmathresult
            \fi
        \fi
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}%


\def\pgfutilsolvetwotwoleqfloat@to@pgf@range#1#2{%
    \pgfmathfloatcreate{1}{1.6}{4}\let\pgfutilsolvetwotwoleqfloat@to@pgf@range@max=\pgfmathresult
    \pgfmathfloatabs@{#1}%
    \expandafter\pgfmathfloatlessthan@\expandafter{\pgfmathresult}{\pgfutilsolvetwotwoleqfloat@to@pgf@range@max}%
    \ifpgfmathfloatcomparison
        \pgfmathfloatabs@{#2}%
        \expandafter\pgfmathfloatlessthan@\expandafter{\pgfmathresult}{\pgfutilsolvetwotwoleqfloat@to@pgf@range@max}%
        \ifpgfmathfloatcomparison
            % ok.
            \pgfmathfloattofixed{#1}\let\tmpa=\pgfmathresult
            \pgfmathfloattofixed{#2}%
            \edef\pgfmathresult{{\tmpa}{\pgfmathresult}}%
        \else
            % singular (because PGF cannot represent its result
            \let\pgfmathresult=\pgfutil@empty
        \fi
    \else
        % singular (because PGF cannot represent its result
        \let\pgfmathresult=\pgfutil@empty
    \fi
}%

% there are funny programs which overwrite \read and \write (like
% tabularx).
\let\pgfutil@write=\write
\let\pgfutil@read=\read

% curtesy for latex:
\let\pgfutil@protect\relax

% Used by latex for doing reruns
% #1 = an internal label
% #2 = a to-be-tested text
\def\pgfutil@check@rerun#1#2{}

% new tempdims:
\newdimen\pgfutil@tempdima
\newdimen\pgfutil@tempdimb


% luatex stuff
% We assume luatex version > 0.39:
%   - \directlua <general text> will work
%   - \directlua is the only luatex primitive that we can assume
%     accessible without being prefixed by the format via
%     tex.enableprimitives.
% Ideas taken from the ifluatex package (Heiko Oberdiek)
\let\pgfutil@ifluatex\iffalse
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
\else
  \expandafter\let\csname pgfutil@ifluatex\expandafter\endcsname
    \csname iftrue\endcsname
\fi

\pgfutil@ifluatex
  \let\pgfutil@directlua\directlua
  \pgfutil@directlua{%
    tex.enableprimitives('pgfutil@',{'luaescapestring'})}
\else
  \def\pgfutil@directlua#1{}
  \def\pgfutil@luaescapestring#1{}
\fi


\def\pgfutil@shellescape@lua@eightseven#1{%
    \pgfutil@directlua{os.execute("\pgfutil@luaescapestring{#1}")}%
}%
\def\pgfutil@shellescape#1{%
    \immediate\write18{#1}%
}%
\pgfutil@IfUndefined{directlua}{%
}{%
    \pgfutil@IfUndefined{lastsavedimageresourcepages}{%
        % Ah - an old version of luatex. It still supports \write18
    }{%
        % take the new variant...
        \let\pgfutil@shellescape=\pgfutil@shellescape@lua@eightseven
    }%
}%

% End of luatex stuff

% Advances a number stored in a macro and writes the result back into
% the macro.
% #1 is a macro containing a number.
\def\pgfutil@advancestringcounter#1{%
    \begingroup
        \c@pgf@counta=#1\relax
        \advance\c@pgf@counta by1
        \edef#1{\the\c@pgf@counta}%
        \pgfmath@smuggleone#1%
    \endgroup
}%
\input pgfutil-common-lists.tex

\endinput


==> tikz.code.tex <==
% Copyright 2019 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS{tikz.code.tex}


\def\tikzerror#1{\pgfutil@packageerror{tikz}{#1}{}}

% Always-present libraries (|\usepgflibrary| defined in
% \file{pgfutil-common.tex}).
\usepgflibrary{plothandlers}

\newdimen\tikz@lastx
\newdimen\tikz@lasty
\newdimen\tikz@lastxsaved
\newdimen\tikz@lastysaved
\newdimen\tikz@lastmovetox
\newdimen\tikz@lastmovetoy

\newdimen\tikzleveldistance
\newdimen\tikzsiblingdistance

\newbox\tikz@figbox
\newbox\tikz@figbox@bg
\newbox\tikz@tempbox
\newbox\tikz@tempbox@bg

\newcount\tikztreelevel
\newcount\tikznumberofchildren
\newcount\tikznumberofcurrentchild

\newcount\tikz@fig@count

\newif\iftikz@node@is@a@label
\newif\iftikz@snaked
\newif\iftikz@decoratepath

\let\tikz@options\pgfutil@empty
% |\tikz@addoption| adds \texttt{#1} at the end of the replacement
% text of |\tikz@options| without expansion.
\def\tikz@addoption#1{%
  \expandafter\def\expandafter\tikz@options\expandafter{\tikz@options#1}}%
% Same as |tikz@addoption| for |\tikz@mode|. Note that |\tikz@mode| is
% initially let to |\pgfutil@empty| later (see path usage options).
\def\tikz@addmode#1{%
  \expandafter\def\expandafter\tikz@mode\expandafter{\tikz@mode#1}}%
% Same as |tikz@addoption| for |\tikz@transform|. Works even if
% |\tikz@transform| is not defined. In that case, nothing is added to
% |\tikz@transform|: \texttt{#1} is expanded.
\def\tikz@addtransform#1{%
  \ifx\tikz@transform\relax
    #1%
  \else
    \expandafter\def\expandafter\tikz@transform\expandafter{\tikz@transform#1}%
  \fi
}%


% TikZ options management.

% Setting up the tikz key family (key management needs
% \file{pgfkeys.code.tex});
\pgfkeys{/tikz/.is family}%

% |\tikzset| is a shortcut to set keys that belongs to the tikz
% family.
\def\tikzset{\pgfqkeys{/tikz}}%

% Note: |\tikzoption| is supported for compatibility only. |\tikzset|
% should be used instead.
\def\tikzoption#1{%
  \pgfutil@ifnextchar[%]
    {\tikzoption@opt{#1}}{\tikzoption@noopt{#1}}}%
\def\tikzoption@opt#1[#2]#3{%
  \pgfkeysdef{/tikz/#1}{#3}%
  \pgfkeyssetvalue{/tikz/#1/.@def}{#2}}%
\def\tikzoption@noopt#1#2{%
  \pgfkeysdef{/tikz/#1}{#2}%
  \pgfkeyssetvalue{/tikz/#1/.@def}{\pgfkeysvaluerequired}}%

% Baseline options
\tikzoption{baseline}[0pt]{%
  \pgfutil@ifnextchar(%)
    {\tikz@baseline@coordinate}{\tikz@baseline@simple}#1\@nil}%
\def\tikz@baseline@simple#1\@nil{\pgfsetbaseline{#1}}%
\def\tikz@baseline@coordinate#1\@nil{%
  \pgfsetbaselinepointlater{\tikz@scan@one@point\pgfutil@firstofone#1}}%

\tikzoption{trim left}[0pt]{\pgfutil@ifnextchar({\tikz@trim@coordinate{left}}{\tikz@trim@simple{left}}#1\@nil}%)%
\tikzoption{trim right}{\pgfutil@ifnextchar({\tikz@trim@coordinate{right}}{\tikz@trim@simple{right}}#1\@nil}%)%
\def\tikz@trim@simple#1#2\@nil{\csname pgfsettrim#1\endcsname{#2}}%
\def\tikz@trim@coordinate#1#2\@nil{\csname pgfsettrim#1pointlater\endcsname{\tikz@scan@one@point\pgfutil@firstofone#2}}%

% Draw options
\tikzoption{line width}{\tikz@semiaddlinewidth{#1}}%

\def\tikz@semiaddlinewidth#1{\tikz@addoption{\pgfsetlinewidth{#1}}\pgfmathsetlength\pgflinewidth{#1}}%

\tikzoption{cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}%
\tikzoption{join}{\tikz@addoption{\csname pgfset#1join\endcsname}}%
\tikzoption{line cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}%
\tikzoption{line join}{\tikz@addoption{\csname pgfset#1join\endcsname}}%
\tikzoption{miter limit}{\tikz@addoption{\pgfsetmiterlimit{#1}}}%

\tikzoption{dash pattern}{% syntax: on 2pt off 3pt on 4pt ...
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi}%
\tikzoption{dash phase}{%
  \def\tikz@dashphase{#1}%
  \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
  \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
}%
\tikzoption{dash}{\tikz@parse@full@dash#1\pgf@stop}%
\def\tikz@parse@full@dash#1phase#2\pgf@stop{%
  \def\tikz@dashphase{#2}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi%
}%
\def\tikz@dashphase{0pt}%
\def\tikz@dashpattern{}%

\def\tikz@scandashon n#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashoff}}%
\def\tikz@scandashoff ff#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashon}}%

% use a decoration to expand the `off' section of a dash pattern.
% https://tex.stackexchange.com/a/133357
\tikzset{
    dash expand off/.code={%
        \ifcsname tikz@library@decorations@loaded\endcsname\else
            \tikzerror{You need \string\usetikzlibrary{decorations} for ``dash offexpand''}%
        \fi
        \tikz@addoption{%
            \pgfgetpath\currentpath
            \pgfprocessround{\currentpath}{\currentpath}%
            \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
            % Parse \on and \off from the current path
            \edef\on{\expandafter\pgfutil@firstoftwo\tikz@dashpattern}%
            \edef\off{\expandafter\pgfutil@secondoftwo\tikz@dashpattern}%
            % \dashphase = max(\on - \dashphase, 0)
            \pgfmathsubtract@{\on}{\tikz@dashphase}%
            \pgfmathmax@{\pgfmathresult}{0}%
            \edef\dashphase{\the\dimexpr\pgfmathresult pt\relax}%
            % \rest = \pgf@decorate@totalpathlength - \on
            \edef\rest{\expandafter\pgf@sys@tonumber\dimexpr\pgf@decorate@totalpathlength - \on + 2\dimexpr\dashphase\relax\relax}%
            % \onoff = \on + \off
            \edef\onoff{\expandafter\pgf@sys@tonumber\dimexpr\on+\off\relax}%
            % \nfullonoff = max(floor(\rest/\onoff), 1)
            \pgfmathdivide@{\rest}{\onoff}%
            \pgfmathfloor@{\pgfmathresult}%
            \pgfmathmax@{\pgfmathresult}{1}%
            % \offexpand = max(\rest/\nfullonoff - \on, \off)
            \pgfmathdivide@{\rest}{\pgfmathresult}%
            \pgfmathsubtract@{\pgfmathresult}{\on}%
            \pgfmathmax@{\pgfmathresult}{\off}%
            \edef\tikz@marshal{\noexpand\pgfsetdash{{\on}{\pgfmathresult}}{\dashphase}}%
            \tikz@marshal
        }%
    }
}

\tikzoption{draw opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}}}%

% Double draw options
\tikzoption{double}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@doublefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \pgfsetinnerstrokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@doubletrue}%
    \tikzset{every double/.try}%
  \fi}%
\tikzoption{double distance}{%
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@setup{%
    \pgf@x=\the\pgf@x%
    \advance\pgf@x by2\pgflinewidth%
    \pgflinewidth=\pgf@x%
    \noexpand\pgfsetlinewidth{\pgflinewidth}%
    \noexpand\pgfsetinnerlinewidth{\the\pgf@x}%
  }%
  \tikzset{double}}%
\def\tikz@double@setup{%
  \pgf@x=2\pgflinewidth%
  \advance\pgf@x by0.6pt%
  \pgflinewidth=\pgf@x%
  \pgfsetlinewidth{\pgflinewidth}%
  \pgfsetinnerlinewidth{0.6pt}%
}%
\tikzset{double distance between line centers/.code={
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@setup{%
    \pgf@x=\pgflinewidth%
    \pgf@xa=\the\pgf@x%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@xa by-\pgflinewidth%
    \pgflinewidth=\pgf@x%
    \noexpand\pgfsetlinewidth{\pgflinewidth}%
    \noexpand\pgfsetinnerlinewidth{\pgf@xa}%
  }%
  \tikzset{double}}}%
\tikzset{double equal sign distance/.style={double distance between line centers=0.45ex}}%




% Fill options

\tikzoption{even odd rule}[]{\tikz@addoption{\pgfseteorule}}%
\tikzoption{nonzero rule}[]{\tikz@addoption{\pgfsetnonzerorule}}%

\tikzoption{fill opacity}{\tikz@addoption{\pgfsetfillopacity{#1}}}%


% Joined fill/draw options

\tikzoption{opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}\pgfsetfillopacity{#1}}}%


% Blend mode

\tikzset{blend mode/.code={\tikz@addoption{\pgfsetblendmode{#1}}}}%


% Main color options
\tikzoption{color}{%
  \tikz@addoption{%
    \ifx\tikz@fillcolor\pgfutil@empty%
      \ifx\tikz@strokecolor\pgfutil@empty%
      \else%
        \pgfsys@color@reset@inorderfalse%
        \let\tikz@strokecolor\pgfutil@empty%
        \let\tikz@fillcolor\pgfutil@empty%
      \fi%
    \else%
      \pgfsys@color@reset@inorderfalse%
      \let\tikz@strokecolor\pgfutil@empty%
      \let\tikz@fillcolor\pgfutil@empty%
    \fi%
    \pgfutil@colorlet{tikz@color}{#1}%
    \pgfutil@colorlet{.}{tikz@color}%
    %
    \pgfsetcolor{.}%
    \pgfsys@color@reset@inordertrue%
  }%
  \def\tikz@textcolor{#1}}%



% Rounding options
\tikzoption{rounded corners}[4pt]{\pgfsetcornersarced{\pgfpoint{#1}{#1}}}%
\tikzoption{sharp corners}[]{\pgfsetcornersarced{\pgfpointorigin}}%

% Radii and arc options
\tikzset{x radius/.initial=0pt}%
\tikzset{y radius/.initial=0pt}%
\tikzset{%
  radius/.code={%
    \pgfmathparse{#1}%
    \ifpgfmathunitsdeclared
      \pgfkeyssetevalue{/tikz/x radius}{\pgfmathresult pt}%
      \pgfkeyssetevalue{/tikz/y radius}{\pgfmathresult pt}%
    \else
      \pgfkeyssetevalue{/tikz/x radius}{\pgfmathresult}%
      \pgfkeyssetevalue{/tikz/y radius}{\pgfmathresult}%
    \fi
  }%
}%
\tikzset{start angle/.initial=}%
\tikzset{end angle/.initial=}%
\tikzset{delta angle/.initial=}%


% Coordinate options
\tikzoption{x}{\tikz@handle@vec{\pgfsetxvec}{\tikz@handle@x}#1\relax}%
\tikzoption{y}{\tikz@handle@vec{\pgfsetyvec}{\tikz@handle@y}#1\relax}%
\tikzoption{z}{\tikz@handle@vec{\pgfsetzvec}{\tikz@handle@z}#1\relax}%

\def\tikz@handle@vec#1#2{\pgfutil@ifnextchar({\tikz@handle@coordinate#1}{\tikz@handle@single#2}}%
\def\tikz@handle@coordinate#1{\tikz@scan@one@point#1}%
\def\tikz@handle@single#1#2\relax{#1{#2}}%
\def\tikz@handle@x#1{\pgfsetxvec{\pgfpoint{#1}{0pt}}}%
\def\tikz@handle@y#1{\pgfsetyvec{\pgfpoint{0pt}{#1}}}%
\def\tikz@handle@z#1{\pgfsetzvec{\pgfpoint{#1}{#1}}}%


% Transformation options
\tikzoption{scale}{\tikz@addtransform{\pgftransformscale{#1}}}%
\tikzoption{scale around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformscale}\tikz@doaround{#1}}}%
\tikzoption{xscale}{\tikz@addtransform{\pgftransformxscale{#1}}}%
\tikzoption{xslant}{\tikz@addtransform{\pgftransformxslant{#1}}}%
\tikzoption{yscale}{\tikz@addtransform{\pgftransformyscale{#1}}}%
\tikzoption{yslant}{\tikz@addtransform{\pgftransformyslant{#1}}}%
\tikzoption{rotate}{\tikz@addtransform{\pgftransformrotate{#1}}}%
\tikzoption{rotate around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformrotate}\tikz@doaround{#1}}}%
\def\tikz@doaround#1{%
  \edef\tikz@temp{#1}% get rid of active stuff
  \expandafter\tikz@doparseA\tikz@temp%
}%
\def\tikz@doparseA#1:{%
  \def\tikz@temp@rot{#1}%
  \tikz@scan@one@point\tikz@doparseB%
}%
\def\tikz@doparseB#1{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@aroundaction{\tikz@temp@rot}%
  \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
}%

\tikzoption{shift}{\tikz@addtransform{\tikz@scan@one@point\pgftransformshift#1\relax}}%
\tikzoption{xshift}{\tikz@addtransform{\pgftransformxshift{#1}}}%
\tikzoption{yshift}{\tikz@addtransform{\pgftransformyshift{#1}}}%
\tikzoption{cm}{\tikz@addtransform{\tikz@parse@cm#1\relax}}%
\tikzoption{reset cm}[]{\tikz@addtransform{\pgftransformreset}}%
\tikzoption{shift only}[]{\tikz@addtransform{\pgftransformresetnontranslations}}%

\def\tikz@parse@cm#1,#2,#3,#4,{%
  \def\tikz@p@cm{{#1}{#2}{#3}{#4}}%
  \tikz@scan@one@point\tikz@parse@cmA}%
\def\tikz@parse@cmA#1{%
  \expandafter\pgftransformcm\tikz@p@cm{#1}%
}%

\tikzset{transform canvas/.code=%
  {%
    \tikz@addoption
    {%
      {%
        \pgftransformreset%
        \let\tikz@transform=\relax%
        \tikzset{#1}%
        \pgflowlevelsynccm%
      }%
      \pgf@relevantforpicturesizefalse%
    }%
  }%
}%

\tikzset{turn/.code={%
    \pgf@x=0pt%
    \pgf@y\pgf@x%
    \pgf@process{\tikz@tangent}%
    \advance\pgf@x by-\tikz@lastx%
    \advance\pgf@y by-\tikz@lasty%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@x=-\pgf@x%
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@ya}}%
    {\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@x}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  }%
}%

\def\tikz@tangent@lookup{%
  \pgfgetpath\tikz@temp%
  \pgfprocesspathextractpoints\tikz@temp%
  \pgfpointsecondlastonpath%
}%

% Code for rotating the xyz coordinate system
% around the x, y, or z vector.
%
\def\tikz@xyz@rotate@let{%
  \let\pgf@z=\pgf@yc%
  \let\pgf@za=\pgf@xc%
}%

\def\tikz@xyz@rotate@xyz@xaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@x=#1\relax%
  \pgf@ya=#2\relax%
  \pgf@za=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@y=\tikz@xyz@cos\pgf@ya%
  \advance\pgf@y by-\tikz@xyz@sin\pgf@za%
  \pgf@z=\tikz@xyz@sin\pgf@ya%
  \advance\pgf@z by\tikz@xyz@cos\pgf@za%
}%

\def\tikz@xyz@rotate@xyz@yaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@xa=#1\relax%
  \pgf@y=#2\relax%
  \pgf@za=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@x=\tikz@xyz@cos\pgf@xa%
  \advance\pgf@x by\tikz@xyz@sin\pgf@za%
  \pgf@z=-\tikz@xyz@sin\pgf@xa%
  \advance\pgf@z by\tikz@xyz@cos\pgf@za%
}%

\def\tikz@xyz@rotate@xyz@zaxis#1#2#3#4{%
  \tikz@xyz@rotate@let%
  \pgf@xa=#1\relax%
  \pgf@ya=#2\relax%
  \pgf@z=#3\relax%
  \pgfmathsin@{#4}\let\tikz@xyz@sin=\pgfmathresult%
  \pgfmathcos@{#4}\let\tikz@xyz@cos=\pgfmathresult%
  \pgf@x=\tikz@xyz@cos\pgf@xa%
  \advance\pgf@x by-\tikz@xyz@sin\pgf@ya%
  \pgf@y=\tikz@xyz@sin\pgf@xa%
  \advance\pgf@y by\tikz@xyz@cos\pgf@ya%
}%

\tikzset{rotate around x/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@xaxis{0pt}{1pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@yvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@xaxis{0pt}{0pt}{1pt}{\tikz@xyz@angle}%
    \pgfsetzvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetyvec{\tikz@xyz@rotate@yvec}%
  },
  rotate around y/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@yaxis{1pt}{0pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@xvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@yaxis{0pt}{0pt}{1pt}{\tikz@xyz@angle}%
    \pgfsetzvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetxvec{\tikz@xyz@rotate@xvec}%
  },
  rotate around z/.code={%
    \tikz@xyz@rotate@let%
    \pgfmathparse{#1}\let\tikz@xyz@angle=\pgfmathresult%
    \tikz@xyz@rotate@xyz@zaxis{1pt}{0pt}{0pt}{\tikz@xyz@angle}%
    \pgfextract@process\tikz@xyz@rotate@xvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \tikz@xyz@rotate@xyz@zaxis{0pt}{1pt}{0pt}{\tikz@xyz@angle}%
    \pgfsetyvec{\pgfpointxyz{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@z}}}%
    \pgfsetxvec{\tikz@xyz@rotate@xvec}%
  },
}%

% Grid options
\tikzoption{xstep}{\def\tikz@grid@x{#1}}%
\tikzoption{ystep}{\def\tikz@grid@y{#1}}%
\tikzoption{step}{\tikz@handle@vec{\tikz@step@point}{\tikz@step@single}#1\relax}%
\def\tikz@step@single#1{\def\tikz@grid@x{#1}\def\tikz@grid@y{#1}}%
\def\tikz@step@point#1{\pgf@process{#1}\edef\tikz@grid@x{\the\pgf@x}\edef\tikz@grid@y{\the\pgf@y}}%

\def\tikz@grid@x{1cm}%
\def\tikz@grid@y{1cm}%


% Current point updates
\newif\iftikz@current@point@local
\tikzset{current point is local/.is if=tikz@current@point@local}%

% Path usage options
\newif\iftikz@mode@double
\newif\iftikz@mode@fill
\newif\iftikz@mode@draw
\newif\iftikz@mode@clip
\newif\iftikz@mode@boundary
\newif\iftikz@mode@shade
\newif\iftikz@mode@fade@path
\newif\iftikz@mode@fade@scope
\let\tikz@mode=\pgfutil@empty

\def\tikz@nonetext{none}%

\tikzoption{path only}[]{\let\tikz@mode=\pgfutil@empty}%
\tikzset{
  shade/.is choice,
  shade/.default=true,
  shade/true/.code=\tikz@addmode{\tikz@mode@shadetrue},
  shade/false/.code=\tikz@addmode{\tikz@mode@shadefalse},
  shade/none/.code=\tikz@addmode{\tikz@mode@shadefalse},
}%

\tikzoption{fill}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillcolor{#1}}%
      \def\tikz@fillcolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}%
\tikzoption{draw}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@drawfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetstrokecolor{#1}}%
      \def\tikz@strokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@drawtrue}%
  \fi%
}%
\tikzoption{clip}[]{\tikz@addmode{\tikz@mode@cliptrue}}%
\tikzoption{use as bounding box}[]{\tikz@addmode{\tikz@mode@boundarytrue}}%

\tikzoption{save path}{\tikz@addmode{\pgfsyssoftpath@getcurrentpath#1\global\let#1=#1}}%
\tikzoption{use path}{\tikz@addmode{\pgfsyssoftpath@setcurrentpath#1}}%

\let\tikz@fillcolor=\pgfutil@empty
\let\tikz@strokecolor=\pgfutil@empty

% Insert a path using an option
\tikzset{insert path/.code=\tikz@scan@next@command#1\pgf@stop}%

% Pattern options
\tikzset{pattern/.code=\tikzerror{You need to say \string\usetikzlibrary{patterns}},
         pattern color/.style=pattern}%

% Path pictures
\tikzset{path picture/.code=\tikz@addmode{\def\tikz@path@picture{#1}}}%

% Fading options
\tikzset{path fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@pathfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@path@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@pathtrue}%
  \fi%
  },
  path fading/.default=,
  scope fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@scopefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@scope@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@scopetrue}%
  \fi%
  },
  scope fading/.default=}%
\tikzset{fit fading/.is if=tikz@fade@adjust}%
\tikzset{fading transform/.store in=\tikz@fade@transform}%
\tikzset{fading angle/.style={fading transform={rotate=#1}}}%

\newif\iftikz@fade@adjust%
\tikz@fade@adjusttrue%
\let\tikz@fade@transform\pgfutil@empty%

\pgfutil@colorlet{transparent}{pgftransparent}%
\def\tikz@do@fade@transform{\let\tikz@transform=\relax\expandafter\tikzset\expandafter{\tikz@fade@transform}}%



% Transparency groups
\newif\iftikz@transparency@group%
\tikzset{/tikz/transparency group/.code=\tikz@transparency@grouptrue\def\tikz@transparency@group@options{isolated=true,#1}\let\tikz@blend@group\pgfutil@empty}%
\tikzset{/tikz/blend group/.code=\tikz@transparency@grouptrue\def\tikz@transparency@group@options{isolated=true}\def\tikz@blend@group{\pgfsetblendmode{#1}}}%

\let\tikz@blend@group\pgfutil@empty

% Shading options
\tikzoption{shading}{\def\tikz@shading{#1}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{shading angle}{\def\tikz@shade@angle{#1}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{top color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{bottom color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{middle color}{%
  \pgfutil@colorlet{tikz@axis@middle}{#1}%
  \def\tikz@shading{axis}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{left color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{right color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{ball}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{inner color}{\pgfutil@colorlet{tikz@radial@inner}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}%
\tikzoption{outer color}{\pgfutil@colorlet{tikz@radial@outer}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}%

\def\tikz@shading{axis}%
\def\tikz@shade@angle{0}%

\pgfdeclareverticalshading[tikz@axis@top,tikz@axis@middle,tikz@axis@bottom]{axis}{100bp}{%
  color(0bp)=(tikz@axis@bottom);
  color(25bp)=(tikz@axis@bottom);
  color(50bp)=(tikz@axis@middle);
  color(75bp)=(tikz@axis@top);
  color(100bp)=(tikz@axis@top)}%

\pgfutil@colorlet{tikz@axis@top}{gray}%
\pgfutil@colorlet{tikz@axis@middle}{gray!50!white}%
\pgfutil@colorlet{tikz@axis@bottom}{white}%

\pgfdeclareradialshading[tikz@ball]{ball}{\pgfqpoint{-10bp}{10bp}}{%
 color(0bp)=(tikz@ball!15!white);
 color(9bp)=(tikz@ball!75!white);
 color(18bp)=(tikz@ball!70!black);
 color(25bp)=(tikz@ball!50!black);
 color(50bp)=(black)}%

\pgfutil@colorlet{tikz@ball}{blue}%

\pgfdeclareradialshading[tikz@radial@inner,tikz@radial@outer]{radial}{\pgfpointorigin}{%
 color(0bp)=(tikz@radial@inner);
 color(25bp)=(tikz@radial@outer);
 color(50bp)=(tikz@radial@outer)}%

\pgfutil@colorlet{tikz@radial@inner}{gray}%
\pgfutil@colorlet{tikz@radial@outer}{white}%


% Pin options
\tikzset{
  pin distance/.store in=\tikz@pin@distance,
  pin distance=3ex,
  pin position/.store in=\tikz@pin@default@pos,
  pin position=above,
  pin edge/.store in=\tikz@pin@edge@style,
  pin edge={},
  tikz@pin@post/.code={\global\let\tikz@pin@edge@style@smuggle=\tikz@pin@edge@style},
  tikz@pre@pin@edge/.code={%
    \toks0=\expandafter{\tikz@pin@edge@style@smuggle}%
    \edef\pgf@marshal{\noexpand\tikzset{tikz@pin@options/.style={\the\toks0}}}%
    \pgf@marshal
  },%
}%

\tikzset{%
  pin/.code={%
    \begingroup
      \ifnum\the\catcode`\:=\active\relax
        \def\tikz@next{%
          \endgroup
          \tikz@parse@pin@active@i{#1}}%
      \else
        \def\tikz@next{%
          \endgroup
          \pgfutil@ifnextchar[%]
            {\tikz@parse@pin@nonactive}
            {\tikz@parse@pin@nonactive[]}#1:\pgf@nil}%
      \fi
    \tikz@next}}%

\begingroup
  \catcode`\:=\active\relax

  \gdef\tikz@parse@pin@active@i#1{%
    \pgfutil@ifnextchar[%]
      {\tikz@parse@pin@active}
      {\tikz@parse@pin@active[]}#1:\pgf@nil}%

  \long\gdef\tikz@parse@pin@active[#1]#2:#3\pgf@nil{%
    \def\tikz@temp{#3}%
    \ifx\tikz@temp\pgfutil@empty
      % no position, use default
      \tikz@@parse@pin@active[#1]\tikz@pin@default@pos:#2:\pgf@nil%
    \else
      \tikz@@parse@pin@active[#1]#2:#3\pgf@nil%
    \fi}%

  \long\gdef\tikz@@parse@pin@active[#1]#2:#3:\pgf@nil{%
    \tikzset{%
      append after command = {%
        \bgroup
          [current point is local = true]
          \pgfextra{\let\tikz@save@last@node=\tikzlastnode\tikz@node@is@a@labelfalse}%
          node [tikz@label@angle = #2,
                anchor=@auto,
                every pin,
                #1,
                append after command = {%
                  (\tikz@save@last@node)
                  edge [every pin edge,
                        tikz@pre@pin@edge,
                        tikz@pin@options]
                  (\tikzlastnode)},
                tikz@label@post = \tikz@pin@distance,
                tikz@pin@post] {#3}
        \egroup}}}%
\endgroup

\long\def\tikz@parse@pin@nonactive[#1]#2:#3\pgf@nil{%
  \def\tikz@temp{#3}%
  \ifx\tikz@temp\pgfutil@empty
    % no position, use default
    \tikz@@parse@pin@nonactive[#1]\tikz@pin@default@pos:#2:\pgf@nil%
  \else
    \tikz@@parse@pin@nonactive[#1]#2:#3\pgf@nil%
  \fi}%

\long\def\tikz@@parse@pin@nonactive[#1]#2:#3:\pgf@nil{%
  \tikzset{%
    append after command = {%
      \bgroup
        [current point is local = true]
        \pgfextra{\let\tikz@save@last@node=\tikzlastnode\tikz@node@is@a@labelfalse}%
        node [tikz@label@angle = #2,
              anchor=@auto,
              every pin,
              #1,
              append after command = {%
                (\tikz@save@last@node)
                edge [every pin edge,
                      tikz@pre@pin@edge,
                      tikz@pin@options]
                (\tikzlastnode)},
              tikz@label@post = \tikz@pin@distance,
              tikz@pin@post] {#3}
      \egroup}}}%

% Label and pin options

\tikzset{
  label distance/.store in=\tikz@label@distance,
  label distance=0pt,
  label position/.store in=\tikz@label@default@pos,
  label position=above,
  absolute/.is if=tikz@absolute,
  tikz@label@angle/.store in=\tikz@label@angle
}%

\newif\iftikz@absolute
\def\tikz@on@text{center}%

\tikzset{tikz@label@post/.code 2 args={
  \edef\tikz@label@angle{\tikz@label@angle}%
  \expandafter\pgfkeys@spdef\expandafter\tikz@label@angle\expandafter{\tikz@label@angle}%
  \csname tikz@label@angle@is@\tikz@label@angle\endcsname
  \ifx\tikz@label@angle\tikz@on@text%
    \def\tikz@node@at{\pgfpointanchor{\tikzlastnode}{center}}%
    \def\tikz@anchor{center}%
  \else%
    \iftikz@absolute%
      \pgftransformreset%
      \pgf@process{%
        \pgfpointshapeborder{\tikzlastnode}%
        {\pgfpointadd{\pgfpointanchor{\tikzlastnode}{center}}{\pgfpointpolar{\tikz@label@angle}{1pt}}}}%
      \edef\tikz@node@at{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      \tikz@compute@direction{\tikz@label@angle}%
      \tikz@addtransform{\pgftransformshift{\pgfpointpolar{\tikz@label@angle}{#1}}}%
    \else%
      \pgf@process{\pgfpointanchor{\tikzlastnode}{\tikz@label@angle}}%
      \edef\tikz@node@at{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
      \pgf@xb=\pgf@x%
      \pgf@yb=\pgf@y%
      \pgf@process{\pgfpointanchor{\tikzlastnode}{center}}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@y%
      \tikz@label@simplefalse%
      \ifdim\pgf@xc=\pgf@xb\relax%
        \ifdim\pgf@yc=\pgf@yb\relax%
          \tikz@label@simpletrue%
        \fi%
      \fi%
      \iftikz@label@simple%
        \tikz@compute@direction{\tikz@label@angle}%
        \tikz@addtransform{\pgftransformshift{\pgfpointpolar{\tikz@label@angle}{#1}}}%
      \else%
        \pgf@process{\pgfpointnormalised{%
            \pgfpointdiff{\pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}}{\pgfpointtransformed{\pgfqpoint{\pgf@xb}{\pgf@yb}}}}}%
        \edef\pgf@marshal{%
          \noexpand\tikz@addtransform{\noexpand\pgftransformshift{\noexpand\pgfpointscale{#1}{
                \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}}%
        \pgf@marshal%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgf@x=\pgf@yc%
        \pgf@y=-\pgf@xc%
        \ifx\tikz@anchor\tikz@auto@text%
          \tikz@auto@anchor%
        \fi%
      \fi%
    \fi%
  \fi}
}%

\newif\iftikz@label@simple%

\tikzset{%
  label/.code={%
    \begingroup
      \ifnum\the\catcode`\:=\active\relax
        \def\tikz@next{%
          \endgroup
          \tikz@parse@label@active@i{#1}}%
      \else
        \def\tikz@next{%
          \endgroup
          \pgfutil@ifnextchar[%]
            {\tikz@parse@label@nonactive}
            {\tikz@parse@label@nonactive[]}#1:\pgf@nil}%
      \fi
    \tikz@next}}%

\begingroup
  \catcode`\:=\active\relax

  \gdef\tikz@parse@label@active@i#1{%
    \pgfutil@ifnextchar[%]
      {\tikz@parse@label@active}
      {\tikz@parse@label@active[]}#1:\pgf@nil}%

  \gdef\tikz@parse@label@active[#1]#2:#3\pgf@nil{%
    \def\tikz@temp{#3}%
    \ifx\tikz@temp\pgfutil@empty
    % no position, use default
      \tikz@@parse@label@active[#1]\tikz@label@default@pos:#2:\pgf@nil%
    \else
      \def\tikz@temp{#2}%
      \ifx\tikz@temp\pgfutil@empty
        \tikz@@parse@label@active[#1]\tikz@label@default@pos:#3\pgf@nil%
      \else
        \tikz@@parse@label@active[#1]#2:#3\pgf@nil%
      \fi
    \fi
  }%

  \gdef\tikz@@parse@label@active[#1]#2:#3:\pgf@nil{%
    \tikzset{%
      append after command = {%
        \bgroup
          [current point is local=true]
          \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name\tikz@node@is@a@labelfalse}
          node [tikz@label@angle = #2,
                anchor=@auto,
                every label,
                #1,
                tikz@label@post = \tikz@label@distance] {\iftikz@handle@active@nodes\expandafter\scantokens\else\expandafter\pgfutil@firstofone\fi{#3\noexpand}}
          \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}
        \egroup}}}%
\endgroup

\def\tikz@parse@label@nonactive[#1]#2:#3\pgf@nil{%
  \def\tikz@temp{#3}%
  \ifx\tikz@temp\pgfutil@empty
    % no position, use default
    \tikz@@parse@label@nonactive[#1]\tikz@label@default@pos:#2:\pgf@nil%
  \else
    \def\tikz@temp{#2}%
    \ifx\tikz@temp\pgfutil@empty
      \tikz@@parse@label@nonactive[#1]\tikz@label@default@pos:#3\pgf@nil%
    \else
      \tikz@@parse@label@nonactive[#1]#2:#3\pgf@nil%
    \fi
  \fi
}%

\def\tikz@@parse@label@nonactive[#1]#2:#3:\pgf@nil{%
  \tikzset{%
    append after command = {%
      \bgroup
        [current point is local=true]
        \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name\tikz@node@is@a@labelfalse}
        node [tikz@label@angle = #2,
              anchor=@auto,
              every label,
              #1,
              tikz@label@post = \tikz@label@distance] {\iftikz@handle@active@nodes\expandafter\scantokens\else\expandafter\pgfutil@firstofone\fi{#3\noexpand}}
        \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}
      \egroup}}}%

\expandafter\def\csname tikz@label@angle@is@right\endcsname{\def\tikz@label@angle{0}}%
\expandafter\def\csname tikz@label@angle@is@above right\endcsname{\def\tikz@label@angle{45}}%
\expandafter\def\csname tikz@label@angle@is@above\endcsname{\def\tikz@label@angle{90}}%
\expandafter\def\csname tikz@label@angle@is@above left\endcsname{\def\tikz@label@angle{135}}%
\expandafter\def\csname tikz@label@angle@is@left\endcsname{\def\tikz@label@angle{180}}%
\expandafter\def\csname tikz@label@angle@is@below left\endcsname{\def\tikz@label@angle{225}}%
\expandafter\def\csname tikz@label@angle@is@below\endcsname{\def\tikz@label@angle{270}}%
\expandafter\def\csname tikz@label@angle@is@below right\endcsname{\def\tikz@label@angle{315}}%

\def\tikz@compute@direction#1{%
  \ifx\tikz@anchor\tikz@auto@text%
  \let\tikz@do@auto@anchor=\relax
  \pgfmathsetcount{\c@pgf@counta}{#1}%
  \ifnum\c@pgf@counta<0\relax
    \advance\c@pgf@counta by 360\relax%
  \fi%
  \ifnum\c@pgf@counta>359\relax
    \advance\c@pgf@counta by-360\relax%
  \fi%
  \ifnum\c@pgf@counta<4\relax%
    \def\tikz@anchor{west}%
  \else\ifnum\c@pgf@counta<87\relax%
    \def\tikz@anchor{south west}%
  \else\ifnum\c@pgf@counta<94\relax%
    \def\tikz@anchor{south}%
  \else\ifnum\c@pgf@counta<177\relax%
    \def\tikz@anchor{south east}%
  \else\ifnum\c@pgf@counta<184\relax%
    \def\tikz@anchor{east}%
  \else\ifnum\c@pgf@counta<267\relax%
    \def\tikz@anchor{north east}%
  \else\ifnum\c@pgf@counta<274\relax%
    \def\tikz@anchor{north}%
  \else\ifnum\c@pgf@counta<357\relax%
    \def\tikz@anchor{north west}%
  \else%
    \def\tikz@anchor{west}%
  \fi\fi\fi\fi\fi\fi\fi\fi%
  \fi%
}%
\def\tikz@auto@text{@auto}%

% General node options
\tikzset{
  name/.code={\edef\tikz@fig@name{\tikz@pp@name{#1}}\let\tikz@id@name\tikz@fig@name},%
  name prefix/.initial=,%
  name suffix/.initial=%
}%
\def\tikz@pp@name#1{\csname pgfk@/tikz/name prefix\endcsname#1\csname pgfk@/tikz/name suffix\endcsname}%


\tikzset{
  node contents/.code=\def\tikz@node@content{#1},
  pic type/.code=\def\tikz@node@content{#1}, % alias
}%

\tikzset{
  behind path/.code=\def\tikz@whichbox{\tikz@figbox@bg},
  in front of path/.code=\def\tikz@whichbox{\tikz@figbox}
}%
\def\tikz@whichbox{\tikz@figbox}%

\tikzoption{at}{\tikz@scan@one@point\tikz@set@at#1}%
\def\tikz@set@at#1{\def\tikz@node@at{#1}}%

\tikzoption{shape}{\edef\tikz@shape{#1}}%

\tikzoption{nodes}{\tikzset{every node/.append style={#1}}}%

\tikzset{alias/.code={%
    \tikz@fig@mustbenamed
    \begingroup
    \toks0=\expandafter{\tikz@alias}%
    \edef\pgf@temp{\noexpand\pgfnodealias{\tikz@pp@name{#1}}{\noexpand\tikz@fig@name}}%
    \toks1=\expandafter{\pgf@temp}%
    \xdef\pgf@marshal{%
        \noexpand\def\noexpand\tikz@alias{\the\toks0 \the\toks1 }%
    }%
    \endgroup
    \pgf@marshal
}}%

% deprecated:
\def\tikzaddafternodepathoption#1{#1\tikzset{prefix after command={\pgfextra{#1}}}}%
\tikzset{after node path/.style={append after command={#1}}}%


% Pic options
\newif\iftikz@node@is@pic
\tikzset{pic text/.store in=\tikzpictext}%
\let\tikzpictext\relax
\tikzset{pic text options/.store in=\tikzpictextoptions}%
\let\tikzpictextoptions\pgfutil@empty


% Anchoring

\tikzoption{anchor}{\def\tikz@anchor{#1}\let\tikz@do@auto@anchor=\relax}%

\tikzoption{left}[]{\def\tikz@anchor{east}\tikz@possibly@transform{x}{-}{#1}}%
\tikzoption{right}[]{\def\tikz@anchor{west}\tikz@possibly@transform{x}{}{#1}}%
\tikzoption{above}[]{\def\tikz@anchor{south}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{below}[]{\def\tikz@anchor{north}\tikz@possibly@transform{y}{-}{#1}}%
\tikzoption{above left}[]%
  {\def\tikz@anchor{south east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{above right}[]%
  {\def\tikz@anchor{south west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{}{#1}}%
\tikzoption{below left}[]%
  {\def\tikz@anchor{north east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{-}{#1}}%
\tikzoption{below right}[]%
  {\def\tikz@anchor{north west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{-}{#1}}%
\tikzset{centered/.code=\def\tikz@anchor{center}}%

\tikzoption{node distance}{\def\tikz@node@distance{#1}}%
\def\tikz@node@distance{1cm}%

% The following are deprecated:
\tikzoption{above of}{\tikz@of{#1}{90}}%
\tikzoption{below of}{\tikz@of{#1}{-90}}%
\tikzoption{left of}{\tikz@of{#1}{180}}%
\tikzoption{right of}{\tikz@of{#1}{0}}%
\tikzoption{above left of}{\tikz@of{#1}{135}}%
\tikzoption{below left of}{\tikz@of{#1}{-135}}%
\tikzoption{above right of}{\tikz@of{#1}{45}}%
\tikzoption{below right of}{\tikz@of{#1}{-45}}%
\def\tikz@of#1#2{%
  \def\tikz@anchor{center}%
  \let\tikz@do@auto@anchor=\relax%
  \tikz@addtransform{%
    \expandafter\tikz@extract@node@dist\tikz@node@distance and\pgf@stop%
    \pgftransformshift{\pgfpointpolar{#2}{\tikz@extracted@node@distance}}}%
  \def\tikz@node@at{\pgfpointanchor{\tikz@pp@name{#1}}{center}}}%
\def\tikz@extract@node@dist#1and#2\pgf@stop{%
  \def\tikz@extracted@node@distance{#1}}%

\tikzset{
  transform shape nonlinear/.is choice,
  transform shape nonlinear/.default=true,
  transform shape nonlinear/true/.code=\let\tikz@nlt\relax,
  transform shape nonlinear/false/.code=\def\tikz@nlt{\pgfapproximatenonlineartranslation},
  transform shape nonlinear=false,
}%


\tikzoption{transform shape}[true]{%
  \csname tikz@fullytransformed#1\endcsname%
  \iftikz@fullytransformed%
    \pgfresetnontranslationattimefalse%
  \else%
    \pgfresetnontranslationattimetrue%
  \fi%
}%

\newif\iftikz@fullytransformed
\pgfresetnontranslationattimetrue%

\def\tikz@anchor{center}%
\def\tikz@shape{rectangle}%

\def\tikz@possibly@transform#1#2#3{%
  \let\tikz@do@auto@anchor=\relax%
  \def\tikz@test{#3}%
  \ifx\tikz@test\pgfutil@empty%
  \else%
    \pgfmathsetlength{\pgf@x}{#3}%
    \pgf@x=#2\pgf@x\relax%
    \edef\tikz@marshal{\noexpand\tikz@addtransform{%
        \expandafter\noexpand\csname  pgftransform#1shift\endcsname{\the\pgf@x}}}%
    \tikz@marshal%
  \fi%
}%


% Inter-picture options
\tikzoption{remember picture}[true]{\csname pgfrememberpicturepositiononpage#1\endcsname}
\tikzset{
    overlay/.is choice,
    overlay/true/.code={\pgf@relevantforpicturesizefalse},
    overlay/false/.code={\pgf@relevantforpicturesizetrue},
    overlay/.default=true
}



% Line/curve label placement options
\tikzoption{sloped}[true]{\csname pgfslopedattime#1\endcsname}%
\tikzoption{allow upside down}[true]{\csname pgfallowupsidedownattime#1\endcsname}%

\tikzoption{pos}{\edef\tikz@time{#1}\ifx\tikz@time\pgfutil@empty\else\pgfmathsetmacro\tikz@time{\tikz@time}\fi}%

\tikzoption{auto}[]{\csname tikz@install@auto@anchor@#1\endcsname}%
\tikzoption{swap}[]{%
  \def\tikz@temp{left}%
  \ifx\tikz@auto@anchor@direction\tikz@temp%
    \def\tikz@auto@anchor@direction{right}%
  \else%
    \def\tikz@auto@anchor@direction{left}%
  \fi%
}%
\tikzset{'/.style=swap}% shorthand


\def\tikz@install@auto@anchor@{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on}%
\def\tikz@install@auto@anchor@false{\let\tikz@do@auto@anchor=\relax}%
\def\tikz@install@auto@anchor@left{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{left}}%
\def\tikz@install@auto@anchor@right{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{right}}%

\let\tikz@do@auto@anchor=\relax%

\def\tikz@auto@anchor@on{\csname tikz@auto@anchor@\tikz@auto@anchor@direction\endcsname}

\def\tikz@auto@anchor@left{\tikz@auto@pre\tikz@auto@anchor\tikz@auto@post}%
\def\tikz@auto@anchor@right{\tikz@auto@pre\tikz@auto@anchor@prime\tikz@auto@post}%

\def\tikz@auto@anchor@direction{left}%

% Text options
\tikzoption{text}{\def\tikz@textcolor{#1}}%
\tikzoption{font}{\def\tikz@textfont{#1}}%
\tikzoption{node font}{\def\tikz@node@textfont{#1}}%
\tikzoption{text opacity}{\def\tikz@textopacity{#1}}%
\tikzoption{text width}{\def\tikz@text@width{#1}}%
\tikzoption{text height}{\def\tikz@text@height{#1}}%
\tikzoption{text depth}{\def\tikz@text@depth{#1}}%
\tikzoption{text ragged}[]%
{\def\tikz@text@action{\pgfutil@raggedright\rightskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}}%
\tikzoption{text badly ragged}[]{\def\tikz@text@action{\pgfutil@raggedright\relax}}%
\tikzoption{text ragged left}[]%
{\def\tikz@text@action{\pgfutil@raggedleft\leftskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}}%
\tikzoption{text badly ragged left}[]{\def\tikz@text@action{\pgfutil@raggedleft\relax}}%
\tikzoption{text justified}[]{\def\tikz@text@action{\leftskip0pt\rightskip0pt\relax}}%
\tikzoption{text centered}[]{\def\tikz@text@action{%
  \leftskip0pt plus2em%
  \rightskip0pt plus2em%
  \spaceskip.3333em \xspaceskip.5em%
  \parfillskip=0pt%
  \iftikz@warn@for@narrow@centered\else\hbadness10000\fi%
  \let\\=\@centercr% for latex
  \relax}}%
\tikzoption{text badly centered}[]%
{\def\tikz@text@action{%
  \let\\=\@centercr% for latex
  \parfillskip=0pt%
  \rightskip\pgfutil@flushglue%
  \leftskip\pgfutil@flushglue\relax}}%
\tikzset{badness warnings for centered text/.is if=tikz@warn@for@narrow@centered}%
\newif\iftikz@warn@for@narrow@centered

\def\tikz@text@reset{%
  \let\tikz@text@width=\pgfutil@empty
  \let\tikz@text@height=\pgfutil@empty
  \let\tikz@text@depth=\pgfutil@empty
  \let\tikz@textcolor=\pgfutil@empty
  \let\tikz@textfont=\pgfutil@empty
  \let\tikz@textopacity=\pgfutil@empty
  \let\tikz@node@textfont=\pgfutil@empty
  \def\tikz@text@action{\pgfutil@raggedright\rightskip0pt plus2em \spaceskip.3333em \xspaceskip.5em\relax}%
}
\tikz@text@reset


% Alignment
\tikzset{
  node halign header/.initial=,
  align/.is choice,
  align/left/.style  ={text ragged,node halign header=\tikz@align@left@header},
  align/flush left/.style  ={text badly ragged,node halign header=\tikz@align@left@header},
  align/right/.style ={text ragged left,node halign header=\tikz@align@right@header},
  align/flush right/.style ={text badly ragged left,node halign header=\tikz@align@right@header},
  align/center/.style={text centered,node halign header=\tikz@align@center@header},
  align/flush center/.style={text badly centered,node halign header=\tikz@align@center@header},
  align/justify/.style ={text justified,node halign header=\tikz@align@left@header},
  align/none/.style ={text justified,node halign header=},
}%
\def\tikz@align@left@header{##\hfil\cr}%
\def\tikz@align@right@header{\hfil##\cr}%
\def\tikz@align@center@header{\hfil##\hfil\cr}%



% Arrow options
\tikzoption{arrows}{\tikz@processarrows{#1}}%


\tikzoption{>}{\pgfdeclarearrow{name=<->,means={#1}}}%
\pgfdeclarearrow{name=|<->|,   means={>[sep=0pt].|}}%

\tikzoption{shorten <}{\pgfsetshortenstart{#1}}%
\tikzoption{shorten >}{\pgfsetshortenend{#1}}%

\def\tikz@processarrows#1{%
  \def\tikz@current@arrows{#1}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else%
    \pgfsetarrows{#1}%
  \fi%
}%

\def\tikz@current@arrows{-}%

% Parabola options
\tikzoption{bend}{\tikz@scan@one@point\tikz@set@parabola@bend#1\relax}%
\tikzoption{bend pos}{\def\tikz@parabola@bend@factor{#1}}%
\tikzoption{parabola height}{%
  \def\tikz@parabola@bend@factor{.5}%
  \def\tikz@parabola@bend{\pgfpointadd{\pgfpoint{0pt}{#1}}{\tikz@last@position@saved}}}%

\def\tikz@parabola@bend{\tikz@last@position@saved}%
\def\tikz@parabola@bend@factor{0}%

\def\tikz@set@parabola@bend#1{\def\tikz@parabola@bend{#1}}%

% Axis options
\tikzoption{domain}{\edef\tikz@plot@domain{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}%
\tikzoption{range}{\def\tikz@plot@range{#1}}%
\tikzoption{yrange}{\def\tikz@plot@range{#1}}%
\let\tikz@plot@range=\pgfutil@empty
\tikzoption{xrange}{\def\tikz@plot@xrange{#1}}%
\let\tikz@plot@xrange=\pgfutil@empty

% Plot options
\tikzoption{smooth}[]{\let\tikz@plot@handler=\pgfplothandlercurveto}%
\tikzoption{smooth cycle}[]{\let\tikz@plot@handler=\pgfplothandlerclosedcurve}%
\tikzoption{sharp plot}[]{\let\tikz@plot@handler\pgfplothandlerlineto}%
\tikzoption{sharp cycle}[]{\let\tikz@plot@handler\pgfplothandlerpolygon}%

\tikzoption{tension}{\pgfsetplottension{#1}}%

\tikzoption{xcomb}[]{\let\tikz@plot@handler=\pgfplothandlerxcomb}%
\tikzoption{ycomb}[]{\let\tikz@plot@handler=\pgfplothandlerycomb}%
\tikzoption{polar comb}[]{\let\tikz@plot@handler=\pgfplothandlerpolarcomb}%
\tikzoption{ybar}[]{\let\tikz@plot@handler=\pgfplothandlerybar}%
\tikzoption{ybar interval}[]{\let\tikz@plot@handler=\pgfplothandlerybarinterval}%
\tikzoption{xbar interval}[]{\let\tikz@plot@handler=\pgfplothandlerxbarinterval}%
\tikzoption{xbar}[]{\let\tikz@plot@handler=\pgfplothandlerxbar}%
\tikzoption{const plot}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}%
\tikzoption{const plot mark left}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlineto}%
\tikzoption{const plot mark right}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkright}%
\tikzoption{const plot mark mid}[]{\let\tikz@plot@handler=\pgfplothandlerconstantlinetomarkmid}%
\tikzoption{jump mark right}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkright}%
\tikzoption{jump mark mid}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkmid}%
\tikzoption{jump mark left}[]{\let\tikz@plot@handler=\pgfplothandlerjumpmarkleft}%

\tikzoption{raw gnuplot}[true]{\csname tikz@plot@raw@gnuplot#1\endcsname}%
\tikzoption{prefix}{\def\tikz@plot@prefix{#1}}%
\tikzoption{id}{\def\tikz@plot@id{#1}}%

\tikzoption{samples}{\pgfmathsetmacro\tikz@plot@samples{max(2,#1)}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}%
\tikzoption{samples at}{\def\tikz@plot@samplesat{#1}}%
\tikzoption{parametric}[true]{\csname tikz@plot@parametric#1\endcsname}%

\tikzoption{variable}{\def\tikz@plot@var{#1}}%

\tikzoption{only marks}[]{\let\tikz@plot@handler\pgfplothandlerdiscard}%

\tikzoption{mark}{%
    \def\tikz@plot@mark{#1}%
    \def\tikz@temp{none}%
    \ifx\tikz@temp\tikz@plot@mark
        \let\tikz@plot@mark=\pgfutil@empty
    \fi
}%
\tikzset{
    no marks/.style={mark=none},%
    no markers/.style={mark=none},%
    every mark/.style={},
    mark options/.style={%
        every mark/.style={#1}%
    }}%
\tikzoption{mark size}{\pgfsetplotmarksize{#1}}%

\tikzoption{mark indices}{\def\tikz@mark@list{#1}}%
\tikzoption{mark phase}{\pgfsetplotmarkphase{#1}}%
\tikzoption{mark repeat}{\pgfsetplotmarkrepeat{#1}}%

\let\tikz@mark@list=\pgfutil@empty

\let\tikz@plot@handler=\pgfplothandlerlineto
\let\tikz@plot@mark=\pgfutil@empty

\def\tikz@plot@samples{25}%
\def\tikz@plot@domain{-5:5}%
\def\tikz@plot@var{\x}%
\def\tikz@plot@samplesat{-5,-4.5833333,...,5}%
\def\tikz@plot@samples@recalc#1:#2\relax{%
  \begingroup
  \pgfmathparse{#1}%
  \let\tikz@temp@start=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\tikz@temp@end=\pgfmathresult%
  \pgfmathsetmacro\tikz@temp@diff{(\tikz@temp@end-\tikz@temp@start)/(\tikz@plot@samples-1)}%
  %
  % this particular item is for backwards compatibility.
  % Pgfplots <= 1.8 called 'samples' in a context where the 'fpu' was
  % active... and I fear there is no simple solution to replace the
  % new \ifdim below. Sorry.
  \pgfkeys{/pgf/fpu/output format/fixed/.try}%
  %
  \pgfmathsetmacro\tikz@temp@diff@abs{abs(\tikz@temp@diff)}%
  \ifdim\tikz@temp@diff@abs pt<0.0001pt\relax%
    \edef\tikz@plot@samplesat{\tikz@temp@start,\tikz@temp@end}%
  \else%
    \pgfmathparse{\tikz@temp@start+\tikz@temp@diff}%
    \edef\tikz@plot@samplesat{\tikz@temp@start,\pgfmathresult,...,\tikz@temp@end}%
  \fi%
  \pgfmath@smuggleone\tikz@plot@samplesat
  \endgroup
}%


\def\tikz@plot@prefix{\jobname.}%
\def\tikz@plot@id{pgf-plot}%

\newif\iftikz@plot@parametric
\newif\iftikz@plot@raw@gnuplot


%
% To and edge options
%
\tikzoption{to path}{\def\tikz@to@path{#1}}%

\def\tikz@to@path{-- (\tikztotarget) \tikztonodes}%

\tikzset{edge macro/.store in=\tikz@edge@macro}%
\let\tikz@edge@macro\pgfutil@empty

\tikzset{
  edge node/.code={
    \expandafter\def\expandafter\tikz@tonodes\expandafter{\tikz@tonodes #1}
  },
  edge label/.style={/tikz/edge node={node[auto]{#1}}},
  edge label'/.style={/tikz/edge node={node[auto,swap]{#1}}},
}%


% After command options
\tikzset{
  append after command/.code=\expandafter\def\expandafter\tikz@after@path\expandafter{\tikz@after@path#1},
  prefix after command/.code={%
    \def\tikz@temp{#1}%
    \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter\tikz@after@path%
    \expandafter\expandafter\expandafter{%
      \expandafter\tikz@temp\tikz@after@path}%
  },
}%
\let\tikz@after@path\pgfutil@empty


% Tree options
\newif\iftikz@child@missing
\pgfkeys{/tikz/missing/.is if=tikz@child@missing}%

\tikzset{edge from parent macro/.initial=\tikz@edge@from@parent@macro}%
\def\tikz@edge@from@parent@macro#1#2{
  [style=edge from parent, #1, /utils/exec=\tikz@node@is@a@labeltrue] \tikz@edge@to@parent@path #2}%

\tikzoption{edge from parent path}{\def\tikz@edge@to@parent@path{#1}}%

\tikzoption{parent anchor}{\def\tikzparentanchor{.#1}\ifx\tikzparentanchor\tikz@border@text\let\tikzparentanchor\pgfutil@empty\fi}%
\tikzoption{child anchor}{\def\tikzchildanchor{.#1}\ifx\tikzchildanchor\tikz@border@text\let\tikzchildanchor\pgfutil@empty\fi}%

\tikzoption{level distance}{\pgfmathsetlength\tikzleveldistance{#1}}%
\tikzoption{sibling distance}{\pgfmathsetlength\tikzsiblingdistance{#1}}%

\tikzoption{growth function}{\let\tikz@grow=#1}%

\tikzset{grow siblings on line/.style={growth function=\tikz@grow@direction}}%

\tikzoption{growth parent anchor}{\def\tikz@growth@anchor{#1}}%
\tikzoption{grow}{\tikz@set@growth{#1}\edef\tikz@special@level{\the\tikztreelevel}}%
\tikzoption{grow'}{\tikz@set@growth{#1}\tikz@swap@growth\edef\tikz@special@level{\the\tikztreelevel}}%

\def\tikz@growth@anchor{center}%

\def\tikz@special@level{-1}% never

\def\tikz@swap@growth{%
  % Swap left and right
  \let\tikz@temp=\tikz@angle@grow@right%
  \let\tikz@angle@grow@right=\tikz@angle@grow@left%
  \let\tikz@angle@grow@left=\tikz@temp%
}%

\def\tikz@set@growth#1{%
  \let\tikz@grow=\tikz@grow@direction%
  \expandafter\ifx\csname tikz@grow@direction@#1\endcsname\relax%
    \c@pgf@counta=#1\relax%
  \else%
    \c@pgf@counta=\csname tikz@grow@direction@#1\endcsname%
  \fi%
  \edef\tikz@angle@grow{\the\c@pgf@counta}%
  \advance\c@pgf@counta by-90\relax%
  \edef\tikz@angle@grow@left{\the\c@pgf@counta}%
  \advance\c@pgf@counta by180\relax%
  \edef\tikz@angle@grow@right{\the\c@pgf@counta}%
}%

\def\tikz@border@text{.border}%
\let\tikzparentanchor=\pgfutil@empty
\let\tikzchildanchor=\pgfutil@empty
\def\tikz@edge@to@parent@path{(\tikzparentnode\tikzparentanchor) -- (\tikzchildnode\tikzchildanchor)}%

\tikzleveldistance=15mm%
\tikzsiblingdistance=15mm%

\def\tikz@grow@direction@down{-90}%
\def\tikz@grow@direction@up{90}%
\def\tikz@grow@direction@left{180}%
\def\tikz@grow@direction@right{0}%

\def\tikz@grow@direction@south{-90}%
\def\tikz@grow@direction@north{90}%
\def\tikz@grow@direction@west{180}%
\def\tikz@grow@direction@east{0}%

\expandafter\def\csname tikz@grow@direction@north east\endcsname{45}%
\expandafter\def\csname tikz@grow@direction@north west\endcsname{135}%
\expandafter\def\csname tikz@grow@direction@south east\endcsname{-45}%
\expandafter\def\csname tikz@grow@direction@south west\endcsname{-135}%

\def\tikz@grow@direction{%
  \pgftransformshift{\pgfpointpolar{\tikz@angle@grow}{\tikzleveldistance}}%
  \ifnum\tikztreelevel=\tikz@special@level%
  \else%
    \pgf@xc=.5\tikzsiblingdistance%
    \c@pgf@counta=\tikznumberofchildren%
    \advance\c@pgf@counta by1\relax%
    \pgfutil@tempdima=\c@pgf@counta\pgf@xc%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@left}{\pgfutil@tempdima}}%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@right}{\tikznumberofcurrentchild\tikzsiblingdistance}}%
  \fi%
}%

\tikzset{grow=down}%


% Snakes are in a lib:
\tikzset{snake/.code=\tikzerror{You need to say \string\usetikzlibrary{snakes}}}%

% Decorations
\tikzset{decorate/.code=\tikzerror{You need to load a  decoration library}}%

% Matrix options
\usepgfmodule{matrix}%

\tikzoption{matrix}[true]{\csname tikz@is@matrix#1\endcsname}%

\tikzoption{matrix anchor}{\def\tikz@matrix@anchor{#1}}%

\tikzoption{column sep}{\def\pgfmatrixcolumnsep{#1}}%
\tikzoption{row sep}{\def\pgfmatrixrowsep{#1}}%

\tikzoption{cells}{\tikzset{every cell/.append style={#1}}}%

\tikzoption{ampersand replacement}{\def\tikz@ampersand@replacement{#1}}%

\newif\iftikz@is@matrix
\let\tikz@matrix@anchor=\pgfutil@empty
\let\tikz@ampersand@replacement=\pgfutil@empty


% Automatic shorthand management
\tikzset{%
  handle active characters in code/.is if=tikz@handle@active@code,
  handle active characters in nodes/.is if=tikz@handle@active@nodes,
}%
\newif\iftikz@handle@active@code
\newif\iftikz@handle@active@nodes


% Execute option
\tikzoption{execute at begin picture}{\expandafter\def\expandafter\tikz@atbegin@picture\expandafter{\tikz@atbegin@picture#1}}%
\tikzoption{execute at end picture}{\expandafter\def\expandafter\tikz@atend@picture\expandafter{\tikz@atend@picture#1}}%
\tikzoption{execute at begin scope}{\expandafter\def\expandafter\tikz@atbegin@scope\expandafter{\tikz@atbegin@scope#1}}%
\tikzoption{execute at end scope}{\expandafter\def\expandafter\tikz@atend@scope\expandafter{\tikz@atend@scope#1}}%
\tikzoption{execute at begin to}{\expandafter\def\expandafter\tikz@atbegin@to\expandafter{\tikz@atbegin@to#1}}%
\tikzoption{execute at end to}{\expandafter\def\expandafter\tikz@atend@to\expandafter{\tikz@atend@to#1}}%
\tikzoption{execute at begin node}{\expandafter\def\expandafter\tikz@atbegin@node\expandafter{\tikz@atbegin@node#1}}%
\tikzoption{execute at end node}{\expandafter\def\expandafter\tikz@atend@node\expandafter{\tikz@atend@node#1}}%
\tikzoption{execute at begin matrix}{\expandafter\def\expandafter\tikz@atbegin@matrix\expandafter{\tikz@atbegin@matrix#1}}%
\tikzoption{execute at end matrix}{\expandafter\def\expandafter\tikz@atend@matrix\expandafter{\tikz@atend@matrix#1}}%
\tikzoption{execute at begin cell}{\expandafter\def\expandafter\tikz@atbegin@cell\expandafter{\tikz@atbegin@cell#1}}%
\tikzoption{execute at end cell}{\expandafter\def\expandafter\tikz@atend@cell\expandafter{\tikz@atend@cell#1}}%
\tikzoption{execute at empty cell}{\expandafter\def\expandafter\tikz@at@emptycell\expandafter{\tikz@at@emptycell#1}}%

\let\tikz@atbegin@picture=\pgfutil@empty
\let\tikz@atend@picture=\pgfutil@empty
\let\tikz@atbegin@scope=\pgfutil@empty
\let\tikz@atend@scope=\pgfutil@empty
\let\tikz@atbegin@to=\pgfutil@empty
\let\tikz@atend@to=\pgfutil@empty
\let\tikz@atbegin@node=\pgfutil@empty
\let\tikz@atend@node=\pgfutil@empty
\let\tikz@atbegin@cell=\pgfutil@empty
\let\tikz@atend@cell=\pgfutil@empty
\let\tikz@at@emptycell=\pgfutil@empty
\let\tikz@atbegin@matrix=\pgfutil@empty
\let\tikz@atend@matrix=\pgfutil@empty


% Pre and post actions
\tikzset{preaction/.code=\expandafter\def\expandafter\tikz@preactions\expandafter{\tikz@preactions\tikz@extra@preaction{#1}}}%
\tikzset{postaction/.code=\expandafter\def\expandafter\tikz@postactions\expandafter{\tikz@postactions\tikz@extra@postaction{#1}}}%
\let\tikz@preactions=\pgfutil@empty
\let\tikz@postactions=\pgfutil@empty

% Styles
\tikzoption{set style}{\tikzstyle#1}%

% Handled in a special way.
\def\tikzstyle{\pgfutil@ifnextchar\bgroup\tikz@style@parseA\tikz@style@parseB}%
\def\tikz@style@parseB#1={\tikz@style@parseA{#1}=}%
\def\tikz@style@parseA#1#2=#3[#4]{% check for an optional argument
  \pgfutil@in@[{#2}%]
  \ifpgfutil@in@%
    \tikz@style@parseC{#1}#2={#4}%
  \else%
    \tikz@style@parseD{#1}#2={#4}%
  \fi%
}%

\def\tikz@style@parseC#1[#2]#3=#4{%
  \pgfkeys{/tikz/#1/.default={#2}}%
  \pgfutil@in@+{#3}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#4}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#4}}%
  \fi}%
\def\tikz@style@parseD#1#2=#3{%
  \pgfutil@in@+{#2}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#3}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#3}}%
  \fi}%


%
%
% Predefined styles
%
%

\tikzset{help lines/.style=              {color=gray,line width=0.2pt}}%

\tikzset{every picture/.style=           {}}%
\tikzset{every path/.style=              {}}%
\tikzset{every scope/.style=             {}}%
\tikzset{every plot/.style=              {}}%
\tikzset{every node/.style=              {}}%
\tikzset{every child/.style=             {}}%
\tikzset{every child node/.style=        {}}%
\tikzset{every to/.style=                {}}%
\tikzset{every cell/.style=              {}}%
\tikzset{every matrix/.style=            {}}%
\tikzset{every edge/.style=              {draw}}%
\tikzset{every label/.style=             {draw=none,fill=none}}%
\tikzset{every pin/.style=               {draw=none,fill=none}}%
\tikzset{every pin edge/.style=          {help lines}}%

\tikzset{ultra thin/.style=              {line width=0.1pt}}%
\tikzset{very thin/.style=               {line width=0.2pt}}%
\tikzset{thin/.style=                    {line width=0.4pt}}%
\tikzset{semithick/.style=               {line width=0.6pt}}%
\tikzset{thick/.style=                   {line width=0.8pt}}%
\tikzset{very thick/.style=              {line width=1.2pt}}%
\tikzset{ultra thick/.style=             {line width=1.6pt}}%

\tikzset{solid/.style=                   {dash pattern=}}%
\tikzset{dotted/.style=                  {dash pattern=on \pgflinewidth off 2pt}}%
\tikzset{densely dotted/.style=          {dash pattern=on \pgflinewidth off 1pt}}%
\tikzset{loosely dotted/.style=          {dash pattern=on \pgflinewidth off 4pt}}%
\tikzset{dashed/.style=                  {dash pattern=on 3pt off 3pt}}%
\tikzset{densely dashed/.style=          {dash pattern=on 3pt off 2pt}}%
\tikzset{loosely dashed/.style=          {dash pattern=on 3pt off 6pt}}%
\tikzset{dashdotted/.style=              {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{dash dot/.style=                {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dashdotted/.style=      {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{densely dash dot/.style=        {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dashdotted/.style=      {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{loosely dash dot/.style=        {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{dashdotdotted/.style=           {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dashdotdotted/.style=   {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dashdotdotted/.style=   {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt on \the\pgflinewidth off 4pt}}%
\tikzset{dash dot dot/.style=         {dash pattern=on 3pt off 2pt on \the\pgflinewidth off 2pt on \the\pgflinewidth off 2pt}}%
\tikzset{densely dash dot dot/.style=   {dash pattern=on 3pt off 1pt on \the\pgflinewidth off 1pt on \the\pgflinewidth off 1pt}}%
\tikzset{loosely dash dot dot/.style=   {dash pattern=on 3pt off 4pt on \the\pgflinewidth off 4pt on \the\pgflinewidth off 4pt}}%


\tikzset{transparent/.style=             {opacity=0}}%
\tikzset{ultra nearly transparent/.style={opacity=0.05}}%
\tikzset{very nearly transparent/.style= {opacity=0.1}}%
\tikzset{nearly transparent/.style=      {opacity=0.25}}%
\tikzset{semitransparent/.style=         {opacity=0.5}}%
\tikzset{nearly opaque/.style=           {opacity=0.75}}%
\tikzset{very nearly opaque/.style=      {opacity=0.9}}%
\tikzset{ultra nearly opaque/.style=     {opacity=0.95}}%
\tikzset{opaque/.style=                  {opacity=1}}%

\tikzset{at start/.style=                {pos=0}}%
\tikzset{very near start/.style=         {pos=0.125}}%
\tikzset{near start/.style=              {pos=0.25}}%
\tikzset{midway/.style=                  {pos=0.5}}%
\tikzset{near end/.style=                {pos=0.75}}%
\tikzset{very near end/.style=           {pos=0.875}}%
\tikzset{at end/.style=                  {pos=1}}%

\tikzset{bend at start/.style=           {bend pos=0,bend={+(0,0)}}}%
\tikzset{bend at end/.style=             {bend pos=1,bend={+(0,0)}}}%

\tikzset{edge from parent/.style=        {draw}}%



% Animation callbacks
\tikzset{
  animate/.code=\tikzerror{You need to say \string\usetikzlibrary{animations} to use animations}
}

% ID callbacks
\newif\iftikz@is@node
\let\tikz@id@name\pgfutil@empty
\let\tikz@id@hook\pgfutil@empty
\def\tikz@call@id@hook{\ifx\tikz@id@hook\pgfutil@empty\else\tikz@id@hook\pgfuseid{\tikz@id@name}\fi}%


% RDF stuff
\let\tikz@clear@rdf@options\relax
\let\tikz@do@rdf@post@options\relax
\let\tikz@do@rdf@pre@options\relax


%
% Setting keys
%

\pgfkeys{/tikz/style/.style=#1}%

\pgfkeys{/tikz/.unknown/.code=%
  % Is it a pgf key?
  \let\tikz@key\pgfkeyscurrentname%
  \pgfkeys{/pgf/\tikz@key/.try={#1}}%
  \ifpgfkeyssuccess%
  \else%
    \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
    \ifpgfutil@in@%
      % this is a color!
      \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
      \edef\tikz@textcolor{\tikz@key}%
    \else%
      \pgfutil@doifcolorelse{\tikz@key}
      {%
        \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
        \edef\tikz@textcolor{\tikz@key}%
      }%
      {%
        % Ok, second chance: This might be an arrow specification:
        \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          % Ah, an arrow spec!
          \expandafter\tikz@processarrows\expandafter{\tikz@key}%
        \else%
          % Ok, third chance: A shape!
          \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
            \pgfkeys{/errors/unknown key/.expand
              once=\expandafter{\expandafter/\expandafter t\expandafter i\expandafter k\expandafter z\expandafter/\tikz@key}{#1}}%
          \else%
            \edef\tikz@shape{\tikz@key}%
          \fi%
        \fi%
      }%
    \fi%
  \fi%
}%
\def\tikz@compat@color@set#1{%
  \pgfutil@color{#1}\pgfutil@colorlet{pgffillcolor}{#1}%
  \expandafter\let\expandafter\pgf@temp\csname\string\color@pgffillcolor\endcsname%
  % for arrow tips:
  \global\let\pgf@strokecolor@global=\pgf@temp
  \global\let\pgf@fillcolor@global=\pgf@temp
}%

\def\tikz@startup@env{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\expandafter\tikz@origsemi\expandafter=\tikz@activesemicolon\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\expandafter\tikz@origcolon\expandafter=\tikz@activecolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\expandafter\tikz@origbar\expandafter=\tikz@activebar\fi%
  \tikz@deactivatthings%
  \iftikz@handle@active@code%
    \tikz@switchoff@shorthands%
  \fi%
}%

%
% Main TikZ Environment
%
\newif\iftikz@inside@picture
\tikz@inside@picturefalse
\def\tikz@check@inside@picture{%
  \iftikz@inside@picture%
    \pgfwarning{Nesting tikzpictures is NOT supported}%
  \fi%
  \tikz@inside@picturetrue%
}

\def\tikzpicture{%
  \begingroup%
    \tikz@startup@env%
    \tikz@collect@scope@anims\tikz@picture}%
\def\tikz@picture[#1]{%
  %\tikz@check@inside@picture%
  \pgfpicture%
  \let\tikz@atbegin@picture=\pgfutil@empty%
  \let\tikz@atend@picture=\pgfutil@empty%
  \let\tikz@transform=\relax%
  \def\tikz@time{.5}%
  \tikz@installcommands%
  \scope[every picture,#1]%
  \iftikz@handle@active@code%
    \tikz@switchoff@shorthands%
  \fi%
  \expandafter\tikz@atbegin@picture%
  \tikz@lib@scope@check%
}%
\def\endtikzpicture{%
    \tikz@atend@picture%
    \global\let\pgf@shift@baseline@smuggle=\pgf@baseline%
    \global\let\pgf@trimleft@final@smuggle=\pgf@trimleft%
    \global\let\pgf@trimright@final@smuggle=\pgf@trimright%
    \global\let\pgf@remember@smuggle=\ifpgfrememberpicturepositiononpage%
    \pgf@remember@layerlist@globally
    \endscope%
    \let\pgf@baseline=\pgf@shift@baseline@smuggle%
    \let\pgf@trimleft=\pgf@trimleft@final@smuggle%
    \let\pgf@trimright=\pgf@trimright@final@smuggle%
    \let\ifpgfrememberpicturepositiononpage=\pgf@remember@smuggle%
    \pgf@restore@layerlist@from@global
  \endpgfpicture\endgroup}%


% Inlined picture
%
% #1 - some code to be put in a tikzpicture environment.
%
% If the command is not followed by braces, everything up to the next
% semicolon is used as argument.
%
% Example:
%
% The rectangle \tikz{\draw (0,0) rectangle (1em,1ex)} has width 1em and
% height 1ex.


\def\tikz{%
  \begingroup%
    \tikz@startup@env%
    \tikz@collect@scope@anims\tikz@opt}%
\def\tikz@opt[#1]{\tikzpicture[#1]\pgfutil@ifnextchar\bgroup{\tikz@}{\tikz@@single}}%
\def\tikz@{\bgroup\tikz@auto@end@pathtrue\aftergroup\endtikzpicture\aftergroup\endgroup\let\pgf@temp=}%
\def\tikz@@single#1{%
  \expandafter\ifx\csname tikz@protected@command\string#1\endcsname\relax%
    \expandafter\tikz@@%
  \else%
    \begingroup\def\tikz@path@do@at@end{\endgroup\endtikzpicture\endgroup}%
  \fi%
  #1%
}%

\expandafter\let\csname tikz@protected@command\string\draw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\pattern\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\fill\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\filldraw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\shade\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\shadedraw\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\clip\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\graph\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\useasboundingbox\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\node\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\coordinate\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\matrix\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\datavisualization\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\path\endcsname\pgfutil@empty%
\expandafter\let\csname tikz@protected@command\string\pic\endcsname\pgfutil@empty%

% Comment by TT: I hope I fixed the \tikz \foreach problem. The new
% version will take a conservative approach and will only do fancy
% stuff when the next keyword after \tikz is one of the following:
% \draw, \fill, \filldraw, \graph, \matrix,
\def\tikz@@{%
  \let\tikz@next=\tikz@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@collectactivesemicolon%
  \fi%
  \tikz@next}%
\def\tikz@collectnormalsemicolon#1;{#1;\endtikzpicture\endgroup}
{
  \catcode`\;=\active
  \gdef\tikz@collectactivesemicolon#1;{#1;\endtikzpicture\endgroup}
}%
% End old code

% Invokes '#1' if the command is invoked within a tikzpicture and
% '#2' if not.
\def\tikzifinpicture#1#2{%
    \pgfutil@ifundefined{filldraw}{#2}{#1}% TT: This is a wrong
                                % test! Who uses this?...
}%


\def\tikz@collect@scope@anims#1{%
  \pgfutil@ifnextchar[#1{#1[]}%]
}%

%
% Environment for scoping graphic state settings
%
\def\tikz@scope@env{%
  \pgfscope%
  \begingroup%
  \let\tikz@atbegin@scope=\pgfutil@empty%
  \let\tikz@atend@scope=\pgfutil@empty%
  \let\tikz@options=\pgfutil@empty%
  \tikz@clear@rdf@options%
  \let\tikz@mode=\pgfutil@empty%
  \let\tikz@id@name=\pgfutil@empty%
  \tikz@transparency@groupfalse%
  \tikzset{every scope/.try}%
  \tikz@collect@scope@anims\tikz@scope@opt%
}%
\def\tikz@scope@opt[#1]{%
  \tikzset{#1}%
  \tikz@options%
  \tikz@do@rdf@pre@options%
  \iftikz@transparency@group\expandafter\pgftransparencygroup\expandafter[\tikz@transparency@group@options]\tikz@blend@group\fi%
  \tikz@is@nodefalse%
  \tikz@call@id@hook%
  \pgfidscope%
    \tikz@do@rdf@post@options%
    \begingroup%
      \let\tikz@id@name\pgfutil@empty%
      \expandafter\tikz@atbegin@scope%
      \expandafter\pgfclearid%
      \tikz@lib@scope@check%
}%
\def\endtikz@scope@env{%
      \tikz@atend@scope%
    \endgroup%
  \endpgfidscope%
  \iftikz@transparency@group\endpgftransparencygroup\fi%
  \endgroup%
  \endpgfscope%
  \tikz@lib@scope@check%
}%


\def\tikz@scoped{\tikz@collect@scope@anims\tikz@scoped@opt}%
\def\tikz@scoped@opt[#1]{\scope[#1]\pgfutil@ifnextchar\bgroup{\tikz@scoped@}{\tikz@scoped@@single}}%
\def\tikz@scoped@{\bgroup\tikz@auto@end@pathtrue\aftergroup\endscope\let\pgf@temp=}%
\def\tikz@scoped@@single#1{%
  \expandafter\ifx\csname tikz@scoped@protected@command\string#1\endcsname\relax%
    \expandafter\tikz@scoped@@%
  \else%
    \begingroup\def\tikz@scoped@path@do@at@end{\endgroup\endscope}%
  \fi%
  #1%
}%
\def\tikz@scoped@@{%
  \let\tikz@scoped@next=\tikz@scoped@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@scoped@next=\tikz@scoped@collectactivesemicolon%
  \fi%
  \tikz@scoped@next}%
\def\tikz@scoped@collectnormalsemicolon#1;{#1;\endscope}
{
  \catcode`\;=\active
  \gdef\tikz@scoped@collectactivesemicolon#1;{#1;\endscope}
}%


% Install a shortcut command which is only valid inside of a
% tikzpicture.
%
% It works in the same way as the '\path' shortcut does: it introduces
% a \let#1=#2 at the beginning of tikzpicture.
%
% #1: shortcut command inside of tikzpicture
% #2: real command name
\def\tikzaddtikzonlycommandshortcutlet#1#2{%
    \expandafter\def\expandafter\tikz@installcommands\expandafter{\tikz@installcommands
        \let#1=#2%
    }%
}%

% Has the same effect as \tikzaddtikzonlycommandshortcutlet but uses
% \def#1{#2} instead of \let.
\def\tikzaddtikzonlycommandshortcutdef#1#2{%
    \expandafter\def\expandafter\tikz@installcommands\expandafter{\tikz@installcommands
        \def#1{#2}%
    }%
}%

%
% Install the abbreviated commands
%
\def\tikz@installcommands{%
  \let\tikz@origscope=\scope%
  \let\tikz@origscoped=\scoped%
  \let\tikz@origendscope=\endscope%
  \let\tikz@origstartscope=\startscope%
  \let\tikz@origstopscope=\stopscope%
  \let\tikz@origpath=\path%
  \let\tikz@origagainpath=\againpath%
  \let\tikz@origdraw=\draw%
  \let\tikz@origpattern=\pattern%
  \let\tikz@origfill=\fill%
  \let\tikz@origfilldraw=\filldraw%
  \let\tikz@origshade=\shade%
  \let\tikz@origshadedraw=\shadedraw%
  \let\tikz@origclip=\clip%
  \let\tikz@origuseasboundingbox=\useasboundingbox%
  \let\tikz@orignode=\node%
  \let\tikz@origpic=\pic%
  \let\tikz@origcoordinate=\coordinate%
  \let\tikz@origmatrix=\matrix%
  \let\tikz@origcalendar=\calendar%
  \let\tikz@origdv=\datavisualization%
  \let\tikz@origgraph=\graph%
  %
  \let\scope=\tikz@scope@env%
  \let\scoped=\tikz@scoped%
  \let\endscope=\endtikz@scope@env%
  \let\startscope=\scope%
  \let\stopscope=\endscope%
  \let\path=\tikz@command@path%
  \let\againpath=\tikz@command@againpath%
  %
  \def\draw{\path[draw]}%
  \def\pattern{\path[pattern]}%
  \def\fill{\path[fill]}%
  \def\filldraw{\path[fill,draw]}%
  \def\shade{\path[shade]}%
  \def\shadedraw{\path[shade,draw]}%
  \def\clip{\path[clip]}%
  \def\graph{\path graph}%
  \def\useasboundingbox{\path[use as bounding box]}%
  \def\node{\tikz@path@overlay{node}}%
  \def\pic{\tikz@path@overlay{pic}}%
  \def\coordinate{\tikz@path@overlay{coordinate}}%
  \def\matrix{\tikz@path@overlay{node[matrix]}}%
  \def\calendar{\tikz@lib@cal@calendar}%
  \def\datavisualization{\tikz@lib@datavisualization}%
}%
\ifx\tikz@lib@cal@calendar\@undefined
\def\tikz@lib@cal@calendar{\tikzerror{You need to say \string\usetikzlibrary{calendar} to use the \string\calendar{} command}}%
\fi
\ifx\tikz@lib@datavisualization\@undefined
\def\tikz@lib@datavisualization{\tikzerror{You need to say \string\usetikzlibrary{datavisualization} to use the \string\datavisualization{} command}}%
\fi

\def\tikz@path@overlay#1{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar<{\tikz@path@overlayed{#1}}{\path #1}}%
\def\tikz@path@overlayed#1<#2>{\path<#2> #1}%

\def\tikz@uninstallcommands{%
  \let\scope=\tikz@origscope%
  \let\scoped=\tikz@origscoped%
  \let\endscope=\tikz@origendscope%
  \let\startscope=\tikz@origstartscope%
  \let\stopscope=\tikz@origstopscope%
  \let\path=\tikz@origpath%
  \let\againpath=\tikz@origagainpath%
  \let\draw=\tikz@origdraw%
  \let\pattern=\tikz@origpattern%
  \let\fill=\tikz@origfill%
  \let\filldraw=\tikz@origfilldraw%
  \let\shade=\tikz@origshade%
  \let\shadedraw=\tikz@origshadedraw%
  \let\clip=\tikz@origclip%
  \let\useasboundingbox=\tikz@origuseasboundingbox%
  \let\node=\tikz@orignode%
  \let\pic=\tikz@origpic%
  \let\coordinate=\tikz@origcoordinate%
  \let\matrix=\tikz@origmatrix%
  \let\calendar=\tikz@origcalendar%
  \let\datavisualization=\tikz@origdv%
  \let\graph=\tikz@origgraph%
}%


{%
  \catcode`\;=12
  \gdef\tikz@nonactivesemicolon{;}%
  \catcode`\:=12
  \gdef\tikz@nonactivecolon{:}%
  \catcode`\|=12
  \gdef\tikz@nonactivebar{|}%
  \catcode`\!=12
  \gdef\tikz@nonactiveexlmark{!}%
  \catcode`\;=\active
  \catcode`\:=\active
  \catcode`\|=\active
  \catcode`\"=\active
  \catcode`\!=\active
  \gdef\tikz@activesemicolon{;}%
  \gdef\tikz@activecolon{:}%
  \gdef\tikz@activebar{|}%
  \gdef\tikz@activequotes{"}%
  \global\let\tikz@active@quotes@token="%
  \gdef\tikz@activeexlmark{!}%
  \gdef\tikz@deactivatthings{%
    \def;{\tikz@nonactivesemicolon}%
    \def:{\tikz@nonactivecolon}%
    \def|{\tikz@nonactivebar}%
    \def!{\tikz@nonactiveexlmark}%
  }%
}%

\let\tikz@orig@shorthands\pgfutil@empty
\def\tikz@switchoff@shorthands{%
  \ifx\tikz@orig@shorthands\pgfutil@empty%
    \edef\tikz@orig@shorthands{%
      \catcode\noexpand`\noexpand\;\the\catcode`\;\relax%
      \catcode\noexpand`\noexpand\:\the\catcode`\:\relax%
      \catcode\noexpand`\noexpand\|\the\catcode`\|\relax%
      \catcode\noexpand`\noexpand\!\the\catcode`\!\relax%
      \catcode\noexpand`\noexpand\,\the\catcode`\,\relax%
      \catcode\noexpand`\noexpand\<\the\catcode`\<\relax%
      \catcode\noexpand`\noexpand\>\the\catcode`\>\relax%
      \catcode\noexpand`\noexpand\"\the\catcode`\"\relax%
      \catcode\noexpand`\noexpand\'\the\catcode`\'\relax%
      \catcode\noexpand`\noexpand\-\the\catcode`\-\relax%
      \catcode\noexpand`\noexpand\=\the\catcode`\=\relax%
      \catcode\noexpand`\noexpand\.\the\catcode`\.\relax%
      \catcode\noexpand`\noexpand\$\the\catcode`\$\relax%
    }%
    \catcode`\;12\relax%
    \catcode`\:12\relax%
    \catcode`\|12\relax%
    \catcode`\!12\relax%
    \catcode`\,12\relax%
    \catcode`\<12\relax%
    \catcode`\>12\relax%
    \catcode`\"12\relax%
    \catcode`\'12\relax%
    \catcode`\-12\relax%
    \catcode`\=12\relax%
    \catcode`\.12\relax%
    \catcode`\$3\relax%
  \fi%
}%



% Constructs a path and draws/fills them according to the current
% settings.

\def\tikz@command@path{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar[{\tikz@check@earg}%]
  {\pgfutil@ifnextchar<{\tikz@doopt}{\tikz@@command@path}}}%
\pgfutil@protected\def\tikz@signal@path{\tikz@signal@path}%
\def\tikz@check@earg[#1]{%
  \pgfutil@ifnextchar<{\tikz@swap@args[#1]}{\tikz@@command@path[#1]}}
\def\tikz@swap@args[#1]<#2>{\tikz@command@path<#2>[#1]}%

\def\tikz@doopt{%
  \let\tikz@next=\tikz@eargnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@eargactivesemicolon%
  \fi%
  \tikz@next}%
\long\def\tikz@eargnormalsemicolon<#1>#2;{\alt<#1>{\tikz@@command@path#2;}{\tikz@path@do@at@end}}%
{
  \catcode`\;=\active
  \long\global\def\tikz@eargactivesemicolon<#1>#2;{\alt<#1>{\tikz@@command@path#2;}{\tikz@path@do@at@end}}%
}

\def\tikz@@command@path{%
  \edef\tikzscope@linewidth{\the\pgflinewidth}%
  \begingroup%
    \setbox\tikz@figbox=\box\pgfutil@voidb@x%
    \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
    \let\tikz@path@do@at@end=\tikz@lib@scope@check%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@mode=\pgfutil@empty%
    \let\tikz@moveto@waiting=\relax%
    \let\tikz@timer=\relax%
    \let\tikz@tangent=\relax%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \let\tikz@preactions=\pgfutil@empty%
    \let\tikz@postactions=\pgfutil@empty%
    \tikz@snakedfalse%
    \tikz@decoratepathfalse%
    \tikz@node@is@a@labelfalse%
    \tikz@resetexpandcount
    \pgf@path@lastx=0pt%
    \pgf@path@lasty=0pt%
    \tikz@lastx=0pt%
    \tikz@lasty=0pt%
    \tikz@lastxsaved=0pt%
    \tikz@lastysaved=0pt%
    \tikzset{every path/.try}%
    \tikz@scan@next@command%
}%
\def\tikz@scan@next@command{%
  \ifx\tikz@collected@onpath\pgfutil@empty%
  \else%
    \tikz@invoke@collected@onpath%
  \fi%
  \afterassignment\tikz@handle\let\pgf@let@token=%
}%
\newcount\tikz@expandcount
\def\tikz@resetexpandcount{\tikz@expandcount=100\relax}
\let\tikz@collected@onpath=\pgfutil@empty%

\edef\tikz@frozen@relax@token{\ifnum0=0\fi}

% Central dispatcher for commands
\def\tikz@handle{%
  \pgfutil@switch\pgfutil@ifx\pgf@let@token{%
    {(}{\let\pgfutil@next\tikz@movetoabs}%)
    {+}{\let\pgfutil@next\tikz@movetorel}%
    {-}{\let\pgfutil@next\tikz@lineto}%
    {.}{\let\pgfutil@next\tikz@dot}%
    {r}{\let\pgfutil@next\tikz@rect}%
    {n}{\let\pgfutil@next\tikz@fig}%
    {[}{\let\pgfutil@next\tikz@parse@options}%]
    {c}{\let\pgfutil@next\tikz@cchar}%
    {\bgroup}{\let\pgfutil@next\tikz@beginscope}%
    {\egroup}{\let\pgfutil@next\tikz@endscope}%
    {;}{\let\pgfutil@next\tikz@finish}%
    {a}{\let\pgfutil@next\tikz@a@char}%
    {e}{\let\pgfutil@next\tikz@e@char}%
    {g}{\let\pgfutil@next\tikz@g@char}%
    {s}{\let\pgfutil@next\tikz@schar}%
    {|}{\let\pgfutil@next\tikz@vh@lineto}%
    {p}{\pgfsetmovetofirstplotpoint\let\pgfutil@next\tikz@pchar}%
    {t}{\let\pgfutil@next\tikz@to}%
    {\pgfextra}{\let\pgfutil@next\tikz@extra}%
    {\foreach}{\let\pgfutil@next\tikz@foreach}%
    {f}{\let\pgfutil@next\tikz@fchar}%
    {\pgf@stop}{\let\pgfutil@next\relax}%
    {\par}{\let\pgfutil@next\tikz@scan@next@command}%
    {d}{\let\pgfutil@next\tikz@decoration}%
    {l}{\let\pgfutil@next\tikz@l@char}%
    {:}{\let\pgfutil@next\tikz@colon@char}%
    {\relax}{\relax\let\pgfutil@next\tikz@scan@next@command}%
  }{\tikz@resetexpandcount\pgfutil@next}{\tikz@expand}%
}%

\def\tikz@l@char{%
  \pgfutil@ifnextchar e{\tikz@let@command}{%
    \pgfutil@ifnextchar i{\tikz@lsystem}{%
      \pgfutil@ifnextchar-{\tikz@@lsystem}{\tikz@expand}%
    }%
  }%
}%

\def\tikz@lsystem{%
  \tikzerror{You need to say \string\usetikzlibrary{lindenmayersystems} to draw Lindenmayer systems}
}%

\def\tikz@@lsystem{%
  \tikzerror{You need to say \string\usetikzlibrary{lindenmayersystems} to draw L-systems}
}%

\def\tikz@pchar{\pgfutil@ifnextchar l{\tikz@plot}{\pgfutil@ifnextchar i{\tikz@subpicture}{\tikz@parabola}}}%
\def\tikz@cchar{%
  \pgfutil@ifnextchar i{\tikz@circle}%
  {\pgfutil@ifnextchar h{\tikz@children}{\tikz@cochar}}}%
\def\tikz@cochar o{%
  \pgfutil@ifnextchar o{\tikz@coordinate}{\tikz@cosine}}%
\def\tikz@e@char{%
  \pgfutil@ifnextchar l{\tikz@ellipse}{\tikz@@e@char}}%
\def\tikz@a@char{%
  \pgfutil@ifnextchar r{\tikz@arcA}{\tikzerror{Arc expected}}}%
\def\tikz@@e@char dge{%
  \pgfutil@ifnextchar f{\tikz@edgetoparent}{\tikz@edge@plain}}%

\def\tikz@schar{\pgfutil@ifnextchar i{\tikz@sine}{\tikz@svg@path}}%

\def\tikz@g@char r{\pgfutil@ifnextchar i{\tikz@grid}{\tikz@graph}}%

% svg syntax
% svg[options] {...}

\def\tikz@svg@path{%
  \tikzerror{You need to say \string\usetikzlibrary{svg.path} to use the svg path command}
}%


\def\tikz@finish{%
  % Rendering pipeline
  %
  % Step 1: The path background box
  %
  \box\tikz@figbox@bg%
  %
  % Step 2: Decorate path
  %
  \iftikz@decoratepath%
    \tikz@lib@dec@decorate@path%
  \fi%
  %
  % Step 3: Preactions
  %
  \pgfsyssoftpath@getcurrentpath\tikz@actions@path%
  \edef\tikz@restorepathsize{%
    \global\pgf@pathmaxx=\the\pgf@pathmaxx%
    \global\pgf@pathmaxy=\the\pgf@pathmaxy%
    \global\pgf@pathminx=\the\pgf@pathminx%
    \global\pgf@pathminy=\the\pgf@pathminy%
  }%
  \tikz@preactions%
  %
  % Step 4: Reset modes
  %
  \let\tikz@path@picture=\pgfutil@empty%
  \tikz@mode@fillfalse%
  \tikz@mode@drawfalse%
  \tikz@mode@doublefalse%
  \tikz@mode@clipfalse%
  \tikz@mode@boundaryfalse%
  \tikz@mode@fade@pathfalse%
  \tikz@mode@fade@scopefalse%
  \edef\tikz@pathextend{%
    {\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
    {\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
  }%
  \tikz@mode% installs the mode settings
  % Path fading counts as an option:
  \iftikz@mode@fade@path%
    \tikz@addoption{%
      \iftikz@fade@adjust%
        \iftikz@mode@draw%
          \pgfsetfadingforcurrentpathstroked{\tikz@path@fading}{\tikz@do@fade@transform}%
        \else%
          \pgfsetfadingforcurrentpath{\tikz@path@fading}{\tikz@do@fade@transform}%
        \fi%
      \else%
        \pgfsetfading{\tikz@path@fading}{\tikz@do@fade@transform}%
      \fi%
      \tikz@mode@fade@pathfalse% no more fading...
    }%
  \fi%
  %
  % Step 5: Install scope fading
  %
  \iftikz@mode@fade@scope%
    \iftikz@fade@adjust%
      \iftikz@mode@draw%
        \pgfsetfadingforcurrentpathstroked{\tikz@scope@fading}{\tikz@do@fade@transform}%
      \else%
        \pgfsetfadingforcurrentpath{\tikz@scope@fading}{\tikz@do@fade@transform}%
      \fi%
    \else%
      \pgfsetfading{\tikz@scope@fading}{\tikz@do@fade@transform}%
    \fi%
    \tikz@mode@fade@scopefalse%
  \fi%
  %
  % Step 5': Setup options
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
    \pgfsys@beginscope%
      \let\pgfscope@stroke@color=\pgf@strokecolor@global%
      \let\pgfscope@fill@color=\pgf@fillcolor@global%
      \begingroup%
        \tikz@options%
  \fi%
  \tikz@do@rdf@pre@options%
  %
  % Step 5'': Setup animations
  %
  \tikz@is@nodefalse%
  \tikz@call@id@hook%
  \iftikz@mode@clip\else%
    \pgfidscope%
      \tikz@do@rdf@post@options%
      \begingroup%
  \fi% open an animation scope here, unless clipping is done
  %
  % Step 6: Do a fill if shade or a path picture follows.
  %
  \iftikz@mode@fill%
    \iftikz@mode@shade%
      \pgfsyssoftpath@getcurrentpath\tikz@temppath
      \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
      \pgfsyssoftpath@setcurrentpath\tikz@temppath%
      \pgfsyssoftpath@invokecurrentpath%
      \pgfpushtype%
      \pgfusetype{.path fill}%
      \pgfsys@fill%
      \pgfpoptype%
      \tikz@mode@fillfalse% no more filling...
    \else%
      \ifx\tikz@path@picture\pgfutil@empty%
      \else%
        \pgfsyssoftpath@getcurrentpath\tikz@temppath
        \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
        \pgfsyssoftpath@setcurrentpath\tikz@temppath%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfpushtype%
        \pgfusetype{.path fill}%
        \pgfsys@fill%
        \pgfpoptype%
        \tikz@mode@fillfalse% no more filling...
      \fi%
    \fi%
  \fi%
  %
  % Step 7: Do a shade if necessary.
  %
  \iftikz@mode@shade%
    \pgfsyssoftpath@getcurrentpath\tikz@temppath
    \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
    \pgfsyssoftpath@setcurrentpath\tikz@temppath%
    \pgfpushtype%
    \pgfusetype{.path shade}%
    \pgfshadepath{\tikz@shading}{\tikz@shade@angle}%
    \pgfpoptype%
    \tikz@mode@shadefalse% no more shading...
  \fi%
  %
  % Step 8: Do a path picture if necessary.
  %
  \ifx\tikz@path@picture\pgfutil@empty%
  \else%
    \begingroup%
      \pgfusetype{.path picture}%
      \pgfidscope%
      \pgfsys@beginscope%
        \let\tikz@id@name\pgfutil@empty%
        \pgfclearid%
        \pgfsyssoftpath@getcurrentpath\tikz@temppath
        \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
        \pgfsyssoftpath@setcurrentpath\tikz@temppath%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsys@clipnext%
        \pgfsys@discardpath%
        \pgf@relevantforpicturesizefalse%
        \expandafter\def\csname pgf@sh@ns@path picture bounding box\endcsname{rectangle}
        \expandafter\edef\csname pgf@sh@np@path picture bounding box\endcsname{%
          \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
          \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
        }
        \expandafter\def\csname pgf@sh@nt@path picture bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
        \expandafter\def\csname pgf@sh@pi@path picture bounding box\endcsname{\pgfpictureid}
        \pgfinterruptpath%
          \tikz@path@picture%
        \endpgfinterruptpath%
      \pgfsys@endscope%
      \endpgfidscope%
    \endgroup%
    \let\tikz@path@picture=\pgfutil@empty%
  \fi%
  %
  % Step 9: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
      % Change line width
      \begingroup%
        \pgfsys@beginscope%
          \tikz@double@setup%
    \fi%
  \fi%
  %
  % Step 10: Do stroke/fill/clip as needed
  %
  \pgfpushtype%
  \edef\tikz@temp{\noexpand\pgfusepath{%
    \iftikz@mode@fill fill,\fi%
    \iftikz@mode@draw draw,\fi%
    \iftikz@mode@clip clip\fi%
    }}%
  \pgfusetype{.path}%
  \tikz@temp%
  \pgfpoptype%
  \tikz@mode@fillfalse% no more filling
  %
  % Step 11: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
        \pgfsys@endscope%
      \endgroup%
    \fi%
  \fi%
  \tikz@mode@drawfalse% no more stroking
  %
  % Step 12: Postactions
  %
  \tikz@postactions%
  %
  % Step 13: Add labels and nodes
  %
  \box\tikz@figbox%
  %
  % Step 14: Close animations
  %
  \iftikz@mode@clip\else\endgroup\endpgfidscope\fi%
  %
  % Step 14: Close option brace
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
      \endgroup%
      \global\let\pgf@strokecolor@global=\pgfscope@stroke@color%
      \global\let\pgf@fillcolor@global=\pgfscope@fill@color%
    \pgfsys@endscope%
    \iftikz@mode@clip%
      \tikzerror{Extra options not allowed for clipping path command.}%
    \fi%
  \fi%
  \iftikz@mode@clip%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \iftikz@mode@boundary%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \endgroup%
  \global\pgflinewidth=\tikzscope@linewidth%
  \tikz@path@do@at@end%
}%
\let\tikz@lib@scope@check\pgfutil@empty% this is a hook for the scopes library
\def\tikz@path@do@at@end{\tikz@lib@scope@check}%
\def\tikz@@pathtext{@path}%

\def\pgf@outer@auto@adjust@hook{%
  {%
    \tikz@mode@drawfalse%
    \tikz@mode%
    \expandafter%
  }%
  \iftikz@mode@draw\else%
    \pgfkeyslet{/pgf/outer xsep}\pgf@zero@text
    \pgfkeyslet{/pgf/outer ysep}\pgf@zero@text
  \fi%
}%

% Extra actions

\def\tikz@extra@preaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \path[#1];% do extra path
      \pgfsyssoftpath@setcurrentpath\tikz@actions@path% restore
      \tikz@restorepathsize%
    \pgfsys@endscope%
  }%
}%

\def\tikz@extra@postaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\pgfutil@voidb@x%
      \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
      \tikz@restorepathsize%
      \path[#1]\pgfextra{\pgfsyssoftpath@setcurrentpath\tikz@actions@path};% do extra path
      \pgf@resetpathsizes%
    \pgfsys@endscope%
  }%
}%



\def\tikz@skip#1{\tikz@scan@next@command#1}%
\def\tikz@expand{%
  \advance\tikz@expandcount by -1
  \ifnum\tikz@expandcount<0\relax%
    \tikzerror{Giving up on this path. Did you forget a semicolon?}%
    \let\pgfutil@next=\tikz@finish%
  \else%
    \let\pgfutil@next=\tikz@@expand
  \fi%
  \pgfutil@next}%

\def\tikz@@expand{%
  \expandafter\tikz@scan@next@command\pgf@let@token}%



% Syntax for scopes:
% {scoped path commands}

\newif\iftikz@auto@end@path

\def\tikz@beginscope{\begingroup\tikz@auto@end@pathfalse\tikz@scan@next@command}%
\def\tikz@endscope{%
  \iftikz@auto@end@path\expandafter\tikz@finish\expandafter\egroup\else\expandafter\tikz@@endscope\fi%
}%
\def\tikz@@endscope{%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
    \global\let\tikz@tangent@temp\tikz@tangent%
    \edef\tikz@marshal{%
      \tikz@lastx=\the\tikz@lastx%
      \tikz@lasty=\the\tikz@lasty%
      \iftikz@current@point@local%
      \else%
        \tikz@lastxsaved=\the\tikz@lastxsaved%
        \tikz@lastysaved=\the\tikz@lastysaved%
        \ifx\tikz@moveto@waiting\relax%
          \let\tikz@moveto@waiting\relax%
        \else%
          \def\noexpand\tikz@moveto@waiting{\tikz@moveto@waiting}%
        \fi%
        \iftikz@shapeborder%
          \noexpand\tikz@shapebordertrue%
          \def\noexpand\tikz@shapeborder@name{\tikz@shapeborder@name}%
        \else%
          \noexpand\tikz@shapeborderfalse%
        \fi%
      \fi%
    }%
    \expandafter%
  \endgroup\tikz@marshal%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \let\tikz@tangent\tikz@tangent@temp%
  \tikz@scan@next@command}%


% Syntax for pgfextra:
% \pgfextra {normal tex text}
% \pgfextra normal tex text \endpgfextra

\def\tikz@extra{\pgfutil@ifnextchar\bgroup\tikz@@extra\relax}%
\long\def\tikz@@extra#1{#1\tikz@scan@next@command}%
\let\endpgfextra=\tikz@scan@next@command

\def\pgfextra{pgfextra}%


% Syntax for foreach:
%
% foreach \var in {list} {path text}
%
% or
%
% \foreach \var in {list} {path text}
%
% Example:
%
% \draw (0,0) \foreach \x in {1,2,3} {-- (\x,0) circle (1cm)} -- (5,5);

\def\tikz@fchar oreach{\tikz@foreach}%

\def\tikz@foreach{%
  \def\pgffor@beginhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \expandafter\tikz@scan@next@command\pgfutil@firstofone}%
  \def\pgffor@endhook{\pgfextra{%
      \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
      \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
      \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
      \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
      \global\setbox\tikz@tempbox=\box\tikz@figbox%
      \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
      \pgfutil@gobble}}%
  \def\pgffor@afterhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \let\pgffor@beginhook\relax%
    \let\pgffor@endhook\relax%
    \let\pgffor@afterhook\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \tikz@scan@next@command}%
  \global\setbox\tikz@tempbox=\box\tikz@figbox%
  \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
  \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
  \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
  \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
  \foreach}%


% Syntax for againpath:
% \againpath \somepathname

\def\tikz@command@againpath#1{%
  \pgfextra{%
    \pgfsyssoftpath@getcurrentpath\tikz@temp%
    \expandafter\pgfutil@g@addto@macro\expandafter\tikz@temp\expandafter{#1}%
    \pgfsyssoftpath@setcurrentpath\tikz@temp%
  }%
}%


% animation syntax
% :attribute = {...}

\def\tikz@colon@char#1=#2{%
  \tikz@scan@next@command{[animate={myself:{#1}={#2}}]}%
}%



%
% When this if is set, a just-scanned point is a shape and its border
% position still needs to be determined, depending on subsequent
% commands.
%

\newif\iftikz@shapeborder


% Syntax for moveto:
% <point>
\def\tikz@movetoabs{\tikz@moveto(}%
\def\tikz@movetorel{\tikz@moveto+}%
\def\tikz@moveto{%
  \tikz@scan@one@point{\tikz@@moveto}}%
\def\tikz@@moveto#1{%
    \tikz@make@last@position{#1}%
  \iftikz@shapeborder%
    % ok, the moveto will have to wait. flag that we have a moveto in
    % waiting:
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@@movetosave{\tikz@last@position}%
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \tikz@scan@next@command%
}%

  % Wrapper around \pgfpathmoveto that adds a save
\def\tikz@@movetosave#1{%
  {\pgftransformreset
    \pgf@process{#1}%
    \xdef\tikz@marshal{%
      \tikz@lastmovetox=\the\pgf@x\relax%
      \tikz@lastmovetoy=\the\pgf@y\relax%
    }%
  }%
  \tikz@marshal
  \pgfpathmoveto{#1}%
}%

  
\let\tikz@moveto@waiting=\relax % normally, nothing is waiting...

\def\tikz@flush@moveto{%
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \tikz@@movetosave{\tikz@last@position}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}%


\def\tikz@flush@moveto@toward#1#2#3{%
  % #1 = a point towards which the last moveto should be corrected
  % #2 = a dimension to which the corrected x-coordinate should be stored
  % #3 = a dimension for the corrected y-coordinate
  \ifx\tikz@moveto@waiting\relax%
    % do nothing
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{#1}}%
    #2=\pgf@x%
    #3=\pgf@y%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \tikz@@movetosave{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}%


%
% Collecting labels on the path
%

\def\tikz@collect@coordinate@onpath#1c{%
  \pgfutil@ifnextchar y{\tikz@cycle@expander@add#1}{\tikz@collect@coordinate@onpath@{#1}}}%
\def\tikz@collect@coordinate@onpath@#1oordinate{%
  \pgfutil@ifnextchar[{\tikz@@collect@coordinate@opt#1}{\tikz@@collect@coordinate@opt#1[]}}%}%
\def\tikz@@collect@coordinate@opt#1[#2]{%
  \pgfutil@ifnextchar({\tikz@@collect@coordinate#1[#2]}{%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2]{}}}%}%
\def\tikz@@collect@coordinate#1[#2](#3){%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2](#3){}}%

\newif\iftikz@collect@pic

\def\tikz@collect@label@onpath#1node{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath node}%
  \let\tikz@collect@cont#1%
  \tikz@collect@picfalse%
  \tikz@collect@label@scan}%

\def\tikz@collect@pic@onpath#1pic{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath pic}%
  \let\tikz@collect@cont#1
  \tikz@collect@pictrue%
  \tikz@collect@label@scan}%

\def\tikz@collect@label@scan{%
  \pgfutil@ifnextchar f{\tikz@collect@nodes}{%
    \pgfutil@ifnextchar({\tikz@collect@paran}%
    {\pgfutil@ifnextchar[{\tikz@collect@options}%
      {\pgfutil@ifnextchar:{\tikz@collect@animation}%
        {\pgfutil@ifnextchar\bgroup{\tikz@collect@arg}%
          {\tikz@collect@cont}}}}}%
}%}}%

\def\tikz@collect@nodes foreach#1in{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath foreach#1in}%
  \pgfutil@ifnextchar\bgroup\tikz@collect@nodes@group\tikz@collect@nodes@one%
}%
\def\tikz@collect@nodes@one#1{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath #1}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@nodes@group#1{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
  \tikz@collect@label@scan%
}%

\def\tikz@collect@animation#1=#2{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1={#2}}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@paran#1){%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1)}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@options#1]{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath#1]}%
  \tikz@collect@label@scan%
}%
\def\tikz@collect@arg#1{%
  \iftikz@handle@active@nodes%
    \iftikz@collect@pic%
      \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
    \else%
      \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{\scantokens{#1}}}%
    \fi%
  \else%
    \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#1}}%
  \fi%
  \tikz@collect@cont%
}%

\def\tikz@invoke@collected@onpath{%
  \tikz@node@is@a@labeltrue%
  \let\tikz@temp=\tikz@collected@onpath%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \expandafter\tikz@scan@next@command\tikz@temp\pgf@stop%
  \tikz@node@is@a@labelfalse%
}%


%
% Macros for the cycle command
%

\def\tikz@cycle@expander#1{\pgfutil@ifnextchar c{\tikz@cycle@expander@{#1}}{#1}}%
\def\tikz@cycle@expander@#1c{\pgfutil@ifnextchar y{\tikz@cycle@expander@add{#1}}{#1c}}%
\def\tikz@cycle@expander@add#1ycle{#1(current subpath start)--cycle}%




% Syntax for lineto:
% -- <point>

\def\tikz@lineto{%
  \pgfutil@ifnextchar |%
  {\expandafter\tikz@hv@lineto\pgfutil@gobble}%
  {\expandafter\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikz@hv@lineto\pgfutil@gobble}%
    {\expandafter\tikz@lineto@mid\pgfutil@gobble}}}%
\def\tikz@lineto@mid{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@lineto@mid}%
  {%
    \pgfutil@ifnextchar c{\tikz@close}{%
      \pgfutil@ifnextchar p{\tikz@lineto@plot@or@pic}{\tikz@scan@one@point{\tikz@@lineto}}}}}%
\def\tikz@lineto@plot@or@pic p{%
  \pgfutil@ifnextchar i{\tikz@collect@pic@onpath\tikz@lineto@mid p}{%
    \pgfsetlinetofirstplotpoint\tikz@plot}%
}%
\def\tikz@@lineto#1{%
  % Record the starting point for later labels on the path:
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate end
    \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@last@position}}%
    \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \tikz@make@last@position{#1}%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    % target is a reasonable point...
    % Record the starting point for later labels on the path:
    \tikz@make@last@position{#1}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@line%
  \let\tikz@tangent\tikz@timer@start%
  \tikz@scan@next@command%
}%

% snake or lineto?
\def\tikz@path@lineto#1{%
  \iftikz@snaked%
    {
      \pgfsyssoftpathmovetorelevantfalse%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }
  \else%
    \pgfpathlineto{#1}%
  \fi%
}%

% snake or lineto?
\def\tikz@path@close#1{%
  \iftikz@snaked%
    {%
      \pgftransformreset%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }%
  \fi%
  \pgfpathclose%
}%


% Syntax for lineto horizontal/vertical:
% -| <point>

\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@hv@lineto}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@hv@lineto}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@hv@lineto}%
    {\tikz@scan@one@point{\tikz@@hv@lineto}}}}}%
\def\tikz@@hv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@yc=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \edef\tikz@tangent{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@x\pgf@yc%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yc}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
  \fi%
  \let\tikz@timer=\tikz@timer@hvline%
  \tikz@scan@next@command%
}%

% Syntax for lineto vertical/horizontal:
% |- <point>

\def\tikz@vh@lineto-{\tikz@vh@lineto@next}%
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@vh@lineto@next}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@vh@lineto@next}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@vh@lineto@next}%
    {\tikz@scan@one@point\tikz@@vh@lineto}}}}%
\def\tikz@@vh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx%
  \tikz@make@last@position{#1}%
  \edef\tikz@tangent{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@y%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xc}{\tikz@lasty}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@vhline%
  \tikz@scan@next@command%
}%

% Syntax for cycle:
% -- cycle
\def\tikz@close c{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@lineto@mid c}% oops, a coordinate
  {\tikz@@close c}}%
\def\tikz@@close cycle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \tikz@make@last@position{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \tikz@path@close{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \def\pgfstrokehook{}%
  \edef\tikz@timer@end{%\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \noexpand\pgfqpoint{\the\tikz@lastmovetox}{\the\tikz@lastmovetoy}}%
  \let\tikz@timer=\tikz@timer@line%
  \let\tikz@tangent\tikz@timer@start%
  \tikz@scan@next@command%
}%


% Syntax for options:
% [options]
\def\tikz@parse@options#1]{%
  \tikzset{#1}%
  \tikz@scan@next@command%
}%

% Syntax for edges:
% edge [options] (coordinate)
% edge [options] node {node text} (coordinate)
% edge :attribute={...} [options] node {node text} (coordinate)
\def\tikz@edge@plain{%
  \begingroup%
    \ifx\tikz@to@use@whom\pgfutil@undefined\else\tikz@to@use@whom\fi
    \let\tikz@to@or@edge@function=\tikz@do@edge%
    \let\tikz@@to@local@options\pgfutil@empty%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \tikz@to@or@edge}%

% Syntax for to paths:
% to [options] (coordinate)
% to [options] node {node text} (coordinate)
% to :attribute={...} [options] node {node text} (coordinate)
\def\tikz@to o{%
  \tikz@to@use@last@coordinate%
  \let\tikz@to@or@edge@function=\tikz@do@to%
  \let\tikz@@to@local@options\pgfutil@empty%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@to@or@edge}%

\def\tikz@to@or@edge{%
  \pgfutil@ifnextchar[{\tikz@to@or@edge@option}{%
    \pgfutil@ifnextchar:{\tikz@to@or@edge@animation}{%
      \tikz@@to@collect}}%]
}%
\def\tikz@to@or@edge@option[#1]{%
  \expandafter\def\expandafter\tikz@@to@local@options\expandafter{\tikz@@to@local@options,#1}%
  \tikz@to@or@edge%
}%
\def\tikz@to@or@edge@animation:#1=#2{%
  \expandafter\def\expandafter\tikz@@to@local@options\expandafter{\tikz@@to@local@options,%
    animate={myself:{#1}={#2}}}%
  \tikz@to@or@edge%
}%
\def\tikz@@to@collect{%
  \pgfutil@ifnextchar(\tikz@@to@or@edge@coordinate%)
  {\pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@to@collect}%
    {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@to@collect}%
      {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@to@collect}%
        {\pgfutil@ifnextchar +{\tikz@scan@one@point\tikz@@to@or@edge@math}%
          {\tikzerror{(, +, coordinate, pic, or node expected}%)
            \tikz@@to@or@edge@coordinate()}}}}}%
}%

\def\tikz@@to@or@edge@coordinate({%
  \pgfutil@ifnextchar${%$
    % Ok, parse directly
    \tikz@scan@one@point\tikz@@to@or@edge@math(%
  }{%
    \pgfutil@ifnextchar[{%]
      \tikz@scan@one@point\tikz@@to@or@edge@math(%
    }{%
      \tikz@@to@or@edge@@coordinate(%
    }%
  }%
}%
\def\tikz@@to@or@edge@math#1{%
  \pgf@process{#1}%
  \iftikz@updatecurrent\else
    \tikz@updatenextfalse
  \fi
  \edef\tikztotarget{\the\pgf@x,\the\pgf@y}%
  \tikz@to@or@edge@function%
}%

\def\tikz@@to@or@edge@@coordinate(#1){%
  \def\tikztotarget{#1}%
  \tikz@to@or@edge@function%
}%

\def\tikz@do@edge{%
  \ifx\tikz@edge@macro\pgfutil@empty%
    \setbox\tikz@whichbox=\hbox\bgroup%
      \unhbox\tikz@whichbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@transform=\pgfutil@empty%
              \let\tikz@options=\pgfutil@empty%
              \tikz@clear@rdf@options%
              \let\tikz@tonodes=\tikz@collected@onpath%
              \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
              \let\tikz@collected@onpath=\pgfutil@empty%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \pgfidscope%
              \tikz@do@rdf@post@options%
              \tikz@transform%
              \let\tikz@transform=\relax%
              % Typeset node:
              \let\tikz@after@path\pgfutil@empty%
              \tikz@atbegin@to%
                \tikz@enable@edge@quotes%
                \path[style=every edge]\expandafter[\tikz@@to@local@options](\tikztostart)\tikz@to@path
                \pgfextra{\global\let\tikz@after@path@smuggle=\tikz@after@path};%
              \tikz@atend@to%
              \endpgfidscope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
    \global\setbox\tikz@tempbox=\box\tikz@whichbox%
    \expandafter\endgroup%
    \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox%
  \else%
      \expandafter\expandafter\expandafter\tikz@edge@macro%
      \expandafter\expandafter\expandafter{\expandafter\tikz@@to@local@options\expandafter}\expandafter{\tikz@collected@onpath}%
    \endgroup%
    \let\tikz@after@path@smuggle=\pgfutil@empty%
  \fi%
  \expandafter\tikz@scan@next@command\tikz@after@path@smuggle%
}%

\def\tikz@do@to{%
  \let\tikz@tonodes=\tikz@collected@onpath%
  \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@scan@next@command%
  {%
    \pgfextra{\let\tikz@after@path\pgfutil@empty}%
    \pgfextra{\tikz@atbegin@to}%
    \pgfextra{\tikz@enable@edge@quotes}%
    [style=every to]\expandafter[\tikz@@to@local@options]\tikz@to@path%
    \pgfextra{\tikz@atend@to}%
    \pgf@stop%
    \expandafter\tikz@scan@next@command\expandafter%
  }\tikz@after@path%
  \pgfextra{\tikz@updatenexttrue\tikz@updatecurrenttrue}%
}%


\def\tikz@to@use@last@coordinate{%
  \iftikz@shapeborder%
    \edef\tikztostart{\tikz@shapeborder@name}%
  \else%
    \edef\tikztostart{\the\tikz@lastx,\the\tikz@lasty}%
  \fi%
}%
\def\tikz@to@use@last@fig@name{%
  \edef\tikztostart{\tikz@to@last@fig@name}%
}%



% Syntax for graph path command:
% graph [options] {...}
% See the graph library for details

\def\tikz@graph aph{\tikz@lib@graph@parser}%

\def\tikz@lib@graph@parser{\pgfutil@ifnextchar[\tikz@graph@error{\tikz@graph@error[]}}%]%
\def\tikz@graph@error[#1]#2{%
  \tikzerror{You need to say \string\usetikzlibrary{graphs} in order to use the graph syntax}%
  \tikz@lib@graph@parser@done%
}%

\def\tikz@lib@graph@parser@done{%
  \tikz@scan@next@command%
}%




% Syntax for edge from parent:
% edge from parent [options]
\def\tikz@edgetoparent from parent{\pgfutil@ifnextchar[\tikz@@edgetoparent{\tikz@@edgetoparent[]}}%}%
\def\tikz@@edgetoparent[#1]{%
  \let\tikz@edge@to@parent@needed=\pgfutil@empty%
  \def\tikz@edgetoparent@options{#1}%
  \begingroup%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \tikz@edgetoparentcollect%
}%
\def\tikz@edgetoparentcollect{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@edgetoparentcollect}%
  {%
      \expandafter%
    \endgroup%
    \expandafter\tikz@edgetoparent@rollout\expandafter{\tikz@collected@onpath}%
  }%
}%

\def\tikz@edgetoparent@rollout#1{%
  \pgfkeysgetvalue{/tikz/edge from parent macro}\tikz@etop@temp
  \expandafter\tikz@scan@next@command\expandafter\tikz@etop@temp\expandafter{\tikz@edgetoparent@options}{#1}%
}%


% Syntax for bezier curves
% .. controls(point) and (point) .. (target)
% .. controls(point) .. (target)
% .. (target) % currently not supported

\def\tikz@dot.{\tikz@@dot}%
\def\tikz@@dot{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@dot}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@dot}%
  {\pgfutil@ifnextchar c{\tikz@curveto@double}{\tikz@curveto@auto}}}%
}%

\def\tikz@curveto@double co{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@@dot co}
  {\tikz@cureveto@@double}}%
\def\tikz@cureveto@@double ntrols#1{%
  \tikz@scan@one@point\tikz@curveA#1%
}%
\def\tikz@curveA#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{#1}%
    \xdef\tikz@curve@first{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  \pgfutil@ifnextchar a
  {\tikz@curveBand}%
  {\let\tikz@curve@second\tikz@curve@first\tikz@curveCdots}%
}%
\def\tikz@curveBand and{%
  \tikz@scan@one@point\tikz@curveB%
}%
\def\tikz@curveB#1{%
  \def\tikz@curve@second{#1}%
  \tikz@curveCdots}
\def\tikz@curveCdots{%
  \afterassignment\tikz@curveCdot\let\pgfutil@next=}%
\def\tikz@curveCdot.{%
  \ifx\pgfutil@next.%
  \else%
    \tikzerror{Dot expected}%
  \fi%
  \iftikz@updatenext
    \tikz@updatecurrenttrue%
  \fi
  \tikz@curveCcheck%
}%
\def\tikz@curveCcheck{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@curveCcheck}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@curveCcheck}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@curveCcheck}
    {\tikz@scan@one@point\tikz@curveC}}}%
}%
\def\tikz@curveC#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{\tikz@curve@second}%
    \xdef\tikz@curve@second{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  %
  % Start recalculating things in case start and end are shapes.
  %
  % First, the start:
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{\tikz@curve@first}}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \tikz@@movetosave{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@timer@cont@one=\tikz@curve@first%
  \let\tikz@timer@cont@two=\tikz@curve@second%
  % Second, the end:
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate third
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@curve@second}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
      \global\let\tikz@timer@end@temp=\tikz@curve@third% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
    \let\tikz@timer@end=\tikz@curve@third
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \let\tikz@timer=\tikz@timer@curve%
  \let\tikz@tangent=\tikz@curve@second%
  \tikz@scan@next@command%
}%


% Syntax for rectangles:
% rectangle <corner point>
\def\tikz@rect ectangle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \tikz@@rect}%
\def\tikz@@rect{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@rect}{%
  \pgfutil@ifnextchar p{\tikz@collect@pic@onpath\tikz@@rect}%
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@rect}%
    {
      \pgf@xa=\tikz@lastx\relax%
      \pgf@ya=\tikz@lasty\relax%
      \tikz@scan@one@point\tikz@rectB}}}}%
\def\tikz@rectB#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \let\tikz@timer=\tikz@timer@line%
          \tikz@@movetosave{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@ya}}%
  \iftikz@snaked%
    \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \fi%
  \pgfpathclose%
          \tikz@@movetosave{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \def\pgfstrokehook{}%
  \let\tikz@tangent\relax%
  \tikz@scan@next@command%
}%



% Syntax for grids:
% grid <corner point>
\def\tikz@grid id{%
  \tikz@flush@moveto%
  \pgf@xa=\tikz@lastx\relax%
  \pgf@ya=\tikz@lasty\relax%
  \pgfutil@ifnextchar[{\tikz@gridA}{\tikz@gridA[]}}%}%
\def\tikz@gridA[#1]{%
  \def\tikz@grid@options{#1}%
  \tikz@cycle@expander{\tikz@scan@one@point\tikz@gridB}}%
\def\tikz@gridB#1{%
  \tikz@make@last@position{#1}%
  \let\tikz@tangent\relax%
  {%
    \let\tikz@after@path\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@grid@options}
    \tikz@checkunit{\tikz@grid@x}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{\tikz@grid@x}{0pt}}%
    \else%
      \pgf@process{\pgfpointxy{\tikz@grid@x}{0}}%
    \fi%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \tikz@checkunit{\tikz@grid@y}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{0pt}{\tikz@grid@y}}%
    \else%
      \pgf@process{\pgfpointxy{0}{\tikz@grid@y}}%
    \fi%
    \advance\pgf@xb by\pgf@x%
    \advance\pgf@yb by\pgf@y%
    \pgfpathgrid[stepx=\pgf@xb,stepy=\pgf@yb]%
      {\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \expandafter}%
  \expandafter\tikz@scan@next@command\tikz@after@path%
}%



% Syntax for plot:
% plot [local options] ...    % starts with a moveto
% -- plot [local options] ... % starts with a lineto
\def\tikz@plot lot{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar[{\tikz@@plot}{\tikz@@plot[]}}%}%
\def\tikz@@plot[#1]{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \begingroup%
    \let\tikz@after@path\pgfutil@empty%
    \let\tikz@options=\pgfutil@empty%
    \tikzset{every plot/.try}%
    \tikzset{#1}%
    \pgfutil@ifnextchar f{\tikz@plot@f}%
    {\pgfutil@ifnextchar c{\tikz@plot@scan@points}%
      {\pgfutil@ifnextchar ({\tikz@plot@expression}{%
      \tikzerror{Cannot parse this plotting data}%
       \endgroup}}}}%
\def\tikz@plot@f f{\pgfutil@ifnextchar i{\tikz@plot@file}{\tikz@plot@function}}%

\def\tikz@plot@file ile#1{\def\tikz@plot@data{\pgfplotxyfile{#1}}\tikz@@@plot}%
\def\tikz@plot@scan@points coordinates#1{%
  \pgfplothandlerrecord\tikz@plot@data%
  \pgfplotstreamstart%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}
  {\tikz@scan@one@point\tikz@plot@next@point}%
  #1\pgf@stop%
}%
\def\tikz@plot@next@point#1{%
  \pgfplotstreampoint{#1}%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}%
  {\tikz@scan@one@point\tikz@plot@next@point}%
}%
\def\tikz@plot@function unction#1{%
  \def\tikz@plot@filename{\tikz@plot@prefix\tikz@plot@id}%
  \iftikz@plot@raw@gnuplot%
    \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{#1}}%
  \else%
    \iftikz@plot@parametric%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          set parametric;
          plot [t=\tikz@plot@domain]
          [\tikz@plot@xrange]
          [\tikz@plot@range]
          #1}}%
    \else%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          plot [x=\tikz@plot@domain]
          \ifx\tikz@plot@range\pgfutil@empty\else[\tikz@plot@range]\fi
          #1}}%
    \fi%
  \fi%
  \tikz@@@plot%
}%

\def\tikz@plot@no@resample{%
  \pgfutil@IfFileExists{\tikz@plot@filename.table}%
  {\def\tikz@plot@data{\pgfplotxyfile{\tikz@plot@filename.table}}}%
  {}%
}%

\def\tikz@plot@expression(#1){%
  \edef\tikz@plot@data{\noexpand\pgfplotfunction{\expandafter\noexpand\tikz@plot@var}{\tikz@plot@samplesat}}%
  \expandafter\def\expandafter\tikz@plot@data\expandafter{\tikz@plot@data{\tikz@scan@one@point\pgfutil@firstofone(#1)}}%
  \tikz@@@plot%
}%

\def\tikz@@@plot{%
    \def\pgfplotlastpoint{\pgfpointorigin}%
    \tikz@plot@handler%
    \tikz@plot@data%
    \global\let\tikz@@@temp=\pgfplotlastpoint%
    \ifx\tikz@plot@mark\pgfutil@empty%
    \else%
      % Marks are drawn after the path.
      \setbox\tikz@whichbox=\hbox{%
        \unhbox\tikz@whichbox%
        \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@options=\pgfutil@empty%
              \let\tikz@transform=\pgfutil@empty%
              \tikzset{every mark}%
              \tikz@options%
              \ifx\tikz@mark@list\pgfutil@empty%
                \pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
              \else
                \pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
              \fi
              \tikz@plot@data%
            \endpgfscope
          \endpgfinterruptpath%
        }}%
      }%
    \fi%
    \global\setbox\tikz@tempbox=\box\tikz@whichbox%
    \global\let\tikz@after@path@smuggle=\tikz@after@path
  \expandafter\endgroup%
  \expandafter\setbox\tikz@whichbox=\box\tikz@tempbox%
  \tikz@make@last@position{\tikz@@@temp}%
  \expandafter\tikz@scan@next@command\tikz@after@path@smuggle%
}%


\pgfdeclareplotmark{ball}
{%
  \def\tikz@shading{ball}%
  \shade (0pt,0pt) circle (\pgfplotmarksize);%
}%




% Syntax for cosine curves:
% cos <end of quarter-period>
\def\tikz@cosine s{\tikz@cycle@expander{\tikz@scan@one@point\tikz@@cosine}}
\def\tikz@@cosine#1{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathcosine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}%

% Syntax for sine curves:
% sin <end of quarter-period>
\def\tikz@sine in{\tikz@cycle@expander{\tikz@scan@one@point\tikz@@sine}}
\def\tikz@@sine#1{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathsine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}%

% Syntax for parabolas:
% parabola[options] bend <coordinate> <coordinate>
\def\tikz@parabola arabola{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \pgfutil@ifnextchar[{\tikz@parabola@options}{\tikz@parabola@options[]}}%}%

\def\tikz@parabola@options[#1]{%
  \def\tikz@parabola@option{#1}%
  \pgfutil@ifnextchar b{\tikz@parabola@scan@bend}{\tikz@cycle@expander{\tikz@scan@one@point\tikz@parabola@semifinal}}}%
\def\tikz@parabola@scan@bend bend{\tikz@scan@one@point\tikz@parabola@scan@bendB}%
\def\tikz@parabola@scan@bendB#1{%
  \def\tikz@parabola@bend{#1}%
  \tikz@cycle@expander{\tikz@scan@one@point\tikz@parabola@semifinal}%
}%
\def\tikz@parabola@semifinal#1{%
  \tikz@flush@moveto%
  % Save original start:
  \pgf@xb=\tikz@lastx%
  \pgf@yb=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \pgf@xc=\tikz@lastx%
  \pgf@yc=\tikz@lasty%
  \begingroup% now calculate bend:
    \let\tikz@after@path\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@parabola@option}%
    \tikz@lastxsaved=\tikz@parabola@bend@factor\tikz@lastx%
    \tikz@lastysaved=\tikz@parabola@bend@factor\tikz@lasty%
    \advance\tikz@lastxsaved by\pgf@xb%
    \advance\tikz@lastysaved by\pgf@yb%
    \advance\tikz@lastxsaved by-\tikz@parabola@bend@factor\pgf@xb%
    \advance\tikz@lastysaved by-\tikz@parabola@bend@factor\pgf@yb%
    \expandafter\tikz@make@last@position\expandafter{\tikz@parabola@bend}%
    % Calculate delta from bend
    \advance\pgf@xc by-\tikz@lastx%
    \advance\pgf@yc by-\tikz@lasty%
    % Ok, now calculate delta to bend
    \advance\tikz@lastx by-\pgf@xb%
    \advance\tikz@lasty by-\pgf@yb%
    \xdef\tikz@parabola@b{{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \expandafter\endgroup%
  \expandafter\expandafter\expandafter\pgfpathparabola\expandafter\tikz@parabola@b%
  \expandafter\tikz@scan@next@command\tikz@after@path%
}%


% Syntax for circles:
% circle [options] % where options should set, at least, radius
% circle (radius) % deprecated
%
% Syntax for ellipses:
% ellipse [options] % identical to circle.
% ellipse (x-radius and y-radius) % deprecated
%
% radii can be dimensionless, then they are in the xy-system
\def\tikz@circle ircle{\tikz@flush@moveto\tikz@@circle}%
\def\tikz@ellipse llipse{\tikz@flush@moveto\tikz@@circle}%
\def\tikz@@circle{%
  \let\tikz@tangent\relax%
  \pgfutil@ifnextchar(\tikz@@@circle
  {\pgfutil@ifnextchar[\tikz@circle@opt{%])
    \advance\tikz@expandcount by -10\relax% go down quickly
    \ifnum\tikz@expandcount<0\relax%
      \let\pgfutil@next=\tikz@@circle@normal%
    \else%
      \let\pgfutil@next=\tikz@@circle@scanexpand%
    \fi%
    \pgfutil@next%
  }}%
}%
\def\tikz@@circle@scanexpand{\expandafter\tikz@@circle}%
\def\tikz@@circle@normal{\tikz@circle@opt[]}%

\def\tikz@circle@opt[#1]{%
  {%
    \def\tikz@node@at{\tikz@last@position}%
    \let\tikz@transform=\pgfutil@empty%
    \tikzset{every circle/.try,#1}%
    \pgftransformshift{\tikz@node@at}%
    \tikz@transform%
    \tikz@do@ellipse{\pgfkeysvalueof{/tikz/x radius}}{\pgfkeysvalueof{/tikz/y radius}}
  }%
  \tikz@scan@next@command%
}%

\def\tikz@@@circle(#1){%
  {%
    \pgftransformshift{\tikz@last@position}%
    \pgfutil@in@{ and }{#1}%
    \ifpgfutil@in@%
      \tikz@@ellipseB(#1)%
    \else%
      \tikz@do@circle{#1}%
    \fi%
  }%
  \tikz@scan@next@command%
}%
\def\tikz@@ellipseB(#1 and #2){%
  \tikz@do@ellipse{#1}{#2}%
}%
\def\tikz@do@circle#1{%
  \pgfmathparse{#1}%
  \let\tikz@ellipse@x=\pgfmathresult
  \ifpgfmathunitsdeclared
    \pgfpathellipse{\pgfpointorigin}%
      {\pgfqpoint{\tikz@ellipse@x pt}{0pt}}%
      {\pgfpoint{0pt}{\tikz@ellipse@x pt}}%
  \else
    \pgfpathellipse{\pgfpointorigin}%
      {\pgfpointxy{\tikz@ellipse@x}{0}}%
      {\pgfpointxy{0}{\tikz@ellipse@x}}%
  \fi
}
\def\tikz@do@ellipse#1#2{
  \pgfmathparse{#1}%
  \let\tikz@ellipse@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \pgfpathellipse{\pgfpointorigin}{%
        \pgfqpoint{\tikz@ellipse@x pt}{0pt}}{\pgfpoint{0pt}{\tikz@ellipse@y pt}}%
    \else%
      \tikzerror{You cannot mix dimensions and dimensionless values in an ellipse}%
    \fi%
  \else%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikzerror{You cannot mix dimensions and dimensionless values in an ellipse}%
    \else%
      \pgfpathellipse{\pgfpointorigin}{%
        \pgfpointxy{\tikz@ellipse@x}{0}}{\pgfpointxy{0}{\tikz@ellipse@y}}%
    \fi%
  \fi%
}%

% Syntax for arcs:
% arc [options]
%
% (The syntax with parentheses is deprecated.)
\def\tikz@arcA rc{\tikz@flush@moveto\tikz@arc@cont}%
\def\tikz@arc@cont{%
  \pgfutil@ifnextchar(%)
  {\tikz@@arcto}{%
    \pgfutil@ifnextchar[%]
    {\tikz@arc@opt}%
    {%
      \advance\tikz@expandcount by -10\relax% go down quickly
      \ifnum\tikz@expandcount<0\relax%
        \let\pgfutil@next=\tikz@@arc@normal%
      \else%
        \let\pgfutil@next=\tikz@@arc@scanexpand%
      \fi%
      \pgfutil@next%
    }%
  }%
}%
\def\tikz@@arc@scanexpand{\expandafter\tikz@arc@cont}%
\def\tikz@@arc@normal{\tikz@arc@opt[]}%


\def\tikz@arc@opt[#1]{%
  {%
    \tikzset{every arc/.try,#1}%
    \pgfkeysgetvalue{/tikz/start angle}\tikz@s
    \pgfkeysgetvalue{/tikz/end angle}\tikz@e
    \pgfkeysgetvalue{/tikz/delta angle}\tikz@d
    \ifx\tikz@s\pgfutil@empty%
      \pgfmathsetmacro\tikz@s{\tikz@e-\tikz@d}
    \else
      \ifx\tikz@e\pgfutil@empty%
        \pgfmathsetmacro\tikz@e{\tikz@s+\tikz@d}
      \fi%
    \fi%
    \xdef\pgf@marshal{\noexpand%
    \tikz@do@arc{\tikz@s}{\tikz@e}
      {\pgfkeysvalueof{/tikz/x radius}}
      {\pgfkeysvalueof{/tikz/y radius}}}%
  }%
  \pgf@marshal%
  \tikz@arcfinal%
}%

\def\tikz@@arcto(#1){%
  \edef\tikz@temp{(#1)}%
  \expandafter\tikz@@@arcto@check@slashand\tikz@temp%
}%

\def\tikz@@@arcto@check@slashand(#1:#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \tikz@parse@arc@and(#1:#2:#3)%
  \else%
    \tikz@parse@arc@and(#1:#2:{#3} and {#3})%
  \fi%
  \tikz@arcfinal%
}%

\def\tikz@parse@arc@and(#1:#2:#3 and #4){%
  \tikz@do@arc{#1}{#2}{#3}{#4}%
}%
\def\tikz@do@arc#1#2#3#4{%
  \let\tikz@tangent\tikz@tangent@lookup%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgfmathsetmacro\tikz@timer@start@angle{#1}%
  \pgfmathsetmacro\tikz@timer@end@angle{#2}%
  \pgfmathparse{#3}%
  \let\tikz@arc@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikz@@@arcfinal{\pgfpatharc{\tikz@timer@start@angle}{\tikz@timer@end@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{\tikz@timer@start@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{\tikz@timer@end@angle}{\tikz@arc@x pt and \tikz@arc@y pt}}%
      \edef\tikz@timer@zero@axis{\noexpand\pgfqpoint{\tikz@arc@x pt}{0pt}}
      \edef\tikz@timer@ninety@axis{\noexpand\pgfqpoint{0pt}{\tikz@arc@y pt}}
    \else%
      \tikzerror{You cannot mix dimensions and dimensionless values in an arc}%
    \fi%
  \else%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikzerror{You cannot mix dimensions and dimensionless values in an arc}%
    \else%
      \tikz@@@arcfinal{\pgfpatharcaxes{\tikz@timer@start@angle}{\tikz@timer@end@angle}{\pgfpointxy{\tikz@arc@x}{0}}{\pgfpointxy{0}{\tikz@arc@y}}}
      {\pgfpointpolarxy{\tikz@timer@start@angle}{\tikz@arc@x and \tikz@arc@y}}{\pgfpointpolarxy{\tikz@timer@end@angle}{\tikz@arc@x and \tikz@arc@y}}%
      \pgf@process{\pgfpointxy{\tikz@arc@x}{0}}
      \edef\tikz@timer@zero@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      \pgf@process{\pgfpointxy{0}{\tikz@arc@y}}
      \edef\tikz@timer@ninety@axis{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
     \fi%
  \fi%
}%

\def\tikz@@@arcfinal#1#2#3{%
  #1%
  \pgf@process{#2}
  \xdef\tikz@arc@save@first{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgf@process{#3}
  \xdef\tikz@arc@save@second{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
}%

\def\tikz@arcfinal{%
  \pgf@process{\tikz@arc@save@first}%
  \advance\tikz@lastx by-\pgf@x%
  \advance\tikz@lasty by-\pgf@y%
  \pgf@process{\tikz@arc@save@second}%
  \advance\tikz@lastx by\pgf@x%
  \advance\tikz@lasty by\pgf@y%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \let\tikz@timer=\tikz@timer@arc%
  \tikz@scan@next@command%
}%


% Syntax for coordinates:
% coordinate[options] (coordinate name) at (point)
% where ``at (point)'' is optional
\def\tikz@coordinate ordinate{%
  \pgfutil@ifnextchar[{\tikz@@coordinate@opt}{\tikz@@coordinate@opt[]}}%
\def\tikz@@coordinate@opt[#1]{%
  \pgfutil@ifnextchar({\tikz@@coordinate[#1]}
  {\tikz@fig ode[shape=coordinate,#1]{}}}%}%
\def\tikz@@coordinate[#1](#2){%
  \pgfutil@ifnextchar a{\tikz@@coordinate@at[#1](#2)}
  {\tikz@fig ode[shape=coordinate,#1](#2){}}}%
\def\tikz@@coordinate@at[#1](#2)a{%
  \pgfutil@ifnextchar t{\tikz@@coordinate@@at[#1](#2)a}%
  {\tikz@fig ode[shape=coordinate,#1](#2){}a}%
}%
\def\tikz@@coordinate@@at[#1](#2)at#3({%
  \def\tikz@coordinate@caller{\tikz@fig ode[shape=coordinate,#1](#2)at}%
  \tikz@scan@one@point\tikz@@coordinate@at@math(%
}%
\def\tikz@@coordinate@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@temp{(\the\pgf@x,\the\pgf@y)}%
  \expandafter\tikz@coordinate@caller\tikz@temp{}%
}%



% Syntax for nodes:
% node foreach \var in {list} ... :attribute={...} [options] (node name) at (pos) {label text}
%
% all of :attribute, [options], (node name), at(pos), and foreach are
% optional. There can be multiple options and the ordering is not
% important as in node[draw] (a) [rotate=10] {text}, *except* that all
% foreach statements must come first.
%
% A label text always ``ends'' the node.
%
\def\tikz@fig ode{%
  \pgfutil@ifnextchar a\tikz@test@also{%
    \pgfutil@ifnextchar f{\tikz@nodes@start}\tikz@normal@fig}}%
\def\tikz@test@also a{\pgfutil@ifnextchar l\tikz@node@also{\tikz@normal@fig a}}%
\def\tikz@normal@fig{%
  \edef\tikz@save@line@width{\the\pgflinewidth}%
  \begingroup%
  \let\tikz@fig@name=\pgfutil@empty%
    \begingroup%
      \tikz@is@matrixfalse%
      \let\nodepart=\tikz@nodepart%
      \let\tikz@atbegin@scope=\pgfutil@empty%
      \let\tikz@atend@scope=\pgfutil@empty%
      \let\tikz@do@after@node=\tikz@scan@next@command%
      \let\tikz@options=\pgfutil@empty%
      \tikz@clear@rdf@options%
      \let\tikz@id@name=\pgfutil@empty%
      \let\tikz@after@path=\pgfutil@empty%
      \let\tikz@transform=\pgfutil@empty%
      \let\tikz@mode=\pgfutil@empty%
      \tikz@decoratepathfalse%
      \let\tikz@preactions=\pgfutil@empty%
      \let\tikz@postactions=\pgfutil@empty%
      \let\tikz@alias=\pgfutil@empty%
      \def\tikz@node@at{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \let\tikz@time@for@matrix\tikz@time%
      \let\tikz@node@content\relax%
      \pgfgetpath\tikzpathuptonow%
      \iftikz@node@is@a@label%
      \else%
        \let\tikz@time\pgfutil@empty%
      \fi%
      \tikz@node@reset@hook%
      \tikzset{every node/.try}%
      \tikz@@scan@fig}%
\def\tikz@@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar:{\tikz@fig@scan@animation}%
        {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
          {\tikzerror{A node must have a (possibly empty) label text}%
            \tikz@fig@main{}}}}}}}%}}%
\def\tikz@fig@scan@at at{%
  \tikz@scan@one@point\tikz@@fig@scan@at}%
\def\tikz@@fig@scan@at#1{%
  \def\tikz@node@at{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@name(#1){%
    \pgfkeysvalueof{/tikz/name/.@cmd}#1\pgfeov% CF : this is now ALWAYS consistent with 'name=' option; allows overrides.
    \tikz@@scan@fig}%
% make it \long to allow \par in "pin" options etc:
\long\def\tikz@fig@scan@options[#1]{\iftikz@node@is@pic\tikz@enable@pic@quotes\else\tikz@enable@node@quotes\fi\tikzset{#1}\ifx\tikz@node@content\relax\expandafter\tikz@@scan@fig\else\tikz@expand@node@contents\fi}%
\def\tikz@fig@scan@animation:#1=#2{\tikzset{animate={myself:{#1}={#2}}}\tikz@@scan@fig}%
\def\tikz@expand@node@contents{%
  \expandafter\tikz@@scan@fig\expandafter{\tikz@node@content}%
}%
\let\tikz@node@reset@hook=\pgfutil@empty%
\let\tikz@node@begin@hook=\pgfutil@empty%
\def\tikz@fig@main{%
  \iftikz@node@is@pic%
    \tikz@node@is@picfalse%
    \expandafter\tikz@subpicture@handle%
  \else%
    \afterassignment\tikz@@fig@main\expandafter\let\expandafter\next\expandafter=%
  \fi}%
\def\tikz@@fig@main{%
    \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
    {\tikzerror{Unknown shape ``\tikz@shape.'' Using ``rectangle'' instead}%
      \def\tikz@shape{rectangle}}%
    {}%
    \expandafter\xdef\csname tikz@dcl@coord@\tikz@fig@name\endcsname{%
      \csname tikz@scan@point@coordinate\endcsname}%
    \tikzset{every \tikz@shape\space node/.try}%
    \tikz@node@textfont%
    \tikz@node@begin@hook%
    \iftikz@is@matrix%
      \let\tikz@next=\tikz@do@matrix%
    \else%
      \let\tikz@next=\tikz@do@fig%
    \fi%
    \tikz@next%
}%
\let\tikz@nodepart@list\pgfutil@empty
\def\tikz@do@fig{%
    % Ok, reset all node part boxes
    \pgfutil@for\tikz@temp:=\tikz@nodepart@list\do{%
      \expandafter\setbox\csname pgfnodepart\tikz@temp box\endcsname=\box\pgfutil@voidb@x%
    }%
    \setbox\pgfnodeparttextbox=\hbox%
      \bgroup%
        \pgfinterruptpicture%
        \pgfsys@begin@text%
          \pgfsys@text@to@black@hook%
          \tikzset{every text node part/.try}%
          \ifx\tikz@textopacity\pgfutil@empty%
          \else%
            \pgfsetfillopacity{\tikz@textopacity}%
            \pgfsetstrokeopacity{\tikz@textopacity}%
          \fi%
          \ifx\tikz@text@width\pgfutil@empty%
            \tikz@textfont%
          \else%
            \begingroup%
                \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
              \pgfutil@minipage[t]{\pgf@x}\leavevmode\hbox{}%
                \tikz@textfont%
                \tikz@text@action%
          \fi%
          \tikz@atbegin@node%
          \bgroup%
            \aftergroup\unskip%
            % Some color stuff has been moved from here to outside; this is
            % necessary for support of dvisvgm and of animation
            % snapshots.
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
              \pgfutil@color{\tikz@textcolor}%
            \fi%
            \setbox\tikz@figbox=\box\pgfutil@voidb@x%
            \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
            \tikz@uninstallcommands%
            \iftikz@handle@active@code%
              \tikz@orig@shorthands%
              \let\tikz@orig@shorthands\pgfutil@empty%
            \fi%
            \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
            \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
            \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
            \aftergroup\tikz@fig@collectresetcolor%
            \tikz@signal@halign@check%
            \tikz@text@reset%
            \tikz@halign@check%
            \ignorespaces%
}%
\def\tikz@fig@collectresetcolor{%
  % Hacks for special packages that mess with \aftergroup
  \pgfutil@ifnextchar\reset@color% hack for color package
  {\reset@color\afterassignment\tikz@fig@collectresetcolor\let\tikz@temp=}\tikz@fig@boxdone%
}%
\def\tikz@fig@boxdone{%
            \tikz@atend@node%
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
              \pgfutil@endminipage%
            \endgroup%
          \fi%
        \pgfsys@end@text%
        \endpgfinterruptpicture%
      \egroup%
    \pgfutil@ifnextchar c{\tikz@fig@mustbenamed\tikz@fig@continue}%
    {\pgfutil@ifnextchar[{\tikz@fig@mustbenamed\tikz@fig@continue}%
      {\pgfutil@ifnextchar t{\tikz@fig@mustbenamed\tikz@fig@continue}
        {\pgfutil@ifnextchar e{\tikz@fig@mustbenamed\tikz@fig@continue}
          {\ifx\tikz@after@path\pgfutil@empty\expandafter\tikz@fig@continue\else\expandafter\tikz@fig@mustbenamed\expandafter\tikz@fig@continue\fi}}}}}%}%

\tikzset{
  matrix/inner style/every cell/.code={%
    \tikzset{every cell/.try={\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  },
  matrix/inner style/column/.code={%
    \tikzset{column \the\pgfmatrixcurrentcolumn/.try}%
  },
  matrix/inner style/even odd column/.code={
    \ifodd\pgfmatrixcurrentcolumn%
      \tikzset{every odd column/.try}%
    \else%
      \tikzset{every even column/.try}%
    \fi
  },
  matrix/inner style/row/.code={%
    \tikzset{row \the\pgfmatrixcurrentrow/.try}%
  },
  matrix/inner style/even odd row/.code={%
    \ifodd\pgfmatrixcurrentrow%
      \tikzset{every odd row/.try}%
    \else%
      \tikzset{every even row/.try}%
    \fi
  },
  matrix/inner style/cell/.code={%
    \tikzset{row \the\pgfmatrixcurrentrow\space column \the\pgfmatrixcurrentcolumn/.try}%
  },
  matrix/inner style order/.store in=\tikz@common@matrix@code@styleorder,
  matrix/inner style order={
    every cell,
    column,
    even odd column,
    row,
    even odd row,
    cell
  },
}%

\def\tikz@do@matrix{%
    \tikzset{every matrix/.try}%
    \tikz@node@transformations%
    \tikz@fig@mustbenamed%
    \setbox\tikz@whichbox=\hbox\bgroup%
      \unhbox\tikz@whichbox%
      \hbox\bgroup\bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \ifx\tikz@time\pgfutil@empty\let\tikz@time\tikz@time@for@matrix\fi%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \tikz@is@nodefalse%
              \tikz@call@id@hook%
              \pgfidscope%
                \tikz@do@rdf@post@options%
                \begingroup%
                \let\tikz@id@name\pgfutil@empty%
                \pgfclearid%
                \setbox\tikz@figbox=\box\pgfutil@voidb@x%
                \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
                \let\tikzmatrixname=\tikz@fig@name%
                \edef\tikz@m@anchor{\ifx\tikz@matrix@anchor\pgfutil@empty\tikz@anchor\else\tikz@matrix@anchor\fi}%
                \expandafter\pgfutil@in@\expandafter{\expandafter.\expandafter}\expandafter{\tikz@m@anchor}%
                \ifpgfutil@in@%
                  \expandafter\tikz@matrix@split\tikz@m@anchor\relax%
                \else%
                  \def\tikz@matrix@shift{\pgfpointorigin}%
                \fi%
                \let\tikz@transform=\relax%
                \pgfmatrixbeforeassemblenode{\tikzset{every outer matrix/.try}}%
                \pgfmatrix%
                {\tikz@shape}%
                {\tikz@m@anchor}%
                {\tikz@fig@name}%
                {%
                  \pgfutil@tempdima=\pgflinewidth%
                  {\begingroup\tikz@finish}%
                  \global\pgflinewidth=\pgfutil@tempdima%
                }%
                {\tikz@matrix@shift}%
                {%
                  \tikz@matrix@make@active@ampersand%
                  \def\pgfmatrixbegincode{%
                    \pgfsys@beginscope%
                    \tikz@common@matrix@code%
                    \tikz@atbegin@cell%
                  }%
                  \def\tikz@common@matrix@code{%
                    \let\tikz@options=\pgfutil@empty%
                    \let\tikz@mode=\pgfutil@empty%
                    \pgfutil@for\pgf@temp:=\tikz@common@matrix@code@styleorder\do{%
                      \toks0=\expandafter{\romannumeral-`0\expandafter\pgfutil@trimspaces\expandafter{\pgf@temp}}%
                      \def\pgf@marshal{}%
                      \pgfutil@ifxempty\pgf@temp{}{%
                        \edef\pgf@marshal{\noexpand\tikzset{matrix/inner style/.cd,\the\toks0}}%
                      }%
                      \pgf@marshal
                    }%
                    \tikz@options%
                  }%
                  \def\pgfmatrixendcode{%
                    \tikz@atend@cell%
                    \pgfsys@endscope%
                  }%
                  \def\pgfmatrixemptycode{%
                    \pgfsys@beginscope%
                    \tikz@common@matrix@code%
                    \tikz@at@emptycell%
                    \pgfsys@endscope%
                  }%
                  \tikz@atbegin@matrix%
                  \aftergroup\tikz@do@matrix@cont}%
                \bgroup%
}%
\def\tikz@do@matrix@cont{%
                \tikz@atend@matrix%
              \endgroup%
              \endpgfidscope%
            \endpgfscope
          \endpgfinterruptpath%
      \egroup\egroup%
    \egroup%
    %
    \tikz@node@finish%
}%
{%
  \catcode`\&=13
  \gdef\tikz@matrix@make@active@ampersand{%
    \ifx\tikz@ampersand@replacement\pgfutil@empty%
      \catcode`\&=13%
      \let&=\pgfmatrixnextcell%
    \else%
      \expandafter\let\tikz@ampersand@replacement=\pgfmatrixnextcell%
    \fi%
  }%
}%


\def\tikz@matrix@split#1.#2\relax{%
  \def\tikz@m@anchor{text}%
  \def\tikz@matrix@shift{\pgfpointanchor{#1}{#2}}%
}%

\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    % Node transformation
    %
    \tikz@node@transformations%
    \tikz@nlt%
    %
    \setbox\tikz@whichbox=\hbox{%
      \unhbox\tikz@whichbox%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \tikz@do@rdf@pre@options%
              \tikz@is@nodetrue%
              \tikz@call@id@hook%
              \pgfidscope%
                \tikz@do@rdf@post@options%
                \let\tikz@id@name\pgfutil@empty%
                \setbox\tikz@figbox=\box\pgfutil@voidb@x%
                \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
                % Add color modifications to text box
                \setbox\pgfnodeparttextbox=\hbox{{%
                    \pgfsys@begin@text% Colors moved here...
                    \ifx\tikz@textcolor\pgfutil@empty%
                    \else%
                      \pgfutil@colorlet{.}{\tikz@textcolor}%
                    \fi%
                    \pgfsetcolor{.}%
                    \pgfusetype{.text}%
                    \pgfidscope%
                      \box\pgfnodeparttextbox%
                    \endpgfidscope%
                    \pgfsys@end@text%
                  }}%
                \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                  \pgfutil@tempdima=\pgflinewidth%
                  {\begingroup\tikz@finish}%
                  \global\pgflinewidth=\pgfutil@tempdima%
                }%
              \endpgfidscope%
            \endpgfscope%
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}%


\def\tikz@fig@mustbenamed{%
  \ifx\tikz@fig@name\pgfutil@empty%
    % Assign a dummy name
    \global\advance\tikz@fig@count by1\relax
    \edef\tikz@fig@name{tikz@f@\the\tikz@fig@count}%
    \let\tikz@id@name\tikz@fig@name%
  \fi%
}%

\def\tikz@node@transformations{%
  %
  % Possibly, we are ``online''
  %
  \ifx\tikz@time\pgfutil@empty%
    \pgftransformshift{\tikz@node@at}%
    \iftikz@fullytransformed%
    \else%
      \pgftransformresetnontranslations%
    \fi%
  \else%
    \tikz@do@auto@anchor%
    \tikz@timer%
  \fi%
  % Invoke local transformations
  \tikz@transform%
}%

\def\tikz@node@finish{%
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@path@smuggle=\tikz@after@path%
    % shift box outside group
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \endgroup\endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \global\pgflinewidth=\tikz@save@line@width%
  \tikz@do@after@path@smuggle%
  \tikz@node@is@picfalse
  \tikz@do@after@node%
}%
\let\tikz@fig@continue@orig=\tikz@fig@continue

\def\tikz@do@after@node{\tikz@scan@next@command}%

\def\tikz@do@after@path@smuggle{%
  \let\tikz@to@last@fig@name=\tikz@last@fig@name%
  \let\tikz@to@use@whom=\tikz@to@use@last@fig@name%
  \let\tikzlastnode=\tikz@last@fig@name%
  \ifx\tikz@after@path@smuggle\pgfutil@empty%
  \else%
    \ifpgflatenodepositioning%
      \expandafter\expandafter\expandafter\tikz@call@late%
      \expandafter\expandafter\expandafter{\expandafter\tikz@last@fig@name\expandafter}\expandafter{\tikz@after@path@smuggle}%
    \else%
      \tikz@scan@next@command{\tikz@after@path@smuggle}\pgf@stop%
    \fi%
  \fi%
}%

\def\tikz@call@late#1#2{\pgfnodepostsetupcode{#1}{\path[late options={name={#1},append after command={#2}}];}}%

\newif\iftikz@do@align

% Alignment handling
\def\tikz@signal@halign@check{%
  \tikz@do@alignfalse
  \ifx\tikz@text@width\pgfutil@empty%
    \pgfkeysgetvalue{/tikz/node halign header}\tikz@align@header%
    \ifx\tikz@align@header\pgfutil@empty%
    \else%
      \tikz@do@aligntrue%
    \fi%
  \fi%
}
\def\tikz@halign@check{%
  \iftikz@do@align%
    % Bingo
    \setbox\tikz@align@aligned@box=\box\pgfutil@voidb@x% void
    \let\\=\tikz@align@newline%
    \expandafter\tikz@start@align%
  \fi%
}%
\def\tikz@align@newline{\pgfutil@protect\tikz@align@newline@}%
\def\tikz@align@newline@{\unskip\pgfutil@ifnextchar[\tikz@@align@newline{\tikz@@align@newline[0pt]}}%}%
\def\tikz@@align@newline[#1]{\egroup\tikz@align@continue\pgfmathparse{#1}\let\tikz@align@temp=\pgfmathresult\tikz@start@align}%
% Two safe boxes for alignment:
\let\tikz@align@aligned@box=\pgfnodeparttextbox
\let\tikz@align@line@box=\tikz@figbox

\def\tikz@start@align{%
  % Start collecting text:
  \setbox\tikz@align@line@box=\hbox\bgroup\bgroup%
    \aftergroup\tikz@align@collectresetcolor\ignorespaces%
}%
\def\tikz@align@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\tikz@align@collectresetcolor\let\tikz@temp=}%
  {\tikz@align@end@check}%
}%
\def\tikz@align@end@check{%
  \egroup%
  \ifvoid\tikz@align@aligned@box%
    \setbox\tikz@align@aligned@box=\box\tikz@align@line@box%
  \else%
    \setbox\tikz@align@aligned@box=\vbox{%
      \expandafter\expandafter\expandafter\halign\expandafter\expandafter\expandafter{\tikz@align@header%
        \box\tikz@align@aligned@box\cr%
        \noalign{\vskip\tikz@align@temp pt}%
        \unhbox\tikz@align@line@box\unskip\cr}}%
  \fi%
  \pgfutil@ifnextchar\tikz@align@continue{}
  {%
    % Main continue
      \box\tikz@align@aligned@box%
    \egroup%
  }%
}%
\def\tikz@align@continue{\tikz@@align@continue}%
\let\tikz@@align@continue=\pgfutil@empty


\def\tikz@node@also lso{\pgfutil@ifnextchar[\tikz@node@also@opt{\tikz@node@also@opt[]}}%
\def\tikz@node@also@opt[#1]{
  \pgfutil@ifnextchar(%)
  {\tikz@node@also@opt@cont[#1]}%
  {\tikzerror{Syntax error in node also: ``('' expected.}%
    \tikz@scan@next@command}%
}%
\def\tikz@node@also@opt@cont[#1](#2){\tikzset{late options={name=#2,#1}}\tikz@scan@next@command}%



% Syntax for parts of  nodes:
% node ... {... \nodepart[options]{name} ... \nodepart{name} ...}

\def\tikz@nodepart{\pgfutil@ifnextchar[\tikz@@nodepart{\tikz@@nodepart[]}}%}%
\def\tikz@@nodepart[#1]#2{%
  \tikz@atend@node%
  \unskip%
  \gdef\tikz@nodepart@options{#1}%
  \gdef\tikz@nodepart@name{#2}%
  \global\let\tikz@fig@continue=\tikz@nodepart@continue%
  \pgfutil@ifnextchar x{\egroup\relax}{\egroup\relax}% gobble spaces
}%
\def\tikz@nodepart@continue{%
  \global\let\tikz@fig@continue=\tikz@fig@continue@orig%
  \ifx\tikz@nodepart@list\pgfutil@empty%
    \let\tikz@nodepart@list\tikz@nodepart@name%
  \else%
    \edef\tikz@nodepart@list{\tikz@nodepart@list,\tikz@nodepart@name}%
  \fi%
  % Now start new box:
   \expandafter\setbox\csname pgfnodepart\tikz@nodepart@name box\endcsname=\hbox%
      \bgroup%
        \pgfinterruptpicture%
        \pgfsys@begin@text%
        \pgfsys@text@to@black@hook%
        \tikzset{every \tikz@nodepart@name\space node part/.try}%
        \expandafter\tikzset\expandafter{\tikz@nodepart@options}%
        \ifx\tikz@textopacity\pgfutil@empty%
        \else%
          \pgfsetfillopacity{\tikz@textopacity}%
          \pgfsetstrokeopacity{\tikz@textopacity}%
        \fi%
        % Colors moved here...
        \ifx\tikz@textcolor\pgfutil@empty%
        \else%
          \pgfutil@colorlet{.}{\tikz@textcolor}%
        \fi%
        \pgfsetcolor{.}%
          \ifx\tikz@text@width\pgfutil@empty%
            \tikz@textfont%
          \else%
            \begingroup%
              \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
              \pgfutil@minipage[t]{\pgf@x}\leavevmode\hbox{}%
                \tikz@textfont%
                \tikz@text@action%
          \fi%
          \bgroup%
            \aftergroup\unskip%
            \setbox\tikz@figbox=\box\pgfutil@voidb@x%
            \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
            \tikz@uninstallcommands%
            \iftikz@handle@active@code%
              \tikz@orig@shorthands%
              \let\tikz@orig@shorthands\pgfutil@empty%
            \fi%
            \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
            \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
            \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
            \tikz@atbegin@node%
            \aftergroup\tikz@fig@collectresetcolor%
            \tikz@signal@halign@check%
            \tikz@text@reset%
            \tikz@halign@check%
            \ignorespaces%
}%


%
% Node foreach
%

\def\tikz@nodes@start{%
  \let\tikz@nodes@list\pgfutil@empty%
  \iftikz@node@is@pic%
    \def\tikz@nodes@collect{pic }%
  \else%
    \def\tikz@nodes@collect{node }%
  \fi%
  \tikz@nodes%
}%
\def\tikz@nodes foreach{\pgfutil@ifnextchar x\tikz@nodes@\tikz@nodes@}% get rid of spaces
\def\tikz@nodes@#1in{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list\foreach#1in}%
  \pgfutil@ifnextchar\bgroup\tikz@nodes@group\tikz@nodes@one%
}%
\def\tikz@nodes@one#1{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list#1}%
  \pgfutil@ifnextchar f\tikz@nodes\tikz@nodes@scan%
}%
\def\tikz@nodes@group#1{%
  \expandafter\def\expandafter\tikz@nodes@list\expandafter{\tikz@nodes@list{#1}}%
  \pgfutil@ifnextchar f\tikz@nodes\tikz@nodes@scan%
}%
\def\tikz@nodes@scan{%
  \pgfutil@ifnextchar a{\tikz@nodes@at}%
  {\pgfutil@ifnextchar({\tikz@nodes@name}%
    {\pgfutil@ifnextchar[{\tikz@nodes@opt}%
      {\pgfutil@ifnextchar\bgroup{\tikz@nodes@main}%
      {\tikzerror{Nodes must have a (possibly empty) label text}%
        \tikz@fig@main{}}}}}}%}}%

% Look ahead whether the next character is a (.  If that is the case, we scan
% until ), otherwise we grab a single token and append.
\def\tikz@nodes@at at{\pgfutil@ifnextchar({\tikz@nodes@at@}{\tikz@nodes@at@@}}%
\def\tikz@nodes@at@#1){%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect at#1)}%
  \tikz@nodes@scan}%
\def\tikz@nodes@at@@#1{%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect at#1}%
  \tikz@nodes@scan}%

\def\tikz@nodes@name#1){%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect#1)}%
  \tikz@nodes@scan}%
\def\tikz@nodes@opt#1]{%
  \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect#1]}%
  \tikz@nodes@scan}%
\def\tikz@nodes@main#1{%
  \iftikz@handle@active@nodes%
    \iftikz@node@is@pic%
      \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{#1}}%
    \else%
      \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{\scantokens{#1}}}%
    \fi%
  \else%
    \expandafter\def\expandafter\tikz@nodes@collect\expandafter{\tikz@nodes@collect{#1}}%
  \fi%
  % Ok, got everything.
  % Now, start building parse text.
  \global\setbox\tikz@tempbox=\box\tikz@figbox%
  \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \tikz@nodes@list{%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \expandafter\tikz@scan@next@command\tikz@nodes@collect\pgfextra\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  }%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \tikz@scan@next@command%
}%



%
% "late" options can be used to "redo" a node
%
\tikzset{late options/.code=\tikz@late@options{#1}}%
\def\tikz@late@options#1{%
  % Do a "virtual" node:
  \begingroup%
    \iftikz@shapeborder%
      \let\tikz@fig@name=\tikz@shapeborder@name%
    \else%
      \let\tikz@fig@name=\pgfutil@empty%
    \fi%
    \tikz@is@matrixfalse%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@after@path=\pgfutil@empty%
    \let\tikz@afternodepathoptions=\pgfutil@empty%
    \let\tikz@alias=\pgfutil@empty%
    \let\tikz@transform=\pgfutil@empty%
    \tikz@decoratepathfalse%
    \tikz@node@reset@hook%
    \tikz@enable@node@quotes%
    \tikzset{every node/.try,#1}%
    \ifx\tikz@fig@name\pgfutil@empty%
      \tikzerror{Late options must reference some existing node}%
    \fi%
    \tikz@node@begin@hook%
    \tikz@alias%
    \tikzgdlatenodeoptionacallback{\tikz@fig@name}%
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@path@smuggle=\tikz@after@path%
  \endgroup%
  \tikz@do@after@path@smuggle%
}%


% Auto placement

\def\tikz@auto@pre{%
  \begingroup
    \pgfresetnontranslationattimefalse
    \ifpgfslopedattime
      \pgfslopedattimefalse%
    \else
      \pgfslopedattimetrue%
    \fi
    \pgfallowupsidedownattimetrue%
    \tikz@timer%
    \pgf@x=\pgf@pt@aa pt%
    \pgf@y=\pgf@pt@ab pt%
    \pgfpointnormalised{}%
}%

\def\tikz@auto@post{%
    \global\let\tikz@anchor@smuggle=\tikz@anchor%
  \endgroup%
  \let\tikz@anchor=\tikz@anchor@smuggle%
}%

\def\tikz@auto@anchor{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south west}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north west}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{east}%
      \else%
        \def\tikz@anchor{west}%
      \fi%
    \fi\fi%
}%

\def\tikz@auto@anchor@prime{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north east}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south east}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{west}%
      \else%
        \def\tikz@anchor{east}%
      \fi%
    \fi\fi%
}%


%
% Callbacks: Please see the documentation of the graph drawing
% lib for info on these callbacks
%
\def\tikzgdeventcallback#1#2{}%
\def\tikzgdeventgroupcallback#1{}%
\def\tikzgdlatenodeoptionacallback#1{}%

% Syntax for trees:
% node {...} child [options] {...} child [options] {...} ...
% node {...} child [options] foreach \var in {list} [options] {...} ...

\def\tikz@children{%
  % Start collecting the children:
  \let\tikz@children@list=\pgfutil@empty%
  \tikznumberofchildren=0\relax%
  \tikz@collect@children c}%

\def\tikz@collect@children{\pgfutil@ifnextchar c{\tikz@collect@children@cchar}{\tikz@children@collected}}%
\def\tikz@collect@children@cchar c{\pgfutil@ifnextchar h{\tikz@collect@child}{\tikz@children@collected c}}%
\def\tikz@collect@child hild{\pgfutil@ifnextchar[{\tikz@collect@childA}{\tikz@collect@childA[]}}%}%
\def\tikz@collect@childA[#1]{\pgfutil@ifnextchar f{\tikz@collect@children@foreach[#1]}{\tikz@collect@childB[#1]}}%
\def\tikz@collect@childB[#1]{%
  \advance\tikznumberofchildren by1\relax
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list \tikz@childnode[#1]}%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@child@code}{\tikz@collect@child@code{}}}%
\def\tikz@collect@child@code#1{%
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list{#1}}%
  \tikz@collect@children%
}%
\def\tikz@collect@children@foreach[#1]foreach#2in#3{%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@children@foreachA{#1}{#2}{#3}}{\tikz@collect@children@foreachA{#1}{#2}{#3}{}}}%
\def\tikz@collect@children@foreachA#1#2#3#4{%
  \expandafter\def\expandafter\tikz@children@list\expandafter
    {\tikz@children@list\tikz@childrennodes[#1]{#2}{#3}{#4}}%
  \c@pgf@counta=\tikznumberofchildren%
  \foreach#2in{#3}%
  {%
    \global\advance\c@pgf@counta by1\relax%
  }%
  \tikznumberofchildren=\c@pgf@counta%
  \tikz@collect@children%
}%
\long\def\tikz@children@collected{%
  \begingroup%
    \advance\tikztreelevel by 1\relax%
    \tikzgdeventgroupcallback{descendants}%
    \let\tikz@options=\pgfutil@empty%
    \tikz@clear@rdf@options%
    \let\tikz@transform=\pgfutil@empty%
    \tikzset{level/.try=\the\tikztreelevel,level \the\tikztreelevel/.try}%
    \tikz@transform%
    \let\tikz@transform=\relax%
    \let\tikzparentnode=\tikz@last@fig@name%
    \ifx\tikz@grow\relax\else%
      % Transform to center of node
      \pgftransformshift{\pgfpointanchor{\tikzparentnode}{\tikz@growth@anchor}}%
    \fi%
    \tikznumberofcurrentchild=0\relax%
    \tikz@children@list%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
  \tikz@scan@next@command%
}%

% Syntax for children:
%
% child [all children options] foreach \var in {values} [child options] {...}
\def\tikz@childrennodes[#1]#2#3#4{%
  \c@pgf@counta=\tikznumberofcurrentchild\relax%
  \setbox\tikz@tempbox=\box\tikz@figbox%
  \setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  \foreach#2in{#3}{%
    \tikznumberofcurrentchild=\c@pgf@counta\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
    \tikz@childnode[#1]{#4}%
    % we must now make the current child number and the figbox survive
    % the group
    \global\c@pgf@counta=\tikznumberofcurrentchild\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \global\setbox\tikz@tempbox@bg=\box\tikz@figbox@bg%
  }%
  \tikznumberofcurrentchild=\c@pgf@counta\relax%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \setbox\tikz@figbox@bg=\box\tikz@tempbox@bg%
}%


% Syntax for child:
%
% child
%
% child[options]
%
% child[options] {node (name) {child node text} ...
%   edge from parent[options] node {label text} node {label text}}

\def\tikz@childnode[#1]#2{%
  \advance\tikznumberofcurrentchild by1\relax%
  {\tikzset{every child/.try,#1}\expandafter}%
  \iftikz@child@missing%
    \tikzgdeventcallback{node}{}%
  \else%
  \setbox\tikz@whichbox=\hbox\bgroup%
    \unhbox\tikz@whichbox%
    \hbox\bgroup\bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \tikzset{every child/.try,#1}%
            \tikz@options%
            \tikz@transform%
            \let\tikz@transform=\relax%
            \tikz@grow%
            % Typeset node:
            \edef\tikz@parent@node@name{[name=\tikzparentnode-\the\tikznumberofcurrentchild,style=every child node]}%
            \def\tikz@child@node@text{[shape=coordinate]{}}
            \tikz@parse@child@node#2\pgf@stop%
            \expandafter\expandafter\expandafter\node
            \expandafter\tikz@parent@node@name
              \tikz@child@node@text
              \pgfextra{\global\let\tikz@childnode@name=\tikz@last@fig@name};%
            \let\tikzchildnode=\tikz@childnode@name%
            {%
              \def\tikz@edge@to@parent@needed{edge from parent}
              \ifx\tikz@child@node@rest\pgfutil@empty%
                \path edge from parent;%
              \else%
                \path \tikz@child@node@rest \tikz@edge@to@parent@needed;%
              \fi%
            }%
        \endpgfscope%
      \endpgfinterruptpath%
    \egroup\egroup%
  \egroup%
  \fi%
}%

\def\tikz@parse@child@node{%
  \pgfutil@ifnextchar n{\tikz@parse@child@node@n}%
  {\pgfutil@ifnextchar c{\tikz@parse@child@node@c}%
    {\pgfutil@ifnextchar\pgf@stop\tikz@parse@child@node@rest\tikz@parse@child@node@expand}}}%
\def\tikz@parse@child@node@expand{%
  \advance\tikz@expandcount by-1\relax%
  \ifnum\tikz@expandcount<0\relax%
    \expandafter\tikz@parse@child@node@rest%
  \else%
    \expandafter\expandafter\expandafter\tikz@parse@child@node%
  \fi%
}%
\def\tikz@parse@child@node@rest#1\pgf@stop{\tikz@resetexpandcount\def\tikz@child@node@rest{#1}}%
\def\tikz@parse@child@node@c c{\tikz@resetexpandcount\pgfutil@ifnextchar o{\tikz@parse@child@node@co}{\tikz@parse@child@node@rest c}}%
\def\tikz@parse@child@node@co o{\pgfutil@ifnextchar o{\tikz@parse@child@node@coordinate}{\tikz@parse@child@node@rest co}}%
\def\tikz@parse@child@node@coordinate ordinate{%
  \pgfutil@ifnextchar ({\tikz@@parse@child@node@coordinate}{%
    \def\tikz@child@node@text{[shape=coordinate]{}}%
    \tikz@parse@child@node@rest}}%}%
\def\tikz@@parse@child@node@coordinate(#1){%
  \pgfutil@ifnextchar a{\tikz@p@c@n@c@at(#1)}{%
    \def\tikz@child@node@text{[shape=coordinate,name=#1]{}}%
    \tikz@parse@child@node@rest}}%
\def\tikz@p@c@n@c@at(#1)at#2({%
  \def\tikz@child@node@text@pre{[shape=coordinate,name=#1]at}%
  \tikz@scan@one@point\tikz@p@c@n@c@at@math(%
}%
\def\tikz@p@c@n@c@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{(\the\pgf@x,\the\pgf@y){}}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text@pre\tikz@marshal}%
  \tikz@parse@child@node@rest%
}%
\def\tikz@parse@child@node@n node{\tikz@resetexpandcount%
  \let\tikz@child@node@text=\pgfutil@empty%
  \tikz@p@c@s}%
\def\tikz@p@c@s{%
  \pgfutil@ifnextchar a{\tikz@p@c@s@at}
  {\pgfutil@ifnextchar ({\tikz@p@c@s@paran}
    {\pgfutil@ifnextchar [{\tikz@p@c@s@bra}
      {\pgfutil@ifnextchar \bgroup{\tikz@p@c@s@group}
        {\tikzerror{Cannot parse this node}}}}}}%}}%
\def\tikz@p@c@s@at at#1({%
  \tikz@scan@one@point\tikz@p@c@s@at@math(%
}%
\def\tikz@p@c@s@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{ at(\the\pgf@x,\the\pgf@y)}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text\tikz@marshal}
  \tikz@p@c@s}%
\def\tikz@p@c@s@paran(#1){%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text(#1)}
  \tikz@p@c@s}%
\def\tikz@p@c@s@bra[#1]{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text[#1]}
  \tikz@p@c@s}%
\def\tikz@p@c@s@group#1{%
  \iftikz@handle@active@nodes%
    \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{\scantokens{#1}}}%
  \else%
    \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{#1}}
  \fi%
  \tikz@parse@child@node@rest%
}%



%
% Syntax for decorated subpaths:
%
% decorate [option] { subpath }
%
\def\tikz@decoration ecorate{%
  \pgfutil@ifnextchar[{\tikz@lib@decoration}{\tikz@lib@decoration[]}%]
}%

\def\tikz@lib@decoration[#1]#2{\tikzerror{You need to load a decoration library}}%

% The decorate path command:
\def\tikz@lib@dec@decorate@path{\tikzerror{You need to load a decoration library}}%



%
% Syntax for let :
%
% let \p1 = (coordinate), \p2 = (coordinate),... in
%
\def\tikz@let@command et#1in{%
  \tikzerror{You need to say \string\usetikzlibrary{calc} to use the let command}%
  \tikz@scan@next@command%
}%


%
% Syntax for pictures:
%
% as for nodes, but with "pic" instead of "node"
%
\newif\iftikz@node@is@pic
\def\tikz@subpicture ic{\tikz@node@is@pictrue\tikz@scan@next@command node}%
\def\tikz@subpicture@handle#1{%
  \pgfkeys@spdef\tikz@temp{#1}%
  \expandafter\tikz@subpicture@handle@\expandafter{\tikz@temp}%
}%
\def\tikz@subpicture@handle@#1{
  \pgfkeys{/tikz/pics/.cd,#1}%
  \tikz@node@transformations%
  \let\tikz@transform=\relax%
  \let\tikz@picmode\tikz@mode%
  \tikzset{name prefix ../.style/.expanded={/tikz/name prefix=\pgfkeysvalueof{/tikz/name prefix}}}%
  \ifx\tikz@fig@name\pgfutil@empty\else%
    \tikzset{name prefix/.expanded=\tikz@fig@name}%
  \fi%
  \pgfkeysvalueof{/tikz/pics/setup code}%
  \pgfkeysgetvalue{/tikz/pics/code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@whichbox=\hbox\bgroup%
    \unhbox\tikz@whichbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \pgfkeysgetvalue{/tikz/pics/foreground code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every front pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \pgfkeysgetvalue{/tikz/pics/background code}{\tikz@pic@code}
  \ifx\tikz@pic@code\pgfutil@empty\else%
  \setbox\tikz@figbox@bg=\hbox\bgroup%
    \unhbox\tikz@figbox@bg%
      \hbox\bgroup
        \bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \setbox\tikz@figbox@bg=\box\pgfutil@voidb@x%
              \tikz@atbegin@scope%
              \scope[every behind pic/.try]%
                \tikz@pic@code%
              \endscope%
              \tikz@atend@scope%
            \endpgfscope%
          \endpgfinterruptpath%
        \egroup
      \egroup%
    \egroup%
  \fi%
  \tikz@node@finish%
}%
\tikzset{
  pic actions/.code=\tikz@addmode{\tikz@picmode}
}%

% Setting up the picture codes:
\tikzset{
  pics/setup code/.initial=,
  pics/code/.initial=,
  pics/background code/.initial=,
  pics/foreground code/.initial=
}%

% Defining pictures:

\def\tikzdeclarepic#1#2{\pgfkeys{/tikz/#1/.cd,#2}}%

\pgfkeysdef{/handlers/.pic}{%
  \edef\pgf@temp{\pgfkeyscurrentpath}%
  \edef\pgf@temp{\expandafter\tikz@smuggle@pics@in\pgf@temp\pgf@stop}%
  \expandafter\pgfkeys\expandafter{\pgf@temp/.style={code={#1}}}%
}%
\def\tikz@smuggle@pics@in/tikz/#1\pgf@stop{/tikz/pics/#1}%

%
% Timers
%

\def\tikz@timer@line{%
  \pgftransformlineattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@end}%
}%

\def\tikz@timer@vhline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}%

\def\tikz@timer@hvline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}%

\def\tikz@timer@curve{%
  \pgftransformcurveattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@cont@one}{\tikz@timer@cont@two}{\tikz@timer@end}%
}%


\def\tikz@timer@arc{%
  \pgfmathcos@{\tikz@timer@start@angle}%
  \let\tikz@angle@cos\pgfmathresult%
  \pgfmathsin@{\tikz@timer@start@angle}%
  \let\tikz@angle@sin\pgfmathresult%
  \pgftransformarcaxesattime{\tikz@time}{%
    \pgfpointdiff{%
      \pgfpointadd{%
        \pgfpointscale{\tikz@angle@cos}{\tikz@timer@zero@axis}%
      }{%
        \pgfpointscale{\tikz@angle@sin}{\tikz@timer@ninety@axis}%
      }%
    }%
    {\tikz@timer@start}%
  }%
  {\tikz@timer@zero@axis}%
  {\tikz@timer@ninety@axis}%
  {\tikz@timer@start@angle}{\tikz@timer@end@angle}%
}%



%
% Coordinate systems
%

\def\tikzdeclarecoordinatesystem#1#2{%
  \expandafter\def\csname tikz@parse@cs@#1\endcsname(##1){%
    \pgf@process{%
      #2%
      \global\let\tikz@smubble@b=\tikz@shapeborder@name%
    }%
    \let\tikz@shapeborder@name=\tikz@smubble@b%
    \edef\tikz@return@coordinate{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
}%
\def\tikzaliascoordinatesystem#1#2{%
  \edef\pgf@marshal{\noexpand\let\expandafter\noexpand\csname
    tikz@parse@cs@#1\endcsname=\expandafter\noexpand\csname
    tikz@parse@cs@#2\endcsname}%
  \pgf@marshal%
}%


% Default coordinate systems:

\tikzdeclarecoordinatesystem{canvas}
{%
  \tikzset{cs/.cd,x=0pt,y=0pt,#1}%
  \pgfpoint{\tikz@cs@x}{\tikz@cs@y}%
}%

\tikzdeclarecoordinatesystem{canvas polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0cm,#1}%
  \pgfpointpolar{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}%

\tikzdeclarecoordinatesystem{xyz}
{%
  \tikzset{cs/.cd,x=0,y=0,z=0,#1}%
  \pgfpointxyz{\tikz@cs@x}{\tikz@cs@y}{\tikz@cs@z}%
}%

\tikzdeclarecoordinatesystem{xyz polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0,#1}%
  \pgfpointpolarxy{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}%
\tikzaliascoordinatesystem{xy polar}{xyz polar}%


\tikzdeclarecoordinatesystem{node}
{%
  \tikzset{cs/.cd,name=,anchor=none,angle=none,#1}%
  \ifx\tikz@cs@anchor\tikz@nonetext%
    \ifx\tikz@cs@angle\tikz@nonetext%
      \expandafter\ifx\csname pgf@sh@ns@\tikz@cs@node\endcsname\tikz@coordinate@text%
      \else
        \aftergroup\tikz@shapebordertrue%
        \edef\tikz@shapeborder@name{\tikz@pp@name{\tikz@cs@node}}%
      \fi%
      \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{center}%
    \else%
      \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{\tikz@cs@angle}%
    \fi%
  \else%
    \pgfpointanchor{\tikz@pp@name{\tikz@cs@node}}{\tikz@cs@anchor}%
  \fi%
}%

% Intersection coordinates
\tikzset{cs/first line/.code=\def\tikz@cs@line@a{#1}\def\tikz@cs@type@a{line}}%
\tikzset{cs/second line/.code=\def\tikz@cs@line@b{#1}\def\tikz@cs@type@b{line}}%

\tikzset{cs/first node/.code=\tikz@cs@unpack{\tikz@cs@node@a}{\tikz@cs@type@a}{#1}}%
\tikzset{cs/second node/.code=\tikz@cs@unpack{\tikz@cs@node@b}{\tikz@cs@type@b}{#1}}%

\def\tikz@cs@unpack#1#2#3{%
  \expandafter\ifx\csname pgf@sh@ns@#3\endcsname\relax%
    \tikzerror{Undefined node ``#3''}%
  \else%
    \def#1{#3}%
    \edef#2{\csname pgf@sh@ns@#3\endcsname}%
  \fi%
}%

\tikzset{cs/solution/.initial=1}%

\tikzset{cs/horizontal line through/.store in=\tikz@cs@hori@line}%
\tikzset{cs/vertical line through/.store in=\tikz@cs@vert@line}%

\tikzdeclarecoordinatesystem{intersection}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\ifx\csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname\relax%
    \tikzerror{I do not know how to compute the intersection
    of a \tikz@cs@type@a and a \tikz@cs@type@b. Try saying
    \string\usetikzlibrary{calc}}%
    \pgfpointorigin%
  \else%
    \csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname%
  \fi%
}%

\def\tikz@intersect@line@and@line{%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@a%
  \pgf@xa=\pgf@xc%
  \pgf@ya=\pgf@yc%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@b%
  \edef\pgf@marshal{%
    {\noexpand\pgfpointintersectionoflines%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}%
  \pgf@marshal%
}%

\def\tikz@parse@line#1--{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \tikz@scan@one@point\pgf@process%
}%


\tikzdeclarecoordinatesystem{perpendicular}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@a\tikz@cs@hori@line%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@b\tikz@cs@vert@line%
  \pgfqpoint{\the\pgf@xb}{\the\pgf@ya}
}%

\tikzdeclarecoordinatesystem{barycentric}
{%
  {%
    \pgf@xa=0pt% point
    \pgf@ya=0pt%
    \pgf@xb=0pt% sum
    \tikz@bary@dolist#1,=,%
    \pgfmathparse{1/\the\pgf@xb}%
    \global\pgf@x=\pgfmathresult\pgf@xa%
    \global\pgf@y=\pgfmathresult\pgf@ya%
  }%
}%

\def\tikz@bary@dolist#1=#2,{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \pgfmathparse{#2}%
    \advance\pgf@xa by\pgfmathresult\pgf@x%
    \advance\pgf@ya by\pgfmathresult\pgf@y%
    \advance\pgf@xb by\pgfmathresult pt%
    \expandafter\tikz@bary@dolist%
  \fi%
}%

\tikzset{cs/x/.store in=\tikz@cs@x}%
\tikzset{cs/y/.store in=\tikz@cs@y}%
\tikzset{cs/z/.store in=\tikz@cs@z}%
\tikzset{cs/angle/.store in=\tikz@cs@angle}%
\tikzset{cs/x radius/.store in=\tikz@cs@xradius}%
\tikzset{cs/y radius/.store in=\tikz@cs@yradius}%
\tikzset{cs/radius/.style={/tikz/cs/x radius=#1,/tikz/cs/y radius=#1}}%
\tikzset{cs/name/.store in=\tikz@cs@node}%
\tikzset{cs/anchor/.store in=\tikz@cs@anchor}%



%
% Coordinate management
%


% Last position visited
\def\tikz@last@position{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
\def\tikz@last@position@saved{\pgfqpoint{\tikz@lastxsaved}{\tikz@lastysaved}}%

% Make given point the last position visited
\def\tikz@make@last@position#1{%
  \pgf@process{#1}%
  \tikz@lastx=\pgf@x\relax%
  \tikz@lasty=\pgf@y\relax%
  \iftikz@updatecurrent%
    \tikz@lastxsaved=\pgf@x\relax%
    \tikz@lastysaved=\pgf@y\relax%
  \fi%
  \iftikz@updatenext
    \tikz@updatecurrenttrue%
  \fi
}%

\newif\iftikz@updatecurrent
\tikz@updatecurrenttrue
\newif\iftikz@updatenext
\tikz@updatenexttrue



% Scanner: Scans a point or a relative point.
% It then calls the first parameter with the argument set to an
% appropriate pgf command representing that point.

\def\tikz@scan@one@point#1{%
  \let\tikz@to@use@whom=\tikz@to@use@last@coordinate%
  \tikz@shapeborderfalse%
  \pgfutil@ifnextchar+{\tikz@scan@relative#1}{\tikz@scan@absolute#1}}%
\def\tikz@scan@absolute#1{%
  \pgfutil@ifnextchar({\tikz@scan@@absolute#1}%)
  {%
    \advance\tikz@expandcount by -1
    \ifnum\tikz@expandcount<0\relax%
      \let\pgfutil@next=\tikz@@scangiveup%
    \else%
      \let\pgfutil@next=\tikz@@scanexpand%
    \fi%
    \pgfutil@next{#1}%
  }%
}%
\def\tikz@@scanexpand#1{\expandafter\tikz@scan@one@point\expandafter#1}%
\def\tikz@@scangiveup#1{\tikzerror{Cannot parse this coordinate}#1{\pgfpointorigin}}%
\def\tikz@scan@@absolute#1({%
  \pgfutil@ifnextchar[% uhoh... options!
  {\def\tikz@scan@point@recall{#1}\tikz@scan@options}%
  {\tikz@@@scan@@absolute#1(}%
}%

\def\tikz@scan@options[#1]#2{%
  \def\tikz@scan@point@options{#1}%
  \tikz@@@scan@@absolute\tikz@scan@handle@options(#2%
}%

\def\tikz@scan@handle@options#1{%
  {%
    % Ok, compute point with options set and zero transformation
    % matrix:
    \pgftransformreset%
    \let\tikz@transform=\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@scan@point@options}%
    \tikz@transform%
    \pgf@process{\pgfpointtransformed{#1}}%
    \xdef\tikz@marshal{\expandafter\noexpand\tikz@scan@point@recall{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  }%
  \tikz@marshal%
}%

\def\tikz@@@scan@@absolute#1({%
  \pgfutil@ifnextchar{$}%$
  {\tikz@parse@calculator#1(}
  {\tikz@scan@no@calculator#1(}%
}%
\def\tikz@scan@no@calculator#1(#2){%
  \edef\tikz@scan@point@coordinate{(#2)}%
  \expandafter\tikz@@scan@@no@calculator\expandafter#1\tikz@scan@point@coordinate%
}%
\def\tikz@@scan@@no@calculator#1(#2){%
  \pgfutil@in@{cs:}{#2}%
  \ifpgfutil@in@%
    \let\pgfutil@next\tikz@parse@coordinatesystem%
  \else%
    \pgfutil@in@{intersection }{#2}%
    \ifpgfutil@in@%
      \let\pgfutil@next\tikz@parse@intersection%
    \else%
      \pgfutil@in@|{#2}%
      \ifpgfutil@in@
        \pgfutil@in@{-|}{#2}%
        \ifpgfutil@in@
          \let\pgfutil@next\tikz@parse@hv%
        \else%
          \let\pgfutil@next\tikz@parse@vh%
        \fi%
      \else%
        \pgfutil@in@:{#2}%
        \ifpgfutil@in@
          \let\pgfutil@next\tikz@parse@polar%
        \else%
          \pgfutil@in@,{#2}%
          \ifpgfutil@in@%
            \let\pgfutil@next\tikz@parse@regular%
          \else%
            \let\pgfutil@next\tikz@parse@node%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgfutil@next#1(#2)%
}%

\def\tikz@parse@calculator#1($#2$){%
  \tikzerror{You need to say \string\usetikzlibrary{calc} for coordinate calculation}%
  #1{\pgfpointorigin}%
}%

\def\tikz@parse@coordinatesystem#1(#2 cs:#3){%
  \let\tikz@return@coordinate=\pgfpointorigin%
  \pgfutil@ifundefined{tikz@parse@cs@#2}
  {\tikzerror{Unknown coordinate system '#2'}}
  {\csname tikz@parse@cs@#2\endcsname(#3)}%
  \expandafter#1\expandafter{\tikz@return@coordinate}%
}%


\newif\iftikz@isdimension
\def\tikz@checkunit#1{%
  \pgfmathparse{#1}%
  \let\iftikz@isdimension=\ifpgfmathunitsdeclared%
}%

\def\tikz@parse@polar#1(#2:#3){%
  \pgfutil@ifundefined{tikz@polar@dir@#2}
  {\tikz@@parse@polar#1({#2}:{#3})}
  {\tikz@@parse@polar#1(\csname tikz@polar@dir@#2\endcsname:{#3})}%
}%
\def\tikz@@parse@polar#1(#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \edef\tikz@args{({#2}:#3)}%
  \else%
    \edef\tikz@args{({#2}:{#3} and {#3})}%
  \fi%
  \expandafter\tikz@@@parse@polar\expandafter#1\tikz@args%
}%
\def\tikz@@@parse@polar#1(#2:#3 and #4){%
  \tikz@checkunit{#3}%
  \iftikz@isdimension%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \def\tikz@next{#1{\pgfpointpolar{#2}{#3 and #4}}}%
    \else%
      \tikzerror{You cannot mix dimension and dimensionless values for polar coordinates}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \fi%
  \else%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \tikzerror{You cannot mix dimension and dimensionless values for polar coordinates}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \else%
      \def\tikz@next{#1{\pgfpointpolarxy{#2}{#3 and #4}}}%
    \fi%
  \fi%
  \tikz@next%
}%
\def\tikz@polar@dir@up{90}%
\def\tikz@polar@dir@down{-90}%
\def\tikz@polar@dir@left{180}%
\def\tikz@polar@dir@right{0}%
\def\tikz@polar@dir@north{90}%
\def\tikz@polar@dir@south{-90}%
\def\tikz@polar@dir@east{0}%
\def\tikz@polar@dir@west{180}%
\expandafter\def\csname tikz@polar@dir@north east\endcsname{45}%
\expandafter\def\csname tikz@polar@dir@north west\endcsname{135}%
\expandafter\def\csname tikz@polar@dir@south east\endcsname{-45}%
\expandafter\def\csname tikz@polar@dir@south west\endcsname{-135}%


% MW:
% Check to see if the y-coordinate is inside {}. If it is, scan it and
% reinsert it into the stream inside an extra group.
%
\def\tikz@parse@regular#1(#2,{%
    \pgfutil@ifnextchar\bgroup{\tikz@@parse@regular#1{#2}}{\tikz@@@parse@regular#1{#2}}%
}%
\def\tikz@@parse@regular#1#2#3{%
    \pgfutil@ifnextchar[{% Uh oh! An array index.
        \tikz@@@parse@regular#1{#2}{#3}}%
      {\tikz@@@parse@regular#1{#2}{{#3}}}}%

% Originally \def\tikz@parse@regular#1(#2,#3){%
%
\def\tikz@@@parse@regular#1#2#3){%
  \pgfutil@in@,{#3}%
  \ifpgfutil@in@%
    \tikz@parse@splitxyz{#1}{#2}#3,%
  \else%
    \tikz@checkunit{#2}%
    \iftikz@isdimension%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\pgfutil@next{#1{\pgfpoint{#2}{#3}}}%
      \else%
        \def\pgfutil@next{#1{\pgfpointadd{\pgfpoint{#2}{0pt}}{\pgfpointxy{0}{#3}}}}%
      \fi%
    \else%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\pgfutil@next{#1{\pgfpointadd{\pgfpoint{0pt}{#3}}{\pgfpointxy{#2}{0}}}}%
      \else%
        \def\pgfutil@next{#1{\pgfpointxy{#2}{#3}}}%
      \fi%
    \fi%
  \fi%
  \pgfutil@next%
}%

\def\tikz@parse@splitxyz#1#2#3,#4,{%
  \def\pgfutil@next{#1{\pgfpointxyz{#2}{#3}{#4}}}%
}%

\def\tikz@coordinate@text{coordinate}%

\def\tikz@parse@node#1(#2){%
  \pgfutil@in@.{#2}% Ok, flag this
  \ifpgfutil@in@
    \tikz@calc@anchor#2\tikz@stop%
  \else%
    \tikz@calc@anchor#2.center\tikz@stop% to be on the save side, in
                                % case iftikz@shapeborder is ignored...
    \ifcsname pgf@sh@ns@\tikz@pp@name{#2}\endcsname
      \expandafter\ifx\csname pgf@sh@ns@\tikz@pp@name{#2}\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{\tikz@pp@name{#2}}%
      \fi%
    \else\ifcsname pgf@sh@ns@#2\endcsname
      \expandafter\ifx\csname pgf@sh@ns@#2\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \def\tikz@shapeborder@name{#2}%
      \fi%
    \fi\fi
  \fi%
  \edef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}%

\def\tikz@calc@anchor#1.#2\tikz@stop{%
  % Check if a shape with name prefix exists, otherwise try the global name
  % without prefix.
  \ifcsname pgf@sh@ns@\tikz@pp@name{#1}\endcsname%
    \pgfpointanchor{\tikz@pp@name{#1}}{#2}%
  \else
    \pgfpointanchor{#1}{#2}%
  \fi
}%


\def\tikz@parse@hv#1(#2){%
  \pgfutil@in@{ -| }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@hvboth%
  \else%
    \pgfutil@in@{ -|}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@hvleft%
    \else%
      \pgfutil@in@{-| }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@hvright%
      \else%
        \let\tikz@next=\tikz@parse@hvdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}%
\def\tikz@parse@hvboth#1(#2 -| #3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvleft#1(#2 -|#3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvright#1(#2-| #3){\tikz@parse@vhdone#1({#3}|-{#2})}%
\def\tikz@parse@hvdone#1(#2-|#3){\tikz@parse@vhdone#1({#3}|-{#2})}%

\def\tikz@parse@vh#1(#2){%
  \pgfutil@in@{ |- }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@vhboth%
  \else%
    \pgfutil@in@{ |-}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@vhleft%
    \else%
      \pgfutil@in@{|- }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@vhright%
      \else%
        \let\tikz@next=\tikz@parse@vhdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}%
\def\tikz@parse@vhboth#1(#2 |- #3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhleft#1(#2 |-#3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhright#1(#2|- #3){\tikz@parse@vhdone#1({#2}|-{#3})}%
\def\tikz@parse@vhdone#1(#2|-#3){%
  {%
    \tikz@@@scan@@absolute\tikz@parse@vh@mid(#2)%
    \tikz@@@scan@@absolute\tikz@parse@vh@end(#3)%
    \xdef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  }%
  \tikz@marshal%
}%
\def\tikz@parse@vh@mid#1{\pgf@process{#1}\pgf@xa=\pgf@x}%
\def\tikz@parse@vh@end#1{\pgf@process{#1}\pgf@ya=\pgf@y}%

\def\tikz@parse@intersection#1(intersection{%
  \pgfutil@ifnextchar o{%
    \tikz@parse@main@intersection#1 1%
  }{%
    \tikz@parse@main@intersection#1%
  }%
}%
\def\tikz@parse@main@intersection#1#2of #3 and #4){%
  \tikzset{cs/solution=#2}%
  \pgfutil@in@{--}{#3}%
  \ifpgfutil@in@%
    \tikz@reparse@line{first}#3\pgf@stop%
  \else%
    \tikzset{cs/first node=#3}%
  \fi%
  \pgfutil@in@{--}{#4}%
  \ifpgfutil@in@%
    \tikz@reparse@line{second}#4\pgf@stop%
  \else%
    \tikzset{cs/second node=#4}%
  \fi%
  \tikz@parse@cs@intersection()% advanced hackery...
  \edef\pgf@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \pgf@marshal%
}%
\def\tikz@reparse@line#1#2--#3\pgf@stop{%
  \tikzset{cs/#1 line={(#2)--(#3)}}%
}%


\def\tikz@parse@intersection@a#1{\pgf@process{#1}\pgf@xa=\pgf@x\pgf@ya=\pgf@y}%
\def\tikz@parse@intersection@b#1{\pgf@process{#1}\pgf@xb=\pgf@x\pgf@yb=\pgf@y}%

\def\tikz@scan@relative#1+{%
  \pgfutil@ifnextchar+{\tikz@scan@plusplus#1}{\tikz@scan@oneplus#1}}%

\def\tikz@scan@plusplus#1+{%
  \def\tikz@doafter{#1}%
  \tikz@scan@absolute\tikz@add%
}%
\def\tikz@add#1{%
  \tikz@doafter{\pgfpointadd{#1}{\tikz@last@position@saved}}%
}%
\def\tikz@scan@oneplus#1{%
  \def\tikz@doafter{#1}%
  \tikz@updatecurrentfalse%
  \tikz@scan@absolute\tikz@add%
}%



%
% Quote handling
%

\let\tikz@enable@node@quotes\relax
\let\tikz@enable@edge@quotes\relax
\let\tikz@enable@pic@quotes\relax



% Loading further libraries

% Include a library file.
%
% #1 = List of names of library file.
%
% Description:
%
% This command includes a list of TikZ library files. For each file X in the
% list, the file tikzlibraryX.code.tex is included, provided this has
% not been done earlier.
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% If no file tikzlibraryX.code.tex exists, the file
% pgflibraryX.code.tex is tried instead. If this file, also, does not
% exist, an error message is printed.
%
% Example:
%
% \usetikzlibrary{arrows}
% \usetikzlibrary[patterns,topaths]

\def\usetikzlibrary{\pgfutil@ifnextchar[{\use@tikzlibrary}{\use@@tikzlibrary}}%}%
\def\use@tikzlibrary[#1]{\use@@tikzlibrary{#1}}%
\def\use@@tikzlibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname tikz@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikz@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikz@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikz@library@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname tikz@library@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \pgfutil@InputIfFileExists{tikzlibrary\pgf@temp.code.tex}{}{
        \pgfutil@IfFileExists{pgflibrary\pgf@temp.code.tex}{%
          \expandafter\usepgflibrary\expandafter{\pgf@temp}%
        }{%
          \tikzerror{I did not find the tikz library
            '\pgf@temp'. I looked for files named
            tikzlibrary\pgf@temp.code.tex and
            pgflibrary\pgf@temp.code.tex, but neither
            could be found in the current texmf trees.}
        }}%
      \catcode`\@=\csname tikz@library@#1@atcode\endcsname
      \catcode`\|=\csname tikz@library@#1@barcode\endcsname
      \catcode`\$=\csname tikz@library@#1@dollarcode\endcsname
      \fi%
    \fi
  }%
}%


% Always-present libraries:

\usetikzlibrary{topaths}%




\endinput

